Autobahn: Seamless high speed BFT

Today's practical, high performance Byzantine Fault Tolerant (BFT) consensus protocols operate in the partial synchrony model. However, existing protocols are inefficient when deployments are indeed partially synchronous. They deliver either low latency during fault-free, synchronous periods (good intervals) or robust recovery from events that interrupt progress (blips). At one end, traditional, view-based BFT protocols optimize for latency during good intervals, but, when blips occur, can suffer from performance degradation (hangovers) that can last beyond the return of a good interval. At the other end, modern DAG-based BFT protocols recover more gracefully from blips, but exhibit lackluster latency during good intervals. To close the gap, this work presents Autobahn, a novel high-throughput BFT protocol that offers both low latency and seamless recovery from blips. By combining a highly parallel asynchronous data dissemination layer with a low-latency, partially synchronous consensus mechanism, Autobahn (i) avoids the hangovers incurred by traditional BFT protocols and (ii) matches the throughput of state of the art DAG-based BFT protocols while cutting their latency in half, matching the latency of traditional BFT protocols.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)
SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done

samples/sample-acmcp.pdf: samples/acm-jdslogo.png

.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut \
	samples/acm-jdslogo.png \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

# distros
distros: all docclean
	zip -r acm-distro.zip  \
	acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.* \
	--exclude samples/sample-acmengage*
	zip -r acmengage-distro.zip samples/sample-acmengage* \
	samples/*.bib \
	acmart.pdf acmguide.pdf  *.cls ACM-Reference-Format.*


.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> Sections/1-Introduction/challenges.tex <==
\section{Our Approach}
\begin{itemize}
    \item 
\end{itemize}

\begin{itemize}
    \item Goal is to achieve 1) async responsive throughput and 2) low latency of traditional agreement
    \item Most of the attention on DAG BFT protocols have been focused on zero-message overhead protocols. These include DAG-Rider, Tusk, Bullshark, Fino, Cordial Miners, etc.
    \item Non-zero message overhead protocols like HotStuff over Narwhal have been largely overlooked
    \item Since the Narwhal DAG runs completely asynchronously independent of consensus, HS-Narwhal achieves async responsive throughput
    \item HotStuff consensus messages are small as they contain just metadata, so the latency is low
    \item This has been shown experimentally where HotStuff over Narwhal has latency of under 2 seconds (slightly lower than Bullshark) and peak throughput of 140k tps (on par with Bullshark)
    \item Even though HS-Narwhal has comparatively low latency it still takes 10 message delays to commit (3 from Narwhal RB plus 7 from HS)
    \item The latency of Bullshark for most commands, however, is 6-12 message delays
    \item The reason why HS-Narwhal still generally has slightly lower latency even though it takes more message delays is that 2-4 of the message delays require disseminating a block (part of DAG round), whereas HS-Narhwal only has 1 message delay which requires disseminating a block. Disseminating blocks take take longer than disseminating messages with small amounts of metadata
    
\end{itemize}

\begin{itemize}
    %\item Insight 1: Removing reliable/consistent broadcast (Cordial Miners) in the DAG layer removes the ability to achieve async responsive throughput. Without the reliable broadcast during periods of asynchrony, DAG blocks can be lost/not available, lowering throughput
    \item Insight \#1: Most DAG BFT protocols are focused on achieving zero-message overhead
    
    Prior work either reliably broadcasts every consensus message as part of the DAG ("zero message overhead") or every consensus message is done externally outside of the DAG.
    Zero message overhead DAG protocols RB both consensus proposals and votes, therefore taking multiple instances of RB to reach consensus. We observe, however, a single instance of RB does most of the work of full consensus. So instead of having a zero-message overhead we have a small-message overhead that avoids needing multiple instances of RB for consensus.
    \item 
\end{itemize}

Our approach is to have the DAG and consensus be logically independent but have them share as many messages as possible that do the same work. This approach, however, has the following challenges.

\subsection{Challenge \#1: Async Responsive Throughput with a Psync Consensus}
\begin{itemize}
    \item Since a Psync consensus protocol needs timeouts we need to be careful 
    that timeouts from consensus do not reduce throughput during asynchronous periods
    \item To see how this can happen consider this naive approach where certain blocks are marked to be processed by a consensus black box
    \item 
\end{itemize}

\subsection{Challenge \#2: How to reconcile the independent speeds of DAG and consensus}
\begin{itemize}
    \item The challenge is that since consensus shares messages with the DAG layer, but is also independent it may need to wait for the DAG to be ready to include a metadata
    \item This problem was identified by Bullshark for logical DAG where consensus would be ready to start but the DAG was still processing a block in flight and would therefore have to wait for the DAG to finish before starting
    \item This is exacerbated by the fact that Logical DAG/Fin are zero message overhead protocols and every consensus message must be reliably broadcasted as part of a physical DAG block
\end{itemize}

\subsection{Challenge \#3: }

\begin{enumerate}
    \item How to compose DAG and consensus in such a way to have async responsive throughput while also having low latency?
    \item If DAG growth and consensus are independent, how do we maintain bounded round advancement, while also supporting async responsive throughput?
    \item How do we design a view change that supports a fast path in the common case?
    \item Implementation details such as syncing, garbage collection
\end{enumerate}

\subsection{Async Responsive Throughput}
How to have a partially synchronous consensus protocol composed with an asynchronous DAG/mempool protocol such that the DAG protocol does not become partially synchronous?
\begin{enumerate}
    \item Approach 1: Certain blocks in the DAG are marked as consensus blocks, and others are marked as DAG blocks. Consensus blocks are run through a blackbox partially synchronous consensus protocol, and DAG blocks are run through the blackbox reliable broadcast protocol.
    \item Approach 2: Still maintain division of DAG blocks and consensus blocks. Consensus blocks go through the blackbox reliable broadcast protocol, and afterwards a single round of voting occurs to complete consensus. DAG blocks go through blackbox reliable broadcast
\end{enumerate}

Advantages of approach 1:
-Clean modularity and simplicity, can plug in any consensus protocol and DAG protocol
-Easy to take advantage of consensus optimizations such as pipelining
Disadvantages:
-Does not satisfy async responsive throughput. This is because if consensus timeouts are slow then consensus blocks will still be waiting the timeout while the DAG advances, thus the DAG becomes partially sync

Challenges with approach 2:
-If consensus timeouts are too big this is fine because the reliable broadcast will finish first maintaining async
-If consensus timeouts are too short then this is problematic since replicas will refuse to vote for consensus blocks because they have already advanced views
-We need some way to "invalidate" or downgrade a consensus block to a DAG block in order to get responsive throughput
-Challenge: how to avoid byzantine replicas always voting to invalidate a consensus block causing a consensus block to lose progress
-Idea 1: to invalidate a consensus block a byzantine replica needs proof that it actually advanced to a higher view. This is the TC (indicates at least f+1 honest voted to advance views).
-Problem with Idea 1: What if a byz replica times out in the consensus layer but has not received a TC. A byz replica has to wait for the TC to arrive -> DAG becomes partially sync. A byz replica votes to invalidate -> no proof and a byz replica spuriously votes to invalidate. Voting twice can lead to problems with ensuring non-equivocation.
Idea 2: Have special votes and normal votes. Special votes are also normal votes. If receive a consensus block that is invalid then send a normal vote invalidating it, otherwise if consensus block is valid then send a special vote. This allows 2f+1 normal votes to create a DAG certificate (consistent broadcast). If byz replicas always sends normal votes then we may have situation with f+1 special votes and f normal votes. Then an honest consensus leader can wait a timeout \fs{actually indefinitely} to receive 2f+1 special votes. f byz replicas cannot prevent liveness in the good case because honest replicas will always send a special vote and an honest leader will wait the timeout. Note this maintains async responsive throughput because leader can always advance the DAG upon receiving the first 2f+1 votes (since special votes double as normal votes)
\fs{Note that if one honest votes invalid then consensus has timed out and thus it's ok to not receive 2f+1 special votes (since they are outdated anyways)}

==> Sections/1-Introduction/old/intro-old-poster.tex <==
\section{Introduction}
This work presents \sys, a highly performant Byzantine Fault Tolerant (BFT) consensus protocol that offers low latency, high throughput, and seamless recovery from periods of asynchrony.

Blockchain systems have emerged as a promising way for mutually distrustful parties to compute over shared data. Byzantine Fault Tolerant (BFT) state machine replication (SMR), the core protocol in most blockchains, provides to applications the abstraction of a centralized, trusted, and always available server. BFT SMR guarantees that a set of replicas will agree on a common sequence of operations, even though some nodes may misbehave. 

While there have been a lot of advancements on BFT SMR efficiency over the last two decades, today's state of the art still falls short of their less robust, crash fault tolerant (CFT), counterparts. %BFT protocols offer increased robustness to malicious faults, at the cost of performance. 
To reach mainstream adoption we submit that a BFT protocol must excel across three axes:
\one It must offer high throughput, \two It must offer low \textbf{end-to-end} latency\footnote{We remark that thoughput and latency are not exclusive: under high demand, low tput implies high end-to-end latency.}, and \three It must behave robustly under realistic network conditions; all whilst being simple enough to build. %\neil{The simple argument may be controversial given our protocol} 
%\fs{-- what about fairness?}\neil{Again a bit controversial since the Star people would argue that byz replicas can run ahead and progress faster with their chains}

As it is, today's systems are faced with a trade-off: they must choose between \textit{either} low latency or robustness. The root of this tension, we submit, traces to their choice of network model.
\iffalse
The root cause for this tension can be traced to the choice of network models. Protocols in the \textit{partially synchronous} model strive to be practical, and achieve optimal \textbf{consensus latency} by limiting progress guarantees to periods of synchrony. On the flip-side \textit{asynchronous} consensus protocols make progress consistently, but do so at a slower, often prohibitive pace; consequently, these protocols see little adoption.
The problem in either case is that most existing protocols adopt one model across the whole system. While hybrid approaches exist, they typically swap between two separate protocols, resulting in inefficient designs.
\fi

Broadly speaking, there are two popular approaches to BFT SMR, each of which enjoys different tradeoffs:
\paragraph{Traditional BFT} (PBFT, Hotstuff, Zyzzyva) protocols employ the \textit{partial synchronous} model to optimize for a minimal number of message exchanges (herafter \textbf{consensus} latency) by limiting progress guarantees to periods of synchrony (cite FLP). Unfortunately, these protocols are not guaranteed to resume operations gracefully once synchrony returns. Under continuous load, lack of progress can cause large request backlogs to form, manifesting -- akin to a metastable failure -- in a constant \textbf{end-to-end} latency degradation. %\neil{Could also mention that HotStuff suffers from sequential latency}
Notably, these protocols typically employ a dedicated (single-leader) to submit proposals and drive agreement, which can easily become a throughput bottleneck. To overcome the latter, recent advances (cite BFT-Mir/ISS, others?) propose \textit{Multi-log BFT} frameworks that carefully orchestrate several (blackbox) instances of traditional BFT protocols in parallel, and intertwine their output logs to arrive at a single, total order. \fs{Doing so is not free: the required orchestration demands additional complexity, and may result in suboptimal performance in the presence of faults.}
Multi-log frameworks inherit both the good and the bad of their building blocks: consenus latencies are low, but \textit{network robustness remains poor}. 

\paragraph{DAG-based BFT,} a newly popular class of consensus protocols (cite HashGraph, Dagrider, Narwahl, Bullshark, Fin, Shoal), takes a different approach all-together, and is rooted in the \textit{asynchronous} model. DAG BFT protocols employ as backbone a high throughput asynchronous data dissemination layer, that proceeds in a series of structured, tightly synchronized rounds, forming a DAG. Consensus leverages this structure to act as a common clock, and is embedded with zero message overhead: it \textit{interprets} the DAG structure, and forms an ordered log by committing and flattening causal histories in the DAG. This design enjoys both excellent throughput and network resilience. However, while asynchronous consensus protocols make progress consistently, they do so at a slower, often prohibitive pace; consequently, these protocols see little practical adoption. Recent DAG protocols (cite Bullshark/Shoal) make use of partial synchrony to improve consensus latency (notably, data dissemination remains asynchronous), yet consensus still requires several rounds of Reliable Broadcast communication, with the state of the art (cite Shoal) exhibiting an average case commit latency of 9 message exchanges.

%\neil{Tail latency could also be an issue since you have to wait for n-f broadcasts to finish in each round}
%\neil{Async fallback. Another approach is to have two protocol paths: an optimistic partially synchronous path that guarantees progress under synchrony and a pessimistic asynchronous path that guarantees progress under asynchrony. Even though protocols like Ditto and Bolt-Dumbo Transformer can commit during asynchronous periods, they suffer from high switching costs between both paths. Thus, once synchronous conditions resume, they incur extra latency to switch back to the faster partially synchronous path. Additionally, the asynchronous paths (VABA) often have poor throughput since they throw away/waste a lot of the broadcasts, which use up a lot of bandwidth. }

\fs{TODO: find a better way to say this/cut alltogether. Still need to smooth over the flow over the next paragraph}
Both classic BFT protocols and recent DAG BFT protocols fall short of simultaneously achieving low consensus latency and network robustness. 

\par \textbf{This work asks whether it is possible to mend the tension between low consensus latencies and robustness, and arrive at practical designs with low end-to-end latency.} We answer in the affirmative and present \sys, a novel BFT consensus protocols with low end-to-end latency, high (multi-proposer) throughput, and seamless recovery from asynchrony. 

Most existing protocols adopt either partial synchrony or asynchrony \textit{across the whole system} (or closely evolve from systems that do), and thus inherit the respective inherent tradeoffs.\footnote{While some hybrid approaches exist (cite), they swap between two separate protocols (one in each model), resulting in inefficient designs.}
%While existing works evolve from one design extreme. in traditional, psync BFT, and async-originating.. It makes data layer async, and protocol psync.
\sys resolves this tension by taking a step back -- rather than evolve from one design corner, \sys aims to start from a clean slate, and layers a partially synchronous traditional-style consensus protocol atop a cheap asynchronous data dissemination layer to combine the best properties of past approaches. 

%%%%%%% END HERE.


\paragraph{Asynchronous data dissemination. }Akin to recent DAG-protocols, \sys leverages an asynchronous data dissemination layer as the backbone of it's protocol, ensuring continuous dissemination progress. Unlike them however, \sys lifts the \textit{speedlimit} and eschews round-based synchronization (and the entailing rigid DAG structure) to allow proposers to make progress fully independently. Each replica acts as proposer, disseminating data in it's \textit{own lane}, and \textit{as fast as it can}. \sys{}'s dissemination layer is unstructured and best-effort: it does not causally relate independent lanes, and makes no guarantees whether or not a lane can fork. We rely on a logically separate consensus layer to decree a consistent total ordering.

\iffalse
To disseminate, a replica uses a lightweight version of provable broadcast primitive (\href{https://decentralizedthoughts.github.io/2022-09-10-provable-broadcast/#:~:text=Provable%20Broadcast%3A%20is%20a%20simple,is%20the%20Weak%2DAvailability%20property.}{cite Ittai's blog post?}) to ensure availability; a simple broadcast followed by $f+1$ acknowlegements suffices to form a Proof of Availability (PoA) \fs{smaller quorums reduce tail latencies -- though it can result in more synchronization being necessary (marginal concern imo) . 2f+1 is not needed, since that's for equivocation. }. Consecutive proposals are chained via hashes to transitively prove availability, and pipelined \fs{(with certificate forwarding)} to minimize latency. \fs{do we need more detail than this here?  less? }

Note, that our dissemination layer is unstructured and best-effort: it does not causally relate independent lanes, and makes no guarantees whether or not a lane can fork. We rely on a logically separate consensus layer to decree a consistent total ordering. \fs{maybe talk about what this async data dissemination layer gives us?}
\fi

\paragraph{Embedded consensus instances. }
In order to reach consensus, \sys constructs a partially synchronous consensus protocol that requires only 3md in fault-free scenarios, and 5md otherwise. We embed all protocol messages into the data dissemination layer's message exchanges, thus sidestepping any coordination redundancies. Instead of proposing data as in traditional BFT protocols, \sys consensus proposes a snapshot vector of each data lanes latest state (or \textit{tip}), thus enjoying the throughput of $O(n)$ parallel proposers. Upon committing the snapshot, \sys deterministically intertwines each tip's causal history, constructing a single totally ordered log \fs{, and implicitly resolving all forked lanes}. Finally, to minimize the wait-time for a tip to be proposed (and thus end-to-end latency), \sys begins and pipelines a new consensus instance as soon as there are new tips -- rather than upon completing the previous instance.

\sys{}'s finely integrated consensus design allows it to enjoy both \textit{optimal} consensus latency and low end-to-end latency, while simultaneously reaping the high throughput and robustness offered by asynchronous data dissemination. Though there is no consensus progress during periods of asynchrony, the data layer (and consequently the lane tips) keep growing. Upon return of synchrony, \sys{} seamlessly recovers by instantly committing it's tips causal histories, making it appear as if progress were never suspended.


\iffalse 
\fs{TODO: Summary how the whole thing ties together: }
throughput: multi-proposer -- maxing out; arbitrarily scalable with orthogonal worker layer
Latency:  3md Fast path, 5 slow path. Could also use all to all. minimal sequential wait time, consensus instances overlap
Robustness: no new instances for a while (k open ones are stuck view changing). When the next new instance opens, it proposes the newest tips (organic batching) => data dissemination was async (can include TX verification). => no backlog. Get a bump in Tput that balances out the dip. And latency recovers seamlessly. 

\iffalse
\fi

\fs{I feel like we can have a separate section (at the end of the protocol description, where we describe the Hotstuff instantiation. } Could also pipeline if we used Hotstuff (e.g. each leader only does one provable broadcast, and the next one starts either with the QC, or just the proposal)

~\\
\fs{TODO: Summary of system performance + overall contributions}
- comparable tput to Bullshark
- but lower latency
- robust behavior to asynchrony  (compare against Hotstuff)

~\\
Contributions:
- (maybe some new definitions: better latency metric, characterization of the async robustness)
- \sys design
- \sys systems


~\\
\fs{TODO: Think about worst case latency:}
Worst case: Async and k honest leaders. All proposed something that was agreed on, but then time out during cert generation/forwarding. Then new instance (with max tips) won't start until one instance finishes (so there is 1 sequential latency here).  (worst worst case: f faulty ones amongst k, so you wait f+1)
-> In View Change: if there is a decision in the VC quorum, then one needs one Provable Broadcast to commit that decision. If there is none, it's the same. But if we want to add new tips, then we turn it into a full consensus (2 PVB) again. That slightly increases the wait for the next slot -- but it doesn't matter: if the replica was honest, then it proposed new data (that might subsume the next slot); if it was byz, we'd VC ANOTHER round anyways.
\fi

\iffalse
Problem: systems use one model for whole sys
Problem: latency != progress. While progress resumes, end-to-end latency suffers.

Tension is between latency and robustness
As it is sys have to favor 2 of three. Why? root cause: async/psync for everything
- some protocols start from psync, add async fallback
- some add psync fast path
- psync overly optimistic; suffer during async.
- async too pessimistic; 
- hybrids kind of naive
(distinguish original and psync bullshark?)

what's the best we can do given the properties we want. 

key insight: only need data diss asynchronous. 

\fi

%%%%%%%%%%%%%% OLD %%%%%%%%%%%%%%%%%%%%%%
\iffalse
\one \sys commits with minimal latency: 3/5. Additional \sys avoid sequential latencies/ minimizes end-to-end latency by aggressively pipelining (otherwise sequential) successive consensus instances.
\two It achieves high throughput by leveraging multi-leader data dissemination. \three Finally, akin to recent DAG protocols, \sys logically separates data dissemination to be asynchronous, and independent -- need to figure out how to say this.

\sys resolves these tensions.
\syss core ethos is to treat all 3 goals as first priniciples; as opposed to evolving from one corner (which adds limitations, and complexity)
\syss key insight is... asynchronous paralell data dissemination + do consensus as soon as there is new data (and not when previous consensus is done)

At a high level, \sys achieves this by layering and embedding a partially synchronous pipelined/multi-leader consensus mechanism atop an asynchronous data dissemination layer; but instead of inheriting the black box rigid round based design of DAG protocols, we start from scratch ...

Akin to recent DAG protocols, an asynchronous data dissemination layer forms the backbone of the protocol. Unlike them however, data dissemination is not synchronized across replicas (round based DAG puts a "speed limit" on replicas), but fully independent. Each replica disseminates data in it's \textit{own lane}, and \textit{as fast as it can}. To disseminate, a replica uses a provable broadcast (broadcasts it's request, and waits for f+1 replies -- proving that the data is available. (this is a lightweight BCB/RB -- we only care about availability). The next proposal includes a hash reference, and is piggybacked alongside the previous cert. 


Consensus takes as input the tips of each lane. The leader simply proposes it's locally visible frontier (a snapshot cut of all lanes). Consensus itself is embedded into the data dissemination -- we just change the Quorums to be of size 2f+1. We embed a PBFT like version (with a fast path), but any consensus protocol that can be built with provable broadcast building blocks can be embedded. e.g. hotstuff.

A simple version \fs{I think it might be viable to explain a modified Sailfish version} starts the next consensus slot after the previous one is done -- with a Ticket: Commitment of previous one, or View Change. (The ticket could be external, or embedded in another data proposal). However, this incurs sequential latency. 
Our improved version implements parallel consensus: The next consensus instance starts as soon as there is "new" data. We wait for previous proposal, and have to be newer across n-f. 
Since we parallelize, slots must wait for each other.

View change. Move instance to new leader. One leader might deal with multiple instances. If instance didn't agree on anything yet, can propose NEW tips -- seamless (didn't "lose" any time).

In practice only a few instances active.
Wait for k instances behind to be caught up (done) before starting next

Throughput: multileader -- maxing out; arbitrarily scalable with orthogonal worker layer
Latency:  3md Fast path, 5 slow path. Could also use all to all. minimal sequential wait time, consensus instances overlap
Robustness: no new instances for a while (k open ones are stuck view changing). When the next new instance opens, it proposes the newest tips (organic batching) => data dissemination was async (can include TX verification). => no backlog. Get a bump in Tput that balances out the dip. And latency recovers seamlessly. 

Worst case: Async and k honest leaders. All proposed something that was agreed on, but then time out during cert generation/forwarding. Then new instance (with max tips) won't start until one instance finishes (so there is 1 sequential latency here).  (worst worst case: f faulty ones amongst k, so you wait f+1)
-> In View Change: if there is a decision in the VC quorum, then one needs one Provable Broadcast to commit that decision. If there is none, it's the same. But if we want to add new tips, then we turn it into a full consensus (2 PVB) again. That slightly increases the wait for the next slot -- but it doesn't matter: if the replica was honest, then it proposed new data (that might subsume the next slot); if it was byz, we'd VC ANOTHER round anyways.



\fs{I feel like we can have a separate section (at the end of the protocol description, where we describe the Hotstuff instantiation. } Could also pipeline if we used Hotstuff (e.g. each leader only does one provable broadcast, and the next one starts either with the QC, or just the proposal)












to allow a new consensus round to begin \textit{as soon as} there are new requests available (rather than waiting for previous consensus to finish




\section{Intro Brainstorm Notes}
- want three things: low (end-to-end) latency, high tput, robustness to async (explain each)
- tension between the three. (show that no protocol does well in all 3)

- try to characterize fundamental shortcomings of other multi leader protocols:
\begin{itemize}
    \item Dag started from async (retrofit psync). Failed to realize data dissemination and consensus are two parts of the same coin. - current state is result of evolution: needed clock for async; kept it in psync. Has benefits (no TO) but comes at cost of latency. 
    \item Mir doesnt have data dissemination layer; suffers from robustness. - can't change existing systems; need to start from scratch. (Could layer dissemination layer like in Narwahl + HS; but that introduces redundancies. -> BBCA ledger is probably the "design from scratch" verison. Mir takes blackbox psync, and runs n parallel instances 
    \item Both start from a Base, and are forced to work around it. We start form clean base.
\end{itemize}



\fs{We want three things: High tput, Low (end-to-end) Latency, and async responsiveness}
\fs{No existing system can do all, they each get at most 2}
\fs{we describe a new system, \sys, that gets all 3.}
\fs{it achieves this by layering a partially sync consensus on an async data dissemination layer ==> need to find a much more compelling way to describe this}

high-level tlrd/name:
- each replica disseminates data in it's own "lane", as fast as it can
- we embed consensus onto some of the broadcasts to occasionally take a snapshot of all lanes => we flatten this into a log. 
\fs{testing}

\begin{itemize}
    \item Traditional leader-based partially synchronous BFT (like PBFT) is not sequential and has low latency 
    \item Drawbacks: 1) Leader is a bottleneck for disseminating large batches and 2) throughput severely drops under asynchrony
    \item We want to decouple data dissemination from consensus using the bandwidth available from all replicas
    \item Also want to have data dissemination to be asynchronous so throughput doesn't drop under asynchrony, it must satisfy a property we call async responsive throughput
    \item Decoupling data dissemination from consensus naively (using black boxes) adds redundancy and latency since they do similar work
    \item Our design (key idea?): make consensus and data dissemination completely logically independent but have them share the same physical messages
    \item Trying to combine data dissemination with consensus in this way has the following challenges:
    \begin{enumerate}
    \item How to avoid unwanted synchronization between consensus and data dissemination (don't want consensus to wait on data dissemination or vice versa)
    \item How to combine a partially synchronous consensus protocol with an asynchronous data dissemination layer without making the data dissemination layer also partially synchronous
    \item How to avoid committing stale data without making consensus completely sequential
    \end{enumerate}
    \item Prior work (DAGs, multiple leader BFT) try to solve some of these issues but they suffer from one or more of:
    \begin{enumerate}
        \item No async responsive throughput
        \item Redundant work between consensus and data dissemination (high latency)
        \item Sequential latency
        \item Unwanted synchronization between consensus and data dissemination
    \end{enumerate}
    \item Can we have it all?
    \item Question: Can we design a BFT system that has low (non-sequential) latency while also having high (async responsive) throughput?
    
\end{itemize}

\fi

==> Sections/1-Introduction/old/intro-old.tex <==
\section{Introduction}
This paper presents Autobahn, a high performance Byzantine Fault Tolerant (BFT) consensus protocol that offers low latency, high throughput, and seamless recovery from periods of asynchrony.

%Online data sharing offers exciting opportunities for many industries -- yet as the demand surges, so does the demand for safe and trust-less communication/coordination.
%As the need for online data sharing grows, so does the demand for safe, trustless communication/coordination.
%BFT consensus lies at the heart of blockchain, and have seen considerable adoption across many such systems over the last decade. Yet, application to mainstream traditional applications remains elusive.

\fs{stolen from begees - rephrase}
Blockchain systems have emerged as a promising way for mutually distrustful parties to compute over shared data. Byzantine Fault Tolerant (BFT) state machine replication (SMR), the core protocol in most blockchains, provides to applications the abstraction of a centralized, trusted, and always available server. BFT SMR guarantees that a set of replicas will agree on a common sequence of operations, even though some nodes may misbehave. 

While there have been a lot of advancements on BFT SMR efficiency over the last two decades, today's state of the art still falls short of their less robust, crash fault tolerant (CFT), counterparts. %BFT protocols offer increased robustness to malicious faults, at the cost of performance. 
To reach mainstream adoption we submit that a BFT protocol must excel across three axes:
\one It must offer low \textbf{end-to-end} latency (\fs{expand one what this means)}, \two It must offer high throughput, and \three It must behave robustly under realistic network conditions; all whilst being \textit{simple} enough to explain and build. \neil{The simple argument may be controversial given our protocol} 
\fs{-- what about fairness?}\neil{Again a bit controversial since the Star people would argue that byz replicas can run ahead and progress faster with their chains}

\fs{playing around with new angle}
As it is, today's systems are faced with a trade-off: they must choose between \textit{either} low latency or robustness. 
The root cause for this tension can be traced to the choice of network models. Protocols in the \textit{partially synchronous} model strive to be practical, and achieve optimal \textbf{consensus latency} by limiting progress guarantees to periods of synchrony. On the flip-side \textit{asynchronous} consensus protocols make progress consistently, but do so at a slower, often prohibitive pace.
The problem in either case is that most existing protocols adopt a model across the whole system. While hybrid approaches exist, they typically swap between two (full) separate protocols, resulting in inefficient designs.


Problem: systems use one model for whole sys
Problem: latency != progress. While progress resumes, end-to-end latency suffers.

Tension is between latency and robustness
As it is sys have to favor 2 of three. Why? root cause: async/psync for everything
- some protocols start from psync, add async fallback
- some add psync fast path
- psync overly optimistic; suffer during async.
- async too pessimistic; 
- hybrids kind of naive
(distinguish original and psync bullshark?)

what's the best we can do given the properties we want. 

key insight: only need data diss asynchronous. 
\fs{end -- new angle}

Unfortunately, in today's systems, these requirements exist under tension: to the best of our knowledge no BFT system today reaches satisfactory performance across all three categories simultaneously.

\fs{TODO: group multi-log under traditional}
\paragraph{Traditional BFT} (PBFT, Hotstuff, Zyzzyva) protocols optimize for latency, but fall short in terms of throughput. These protocols typically employ a dedicated (single-leader) to drive agreement, which can easily become a throughput bottleneck. \footnote{We remark that thoughput and latency are not exclusive: under high demand, low tput results in high end-to-end latency.} Moreover, these protocols are designed to be efficient only under synchrony; while always safe, no progress is guaranteed during periods of asynchrony. Worse, these protocols are not guaranteed to resume operations gracefully once synchrony returns. Under continuous load, lack of progress can cause large request backlogs to form, manifesting -- akin to a metastable failure -- in a constant end-to-end latency degradation. \neil{Could also mention that HotStuff suffers from sequential latency}

To overcome the throughput shortcoming more recent BFT protocols employ \textit{multi-leader} designs. Broadly speaking, there are two popular approaches, each of which enjoys different tradeoffs:
\paragraph{Multi-log BFT} frameworks such as BFT-Mir/ISS (others?) carefully orchestrate several (blackbox) instances of classic BFT protocols in parallel, and intertwine their output logs to arrive at a single, total order. Multi-log frameworks inherit both the good and the bad of their building blocks: commit latencies are low, but network robustness is poor. Lastly, the required orchestration demands additional complexity, and may result in suboptimal performance in the presence of faults.
\paragraph{DAG-based BFT.} A different approach all-together are the newly popular DAG-based consensus protocols (Narwahl, Bullshark, Fin, Shoal). DAG BFT protocols employ as backbone an asynchronous data dissemination layer, that proceeds in a series of structured, tightly synchronized rounds, forming a DAG. Consensus leverages this structure to act as a common clock, and is embedded with zero message overhead: it interprets the DAG structure, and forms an ordered log by committing and flattening causal histories in the DAG. This class of protocol originated from asynchronous designs, and enjoys both excellent throughput and network resilience, yet falls short in terms of latency. Consensus requires several rounds of Reliable Broadcast communication  \fs{be more concrete}, with the state of the art (Shoal) exhibiting best and average case latencies of 6md \fs{for leaders} and 9md respectively.
\neil{Tail latency could also be an issue since you have to wait for n-f broadcasts to finish in each round}
\neil{Async fallback. Another approach is to have two protocol paths: an optimistic partially synchronous path that guarantees progress under synchrony and a pessimistic asynchronous path that guarantees progress under asynchrony. Even though protocols like Ditto and Bolt-Dumbo Transformer can commit during asynchronous periods, they suffer from high switching costs between both paths. Thus, once synchronous conditions resume, they incur extra latency to switch back to the faster partially synchronous path. Additionally, the asynchronous paths (VABA) often have poor throughput since they throw away/waste a lot of the broadcasts, which use up a lot of bandwidth. }

\textbf{This work asks whether it is possible to simultaneously succeed across all three categories. We answer in the affirmative and present Autobahn, a novel BFT consensus protocols with low end-to-end latency, high (multi-leader) throughput, and seamless recovery from asynchrony. }

Autobahn resolves the tensions present in Multi-log and DAG-based BFT systems by taking a step back -- rather than evolve from one design corner, Autabahn aims to start from a clean slate, and combine the best properties of past approaches. 

\paragraph{Asynchronous data dissemination. }Akin to recent DAG-protocols, Autobahn leverages an asynchronous data dissemination layer as the backbone of it's protocol. Unlike them however, Autobahn lifts the \textit{speedlimit} and eschews round-based synchronization (and the entailing rigid DAG structure) to allow proposers to make progress fully independently. Each replica acts as proposer, disseminating data in it's \textit{own lane}, and \textit{as fast as it can}. 

To disseminate, a replica uses a lightweight version of provable broadcast primitive (\href{https://decentralizedthoughts.github.io/2022-09-10-provable-broadcast/#:~:text=Provable%20Broadcast%3A%20is%20a%20simple,is%20the%20Weak%2DAvailability%20property.}{cite Ittai's blog post?}) to ensure availability; a simple broadcast followed by $f+1$ acknowlegements suffices to form a Proof of Availability (PoA) \fs{smaller quorums reduce tail latencies -- though it can result in more synchronization being necessary (marginal concern imo) . 2f+1 is not needed, since that's for equivocation. }. Consecutive proposals are chained via hashes to transitively prove availability, and pipelined \fs{(with certificate forwarding)} to minimize latency. \fs{do we need more detail than this here?  less? }

Note, that our dissemination layer is unstructured and best-effort: it does not causally relate independent lanes, and makes no guarantees whether or not a lane can fork. We rely on a logically separate consensus layer to decree a consistent total ordering. \fs{maybe talk about what this async data dissemination layer gives us?}

\paragraph{Embedded consensus instances. }


embed consensus into the async data layer -- has provable broadcast structure!
Avoids redundancy
Free to implement any protocol. E.g. have a fast path for optimal consensus latency

Simple construct: ticketing, start next view.


\paragraph{Parallel consensus. }
run multiple instances in parallel to minimize end-to-end latency (no wait time/sequential latency)
pipeline so they are not wasteful. 
Do consensus on slots;
Finish all slots; view changes handover.

In practice only a few instances open; can bound to be k ahead of latest commit (include cert from slot x-k)


\fs{TODO: Summary how the whole thing ties together: }
throughput: multi-proposer -- maxing out; arbitrarily scalable with orthogonal worker layer
Latency:  3md Fast path, 5 slow path. Could also use all to all. minimal sequential wait time, consensus instances overlap
Robustness: no new instances for a while (k open ones are stuck view changing). When the next new instance opens, it proposes the newest tips (organic batching) => data dissemination was async (can include TX verification). => no backlog. Get a bump in Tput that balances out the dip. And latency recovers seamlessly. 

\fs{I feel like we can have a separate section (at the end of the protocol description, where we describe the Hotstuff instantiation. } Could also pipeline if we used Hotstuff (e.g. each leader only does one provable broadcast, and the next one starts either with the QC, or just the proposal)

~\\
\fs{TODO: Summary of system performance + overall contributions}
- comparable tput to Bullshark
- but lower latency
- robust behavior to asynchrony  (compare against Hotstuff)

~\\
Contributions:
- (maybe some new definitions: better latency metric, characterization of the async robustness)
- Autobahn design
- Autobahn systems


~\\
\fs{TODO: Think about worst case latency:}
Worst case: Async and k honest leaders. All proposed something that was agreed on, but then time out during cert generation/forwarding. Then new instance (with max tips) won't start until one instance finishes (so there is 1 sequential latency here).  (worst worst case: f faulty ones amongst k, so you wait f+1)
-> In View Change: if there is a decision in the VC quorum, then one needs one Provable Broadcast to commit that decision. If there is none, it's the same. But if we want to add new tips, then we turn it into a full consensus (2 PVB) again. That slightly increases the wait for the next slot -- but it doesn't matter: if the replica was honest, then it proposed new data (that might subsume the next slot); if it was byz, we'd VC ANOTHER round anyways.


%%%%%%%%%%%%%% OLD %%%%%%%%%%%%%%%%%%%%%%
\iffalse
For robustness you need asynchrony, for low latency you need partial sync.

1) Traditional BFT: latency -- lacks tput: leader bottleneck; robustness: after async large backlog (metastable)
2) Multileader BFT: latency, tput (more complexity); lacks robustness
3) Async BFT: robustness -- lacks latency: pessimistic network model
4) Partially sync DAG BFT: tput, robustness (simplicity) from parallel and async data dissemination -- lacks latency: comes from async; uses Dag as clock. Suffers from too many rounds + sequential latency.
\fi 

\iffalse
\one Autobahn commits with minimal latency: 3/5. Additional Autobahn avoid sequential latencies/ minimizes end-to-end latency by aggressively pipelining (otherwise sequential) successive consensus instances.
\two It achieves high throughput by leveraging multi-leader data dissemination. \three Finally, akin to recent DAG protocols, Autobahn logically separates data dissemination to be asynchronous, and independent -- need to figure out how to say this.

Autobahn resolves these tensions.
Autobahns core ethos is to treat all 3 goals as first priniciples; as opposed to evolving from one corner (which adds limitations, and complexity)
Autobahns key insight is... asynchronous paralell data dissemination + do consensus as soon as there is new data (and not when previous consensus is done)

At a high level, Autobahn achieves this by layering and embedding a partially synchronous pipelined/multi-leader consensus mechanism atop an asynchronous data dissemination layer; but instead of inheriting the black box rigid round based design of DAG protocols, we start from scratch ...

Akin to recent DAG protocols, an asynchronous data dissemination layer forms the backbone of the protocol. Unlike them however, data dissemination is not synchronized across replicas (round based DAG puts a "speed limit" on replicas), but fully independent. Each replica disseminates data in it's \textit{own lane}, and \textit{as fast as it can}. To disseminate, a replica uses a provable broadcast (broadcasts it's request, and waits for f+1 replies -- proving that the data is available. (this is a lightweight BCB/RB -- we only care about availability). The next proposal includes a hash reference, and is piggybacked alongside the previous cert. 


Consensus takes as input the tips of each lane. The leader simply proposes it's locally visible frontier (a snapshot cut of all lanes). Consensus itself is embedded into the data dissemination -- we just change the Quorums to be of size 2f+1. We embed a PBFT like version (with a fast path), but any consensus protocol that can be built with provable broadcast building blocks can be embedded. e.g. hotstuff.

A simple version \fs{I think it might be viable to explain a modified Sailfish version} starts the next consensus slot after the previous one is done -- with a Ticket: Commitment of previous one, or View Change. (The ticket could be external, or embedded in another data proposal). However, this incurs sequential latency. 
Our improved version implements parallel consensus: The next consensus instance starts as soon as there is "new" data. We wait for previous proposal, and have to be newer across n-f. 
Since we parallelize, slots must wait for each other.

View change. Move instance to new leader. One leader might deal with multiple instances. If instance didn't agree on anything yet, can propose NEW tips -- seamless (didn't "lose" any time).

In practice only a few instances active.
Wait for k instances behind to be caught up (done) before starting next

Throughput: multileader -- maxing out; arbitrarily scalable with orthogonal worker layer
Latency:  3md Fast path, 5 slow path. Could also use all to all. minimal sequential wait time, consensus instances overlap
Robustness: no new instances for a while (k open ones are stuck view changing). When the next new instance opens, it proposes the newest tips (organic batching) => data dissemination was async (can include TX verification). => no backlog. Get a bump in Tput that balances out the dip. And latency recovers seamlessly. 

Worst case: Async and k honest leaders. All proposed something that was agreed on, but then time out during cert generation/forwarding. Then new instance (with max tips) won't start until one instance finishes (so there is 1 sequential latency here).  (worst worst case: f faulty ones amongst k, so you wait f+1)
-> In View Change: if there is a decision in the VC quorum, then one needs one Provable Broadcast to commit that decision. If there is none, it's the same. But if we want to add new tips, then we turn it into a full consensus (2 PVB) again. That slightly increases the wait for the next slot -- but it doesn't matter: if the replica was honest, then it proposed new data (that might subsume the next slot); if it was byz, we'd VC ANOTHER round anyways.



\fs{I feel like we can have a separate section (at the end of the protocol description, where we describe the Hotstuff instantiation. } Could also pipeline if we used Hotstuff (e.g. each leader only does one provable broadcast, and the next one starts either with the QC, or just the proposal)












to allow a new consensus round to begin \textit{as soon as} there are new requests available (rather than waiting for previous consensus to finish




\section{Intro Brainstorm Notes}
- want three things: low (end-to-end) latency, high tput, robustness to async (explain each)
- tension between the three. (show that no protocol does well in all 3)

- try to characterize fundamental shortcomings of other multi leader protocols:
\begin{itemize}
    \item Dag started from async (retrofit psync). Failed to realize data dissemination and consensus are two parts of the same coin. - current state is result of evolution: needed clock for async; kept it in psync. Has benefits (no TO) but comes at cost of latency. 
    \item Mir doesnt have data dissemination layer; suffers from robustness. - can't change existing systems; need to start from scratch. (Could layer dissemination layer like in Narwahl + HS; but that introduces redundancies. -> BBCA ledger is probably the "design from scratch" verison. Mir takes blackbox psync, and runs n parallel instances 
    \item Both start from a Base, and are forced to work around it. We start form clean base.
\end{itemize}



\fs{We want three things: High tput, Low (end-to-end) Latency, and async responsiveness}
\fs{No existing system can do all, they each get at most 2}
\fs{we describe a new system, Autobahn, that gets all 3.}
\fs{it achieves this by layering a partially sync consensus on an async data dissemination layer ==> need to find a much more compelling way to describe this}

high-level tlrd/name:
- each replica disseminates data in it's own "lane", as fast as it can
- we embed consensus onto some of the broadcasts to occasionally take a snapshot of all lanes => we flatten this into a log. 
\fs{testing}

\begin{itemize}
    \item Traditional leader-based partially synchronous BFT (like PBFT) is not sequential and has low latency 
    \item Drawbacks: 1) Leader is a bottleneck for disseminating large batches and 2) throughput severely drops under asynchrony
    \item We want to decouple data dissemination from consensus using the bandwidth available from all replicas
    \item Also want to have data dissemination to be asynchronous so throughput doesn't drop under asynchrony, it must satisfy a property we call async responsive throughput
    \item Decoupling data dissemination from consensus naively (using black boxes) adds redundancy and latency since they do similar work
    \item Our design (key idea?): make consensus and data dissemination completely logically independent but have them share the same physical messages
    \item Trying to combine data dissemination with consensus in this way has the following challenges:
    \begin{enumerate}
    \item How to avoid unwanted synchronization between consensus and data dissemination (don't want consensus to wait on data dissemination or vice versa)
    \item How to combine a partially synchronous consensus protocol with an asynchronous data dissemination layer without making the data dissemination layer also partially synchronous
    \item How to avoid committing stale data without making consensus completely sequential
    \end{enumerate}
    \item Prior work (DAGs, multiple leader BFT) try to solve some of these issues but they suffer from one or more of:
    \begin{enumerate}
        \item No async responsive throughput
        \item Redundant work between consensus and data dissemination (high latency)
        \item Sequential latency
        \item Unwanted synchronization between consensus and data dissemination
    \end{enumerate}
    \item Can we have it all?
    \item Question: Can we design a BFT system that has low (non-sequential) latency while also having high (async responsive) throughput?
    
\end{itemize}

\fi

==> Sections/2-Psync/partial_synchrony.tex <==
\section{Partial Synchrony: Theory meets Practice}
\label{sec:psync}
\neil{I think we should refocus on the good vs bad/not-good intervals. Bad intervals are caused by faulty leaders, partial network partitions, DDoS, etc., which cause hangovers during good intervals. We argue that intervals are not always good but rather transition frequently between good intervals and bad intervals for the above reasons. Existing work either optimizes for good intervals recovering poorly from bad intervals or optimizes recovery from bad intervals but poor performance during good intervals.}\fs{agree!}
%\section{On the quest for \textit{Partial} Synchrony}
%\ia{I like this section! My main comment is perhaps to consider defining "practical partial synchrony" in which there are two additional factors (1) the times of synchrony and asynchrony fluctuate AND (2) there is a constant stream of client requests over time that does not stop during asynchrony. I think that the problems mentioned in this section and their solution need BOTH these conditions to hold and in the current writeup the second is implicit - I would make it explicit and part of the model. The motivation could be that these systems need to be able to handle workloads that continue to request even during asynchrony - otherwise if there are no requires during asynchrony then the hangover is not as significant...  }\fs{good point. For now I just added a footnote making this assumption explicit when talking about Backlogs in traditional BFT}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% RE-WRITE %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
This work is premised on a simple observation: partially synchronous \changebars{BFT}{} protocols today do not \textit{practically} tolerate periods of asynchrony \fs{we mean "progress interruptions"}. Partial synchrony is an appealing theoretical model that captures when consensus protocols can still achieve liveness, in spite of the seminal FLP impossibility result~\cite{fischer1985impossibility}. All partially synchronous protocols are live when the partially synchronous network reaches the Global Stabilization Time (GST), from which point all messages all be delivered within $\Delta$ time~\cite{dwork1988consensus}. While useful for proving liveness, this model does not accurately describe how real networks work \changebars{, and does not account for the impact of Byzantine actors.}{}\fs{can mention eventual synchrony (theoretical) vs partial synchrony (practical)}. 

\par \textbf{Timeouts \& Asynchrony.}
% The partial synchrony that real network experience, however, looks quite different: it manifests in periods of “good” network behaviour, interspersed by regular network blips.  These blips can be of two form: consensus blips and full blips. Consensus blips cause timeouts to trigger but do not necessarily stall data dissemination, while full blips halt all communication between nodes.  Blips can stem from malicious leaders that artificially delay consensus messages, partial network partitions, or run-of-the-mill latency fluctuation. 

\changebars{In practice, partially synchronous protocols must rely on (exponentially increasing) timeouts in order to simulate periods of synchrony.
However, setting accurate timeouts is a notoriously hard challenge~\cite{tennage2023quepaxa, spiegelman2023shoal, liu2023flexible}. Too high, and the protocol too is slow to respond to faults. Too low, and even common network fluctuations break progress.
From the perspective of the protocol, all timeout violations (and most failures) are indistinguishable from asynchrony. In the following, we will thus use “periods of asynchrony” interchangeably to mean “lack of consensus progress caused by faults or violation of timeouts” (or short, a “blip”). Blips can stem from malicious leaders that artificially delay consensus messages, partial network partitions, or run-of-the-mill latency fluctuation.}{} \fs{our focus is on the EFFECT ("asynchrony"), not the cause (network fluctuations/leader failures)}

%All timeout violations (and most failures) are, from the perspective of the protocol, indistinguishable from asynchrony.



\changebars{We submit that periods of asynchrony are not only inevitable in modern BFT deployments, but intrinsic to the fault model. 
For one, Byzantine failures and adversarial network compromises are expected by design; unlike Crash Fault Tolerant systems, asynchronous periods in BFT are \textit{not exclusively} attributable to the network. Replicas may be malicious, or targeted for compromise, ddos attacks, or route hijacking, resulting in loss of consensus progress. Recent work demonstrates that targeted network attacks on leaders are surprisingly easy to mount and may cause acute liveness concerns~\cite{consensus-dos}.}{}
\fs{todo: move away from this... magnitutde is not high enough to warrant worry regarding timeouts. More reasonably would be to quote temporary partitions.}
Second, message delays due to intermittent network failures or packet queuing are frequent; WAN latencies are unpredictable and can vary by order of magnitudes \cite{hoiland2016measuring}, and many RPCs have been showed to suffer from high tail latency~\cite{dean2013tail, seemakhupt2023cloud}\fs{add: blockchains are deployed in WAN where latencies are often unpredictable? Quote from MyTumbler}. \changebars{Likewise, partitions can happen...? Is this something we can cite?}{}

In short, \changebars{practical deployments}{modern networks} are truly partially synchronous: most messages will arrive within $\Delta$ most of the times, but not always. 
%There will be periods of asynchrony in which the network behaves poorly. 

\par \textbf{Reasoning about Robustness.}
To properly assess the performance of a partially synchronous system, we should consider how it behaves \textit{at all times}, during periods of full synchrony, but also \textit{after} periods of asynchrony.\la{Well said}

While Aardvark introduced the concept of synchronous intervals~\cite{aardvark} when describing the need for robust BFT systems, there does not currently exist a precise way to capture the performance of partially synchronous protocols during synchronous intervals \textit{after} experiencing periods of asynchrony. To this effect, we introduce the dual notions of asynchrony hangovers and seamless partially synchronous protocols. Informally, a partially synchronous protocol is seamless if it does not suffer from protocol-induced hangovers.

% We curtly re-state the terminology introduced by Aardvark for convenience: We say that an execution is \textbf{gracious} if it is \one synchronous (w.r.t. some implementation-dependent timeout on message delay), and \two all clients and servers behave correctly; it is uncivil if up to $f$ servers are Byzantine. To qualify progress, we use the notion of a good interval~\cite{good-case}:

% Synchronous interval: During a synchronous interval any message sent between correct processes is delivered within a bounded delay T if the sender retransmits according to some schedule until it is delivered
% Gracious Exececution: An execution is gracious iff (a) the execution is synchronous with some  implementation-dependent short bound on message delay and (b) all clients and servers behave correctly
% Uncivil: An execution is  uncivil iff (a) the execution is synchronous with some implementation-dependent short bound on message delay, (b) up to f servers and an arbitrary number of clients are Byzantine, and (c) all remaining clients and servers are correct

\par \textbf{Asynchrony Hangovers \& Seamlessness.}
% We first lay some groundwork. We note that all
All deterministic partially synchronous protocols require a coordinator (or \textit{leader}) to propose an input and drive progress; "leaderless" protocols are a misnomer, and typically refer to either \one the use of multiple coordinators driving independent instances in parallel~\cite{gupta2021rcc, stathakopoulou2019mir}, or \two the use of a client as coordinator~\cite{suri2021basil}. Byzantine leaders may establish "progress", but intentionally limit performance; such Byzantine behavior is indistinguishable from \changebars{a slow network}{asynchrony}.
Following Aardvark~\cite{aardvark} and Abraham et al.~\cite{good-case} we say that an interval is \textit{good} if the system is synchronous (w.r.t. some implementation-dependent timeout on message delay), and the consensus process is led by a correct replica; we say it is \textit{gracious} if it is synchronous and all replicas are correct~\cite{aardvark}. \changebars{Intuitively, good intervals capture the periods during which progress is guaranteed.}{}\fs{we could use "bad interval=not good" instead of the confusing "periods of asynchrony" if we wanted to be more precise. That way people might stop getting bogged down on network fluctuations.}
Given this, we define:
\begin{definition}
    An \textbf{asynchrony hangover} is any performance degradation that is caused by a period of asynchrony, and persists beyond the return of a good interval. 
    % \nc{Is there some acceptable delay T, or do we assume that it should "immediately" resume?}\fs{I'm not opposed to the T.  I think "immediately" is impossible, hence the discussion about "quasi-seamlessness". My worry is that picking some T to compare protocols under is not very principled}
\end{definition}

Asynchrony hangovers impact both throughput and latency. We characterize a throughput hangover as the duration required to commit all outstanding requests issued before the start of a good interval. If the provided load is below the system's steady-state throughput, the system will eventually recover all throughput "lost" during asynchrony.\footnote{If the load is equal/greater to the throughput, then the lost committed throughput (or \textit{goodput}) can never be recovered.} The longer the hangover lasts, the more severe it is.
Delayed throughput recovery can, in turn, materialize as increased latency even for commands issued \textit{during} a good interval. Assuming FIFO priority, such commands experience the latency required to first commit both the backlog formed during asynchrony, and the perpetuated backlog induced by new waiting commands. 
\fs{Note: It may be app specific how important or "socially acceptable" a hangover is}
Hangovers can cause not only immediate headaches, but also make the system more susceptible to future asynchronous bumps in the road. Good intervals may not last forever, and unresolved hangovers can add up---and continue indefinitely.

% are subject to compound \fs{"compound" the right choice of word?} further--in the worst case continuing in perpetuity. % akin to a meta-stable failure~\cite{huang2022metastable, bronson2021metastable}. \fs{this isn't really precise, since the trigger comes back}

In a hangover-free system, all submitted requests whose progress is interrupted by asynchrony commit instantaneously when progress resumes; further, these are the only requests that experience a hike in latency, and for no more than the remaining duration of the asynchronous period. 

% Put differently, performance during good intervals must be \textit{independent} of the  duration of preceeding asynchrony.

\fs{Massage definition/section: Seamless should only capture what is in our control. I.e. it should refer to hangovers caused by "protocol mechanisms" (not by things like data bandwidth) => Recovery from asynchrony should be instant (subject to data constraints). 
Asynchrony "ends" when all data has arrived at honest.}

\par \textbf{Practical Limits.} Careful protocol design cannot of course eliminate all hangovers, {\em e.g.}, those due to insufficient network bandwidth or to bottlenecks caused by message deliveries, but it can avoid introducing unforced ones. \changebars{No \textit{consensus} protocol, not even asynchronous ones, can provide progress beyond the pace of the network. Without new data being disseminated, there is nothing to agree on.}{} 
% Not all hangovers are avoidable at a protocol level. We can, for instance, not overcome network limitations such as data bandwidth capacities, or bottlenecks caused by message deliveries. We can, however, strive to avoid hangovers caused by protocol design considerations.
\changebars{For instance, hangovers caused by a slowdown of the network pace below the request input rate will inevitably form a backlog; avoiding such requires admitting fewer client proposals and is beyond the scope of the consensus protocol. We can, however, strive to avoid frictions caused by protocol-level mechanisms such as timeouts: data dissemination, for instance, need not be subject to timeouts, and should continue at the available network pace.}{} 
\changebars{We thus distinguish two forms of blips: consensus blips and full blips. Consensus blips cause timeouts to trigger but do not necessarily stall data dissemination, while full blips may arbitrarily impact (e.g. halt) communication between nodes.}{}
\changebars{We say that a partially synchronous protocol behaves optimally, or \textit{seamlessly}, if it experiences no asynchrony hangovers caused by only \textbf{consensus blips}.}{Thus, we say that a partially synchronous protocol behaves optimally (w.r.t to periods of asynchrony), or \textit{seamlessly}, if it experiences no asynchrony hangovers solely due to consensus protocol design choices.}

%Thus, we say that a partially synchronous protocol behaves optimally (w.r.t to periods of asynchrony), or \textit{seamlessly}, if it experiences no asynchrony hangovers solely due to consensus protocol design choices.
\fs{a consensus protocol can be seamless without the system being seamless!}
\begin{definition}
\fs{Some reviewers complained "protocol mechanisms" is too vague}
    %A partially synchronous system is \textbf{seamless} if it is free of protocol mechanisms subject to asynchrony hangovers. 
    \changebars{A partially synchronous system is \textbf{seamless} if it is not subject to asynchrony hangovers that are caused by consensus blips only. }{A partially synchronous system is \textbf{seamless} if it is free of protocol mechanisms subject to asynchrony hangovers.}
\end{definition}

\changebars{Seamlessness is a desirable property for any partially synchronous consensus protocol, yet it is especially important for BFT protocols as Byzantine leaders may produce hangovers by simply not participating, thus negatively impacting performance \textit{beyond} their tenure. This, we find, is at odds with the \textit{Byzantine fault tolerant} tenet: BFT protocols should be robust to Byzantine faults~\cite{aardvark}.}{} \fs{cite Aardvark Robustness doctrine}

\fs{Other things we could }

%%%%%

\par \textbf{Analysis of existing approaches.}
Traditional BFT protocols\cite{castro1999pbft, yin2019hotstuff} are not seamless. They disseminate batches of requests and reach consensus on each batch independently; \fs{Note: I am intentionally not specifying whether batches are sent alongside consensus -- this does not matter}the number of consensus instances required to commit all requests is directly proportional to the input rate of requests divided by the batch size. Consequently, the time required by these protocols to process the backlog accumulated during progress-free (asynchronous) intervals is in the order of the backlog's size--assuming continuous client load.
%We demonstrate empirically in \S\ref{sec:eval} that Hotstuff~\cite{yin2019hotstuff}, for instance, suffers a latency hangover. 

We demonstrate empirically in Fig. \ref{fig:hangover} that Hotstuff~\cite{yin2019hotstuff}, for instance, suffers a latency hangover because it is bottlenecked by the (processing) bandwidth of each proposal (\S\ref{sec:eval}). % (we defer to \S\ref{sec:eval} for a more detailed discussion).
\begin{figure}[h!]
    \vskip -2pt
   \centering
   %\includegraphics[width=0.45\textwidth]{Figures/consensus.pdf}
   \includegraphics[width=0.38\textwidth]{Figures/eval/hangover-blips-intro-cut-visibility.pdf}
   %{Figures/eval/hangover-blips-intro-cut.pdf}
   \vskip -4pt
   \caption{Latency Hangover (nearly 4 seconds) in Hotstuff~\cite{yin2019hotstuff} following a 3 second blip (e.g. leader failures).}
   %\caption{Core Consensus coordination pattern. Messages may be piggybacked on existing cars (\S\ref{sec:ride_sharing}): P1 = \textsc{Prepare}, P2 = \textsc{Confirm}, C = \textsc{Commit}.}
   \label{fig:hangover}
   \vskip -0pt
\end{figure}


Simply proposing larger batches is not a viable option for reducing the number of required agreement instances as it comes at the cost of increased latency in the common case.
Similarly, a straightforward decoupling of dissemination and consensus (proposing only a batch digest)~\cite{bagaria2019prism, danezis2022narwhal}\fs{this is what the HS baseline does; it starts dropping messages at some point} %or tiered batching (proposing batches of "mini-batches")~\cite{danezis2022narwhal} 
can alleviate data transfers and request verification on the critical path of consensus, \changebars{but does not address the princal concern.}{but the fundamental complexity remains proportional to the backlog.} \changebars{Such designs are consequently unable to robustly scale throughput beyond the leader dissemination capacity; we confirm this empirically in \S\ref{sec:eval}.}{} \fs{our experiments of batchedHS show that separating dissemination just blindly is not enough - not only is it not robust during async, but it doesn't seem to hold up under high load}
\fs{I changed the argument from being about the size of a proposal growing proportionally to the number of consensus instances required -- I think the batch-latency tradeoff is much more obvious}
%but not the principled concern. 

A class of recent DAG-based BFT protocols~\cite{danezis2022narwhal, Bullshark}, in contrast, is seamless. \fs{not all are seamless: the un-certified ones like Cordial are not} These protocols decouple data dissemination and consensus, and construct an asynchronously growing DAG consisting of data batches chained together. The construction leverages Reliable Broadcast to generate proofs that transitively vouch for data availability and request verification of \textit{all} topologically preceding batches in the DAG. The consensus mechanism can commit entire backlogs with constant cost by proposing only a single batch, and thus experiences complexity \textit{independent} of asynchronous durations. Unfortunately, existing seamless DAG-BFT protocols exhibit, during {\em good} intervals, up to twice the latency of traditional BFT protocols. \fs{Can talk about why, but I think this is not the right place.}\fs{The root cause is that consensus is hardwired into the structure of the DAG. This allows neither to go as fast as they'd like. Each round of consensus is mapped to one RB (best case)} To bridge the gap, we propose \sys{}, a novel high throughput BFT protocol that delivers low latency during synchrony and handles \textit{partial} synchrony seamlessly.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% OLD VERSION %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\iffalse
No deterministic protocol can guarantee both safety and liveness under asynchrony~\cite{fischer1985impossibility}. Partial synchrony, is a powerful and convenient model that allows us to build practical systems: safety is guaranteed always, while progress guarantees are limited to periods of synchrony.
The dominant partial synchrony model in BFT assumes an eventual Global Stabilization Time (GST) after which synchrony is forever on guaranteed. This model simplifies both the explanation and proofs of consensus protocols, yet is unrealistic in real deployments~\cite{liu2023flexible}. \fs{why? maybe talk a bit about timeouts. All psync protocols need them. But they're "hard"/impossible to set "correctly" in asynchrony. Too low, and we get spurious async periods; too high, and we don't respond timely to failures}\neil{Yeah we can also say that systems that assume this unrealistic model have no incentive to care about the impact of asynchrony since it never returns after synchrony (essentially a one time problem).} \fs{can also reference MyTumbler experience on WAN deployments}
\nc{We say it's unrealistic in real deployments, we don't say what the consequences are. One way to interpret what you're saying is that the protocols aren't actually live. The other way to interpret this is that the protocols are live, but perform horribly. We want to distinguish between the two early. }

This paper argues, that asynchronous periods are not fringe outliers, but constitute a core part of a partially synchronous protocol's common case. It is therefore imperative to take into account, and characterize the impact that asynchrony has on the performance of partially synchronous protocols. While we are typically primarily interested in the pragmatic metrics of latency and throughput, we ought to also analyze the \changebars{robustness}{ \textit{quality}} of performance in the presence of recurring asynchrony. 

During asynchrony, there is no progress, and hence performance is void. But \textit{how fast}, at \textit{what rate}, and \textit{how well} do we regain performance \textbf{after} progress returns?

\nc{I would be a lot more direct in this first two paragraphs. SUGGESTED REWRITE:

This work is premised on a simple observation: partially synchronous protocols cannot practically tolerate periods of asynchrony. Partial synchrony is an appealing theoretical model that captures when consensus protocols can still achieve liveness, in spite of the seminal FLP impossibility result. All partially synchronous protocols are live when the partially synchronous network reaches the Global Stabilization Time (GST), at which point all messages will be delivered within $\Delta$ time. While useful for proving liveness, this model does not accurately describe how real networks work. Message delays due to intermittent failures, packet queuing are frequent; most RPCs for instance suffer from high tail latency (or other example)~\cite{dean2013tail,rpcpaper, liu2023flexible}. Setting accurate timeouts is similarly a notoriously hard challenge~\cite{tennage2023quepaxa}. In short, modern networks are truly partially synchronous: most messages will arrive within $\Delta$ most of the times, but not always. There will be periods of asynchrony in which the network behaves poorly. To properly assess the performance of a partially synchronous system, we should consider how it behaves \textit{at all times}, during periods of full synchrony, but also \textit{after} periods of asynchrony.

While Aardvark introduced the concept of synchronous intervals~\cite{} when describing the need for robust BFT systems, there does not currently exist a precise way to capture the performance of partially synchronous protocols during synchronous intervals \textit{after} experiencing periods of asynchrony. To this effect, we introduce the dual notions of asynchrony hangovers and seamless partially synchronous protocols. Informally, a psync protocol is seamless if it does not suffer from hangovers.}

\nc{To the extent possible, let's reuse the terminology of aadvark, gracious, uncivil, synchronous intervals and let's heavily ack aadvark here to make sure that people don't say "aadvark did it and you don't know about it}

To characterize the quality of performance in partially synchronous protocols we introduce the dual notions of an \textbf{asynchrony hangover}, and a \textbf{seamless partially synchronous protocol}. \fs{NC: loosely inspired by/rooted in principles of control theory?}
As a prerequisite, we note that a Byzantine leader could establish "progress", but intentionally limit performance; we classify Byzantine behavior to be indistinguishable from asynchrony. We thus say that an interval is \textit{good} if the system is synchronous (w.r.t. some implementation-dependent timeout on message delay), and the consensus process is led by a correct replica~\cite{good-case}\footnote{A replica \textit{leads} consensus if it determines the initial input proposal.}\fs{this is the first mention of a leader; can we take it for granted? All deterministic psync protocols must have a leader}; we say that it is \textit{gracious} if all replicas are correct~\cite{aardvark}. Given this, we define:
\nc{We probably want to be specific about what it means for a consensus process to be "led by a correct replica". I know you claim that there is always some form of leader in a psync deterministic protocol, but I worry that this opens up to "what about leaderless protocols, what about multileader protocols}
\nc{Let's maybe reintroduce the definitions of good and gracious as explicit definitions, even if we cite the others}

\fs{TODO: Tweak definition to account for subtle distinction: \sys{} gets seamlessness as soon as there is a new SLOT lead by an honest leader. I.e. put differently: slot instances that were started before or during async have no guarantee of eliminating the hangover -> after all, they might have to commit old tips that were proposed BEFORE getting back to synchrony. E.g. an unfinished slot might view change to an honest replica which has to re-propose the old proposal. This should not be treated as "leading consensus process", the replica is merely "orchestrating recovery". "Leading" should be defined as deciding (on its own) what the proposal should be. => for now I made it a footnote}

\begin{definition}
    An \textbf{asynchrony hangover} is any performance degradation that is caused by a period of asynchrony, and persists beyond the return of \changebars{a good interval.}{consensus progress.} %\fs{more precise: beyond the first HONEST commit.}
    \nc{Is there some acceptable delay T, or do we assume that it should "immediately" resume?}\fs{I'm not opposed to the T.  I think "immediately" is impossible, hence the discussion about "quasi-seamlessness". My worry is that picking some T to compare protocols under is not very principled}
\end{definition}
    

\fs{more rigorous: degradation should be "measured" with respect to the async free case. I.e. which requests would experience different performance under the two cases. I.e. should only look at the "set" of Tx that would've committed without async? Can't talk about the ones that wouldn't be committed anyways (e.g. orphan nodes in DAG/or tips that weren't included) -> those don't have a "hangover"}

We illustrate the concept of asynchrony hangovers for the closely intertwined throughput and latency metrics; we defer a more rigorous analysis of other possible types of asynchrony hangovers to future work.
\nc{Make the sentence more direct. Asynchrony hangovers have an impact on both throughput and latency. A throughput hangover is the duration all commands started outside of a synchronous period (tried to make it more precise than delayed by asynchrony, though I'm realising now i'm making it too strong because i'm including commands proposed by a byz leader}

\par We denote a \textbf{throughput hangover} as the duration required to commit all load whose progress was delayed by asynchrony. Assuming the provided load is below the steady-state throughput the system can offer, the system will eventually recover all throughput "lost" during asynchrony.\footnote{If the load is equal/greater to the throughput, then the lost committed throughput (or \textit{goodput}) can never be recovered.} The longer it takes, the more severe the hangover. \fs{we want this horizon to be short, else by the next async blip we build even more backlog and so on, until we can never recover the tput. It's tricky to talk about this as tput problem in isolation. It's so closely intertwined with latency} \fs{the time it takes to address my tput deficit is a window of vulnerability. The longer it is, the longer there is a possibility of conflict with another event (e.g. async/faults) that further extends. It weakens the system to faults}\nc{I'm not entirely sure the point that you're trying to make here comes through. At least what your'e saying in comments doesn't seem to be the same as hwat you're saying in the text}\fs{we are still discussing; the old text does not yet reflect the new comments. What is the best way to describe it?}
In a throughput hangover-free system, all load submitted -- whose progress is interrupted by asynchrony -- commits instantaneously upon return of progress. \changebars{}{If we "zoom out", the amortized throughput over a period of measurement should be equivalent to that of a system with continuous progress; as though asynchrony never occurred.}
\fs{This is essentially our "async resp tput" but in a more general formulation. Likewise for latency below: "seamless"/metastable-free latency we were talking about} \fs{in a way, the async resp tput is just a latency property though... }
\neil{Yeah I like the way you have talked about this, especially the window of vulnerability.}
\neil{I agree the throughput hangover is very closely related to latency. In fact one can argue that having a throughput hangover implies that you must also have a latency hangover (from the backlog of requests). And similarly you would only have a latency hangover if you had a throughput hangover (if there's no backlog then the latency won't increase)}\fs{exactly: tput and latency don't exist separately. Latency at 1 tput means nothing, just as 1m tput at 100s lat.}
\nc{What's the benefit then of separating them out?} \fs{maybe none. I only came up with the theory of hangovers while writing them out.. we can change it!}

\par A \textbf{latency hangover} $h$ materializes as either \one increased latency (w.r.t to the expected latency under synchrony) for requests that were issued after \changebars{resuming a good interval}{progress returns} ($Lat(req) = E(Lat) + h)$)
\nc{Shall we express this in terms of synchronous intervals instead? Notion of "progress" can be vague}\fs{yes, changed it. Wrote the text before formalizing good intervals}, or \two increased latency \textit{beyond} the asynchrony duration for requests issued before or during the period of asynchrony ($Lat(req) = E(Lat) + duration_{async} + h)$). Put differently, in a latency hangover-free system, only the requests whose progress is interrupted by asynchrony experience a hike in latency; and no more than the duration of the asynchronous period. \fs{more precise would be: if a req is input half way through async, then the hike is only the remainder...}

We say that a partially synchronous system behaves optimally w.r.t to periods of asynchrony, or \textit{seamlessly}, if it experiences no asynchrony hangovers.
%We note, that a byzantine leader could establish "progress", but intentionally limit performance; we classify such byzantine behavior to be indistinguishable from asynchrony, and understand a seamless protocol to be one that does not incur hangovers beyond an \textbf{honest} leaders tenure (after the return of synchrony).

\fs{Massage definition/section: Seamless should only capture what is in our control. I.e. it should refer to hangovers caused by "protocol mechanisms" (not by things like data bandwidth) => Recovery from asynchrony should be instant (subject to data constraints). Asynchrony "ends" when all data has arrived at honest.}

\begin{definition}
    A partially synchronous system is \textbf{seamless} if it is not subject to asynchrony hangovers.
\end{definition}
\fs{other name suggestions. NC: a psync system is "young" if it doesn't get hangovers. Periods of asynchrony are blips or "binges"}

\fs{Note: Seamless refers only to the consensus protocol. The application layer may of course not deal seamlessly with a large backlog of load if it is overloaded. For our purposes however, we assume application layer (execution) has infinite tput, i.e. consensus is not bottlenecked by execution -- more consensus tput == better.}
A seamless (hangover-free) protocol, must commit any proposals that \textit{would have} committed under synchrony -- but did not due to a period of asynchrony -- as soon as progress is restored \fs{kind of redundant with previous sentence on tput}, and without affecting performance of all other proposals. In practice, this demands in particular that performance (throughput/latency) must be independent from the duration of asynchrony.
\nc{These last two sentences seem redundant with what was said before?}

\fs{TODO: I submit that seamlessness is actually impossible in an async system. One may always miss some data (possibly proportional to async period) due to the nature of having Quorums < n.}
\fs{We instead can strive to be just shy of seamlessness. Define "Quasi-seamless": Only data transfer size is proportional to backlog; message exchange protocol latency should be fixed} \fs{Note: with this definition, existing dag protocols are also not quite quasi-seamless. A replica may still need to recursively learn of parents} \fs{Certified DAGs can sidestep this by using the same trick that we do; they just need to ensure that voting on proposals from the same replica is FIFO.} \fs{Uncertified DAGs cannot. a) must sync during consensus, b) cannot certify Fifo => recursion inevitable}


\fs{Challenge: Distinction between consensus and data dissemination. Why is it important to think about data dissemination? Can be doing consensus just fine, but if you have to recursively get data, then end-to-end latency story. Big problem, not nitty gritty detail.}


\par \textbf{Analysis of existing protocols.}
Traditional BFT protocols \fs{cite the usual bunch} are not seamless. Periods of asynchrony result in the formation of backlogs, whose size is directly proportional to the duration of no-progress \nc{of the asynchronous period}\fs{I speficially didn't say async, because there can be progress in async -- it's just not guaranteed. Unless we want to define asynchrony explicitly as the case in which we time-out/make no progress}.
\nc{Fair. I had been implicitly assuming that asynchrony meant no progress but I see your point}This results in both latency and throughput hangovers as "working off" backlogs requires additional data transfers and request verification on the critical path of consensus. Techniques such as mini-batching (proposing batches of digests of already best-effort disseminated batches), or naive chaining (proposing the head of a hash-chain of best-effort disseminated requests) can ameliorate hangovers, but not sidestep them: they introduce data synchronization proportional to the backlog onto the critical path. \fs{- Simply chaining together proposals is not enough either (that just gives them an order). Need transitive certificates of availability. I.e. best effort broadcasts are not enough! -> i.e. Dahlia's BCCA thing}
\nc{This explanation is too encoded right now}
\nc{Ideally, we'd want a graph in this section that demonstrates this} \fs{@Neil: we can slot in here a nicer version of the poster graph?}
\nc{Traditional BFT protocols don't consider "chains", so talking about chaining is a bit confusing/narrow. We want to identify the "root cause" for why they suffer from this backlog. I think this is where we probably want to "break down" the BFT protocols that exist today in "conceptually" different roles, that are intertwined }

Recent DAG-based BFT protocols \fs{cite Bullshark/Shoal}, in contrast, are seamless. The DAG-construction, driven by series of temporally intertwined Reliable Broadcast's (RB) elegantly generates Proofs of Availability (PoA) that transitively vouch for both data transfer and verification of \changebars{}{large causal histories of} asynchronously disseminated data. As a result, the cost of consensus is \textit{independent} and agnostic to periods of asynchrony; the latest PoA subsumes the backlog. The downside of DAG-based BFT is that consensus is hard-wired into the structure of the DAG. For one, the RB at the core of such protocols provides a property stronger than PoA's, resulting in additional cost. Second, consensus must always account for the \textit{worst-case} \fs{I fear this is too vague and not useful -- but I don't want to write an essay about DAGs here. I do want to however appreciate what they do nicely}, resulting in higher than desirable sunny-day latencies. \neil{Instead of saying consensus must always account for the worst case, I would say something like consensus RBs both proposals and votes} \fs{cannot parse}
\neil{was just trying to say why DAGs have higher sunny-day latencies, and the "simple" reason to me is that they reliably broadcast both the leader's proposal and all other replicas' votes. probably need to workshop this explanation a bit}
To bridge the gap, we propose Autobahn, a novel high throughput BFT protocol that exhibits both low latency during synchrony, and seamlessness under \textit{partial} synchrony.



\fs{TODO?? Define effective latency as well? end-to-end; consensus latency isn't the only thing that matters, but sequential latency is important.}\fs{don't think it's needed here. DAGs and Traditional BFT don't need to worry about "missing" the bus. It's something that we introduce, and then want to make better. (Only Dahlia's BBCA also "needs" it but doesn't think about it)}
 
\nc{High level thoughts, we really want to structure this "Analysis of existing protocol" in a more didactic way/structured way. Given the audience is unlikely to be familiar with everything, we have to "teach" them about the different components, design choices one can make in modern BFT protocols. The relationship between the data dissimination layer and the consensus layer is really waht distinguishes most of the protocols in how they handle asynchronous blips, so we're going to have to conceptually talk about this}

\fi

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% END %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%Resolved: \neil{I think we should define two terms: good-case and common-case. Good-case = honest leader after sync (when liveness is guaranteed for psync protocols) and common case is async/sync conditions. Then we can say an asynchrony hangover is a performance degradation that persists beyond the return of good case conditions} \fs{yeah good idea; I like "gracious" execution defined by aardvark -- although it says that all replicas must be correct, and not just the leader...}. \fs{alternatively: we can early on say that async and byz leader are indistinguishable}

\iffalse
We say that a partially synchronous system is \textit{seamless} when it is not subject to hangovers that last beyond an honest leader. No system can manage under byz leaders => we should could them into the period of asynchrony.

TODO: an optimal system is then: .... hangover free! We call this seamless, because it "seems" as async never happened.

TODO: Discuss what protocols are seamless and which are not:
- DAGs are. Very elegant design in which consensus is just an interpretation. The con is that consensus is "hard-wired" onto the structure. Need to account for the worst-case

- Traditional protocols are not. Backlog means that next honest has to propose a much bigger batch (or a batch of "mini-batches). This requires coordination proportional to the duration of asynchrony: a) data transfer, b) request verification, c) synchronization on critical path (in case of mini-batches). 

- Simply chaining together proposals is not enough either (that just gives them an order). Need transitive certificates of availability. I.e. best effort broadcasts are not enough!



Partial synchrony today, is viewed as primarily theoretical property. The GST model grossly simplifies realistic network behavior in a way that makes it easy to use for proofs. Once we deploy the system in practice however, we don't give it a second look.
we chalk up blips in progress/performance to asynchrony, and call it a day.


However, in partially sync systems, that are run on an asynchronous network (the internet...) asynchrony is part of the common case behavior. Partially synchronous systems should perform optimally when the system is \textit{partially} synchronous.

What does optimal mean? Clearly, it is impossible to have progress in async periods. What we want is "seamlessness"

We define a class of behaviors we call "hangovers"
- latency should be affected exactly by the blip in progress; not more. The moment we return to synchrony, latency should be normal. Req during the period of async should just be normal latency + async period
  => Latency hangover: Latency for requests received after synchrony returns is still affected. (this is imprecise: even the ones "later" during the async period, should only pay the "remaining" async cost_

- tput should be unaffected in amortization. I.e. if we "zoom out" it should look like there are no blibs overall. The total amount of goodput (delivered throughput) should be the same as a system that was always synchronous.
  -- Need to add some more stuff here. This is technically satisfied by a system that doesn't fully use its load (i.e. recovres)
  -- Tput should be back THE moment sync returns. (define as hangover)
  => Tput hangover: Tput


TLDR: No hangovers!!
Define: A partially synchronous protocol is seamless if there are no hangovers.



\fs{Thought: In fact, recent protocols like Bullshark might even guarantee seamlessness even with byz progress (stronger than our definition) by not giving proposers a "free choice" what to propose.. It's not entirely true though: a byz replica can always try to not include previous leader, but its not guaranteed to manage. Imo that fits our bill of "changing" what could've been proposed... but it's tricky)  }
\neil{Not sure exactly what you mean here, still think it doesn't guarantee seamlessness with byz because byz leader could just refuse to propose anything?}\fs{yep lol, forgot :D Resolved.}
\fi

==> Sections/2-Psync/partial_synchrony_new.tex <==
\section{Partial Synchrony: Theory meets Practice}
\label{sec:psync}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% RE-WRITE %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
This work is premised on a simple observation: partially synchronous BFTprotocols today do not \textit{practically} tolerate periods of asynchrony \fs{we mean "progress interruptions"}. Partial synchrony is an appealing theoretical model that captures when consensus protocols can still achieve liveness, in spite of the seminal FLP impossibility result~\cite{fischer1985impossibility}. All partially synchronous protocols are live when the partially synchronous network reaches the Global Stabilization Time (GST), from which point all messages all be delivered within $\Delta$ time~\cite{dwork1988consensus}. While useful for proving liveness, this model does not accurately describe the effects real networks may experience, and does not account for the impact of Byzantine actors\fs{can mention eventual synchrony (theoretical) vs partial synchrony (practical)}. 

\par \textbf{Timeouts \& Asynchrony.} In practice, partially synchronous protocols must rely on (exponentially increasing) timeouts in order to simulate periods of synchrony. Unfortunately, setting accurate timeouts is a notoriously hard challenge~\cite{tennage2023quepaxa, spiegelman2023shoal, liu2023flexible}. Too high, and the protocol too is slow to respond to faults. Too low, and even common network fluctuations break progress.
From the perspective of the protocol, all timeout violations (and most failures) are indistinguishable from asynchrony. 
\fs{our focus is on the EFFECT ("asynchrony"), not the cause (network fluctuations/leader failures)}
In the following, we will thus use “periods of asynchrony” (or short, a “blip”) to capture all sources of consensus interruptions. 
%blips can stem from malicious leaders that artificially delay consensus messages, partial network partitions, or run-of-the-mill latency fluctuation. 
Blips can originate for a multitude of reasons and are, we submit, inevitable in modern BFT deployments.
On the one hand, Byzantine failures and adversarial network compromises are intrinstic to the fault model and expected by design; blips are \textit{not exclusively} attributable to the network. Replicas may be malicious, or targeted for compromise, ddos attacks, or route hijacking, resulting in loss of consensus progress. Recent work demonstrates that targeted network attacks on leaders are surprisingly easy to mount and may cause acute liveness concerns~\cite{consensus-dos}.
%\fs{todo: move away from this... magnitutde is not high enough to warrant worry regarding timeouts. More reasonably would be to quote temporary partitions.}
%message delays due to intermittent network failures, or packet queuing are frequent
On the other hand, non-malicious network events are common; Wide area network (WAN) latencies are unpredictable and can vary by order of magnitudes \cite{hoiland2016measuring}, and many RPCs have been showed to suffer from high tail latency~\cite{dean2013tail, seemakhupt2023cloud}. Furthermore, participants in today's blockchain systems often exhibit asymmetric hardware, network resources, and configuration experience, complicating configurations and resulting in frequent interruptions \cite{priv-com-aptos-mysten}.

%\fs{add: blockchains are deployed in WAN where latencies are often unpredictable? Quote from MyTumbler}. \changebars{Likewise, partitions can happen...? Is this something we can cite?}{}


In short, \changebars{practical deployments}{modern networks} are truly partially synchronous: most messages will arrive within $\Delta$ most of the times, but not always. 

% We submit that periods of asynchrony are not only inevitable in modern BFT deployments, but intrinsic to the fault model.
% The partial synchrony that real network experience, however, looks quite different: it manifests in periods of “good” network behaviour, interspersed by regular network blips.  These blips can be of two form: consensus blips and full blips. Consensus blips cause timeouts to trigger but do not necessarily stall data dissemination, while full blips halt all communication between nodes.  Blips can stem from malicious leaders that artificially delay consensus messages, partial network partitions, or run-of-the-mill latency fluctuation. 
%There will be periods of asynchrony in which the network behaves poorly. 

%\par \textbf{Reasoning about Robustness.} 
To properly assess the performance of a partially synchronous system, we should consider how it behaves \textit{at all times}, during periods of full synchrony, but also \textit{after} periods of asynchrony.

While Aardvark introduced the concept of synchronous intervals~\cite{aardvark} when describing the need for robust BFT systems, there does not currently exist a precise way to capture the performance of partially synchronous protocols during synchronous intervals \textit{after} experiencing periods of asynchrony. To this effect, we introduce the dual notions of asynchrony hangovers and seamless partially synchronous protocols. Informally, a partially synchronous protocol is seamless if it does not suffer from protocol-induced hangovers.

% We curtly re-state the terminology introduced by Aardvark for convenience: We say that an execution is \textbf{gracious} if it is \one synchronous (w.r.t. some implementation-dependent timeout on message delay), and \two all clients and servers behave correctly; it is uncivil if up to $f$ servers are Byzantine. To qualify progress, we use the notion of a good interval~\cite{good-case}:

% Synchronous interval: During a synchronous interval any message sent between correct processes is delivered within a bounded delay T if the sender retransmits according to some schedule until it is delivered
% Gracious Exececution: An execution is gracious iff (a) the execution is synchronous with some  implementation-dependent short bound on message delay and (b) all clients and servers behave correctly
% Uncivil: An execution is  uncivil iff (a) the execution is synchronous with some implementation-dependent short bound on message delay, (b) up to f servers and an arbitrary number of clients are Byzantine, and (c) all remaining clients and servers are correct

\par \textbf{Asynchrony Hangovers \& Seamlessness.}
% We first lay some groundwork. We note that all
All deterministic partially synchronous protocols require a coordinator (or \textit{leader}) to propose an input and drive progress; "leaderless" protocols are a misnomer, and typically refer to either \one the use of multiple coordinators driving independent instances in parallel~\cite{gupta2021rcc, stathakopoulou2019mir}, or \two the use of a client as coordinator~\cite{suri2021basil}. Byzantine leaders may establish "progress", but intentionally limit performance; such Byzantine behavior is indistinguishable from \changebars{a slow network}{asynchrony}.
Following Aardvark~\cite{aardvark} and Abraham et al.~\cite{good-case} we say that an interval is \textit{good} if the system is synchronous (w.r.t. some implementation-dependent timeout on message delay), and the consensus process is led by a correct replica; we say it is \textit{gracious} if it is synchronous and all replicas are correct~\cite{aardvark}. \changebars{Intuitively, good intervals capture the periods during which progress is guaranteed.}{}\fs{we could use "bad interval=not good" instead of the confusing "periods of asynchrony" if we wanted to be more precise. That way people might stop getting bogged down on network fluctuations.}
Given this, we define:
\begin{definition}
    An \textbf{asynchrony hangover} is any performance degradation that is caused by a period of asynchrony, and persists beyond the return of a good interval. 
    % \nc{Is there some acceptable delay T, or do we assume that it should "immediately" resume?}\fs{I'm not opposed to the T.  I think "immediately" is impossible, hence the discussion about "quasi-seamlessness". My worry is that picking some T to compare protocols under is not very principled}
\end{definition}

Asynchrony hangovers impact both throughput and latency. We characterize a throughput hangover as the duration required to commit all outstanding requests issued before the start of a good interval. If the provided load is below the system's steady-state throughput, the system will eventually recover all throughput "lost" during asynchrony.\footnote{If the load is equal/greater to the throughput, then the lost committed throughput (or \textit{goodput}) can never be recovered.} The longer the hangover lasts, the more severe it is.
Delayed throughput recovery can, in turn, materialize as increased latency even for commands issued \textit{during} a good interval. Assuming FIFO priority, such commands experience the latency required to first commit both the backlog formed during asynchrony, and the perpetuated backlog induced by new waiting commands. 
\fs{Note: It may be app specific how important or "socially acceptable" a hangover is}
Hangovers can cause not only immediate headaches, but also make the system more susceptible to future asynchronous bumps in the road. Good intervals may not last forever, and unresolved hangovers can add up---and continue indefinitely.

% are subject to compound \fs{"compound" the right choice of word?} further--in the worst case continuing in perpetuity. % akin to a meta-stable failure~\cite{huang2022metastable, bronson2021metastable}. \fs{this isn't really precise, since the trigger comes back}

In a hangover-free system, all submitted requests whose progress is interrupted by \changebars{a blip}{asynchrony} commit instantaneously when progress resumes; further, these are the only requests that experience a hike in latency, and for no more than the remaining duration of the asynchronous period. 

% Put differently, performance during good intervals must be \textit{independent} of the  duration of preceeding asynchrony.


\par \textbf{Practical Limits.} Careful protocol design cannot of course eliminate all hangovers, {\em e.g.}, those due to insufficient network bandwidth or to bottlenecks caused by message deliveries, but it can avoid introducing unforced ones. \changebars{No \textit{consensus} protocol, not even asynchronous ones, can provide progress beyond the pace of the network. Without new data being disseminated, there is nothing to agree on.}{} 
% Not all hangovers are avoidable at a protocol level. We can, for instance, not overcome network limitations such as data bandwidth capacities, or bottlenecks caused by message deliveries. We can, however, strive to avoid hangovers caused by protocol design considerations.
\changebars{For instance, hangovers caused by a slowdown of the network pace below the request input rate will inevitably form a backlog; avoiding such requires admitting fewer client proposals and is beyond the scope of the consensus protocol. We can, however, strive to avoid frictions caused by protocol-level mechanisms such as timeouts: data dissemination, for instance, need not be subject to timeouts, and should continue at the available network pace.}{} 
\changebars{We thus distinguish two forms of blips: consensus blips and full blips. Consensus blips cause timeouts to trigger but do not necessarily stall data dissemination, while full blips may arbitrarily impact (e.g. halt) communication between nodes.}{}
\changebars{We say that a partially synchronous protocol behaves optimally (w.r.t to blips), or \textit{seamlessly}, if it \one experiences no asynchrony hangovers caused by only \textbf{consensus blips}, and \two does not introduce new causes of frictions that make the system more suspectible to experience consensus blips.}{Thus, we say that a partially synchronous protocol behaves optimally (w.r.t to periods of asynchrony), or \textit{seamlessly}, if it experiences no asynchrony hangovers solely due to consensus protocol design choices.} \fs{ is free of protocol mechanisms (beyond timeouts, which are necessary by FLP) that make the system more susceptible to experiencing blips.}

\fs{FIXME: ITERATE ON THE "PROTOCOL MECHANISM PART"!!!}
\fs{Massage definition/section: Seamless should only capture what is in our control. I.e. it should refer to hangovers caused by "protocol mechanisms" (not by things like data bandwidth) => Recovery from asynchrony should be instant (subject to data constraints). 
Asynchrony "ends" when all data has arrived at honest.}

%Thus, we say that a partially synchronous protocol behaves optimally (w.r.t to periods of asynchrony), or \textit{seamlessly}, if it experiences no asynchrony hangovers solely due to consensus protocol design choices.
\fs{a consensus protocol can be seamless without the system being seamless!}
\begin{definition}

    \fS{Idea: a seamless system should minimize/avoid all "frictions" related to asynchrony. Making it more susceptible to asynchrony is friction. Not recovering smoothly is friction. A seamless protocol should avoid hangovers caused by asynchrony WITHOUT making it more susceptible to it.}
    %A partially synchronous system is \textbf{seamless} if it is free of protocol mechanisms subject to asynchrony hangovers. 
    \changebars{A partially synchronous system is \textbf{seamless} if it \one is not subject to asynchrony hangovers that are caused by consensus blips only, and \two does not introduce any protocol mechanisms (beyond timeouts) that are susceptible to introducing more consensus blips. }{A partially synchronous system is \textbf{seamless} if it is free of protocol mechanisms subject to asynchrony hangovers.}
\end{definition}

\changebars{Seamlessness is a desirable property for any partially synchronous consensus protocol, yet it is especially important for BFT protocols as Byzantine leaders may produce hangovers by simply not participating, thus negatively impacting performance \textit{beyond} their tenure. This, we find, is at odds with the \textit{Byzantine fault tolerant} tenet: BFT protocols should be robust to Byzantine faults~\cite{aardvark}.}{} \fs{cite Aardvark Robustness doctrine}

\fs{Other things we could }

%%%%%

\par \textbf{Analysis of existing approaches.}
Traditional BFT protocols\cite{castro1999pbft, yin2019hotstuff} are not seamless. They disseminate batches of requests and reach consensus on each batch independently; \fs{Note: I am intentionally not specifying whether batches are sent alongside consensus -- this does not matter}the number of consensus instances required to commit all requests is directly proportional to the input rate of requests divided by the batch size. Consequently, the time required by these protocols to process the backlog accumulated during progress-free (asynchronous) intervals is in the order of the backlog's size--assuming continuous client load.
%We demonstrate empirically in \S\ref{sec:eval} that Hotstuff~\cite{yin2019hotstuff}, for instance, suffers a latency hangover. 

We demonstrate empirically in Fig. \ref{fig:hangover} that Hotstuff~\cite{yin2019hotstuff}, for instance, suffers a latency hangover because it is bottlenecked by the (processing) bandwidth of each proposal (\S\ref{sec:eval}). % (we defer to \S\ref{sec:eval} for a more detailed discussion).
\begin{figure}[h!]
    \vskip -2pt
   \centering
   %\includegraphics[width=0.45\textwidth]{Figures/consensus.pdf}
   \includegraphics[width=0.38\textwidth]{Figures/eval/hangover-blips-intro-cut-visibility.pdf}
   %{Figures/eval/hangover-blips-intro-cut.pdf}
   \vskip -4pt
   \caption{Latency Hangover (nearly 4 seconds) in Hotstuff~\cite{yin2019hotstuff} following a 3 second blip\changebars{ caused by 2 consecutive leader failures (using a 1s timeout)}{}.}
   %\caption{Core Consensus coordination pattern. Messages may be piggybacked on existing cars (\S\ref{sec:ride_sharing}): P1 = \textsc{Prepare}, P2 = \textsc{Confirm}, C = \textsc{Commit}.}
   \label{fig:hangover}
   \vskip -0pt
\end{figure}


Simply proposing larger batches is not a viable option for reducing the number of required agreement instances as it comes at the cost of increased latency in the common case.
Similarly, a straightforward decoupling of dissemination and consensus (proposing only a batch digest)~\cite{bagaria2019prism, danezis2022narwhal}\fs{this is what the HS baseline does; it starts dropping messages at some point} %or tiered batching (proposing batches of "mini-batches")~\cite{danezis2022narwhal} 
can alleviate data transfers and request verification on the critical path of consensus, \changebars{but does not address the princal concern.}{but the fundamental complexity remains proportional to the backlog.} \changebars{Such designs are consequently unable to robustly scale throughput beyond the leader dissemination capacity; we confirm this empirically in \S\ref{sec:eval}.}{} \fs{our experiments of batchedHS show that separating dissemination just blindly is not enough - not only is it not robust during async, but it doesn't seem to hold up under high load}
\fs{I changed the argument from being about the size of a proposal growing proportionally to the number of consensus instances required -- I think the batch-latency tradeoff is much more obvious}
%but not the principled concern. 

A class of recent DAG-based BFT protocols~\cite{danezis2022narwhal, Bullshark}, in contrast, is \fs{almost...} seamless. \fs{not all are seamless: the un-certified ones like Cordial are not} These protocols decouple data dissemination and consensus, and construct an asynchronously growing DAG consisting of data batches chained together. The construction leverages Reliable Broadcast to generate proofs that transitively vouch for data availability and request verification of \textit{all} topologically preceding batches in the DAG. The consensus mechanism can commit entire backlogs with constant cost by proposing only a single batch, and thus experiences complexity \textit{independent} of asynchronous durations. Unfortunately, existing seamless DAG-BFT protocols exhibit, during {\em good} intervals, up to twice the latency of traditional BFT protocols. \fs{Can talk about why, but I think this is not the right place.} \la{Why not? What do you think is the right place? I must say that as I was reading it, the "why?" question definitely popped in my mind...} \fs{The root cause is that consensus is hardwired into the structure of the DAG. This allows neither to go as fast as they'd like. Each round of consensus is mapped to one RB (best case)} To bridge the gap, we propose \sys{}, a novel high throughput BFT protocol that delivers low latency during synchrony and handles \textit{partial} synchrony seamlessly.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% OLD VERSION %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\iffalse
No deterministic protocol can guarantee both safety and liveness under asynchrony~\cite{fischer1985impossibility}. Partial synchrony, is a powerful and convenient model that allows us to build practical systems: safety is guaranteed always, while progress guarantees are limited to periods of synchrony.
The dominant partial synchrony model in BFT assumes an eventual Global Stabilization Time (GST) after which synchrony is forever on guaranteed. This model simplifies both the explanation and proofs of consensus protocols, yet is unrealistic in real deployments~\cite{liu2023flexible}. \fs{why? maybe talk a bit about timeouts. All psync protocols need them. But they're "hard"/impossible to set "correctly" in asynchrony. Too low, and we get spurious async periods; too high, and we don't respond timely to failures}\neil{Yeah we can also say that systems that assume this unrealistic model have no incentive to care about the impact of asynchrony since it never returns after synchrony (essentially a one time problem).} \fs{can also reference MyTumbler experience on WAN deployments}
\nc{We say it's unrealistic in real deployments, we don't say what the consequences are. One way to interpret what you're saying is that the protocols aren't actually live. The other way to interpret this is that the protocols are live, but perform horribly. We want to distinguish between the two early. }

This paper argues, that asynchronous periods are not fringe outliers, but constitute a core part of a partially synchronous protocol's common case. It is therefore imperative to take into account, and characterize the impact that asynchrony has on the performance of partially synchronous protocols. While we are typically primarily interested in the pragmatic metrics of latency and throughput, we ought to also analyze the \changebars{robustness}{ \textit{quality}} of performance in the presence of recurring asynchrony. 

During asynchrony, there is no progress, and hence performance is void. But \textit{how fast}, at \textit{what rate}, and \textit{how well} do we regain performance \textbf{after} progress returns?

\nc{I would be a lot more direct in this first two paragraphs. SUGGESTED REWRITE:

This work is premised on a simple observation: partially synchronous protocols cannot practically tolerate periods of asynchrony. Partial synchrony is an appealing theoretical model that captures when consensus protocols can still achieve liveness, in spite of the seminal FLP impossibility result. All partially synchronous protocols are live when the partially synchronous network reaches the Global Stabilization Time (GST), at which point all messages will be delivered within $\Delta$ time. While useful for proving liveness, this model does not accurately describe how real networks work. Message delays due to intermittent failures, packet queuing are frequent; most RPCs for instance suffer from high tail latency (or other example)~\cite{dean2013tail,rpcpaper, liu2023flexible}. Setting accurate timeouts is similarly a notoriously hard challenge~\cite{tennage2023quepaxa}. In short, modern networks are truly partially synchronous: most messages will arrive within $\Delta$ most of the times, but not always. There will be periods of asynchrony in which the network behaves poorly. To properly assess the performance of a partially synchronous system, we should consider how it behaves \textit{at all times}, during periods of full synchrony, but also \textit{after} periods of asynchrony.

While Aardvark introduced the concept of synchronous intervals~\cite{} when describing the need for robust BFT systems, there does not currently exist a precise way to capture the performance of partially synchronous protocols during synchronous intervals \textit{after} experiencing periods of asynchrony. To this effect, we introduce the dual notions of asynchrony hangovers and seamless partially synchronous protocols. Informally, a psync protocol is seamless if it does not suffer from hangovers.}

\nc{To the extent possible, let's reuse the terminology of aadvark, gracious, uncivil, synchronous intervals and let's heavily ack aadvark here to make sure that people don't say "aadvark did it and you don't know about it}

To characterize the quality of performance in partially synchronous protocols we introduce the dual notions of an \textbf{asynchrony hangover}, and a \textbf{seamless partially synchronous protocol}. \fs{NC: loosely inspired by/rooted in principles of control theory?}
As a prerequisite, we note that a Byzantine leader could establish "progress", but intentionally limit performance; we classify Byzantine behavior to be indistinguishable from asynchrony. We thus say that an interval is \textit{good} if the system is synchronous (w.r.t. some implementation-dependent timeout on message delay), and the consensus process is led by a correct replica~\cite{good-case}\footnote{A replica \textit{leads} consensus if it determines the initial input proposal.}\fs{this is the first mention of a leader; can we take it for granted? All deterministic psync protocols must have a leader}; we say that it is \textit{gracious} if all replicas are correct~\cite{aardvark}. Given this, we define:
\nc{We probably want to be specific about what it means for a consensus process to be "led by a correct replica". I know you claim that there is always some form of leader in a psync deterministic protocol, but I worry that this opens up to "what about leaderless protocols, what about multileader protocols}
\nc{Let's maybe reintroduce the definitions of good and gracious as explicit definitions, even if we cite the others}

\fs{TODO: Tweak definition to account for subtle distinction: \sys{} gets seamlessness as soon as there is a new SLOT lead by an honest leader. I.e. put differently: slot instances that were started before or during async have no guarantee of eliminating the hangover -> after all, they might have to commit old tips that were proposed BEFORE getting back to synchrony. E.g. an unfinished slot might view change to an honest replica which has to re-propose the old proposal. This should not be treated as "leading consensus process", the replica is merely "orchestrating recovery". "Leading" should be defined as deciding (on its own) what the proposal should be. => for now I made it a footnote}

\begin{definition}
    An \textbf{asynchrony hangover} is any performance degradation that is caused by a period of asynchrony, and persists beyond the return of \changebars{a good interval.}{consensus progress.} %\fs{more precise: beyond the first HONEST commit.}
    \nc{Is there some acceptable delay T, or do we assume that it should "immediately" resume?}\fs{I'm not opposed to the T.  I think "immediately" is impossible, hence the discussion about "quasi-seamlessness". My worry is that picking some T to compare protocols under is not very principled}
\end{definition}
    

\fs{more rigorous: degradation should be "measured" with respect to the async free case. I.e. which requests would experience different performance under the two cases. I.e. should only look at the "set" of Tx that would've committed without async? Can't talk about the ones that wouldn't be committed anyways (e.g. orphan nodes in DAG/or tips that weren't included) -> those don't have a "hangover"}

We illustrate the concept of asynchrony hangovers for the closely intertwined throughput and latency metrics; we defer a more rigorous analysis of other possible types of asynchrony hangovers to future work.
\nc{Make the sentence more direct. Asynchrony hangovers have an impact on both throughput and latency. A throughput hangover is the duration all commands started outside of a synchronous period (tried to make it more precise than delayed by asynchrony, though I'm realising now i'm making it too strong because i'm including commands proposed by a byz leader}

\par We denote a \textbf{throughput hangover} as the duration required to commit all load whose progress was delayed by asynchrony. Assuming the provided load is below the steady-state throughput the system can offer, the system will eventually recover all throughput "lost" during asynchrony.\footnote{If the load is equal/greater to the throughput, then the lost committed throughput (or \textit{goodput}) can never be recovered.} The longer it takes, the more severe the hangover. \fs{we want this horizon to be short, else by the next async blip we build even more backlog and so on, until we can never recover the tput. It's tricky to talk about this as tput problem in isolation. It's so closely intertwined with latency} \fs{the time it takes to address my tput deficit is a window of vulnerability. The longer it is, the longer there is a possibility of conflict with another event (e.g. async/faults) that further extends. It weakens the system to faults}\nc{I'm not entirely sure the point that you're trying to make here comes through. At least what your'e saying in comments doesn't seem to be the same as hwat you're saying in the text}\fs{we are still discussing; the old text does not yet reflect the new comments. What is the best way to describe it?}
In a throughput hangover-free system, all load submitted -- whose progress is interrupted by asynchrony -- commits instantaneously upon return of progress. \changebars{}{If we "zoom out", the amortized throughput over a period of measurement should be equivalent to that of a system with continuous progress; as though asynchrony never occurred.}
\fs{This is essentially our "async resp tput" but in a more general formulation. Likewise for latency below: "seamless"/metastable-free latency we were talking about} \fs{in a way, the async resp tput is just a latency property though... }
\neil{Yeah I like the way you have talked about this, especially the window of vulnerability.}
\neil{I agree the throughput hangover is very closely related to latency. In fact one can argue that having a throughput hangover implies that you must also have a latency hangover (from the backlog of requests). And similarly you would only have a latency hangover if you had a throughput hangover (if there's no backlog then the latency won't increase)}\fs{exactly: tput and latency don't exist separately. Latency at 1 tput means nothing, just as 1m tput at 100s lat.}
\nc{What's the benefit then of separating them out?} \fs{maybe none. I only came up with the theory of hangovers while writing them out.. we can change it!}

\par A \textbf{latency hangover} $h$ materializes as either \one increased latency (w.r.t to the expected latency under synchrony) for requests that were issued after \changebars{resuming a good interval}{progress returns} ($Lat(req) = E(Lat) + h)$)
\nc{Shall we express this in terms of synchronous intervals instead? Notion of "progress" can be vague}\fs{yes, changed it. Wrote the text before formalizing good intervals}, or \two increased latency \textit{beyond} the asynchrony duration for requests issued before or during the period of asynchrony ($Lat(req) = E(Lat) + duration_{async} + h)$). Put differently, in a latency hangover-free system, only the requests whose progress is interrupted by asynchrony experience a hike in latency; and no more than the duration of the asynchronous period. \fs{more precise would be: if a req is input half way through async, then the hike is only the remainder...}

We say that a partially synchronous system behaves optimally w.r.t to periods of asynchrony, or \textit{seamlessly}, if it experiences no asynchrony hangovers.
%We note, that a byzantine leader could establish "progress", but intentionally limit performance; we classify such byzantine behavior to be indistinguishable from asynchrony, and understand a seamless protocol to be one that does not incur hangovers beyond an \textbf{honest} leaders tenure (after the return of synchrony).

\fs{Massage definition/section: Seamless should only capture what is in our control. I.e. it should refer to hangovers caused by "protocol mechanisms" (not by things like data bandwidth) => Recovery from asynchrony should be instant (subject to data constraints). Asynchrony "ends" when all data has arrived at honest.}

\begin{definition}
    A partially synchronous system is \textbf{seamless} if it is not subject to asynchrony hangovers.
\end{definition}
\fs{other name suggestions. NC: a psync system is "young" if it doesn't get hangovers. Periods of asynchrony are blips or "binges"}

\fs{Note: Seamless refers only to the consensus protocol. The application layer may of course not deal seamlessly with a large backlog of load if it is overloaded. For our purposes however, we assume application layer (execution) has infinite tput, i.e. consensus is not bottlenecked by execution -- more consensus tput == better.}
A seamless (hangover-free) protocol, must commit any proposals that \textit{would have} committed under synchrony -- but did not due to a period of asynchrony -- as soon as progress is restored \fs{kind of redundant with previous sentence on tput}, and without affecting performance of all other proposals. In practice, this demands in particular that performance (throughput/latency) must be independent from the duration of asynchrony.
\nc{These last two sentences seem redundant with what was said before?}

\fs{TODO: I submit that seamlessness is actually impossible in an async system. One may always miss some data (possibly proportional to async period) due to the nature of having Quorums < n.}
\fs{We instead can strive to be just shy of seamlessness. Define "Quasi-seamless": Only data transfer size is proportional to backlog; message exchange protocol latency should be fixed} \fs{Note: with this definition, existing dag protocols are also not quite quasi-seamless. A replica may still need to recursively learn of parents} \fs{Certified DAGs can sidestep this by using the same trick that we do; they just need to ensure that voting on proposals from the same replica is FIFO.} \fs{Uncertified DAGs cannot. a) must sync during consensus, b) cannot certify Fifo => recursion inevitable}


\fs{Challenge: Distinction between consensus and data dissemination. Why is it important to think about data dissemination? Can be doing consensus just fine, but if you have to recursively get data, then end-to-end latency story. Big problem, not nitty gritty detail.}


\par \textbf{Analysis of existing protocols.}
Traditional BFT protocols \fs{cite the usual bunch} are not seamless. Periods of asynchrony result in the formation of backlogs, whose size is directly proportional to the duration of no-progress \nc{of the asynchronous period}\fs{I speficially didn't say async, because there can be progress in async -- it's just not guaranteed. Unless we want to define asynchrony explicitly as the case in which we time-out/make no progress}.
\nc{Fair. I had been implicitly assuming that asynchrony meant no progress but I see your point}This results in both latency and throughput hangovers as "working off" backlogs requires additional data transfers and request verification on the critical path of consensus. Techniques such as mini-batching (proposing batches of digests of already best-effort disseminated batches), or naive chaining (proposing the head of a hash-chain of best-effort disseminated requests) can ameliorate hangovers, but not sidestep them: they introduce data synchronization proportional to the backlog onto the critical path. \fs{- Simply chaining together proposals is not enough either (that just gives them an order). Need transitive certificates of availability. I.e. best effort broadcasts are not enough! -> i.e. Dahlia's BCCA thing}
\nc{This explanation is too encoded right now}
\nc{Ideally, we'd want a graph in this section that demonstrates this} \fs{@Neil: we can slot in here a nicer version of the poster graph?}
\nc{Traditional BFT protocols don't consider "chains", so talking about chaining is a bit confusing/narrow. We want to identify the "root cause" for why they suffer from this backlog. I think this is where we probably want to "break down" the BFT protocols that exist today in "conceptually" different roles, that are intertwined }

Recent DAG-based BFT protocols \fs{cite Bullshark/Shoal}, in contrast, are seamless. The DAG-construction, driven by series of temporally intertwined Reliable Broadcast's (RB) elegantly generates Proofs of Availability (PoA) that transitively vouch for both data transfer and verification of \changebars{}{large causal histories of} asynchronously disseminated data. As a result, the cost of consensus is \textit{independent} and agnostic to periods of asynchrony; the latest PoA subsumes the backlog. The downside of DAG-based BFT is that consensus is hard-wired into the structure of the DAG. For one, the RB at the core of such protocols provides a property stronger than PoA's, resulting in additional cost. Second, consensus must always account for the \textit{worst-case} \fs{I fear this is too vague and not useful -- but I don't want to write an essay about DAGs here. I do want to however appreciate what they do nicely}, resulting in higher than desirable sunny-day latencies. \neil{Instead of saying consensus must always account for the worst case, I would say something like consensus RBs both proposals and votes} \fs{cannot parse}
\neil{was just trying to say why DAGs have higher sunny-day latencies, and the "simple" reason to me is that they reliably broadcast both the leader's proposal and all other replicas' votes. probably need to workshop this explanation a bit}
To bridge the gap, we propose Autobahn, a novel high throughput BFT protocol that exhibits both low latency during synchrony, and seamlessness under \textit{partial} synchrony.



\fs{TODO?? Define effective latency as well? end-to-end; consensus latency isn't the only thing that matters, but sequential latency is important.}\fs{don't think it's needed here. DAGs and Traditional BFT don't need to worry about "missing" the bus. It's something that we introduce, and then want to make better. (Only Dahlia's BBCA also "needs" it but doesn't think about it)}
 
\nc{High level thoughts, we really want to structure this "Analysis of existing protocol" in a more didactic way/structured way. Given the audience is unlikely to be familiar with everything, we have to "teach" them about the different components, design choices one can make in modern BFT protocols. The relationship between the data dissimination layer and the consensus layer is really waht distinguishes most of the protocols in how they handle asynchronous blips, so we're going to have to conceptually talk about this}

\fi

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% END %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%Resolved: \neil{I think we should define two terms: good-case and common-case. Good-case = honest leader after sync (when liveness is guaranteed for psync protocols) and common case is async/sync conditions. Then we can say an asynchrony hangover is a performance degradation that persists beyond the return of good case conditions} \fs{yeah good idea; I like "gracious" execution defined by aardvark -- although it says that all replicas must be correct, and not just the leader...}. \fs{alternatively: we can early on say that async and byz leader are indistinguishable}

\iffalse
We say that a partially synchronous system is \textit{seamless} when it is not subject to hangovers that last beyond an honest leader. No system can manage under byz leaders => we should could them into the period of asynchrony.

TODO: an optimal system is then: .... hangover free! We call this seamless, because it "seems" as async never happened.

TODO: Discuss what protocols are seamless and which are not:
- DAGs are. Very elegant design in which consensus is just an interpretation. The con is that consensus is "hard-wired" onto the structure. Need to account for the worst-case

- Traditional protocols are not. Backlog means that next honest has to propose a much bigger batch (or a batch of "mini-batches). This requires coordination proportional to the duration of asynchrony: a) data transfer, b) request verification, c) synchronization on critical path (in case of mini-batches). 

- Simply chaining together proposals is not enough either (that just gives them an order). Need transitive certificates of availability. I.e. best effort broadcasts are not enough!



Partial synchrony today, is viewed as primarily theoretical property. The GST model grossly simplifies realistic network behavior in a way that makes it easy to use for proofs. Once we deploy the system in practice however, we don't give it a second look.
we chalk up blips in progress/performance to asynchrony, and call it a day.


However, in partially sync systems, that are run on an asynchronous network (the internet...) asynchrony is part of the common case behavior. Partially synchronous systems should perform optimally when the system is \textit{partially} synchronous.

What does optimal mean? Clearly, it is impossible to have progress in async periods. What we want is "seamlessness"

We define a class of behaviors we call "hangovers"
- latency should be affected exactly by the blip in progress; not more. The moment we return to synchrony, latency should be normal. Req during the period of async should just be normal latency + async period
  => Latency hangover: Latency for requests received after synchrony returns is still affected. (this is imprecise: even the ones "later" during the async period, should only pay the "remaining" async cost_

- tput should be unaffected in amortization. I.e. if we "zoom out" it should look like there are no blibs overall. The total amount of goodput (delivered throughput) should be the same as a system that was always synchronous.
  -- Need to add some more stuff here. This is technically satisfied by a system that doesn't fully use its load (i.e. recovres)
  -- Tput should be back THE moment sync returns. (define as hangover)
  => Tput hangover: Tput


TLDR: No hangovers!!
Define: A partially synchronous protocol is seamless if there are no hangovers.



\fs{Thought: In fact, recent protocols like Bullshark might even guarantee seamlessness even with byz progress (stronger than our definition) by not giving proposers a "free choice" what to propose.. It's not entirely true though: a byz replica can always try to not include previous leader, but its not guaranteed to manage. Imo that fits our bill of "changing" what could've been proposed... but it's tricky)  }
\neil{Not sure exactly what you mean here, still think it doesn't guarantee seamlessness with byz because byz leader could just refuse to propose anything?}\fs{yep lol, forgot :D Resolved.}
\fi

==> Sections/3-System/Notes_And_Discussions/Notes_and_Discussion.tex <==
\subsection{data dissemination}


\subsection{base consensus}
Assymetry: Consensus needs data layer to advance; but data layer does not need consensus. There should be no consensus for the sake of consensus -- only if there is data waiting to commit.

- Note: By only proposing tips (and not data), we increase latency by an extra RTT. I.e. the slow case latency is 6 md, the fast case one 4md. This can be worse latency than BBCA/ISS/Mir...
 -- Actually, the total latency is 6/8: 2 md to get cert, 1 md to reach leader, 3md to finish fast at all replicas, +2 for slow
- If consensus rides a car, we can also commit the data proposal of the leader; I.e. for the leader we can allow it to propose something in addition to the tips. 
- We can also in general allow tips to be proposals (and not certs), but then we may have to sync on the critical path. I.e. the leader may need to forward the data for the tips that it proposed.

\subsection{fast path}

\subsection{view changes and timeouts}




fs{TODO: to add properly}
-ticket designates leader for (slot, view) pair
- fast path should not make lane wait -- otherwise we may slow down other consensus instances. => receive votes async, send cert externally. If we wait for next proposal=> then we'd be no faster than the slow path. 
 Note. External fast cert broadcast should not include proposal, so that we don't have to reconcile the fork

- tips = certs to avoid synchronization on critical path. Could send proposal tip, but then may need to sync

- signatures not shared across slots/views. If we wanted to share them (not reduce number of sigs) then we'd need to form "weird" Quorums; proofs would require messages for slots/views other than the one in question.

- when to start timeout? 
    Start timeout for slot instance s upon receiving proposal for s-1. Add a small amount of lee-way in case the leader didn't get the proposal (always forward proposal?). Add another bit of lee-way to allow the new proposer to wait for enough new tips.

- In the worst case there are f consecutive slots led by byz leaders. If not careful, each of those instances could itself view change f times, for a total of $f^2$ VC before resuming. Use a bit smarter RR, where the VC election is offset to start at +f replicas. That way at most there is f wait. This is unavoidable in any Byz psync protocol.
Note that as a result, if one slot VC, the new leader is possibly unique from any currently active slot (i.e. it is not already managing another instance).
- Note also: While VC hurts latency, it does not affect our amortized tput.
- With consecutive faulty leaders the latency cost is still sequential; there is no benefit from pipelining. It does not make sense necessarily to start more things in the pipeline, since they have to wait for the previous 


-- Why do we need to wait for prev slots to commit? Don't honest proposals strictly extend each other? That's true! But we don't know whether a prev proposal will commit (or may change due to equiv or VC). So we must wait in order to not commit inconsistent histories. (This is because our lanes allow forking -- two proposals might not necessarily extend the same tree)
-- Commit procedure: For each tip, commit all of it's history, but stop as soon as some tip height is already included (i.e. until we reach the last common commited ancestor in a lane fork). (very very simple -- much easier than doing the DAG flattening imo)
-- NOTE! We don't need to "reconcile" forks -- i.e. we don't need to pick one. We can just commit the forks in some order (i.e. nothing is lost / anything that is proposed can be committed)


-- Alternativey idea: Instead of waiting for a proposal from s-1 (note, a proposal contains as ticket either a proposal from s-2, or a TC from s-1) we could start s as soon as we see any TC from s-1. This TC might have null-proposal. However, it must have a reference to the proposal of s-2 (since we only started timeout for s-1 after seeing proposal for s-2). Thus we could just extend the tips from s-2, and issue a proposal in s that uses as Ticket the TC from s-1 and proposal s-2. It could be that s-1 ends up committing a proposal with bigger tips than s. (But that's also possible in general!!!)  -- alternatively: assemble last proposal by having each replica vote as part of TO votes what are the highest tips they've committed/seen proposed, and then merge them.
-- Note! either way, tip extension is only best effort. The proposal that we extend may not end up being committed. Tip-extension is to avoid redundant work in the graceful case. In the faulty case, we will do redundant work, but that's fine. So a more precise downside of the empty TC approach is that you're going to give up on "trying to" avoid redundancy, even though we KNOW that we'll end up with 2 honest proposers


--VC messages can be embedded on cars, but can also be sent externally.
- since we don't share the signatures, physically there is no data saved anyways. 


-- If we want to share signatures (e.g. one car message includes many things: data dissemination, vc vote for slot k, prepare vote for slot q, commit vote for slot r), then we need to send a message for all the things we signed in order to verify a QC for just one purpose (e.g. to verify Commit Quorum for slot r, need vote message for Vc k). Can reduce this by creating a merkle tree, and sending only the relevant message + a hash path (Basil batching)



\fs{End}

\par \textbf{Protocol notes.}
\begin{itemize}
    \item Tips need to be certs in order to guarantee n-f new tips. Question to ourself: What if we make the tips not certs (as aggressive as possible)? Can we guarantee f+1/n-f new tips? For tips we don't need to check the proofs, whereas for certs need to check f+1/n-f signatures depending on whether tip is a normal or special
    \item Propose new tips if nothing was committed in previous view.
    \item Cert of the tip only has to f+1. We are not forced to pick tips with 2f+1. This is because if there is a tip with 2f+1 it will be deterministically ordered before from consensus. So having a tip of f+1 strictly increases what we are committing after
    \item $2f+1$ streamlines synchronization better. Also for $f+1$ if we can catch equivocation and report
    \item Can we avoid double spends if our slot is committed but not prior slots? Can we say the same as BBCA for payments?
    \item There can be multiple instances but in practice we don't expect there to be $n$. Instances will start and finish quickly. Can remove all metadata but keep the commit proof for committed instances. Try to garbage collect by enforcing that instance x contains proofs for instance x-k back, so you keep only k proofs at a time. Don't need for checkpointing but k can be smaller than checkpoint
    \item If one replica is the leader for multiple instances then its block can contain multiple proposals/tickets/QCs. Each block contains vector of consensus metadata for each instance its sending data for. In the worst case a block contains data for f+1 instances (f byz guys). Can we collapse the proposals for multiple instances? If you have multiple instances then one signature + merkle tree suffices  (to avoid sending all messages)
    \item If nothing has been committed then collapse everything that is guaranteed to have not committed. In the worst case the safe thing to do is keep certs \fs{no clue what this comment was trying to say anymore}
    \item As soon as you see a slot for which nothing could have committed, you can collapse all slots above (rewrite history) because while they could have committed they couldn't have finalized (= all previous slots commit)
    \fs{ if in the view change the winning proposal is $\bot$ then you can propose new tips that cover the old ones. I think the second comment is referring to how for example slot 3 could be committed but slot 2 view changes and proposes new tips that cover slot 3's. This is okay because slot 3 hasn't "executed" slot 2 yet, so once slot 2 is committed, everybody will commit slot 2 tips and essentially ignore slot 3's because it was already covered.}

    \item for consensus we need to sync on the n tips provided; this isn't much different than in Bullshark for example, where one needs to sync on the n-f parents. If want wanted to bring down the amount of tip sync on the critical path then one could try to also included parent edges in a tip, and then only propose one tip such that n-f parents are new. But this is less responsive than it could be -- it ignores possibly newer tips
\end{itemize}


\section{Latest discussion}

\subsection{Minimizing latency}
Can propose un-certified tips. Tradeoff: lower latency for tip proposals; but possible sync cost. Sync adds extra RTT on critical path. Byz will always ask for sync. Can use reputation mechanism to avoid including uncertified tips. Using uncertifies tips feels "natural" as we receive it together with the previous cert (since it's piggybacked)

Only allow tip proposal to be uncertified; any older proposal still needs to be in the certification chain. This is necessary to keep cost constant in case of recovery from periods of asynchrony. Otherwise would have to potentially sync on all proposals. (Alternatively: Could form hash chain on data, and only accept/vote for new data if all ancestors are local -- Byz can still ask for everything though... Likewise, a byz leader could propose an arbitrary chain and cause a lot of sync)

Using certs makes the experience smoother. There are no expected hiccups anymore.

Note: aggressive bcast presumably only helps common case, in which tips are immediately committed, without there forming a waiting "uncommitted" chain.


\subsection{Fairness}
Traditionally, chain quality is = 1/2 of the log is from honest. 1/2 of each round is honest.
- this is achieved by rate limiting everyone to run at the speed of the f+1st slowest replica.
- arguably not "fair". f+1s slowest replica has same impact as fastest, without putting in the same effort.

Our fairness:
- provide only the OPPORTUNITY for 1/2 of log to be honest / for 1/2 of each commit to be honest
- 1/2 of tips are honest, but byz replicas might have much higher tips. That is ok, byz put in more work.
- fairness = equal opportunity, but work is rewarded.
- in common case where all replicas are equally performant this results in traditional chain quality.

\subsection{Responsiveness of Data layer}

Problem: 
If consensus is piggybacked on same car as data layer we wait for 2f+1. But first 2f+1 might not be honest.
Could receive f+1 yes votes; and f byz timeout votes. Cannot distinguish whether those are honest or not.

Consensus needs to wait for 2f+1 yes votes, or 2f+1 timeout votes (to form the respective Quorums)

Data layer shouldn't block arbitrarily. 
3 options:
1) make data layer wait TO -> data layer stays async, but is not responsive
2) let data layer continue, and let consensus Quorum wait to ride next available car
3) drive yourself: let consensus send external messages (Note: shouldn't contain data -- otherwise it will be a fork that may never be reconciled, i.e. lost data. don't want this for honest proposals; could re-concile by having multiple parents, but it's messy)


Realistically, it's not a big deal to briefly halt data layer; we will simply batch more.

Waiting to share cars is beneficial if we want to use batched Basil sigs; i.e. if signatures are a bottleneck.

We would like for our lanes to be High occupancy (many logical messages/passengers sharing same cars). But whether or not we enforce it depends on the bottlenecks. If latency is the most important feature (no crypto bottleneck) then we probably want to drive ourselves asap (send external messages). If crypto is the bottleneck, we may want to encourage or mandate carpooling to save signatures.


\subsubsection{correlated instances}
Example: 2 consensus instances drive same car.
Question: Could this cause issues with Quorum progress?

No.

Cases:
1) different leaders
    - different broadcasts. They are not on the same car = not correlated
2) Same leader
    a: honest
        --> expect all honest replicas to vote yes for both instances
            Tricky case:
            - Timeouts differ (e.g. C1 was in view 2, and C2 in view 13 and has a much higher TO)
            - But we still expect replica to vote for both: Either both yes, one VC one yes, or both VC (i.e. bottom line is we get a reply)
                            (Honest leader cannot distinguish honest reply from byz)
            - As a result, we may get the necessary quorums for progress for the respective instances at different times
            - if we make data layer wait, and require instances to carpool, then we correlated the progress of the two instances
            => need to be able to continue (either externally, or by letting data layer proceed with just one instance -- and other instance waits for next car)
    b: byz
        --> doesn't matter, need to consider timing out anyways.


Note: Aggressive tip proposals may requires sync => may result in honest replicas correlating progress.
        E.g. replica doesn't vote for C1 because it still needs to sync on C2. => would need to separate messages (but this is only possible if we are not carpooling signatures)

==> Sections/3-System/Notes_And_Discussions/autobahn_design.tex <==
\section{\sys{} Design}
\neil{old Notes}
\par \textbf{Central question:} \textit{How can we architect a new BFT system containing an asynchronous data dissemination layer and a partially synchronous ordering layer that maximizes throughput and minimizes latency?}

\par \textbf{Problems with prior designs}
\begin{enumerate}
    \item Elimination of view synchronization and view change
    \item No async responsive throughput (timeouts used in data dissemination)
    \item Sequential latency
\end{enumerate}

\par \textbf{Elimination of view synchronization and view change}
\begin{itemize}
    \item Eliminating view synchronization and view change improves simplicity but hurts performance
    \item Removing view synchronization pushes its functionality to be incorporated in the data dissemination layer, putting unnecessary synchronization on the critical path
    \item Removing the view change requires consensus to incur more message delays in the common case (multiple rounds of RB)
\end{itemize}

\par \textbf{No async responsive throughput}
\begin{itemize}
    \item One main advantage of the data dissemination layer is that it can makes progress during periods of asynchrony (unlike consensus)
    \item Many prior protocols push timeouts on the critical path of the data dissemination layer as a result of trying to overlay a partially synchronous consensus layer on top
\end{itemize}

\par \textbf{Sequential latency}
\begin{itemize}
    \item The problem with sequential latency is that if you are unlucky, requests may miss the upcoming consensus instance and have to wait until the next consensus instance starts to be ordered
    \item This leads to a discrepancy between anchor latency and non-anchor latency in prior protocols
\end{itemize}

\par \textbf{Solutions}
\begin{itemize}
    \item Bring back traditional BFT with view synchronization and view change but piggyback consensus metadata on data dissemination layer, so that it incurs no overhead
    \item Remove timeouts off the critical data dissemination path, and under asynchrony consensus can output blocks to data dissemination (even if consensus doesn't make progress)
    \item Use a hybrid approach between fully parallel and fully sequential BFT: semi-parallel (chain of propose/round 1 messages but other messages can happen in parallel)
\end{itemize}

\par \textbf{\sys{} Data Dissemination}
\begin{itemize}
    \item Each replica maintains its own independent chain (no synchronized rounds)
    \item Blocks only need a quorum of $f+1$ votes (we don't care about non-equivocation)
    \item Can pipeline the proposal sending step with the disseminating of the certificate
    \item A result of pushing synchronization and view change to consensus layer
\end{itemize}

\par \textbf{\sys{} Consensus}
\begin{itemize}
    \item Semi-parallel consensus instances (avoids sequential latency): can start a consensus instance as soon as you receive a proposal for previous instance
    \item Optimistic fast path with 3f+1 quorums (can't do with DAG RB designs)
    \item Logically separate from data dissemination but physically uses the same messages (no overhead, comes for free except for view change)
    \item Special edge rule when data dissemination and consensus aren't synchronized
    \item New consensus instances must cover n-f new certs (avoids degenerating throughput to that of a single chain)
\end{itemize}

==> Sections/3-System/Notes_And_Discussions/design1.tex <==
\section{Design inspired by Dumbo-NG for less blocking}
Instead of a replica r creating a header having n-f edges, a header just has a 
single edge to r's certificate in the previous round. The advantage is that you are
not waiting for n-f other consistent broadcasts to finish and just for your own 
consistent broadcast to finish (to even further reduce blocking I could imagine 
doing parallel consistent broadcasts using logs/sets but for now will just assume 
this sequential sequence of consistent broadcasts). 
The disadvantage is of course DAG coverage 
since you only have a single edge but note that DAG coverage can also be
redundant. If you have n-f headers in some round k all with the same edges to
the same headers in round k-1, you haven't gained additional coverage when
waiting for n-f consistent broadcasts to finish. Instead for coverage we can
actually leverage the consensus/agreement blackbox. As input to the consensus
engine a batch of n DAG-QCs (of which n-f that aren't committed) can be fed in. 
Then the consensus engine will output a committed set of n DAG-QCs which can be 
ordered in some deterministic way.

The fundamental difference is that in these DAG protocols to start the next
broadcast you have to wait for n-f broadcasts to finish, whereas in this Dumbo
inspired design you only wait for your own broadcast to finish before moving on
to the next round of broadcast.

\par \textbf{Log (parallel) vs Chain (sequential).} One of the advantages of the
chain is that it is very compact to send the whole chain. One can simply just send
the tip of the chain (along with a certificate proving availability) and commit
the entire ancestry/history of the tip (using a pull-based approach to get
missing blocks). With a log it is a bit more difficult since a certificate on
the latest sequence number does not imply there are certificates for all prior 
sequence numbers.


\subsection{Design}
When the consensus leader receives a ticket: either a Commit-QC or a Timeout-Cert
then it creates a new special header. Now it is possible that the consensus leader
is in the midst of a consistent broadcast instance when it gets its ticket. To
prevent blocking, we allow special headers to extend a header that doesn't have
a certificate. And in a sense the certificate for a special header also acts as a
certificate for its parent (if it does not exist). A special header consists of
the consensus view, and the ticket to start that view. In the Dumbo-NG inspired
design a special header also consists of n DAG-QCs (of which n-f must be new 
DAG-QCs), otherwise a special header just consists of hashes of mini-batches.
The leader of a special header also does a consistent broadcast as normal. There
are no timeouts for the first 3 message delays, and thus the DAG maintains its
asynchronous responsive throughput (no timeouts). The timer starts when a replica
receives a certificate for a special header, and it then sends a \textsc{Vote}
message to the next consensus leader. Upon receiving a ticket the replica resets
its timer.

==> Sections/3-System/Notes_And_Discussions/outline.tex <==
\section{Outline}
There are a couple of ways to embed consensus within a DAG. We classify prior DAG
BFT consensus protocols along two axes. The first is whether they are 
"zero-message" overhead or if they require additional messages. We call this
physically separate if it requires additional messages or not physically 
separate if consensus messages are completely shared with DAG messages. 
The second is
whether consensus is logically separate from the DAG. This means that the 
consensus process is independent of how the DAG operates. Cordial Miners,
Bullshark, Tusk, and
DAG-Rider are in the not physically separate, not logically separate quadrant. 
Logical DAG, Fin/Fino are in the not physically separate, logically separate 
quadrant. HotStuff over Narwhal is in the physically separate, and logically
separate quadrant.

Prior DAG-based BFT consensus protocols were in complete extremes of physical 
separation. Either they shared all messages with DAG construction or they shared
none (HotStuff over Narwhal). We explore a new trade-off in the design space where
we are in between the two extremes.

Advantages/Disadvantages of each approach:

Not physically separate, not logically separate
Pros
-Easy to implement
-No view change/pacemaker
-High throughput since no consensus messages wasting bandwidth

Cons
-Latency is still high, 6 message delays in the good case. 2 of these message
delays are sending large amounts of data

Not physically separate, logically separate
Same pros as not physically separate, not logically separate

Cons
-Latency is still high
-Tail latency is high

Physically separate, logically separate

Semi-parallel new design:
1) no structure compared to DAG, can be fast/responsive
2) embed consensus
3) no external messages
4) latency is good since can start before next finishes
5) normal blocks f+1

Similar to dashing but we embed consensus and semi-sequential 
When you get VC quorum, include highest QC, if the leader of new view and conclude nothing could have committed, then just propose latest tips you have seen, you can either recover or finish it

Throughput benefits:
-All blocks (special and normal) can be pipelined. In DAG protocols blocks cannot be pipelined because each block has n-f parents instead of 1 parent
-Consensus embedded in normal case (no external messages)

Implementation:
-Independent consensus instance per slot, so modified consensus to elect leaders based on tuple (slot, view)

-With new design there isn't just one kind of special block. Special blocks are split into two categories: special blocks containing a ticket with proposals (starting a consensus instance) and special blocks containing prepare/commit certificates. Created two different structs containing each kind of data

-Since we don't have "synchronized rounds" as in the DAG the proposer needs to be modified to propose when there is sufficient growth (n-f tips certified). Proposer doesn't have the current state as core, so added a channel between core and proposer, where core sends all certs it receives to proposer and proposer keeps track of the latest cert per public key, and it only proposes a new special header when there is sufficient growth from the ticket


==> Sections/3-System/Poster/poster-overview.tex <==
\section{\sys{} Protocol Overview}

%While DAG protocol's rely on carefully structured causality across replica operations both for dissemination and consensus, \sys{}'s key idea is to eschew any causalities \textit{across} replicas. This approach allows \sys{} to lift the \textit{speedlimit}, minimizing consensus and end-to-end latency.
\fs{this is the description from the poster}

In the following, we outline the Autobahn protocol, separating the discussion into data dissemination and consensus layers. 


%DAG protocol's rely on carefully causally structured data dissemination to reduce the problem of total ordering to interpreting the causal order in the DAG, which is inefficient and \textit{sequential} -- reducing the problem of total ordering to causal ordering (DAG protocols transform a causal ordering across replicas to a total ordering) is inefficient and sequential, 


\paragraph{Asynchronous data dissemination. }Akin to recent DAG-protocols, \sys leverages an asynchronous data dissemination layer as the backbone of its protocol, ensuring continuous dissemination progress. Unlike them however, \sys avoids round-based synchronization (and the entailing rigid DAG structure) to allow proposers to make progress fully independently. Each replica acts as proposer, disseminating data in its \textit{own lane}, and \textit{as fast as it can}. 

To disseminate, a replica uses a lightweight version of provable broadcast primitive \cite{provable_abraham}
%(\href{https://decentralizedthoughts.github.io/2022-09-10-provable-broadcast/#:~:text=Provable%20Broadcast%3A%20is%20a%20simple,is%20the%20Weak%2DAvailability%20property.}{cite Ittai's blog post?}) 
to ensure availability; a simple broadcast followed by only $f+1$ acknowlegements suffices to form a Proof of Availability (PoA). This Quorum is smaller than those of Reliable Broadcast primitives used by DAG protocols -- thus minimizing tail latency. 
%Unlike the reliable/consistent broadcast primitives used in DAG protocols this primitive has two advantages: i) lower tail latency from smaller quorums and ii) a reduced number messages from the ability to pipeline multiple instances.

%\fs{smaller quorums reduce tail latencies -- though it can result in more synchronization being necessary (marginal concern imo) . 2f+1 is not needed, since that's for equivocation. }. 
\sys further chains consecutive proposals via hashes to transitively prove availability, and pipelines them to minimize latency. Replicas broadcasts PoA certificates assembled for their proposals, and piggyback a new proposal that causally extends the previous proposals PoA (via a hash reference). This allows \sys to only propose the latest proposal (henceforth \textit{tip}) for consensus, as the tip's PoA transitively asserts the availability of all it's predecessors.


\sys{}'s data dissemination layer is unstructured and best-effort: it does not causally relate lanes across replicas, and makes no guarantees whether or not a lane can fork. We rely on a logically separate consensus layer to intertwine lanes and decree a single consistent total ordering. 
%\fs{maybe talk about what this async data dissemination layer gives us?}


\paragraph{Embedded consensus instances. }
In order to reach consensus, \sys constructs a partially synchronous consensus protocol that requires only 3 message delays in fault-free scenarios, and 5 otherwise. We embed common case protocol messages into the data dissemination layer's message exchanges, thus minimizing coordination redundancies. 
Crucially, we must ensure that shared messages between consensus and dissemination do not unintentionally make data dissemination partially synchronous. \fs{remove rest }In \sys, data dissemination always continues unimpeded. When possible (in the common case) consensus \textit{rides} dissemination messages by embedding some additional meta data into proposals; when it is not possible to do so without slowing down dissemination, consensus sends additional (external) messages.

%Doing so presents two challenges: i) we must ensure that shared messages between consensus and dissemination do not unintentionally make data dissemination partially synchronous, and ii) consensus is not blocked on data dissemination and vice versa. To solve these challenges we add mechanisms for data dissemination to continue to progress even if consensus is stalled under asynchrony, and for consensus to continue to progress even if data dissemination is in the midst of finishing a broadcast.

Instead of proposing data as in traditional BFT protocols, \sys consensus proposes a snapshot of each data lanes latest state (or \textit{tip}), thus enjoying the throughput of $O(n)$ parallel proposers. Upon committing the snapshot (a vector of tips), \sys deterministically intertwines each tip's causal history, constructing a single totally ordered log that implicitly resolves all forked lanes. 

Consensus follows a ticketing-based approach in which a replica may only propose when in possession of a \textit{ticket}. In it's simplest form, a ticket corresponds to a \textit{view} in traditional BFT protocols, which specifies a leader-replica and consists of either \one a Quorum certifying commitment of the previous proposal, or \two a Quorum of votes expressing discontent with the previous proposer's progress (\textit{View Change}). 

While this design is straightforward, a \textit{sequential} ticket-based approach has suboptimal end-to-end latency. If a newer tip "misses the bus", and is not included in a proposal, it's effective latency is that of two consensus instances -- the wait-time, plus the consensus latency after being included. This problem plagues DAG-based BFT protocols, and is inevitable because consensus must wait for all previous leaders to commit to ensure consistent causal histories. \sys however, does not rely on causality across replicas, and can thus aggressively pipeline successive consensus instances. 

\par To minimize the wait-time for a tip to be proposed (and thus end-to-end latency) \sys begins a new consensus instance in parallel; as opposed to upon completing the previous instance. In this optimized pipe-lined form, \sys tickets correspond to slots in the log. While a given slot's consensus instance may complete early, \sys \textit{commits} it only after all prior slots commit; if a slot's consensus instance times out, \sys performs a View Change to turn over leadership of the instance to another replica. To avoid redundant proposals \sys strikes a balance: Slot $s$ uses as ticket the proposal of slot $s-1$, and may only proposes once a Quorum of new tips is available.

Within a consensus instance, processing resembles classic BFT protocols. The ticket-holder broadcasts it's proposal (a snapshot of tips) to all replicas, which in turn vote. Both message exchanges are piggybacked on normal data dissemination messages. Subtly, however, data dissemination does not proceed as soon as $f+1$ votes are received -- for ticket-augmented proposals 2f+1 votes are collected and aggregated into a LockCertificate (LockQC). Note that dissemination still remains asynchronous.
The ticket-holder broadcasts the LockQC alongside the next data proposal, and once again collects 2f+1 votes, forming a CommitCertificate (CommitQC), and broadcasting it once more. A replica commits upon receiving a CommitQC. \sys is amenable to implementing a FastPath, that allows committment within 3 message exchanges if a LockQC with $3f+1$ votes can be formed. For brevity, we omit discussion of the Fast Path and View Change case; like the above common case, they closely resembles traditional BFT protocol procedures. 
%Waiting for Quorums $> n-f$, however, temporarily halts the dissemination layer. While this does not at odds with asynchrony, \sys uses external messages to sidestep the obstruction of responsiveness -- for simplicity we defer a detailed discussion to a full paper.
%For brevity, we also omit discussion of the View Change case; like the above common case, it closely resembles traditional BFT protocol procedures. 

%Finally, to minimize the wait-time for a tip to be proposed (and thus end-to-end latency), \sys begins and pipelines a new consensus instance as soon as there are new tips -- rather than upon completing the previous instance.






\paragraph{Summary}
%\sys enforces causality only within a replica's own lane. This allows us to amortize data dissemination and verification... -- TODO: this is what allows us to only propose tips.

%\sys{}'s data dissemination layer removes transaction dissemination and verification off the critical path of consensus. This has the following advantages: i) transaction dissemination and verification are no longer bottlenecks for consensus ii) they can make progress under asynchrony instead of inheriting partial synchrony from consensus and iii) the cost of disseminating and verifying transactions after recovering from asynchrony is reduced.


\sys{}'s finely integrated consensus design allows it to enjoy both \textit{optimal} consensus latency and low end-to-end latency, and simultaneously reap the high throughput and robustness offered by parallel asynchronous data dissemination. While \sys{} -- like any partially synchronous protocol -- cannot guarantee consensus progress during periods of asynchrony, it's data layer (and consequently the lane tips) keep growing unimpeded. Upon return of synchrony, \sys{} seamlessly recovers by instantly committing it's tips causal histories, making it appear as though progress were never suspended.


==> Sections/3-System/Protocol/consensus-on-lanes.tex <==
%\subsection{On a highway to... throughput}
\subsection{From Lanes to Consensus.}
%\subsection{Layering partially sync consensus.}
\label{sec:consensus_on_lanes}
%Motorway -- layering partially sync consensus atop async dissemination.

\iffalse
- describe what we reach consensus on (lane cuts)
- describe how we order committed tips/lanes
- describe why we want certain data layer proprties: async growth, chaining, cert, fifo
\fi

 \nc{If we're going to distinguish between proposals (in the data layer) and consensus proposals (in the consensus layer), we may want to explicitly call them differently, and acknowledge that this is a feature that makes us different from traditional BFT, that we "decouple" what a proposal at the data layer and the consensus layer is. A "data proposal" is a batch of requests, a "consensus proposal" is a cut of c}\fs{For now I just explicitly highlighted both in italics}
 
\sys{}'s data dissemination layer \one disseminates batches of requests (\textbf{\textit{data proposals}}), and \two succinctly summarizes which data proposals are reliably stored in the system through the use of certified tips. It intentionally provides no consistency guarantee on the state observed by any two honest replicas. For instance, different replicas may observe inconsistent lane states (neither a prefix of another). 

The role of the consensus layer in \sys{} is to reconcile these views and to totally order all certified proposals. 
\nc{Rather than call it disseminated proposal, could we call them "reliable proposals" (basically we want to order all proposals which have been stored at f+1 folks?) and rexplicitly define that term?}
%The role of the consensus layer in \sys{} is to totally order the disseminated proposals. %from all data lanes. 
Unlike traditional BFT consensus protocols, that take as input a batch of requests to commit, a \textit{consensus proposal} in \sys{} consists of a snapshot \textit{cut} of all data lanes (akin to \cite{ding2020scalog, gao2022dumbo}). \fs{added scalog and dumbo-NG citation; though we weren't actively inspired by that}
Concretely, a consensus proposal contains a vector of the $n$ \textit{certified} tips \changebars{}{observed by the leader}. 
%\neil{Would just explicitly emphasize that what's proposed are certificates containing the metadata and not the tip (data) itself} \fs{-> I think that detail can be left to protocol details}
%\sys{}'s consensus tries to commit each lanes' history by taking as input a snapshot (or \textit{cut}) of observed lane tips. 
Fig. \ref{fig:car_lanes} illustrates an example cut that might correspond to the latest certified tips at some replica. %We note different replicas may locally observe inconsistent lane states (neither a prefix on another) -- it is the responsibility of consensus to reconcile these views. 

\fs{note: proposing a vector of locally observed certified tips is pretty much analogous to having edges in the DAG.}

\nc{is there a reason why you don't describe the protocol as you're describing the pseudocode?}
\fs{Moved up this paragraph -- previously I had it at the end of the section. Happy to move it around...}
\par \textbf{Implementing consensus.}
\sys{}'s architecture allows for a flexible choice in implementing the precise consensus mechanism. In theory, any consensus protocol (including asynchronous ones) can be employed. Because \sys{} aims to minimize latency, we opt to design a mechanism that follows a classic two-round (linear) PBFT-style ~\cite{castro1999pbft, gueta2019sbft} (or Jolteon~\cite{jolteon-ditto}) agreement pattern, and augment it with a Fast Path inspired by Zyzzyva~\cite{kotla10zyzzyva} and SBFT~\cite{gueta2019sbft} that reduces latency to a single round in gracious intervals. 
We describe \sys{}'s core consensus protocol in detail in \S\ref{sec:core_consensus}, and focus here on the interplay between lanes and consensus. 

\fs{Suggestion: First mention all of the Normal case consensus here (core consensus). Then follow with discussion. Then talk about view change, and parallelism}

\par \textbf{Discussion.}
Committing a cut of the all lane states allows \sys to achieve consensus throughput that scales horizontally with the number of lanes ($n$ total) and their volume. 
\fs{TODO: Highlight that we only need f+1 signatures and this is a 2x reduction vs DAGs: In DAGs all nodes are pessimistically 2f+1 because they could belong to consensus}

Proposing only certified lane tips in turn allows \sys{} to seamlessly recover from asynchrony. 
Three key structural lane requirements make this possible: 
\one \textbf{Chaining} lanes allow a tip to uniquely identifies its lane's history, allowing \sys{} to commit (arbitrarily long) lane backlogs with constant proposal size. \nc{But due to forking there can be multiple tips for the same lane. Phrasing is maybe slightly confusing here?} \fs{true, but that's an orthogonal point no? The whole point is that we only need to look backwards from A tip}\la{I am with Florian on this one.}
\two \textbf{Certified tips} allow replicas to transitively prove the availability of a lane history \textit{without} observing the history themselves. This allows replicas with locally inconsistent lane states to vote for consensus proposals, and move synchronization off the critical path. \la{I don't understand this last sentence -- just me I am sure, but I'd love to go over it, Florian.}\fs{go for it! (in general feel free to make changes!! just highlight which parts changes (so I can identify) and put the old text in comments}
\three Finally, \textbf{FIFO voting} enforces that a single honest replica must be in possession of \textit{all} data in a certified tip's history. \sys{} leverages this invariant to guarantee that all honest replicas can reconcile states in a single round-trip.



\nc{not clear what you mean here by FIFO delivery. One way to understand it is that you only vote to certify a tip when you are in possesion of its parent's data, but I don't believe that's what you're trying to say. You've never used the world "delivery" before}\fs{that is exactly what I mean -- I tried describing it in the dissemination protocol box => I've also now renamed it to FIFO voting (happy to not use word FIFO explicitly too.} 
\nc{I think it's better, and fine for now, but if you're not careful, it still reads like you're saying three times the same thing, maybe we could "name" the properties? ("chaining", "certified tips", "fifo voting"?), I think otherwise it's hard to view what "different" part of the "chained certified tips" you're referring to (that's the reason why i was saying they're the same, for me certified tips also included chaining)}

\nc{Might be good to then highlight the "challenges" in getting from the data layer to the dissemination layer?}

We discuss next in detail how \sys{} replicas process a committed cut to synchronize their perceived lane states and construct a consistent totally ordered log.  \fs{TODO: highlight challenge here already? I feel like we highlight them enough inside the next sections}

% Challenges:
% - turn independent lanes into one total order
% - data fetching

%%%%%%%%%%%%%% OLD TEXT BEGIN

\fs{cut flexibility discussion for now. CHECK COMMENTED OUT TEXT}
\iffalse
\par \textbf{Flexible horizontal scalability.}
Committing a cut of the lane state allows \sys to achieve consensus throughput that scales horizontally with the number of lanes ($n$ total) and their volume. Upon committing a consensus proposal, \sys{} deterministically orders the not yet committed data proposals of all lanes into one consistent total order.  
\nc{We have to at some point mentiont he relationship to Scalog} \fs{I added citation above. Do you want more?}

Parallel proposers allow scaling past single leader bottlenecks in traditional BFT constructions~\cite{stathakopoulou2019mir}, and are a core motivation shared by recent multi-log~\cite{stathakopoulou2019mir, stathakopoulou2022state} and DAG BFT~\cite{Bullshark, danezis2022narwhal} Both protocol groups however, are bound by rigid proposal structures %hat impose fixed proposal rates
: Multi-log frameworks impose a predetermined request partitioning, and may need to issue wasteful no-ops to facilitate progress~\cite{liu2023flexible}; DAG-based protocols require proceeding in round-by-round lockstep in order for consensus to deterministically interpret an order, and are thus limited by the proposal rate of the \textit{slowest} honest replica.
\nc{But they achieve zero shot. If we say that, we also want to explain in a bit more detail why that is (which is why i think it'll be easier to do that once you've described what we do in a bit more detail). I think explaining that their additional requirements allows them to achieve a deterministic ordering of blocks because, while they might not agree on which block to commit, they'll have consistent "enough" histories will be a lot clearer to explain}.

\sys{} lanes, in contrast, are fully decorrelated, and can thus enjoy flexible proposal speeds. \fs{may want to switch the order} Replicas may experience asymmetric latencies, varying CPU or bandwidth capacities, or heterogeneous loads. For instance, in modern permissioned blockchain settings, replicas might be operated by distinct entities, and propose requests on behalf of their entity~\cite{liu2023flexible}. No matter the cause, \sys{} enables replicas to operate at the maximum speed of \textit{their} load and resource capability. 
\nc{You've said this a few times already, and while we should mentioni t, talking about how good we are before we actually talk about the (even high level) details of the rest of the protocol is confusing. I'd fully remove the last paragraph for now, and possibly even the first one until you've given more info about how you actually run consensus} \fs{I'm not sure what more context from consensus would help here. But I agree the paragraph kind of hangs out there and should change}


\fs{TODO: make para shorter, less abstract.}
\par \textbf{On the quest for seamless consensus.} Proposing only a cut of certified lane tips allows \sys{} to seamlessly recover from asynchrony by committing all disseminated data proposals with constant complexity (per lane), irrespective of the length of a lanes uncommitted suffix. \nc{Technically you're not proposing a lane's certified tip, you're proposing a cut of n tips}\fs{you are right: I intentionally chose to say "a lane" in order to be able to say "constant complexity". I adjusted it now. } 
Three key structural lane requirements make this possible: 
\one First, chained lanes allow a tip to uniquely identifies its lane's history, allowing \sys{} to commit lane backlogs with constant proposal size. \nc{But due to forking there can be multiple tips for the same lane. Phrasing is maybe slightly confusing here?} \fs{true, but that's an orthogonal point no? The whole point is that we only need to look backwards from A tip}
\two Second, \sys{} lanes impose FIFO delivery at honest replicas. This ensures that a single honest replica must be in possession of \textit{all} data in a certified tips history. \nc{not clear what you mean here by FIFO delivery. One way to understand it is that you only vote to certify a tip when you are in possesion of its parent's data, but I don't believe that's what you're trying to say. You've never used the world "delivery" before}\fs{that is exactly what I mean (and what is described in the dissemination protocol box 2)-- I'm happy not not mention "deliver"y or FIFO explicitly though.} \sys{} leverages this invariant, to guarantee that all honest replicas can catch up on all missing data in a single round-trip.
\three Finally, certified tips transitively prove the availability of a lane history. This allows replicas to vote for consensus proposals without needing to locally receive all data first.


% While consensus in \sys{} is partially synchronous, that is, it only guarantees to make progress committing during periods of synchrony, data lanes complete new cars even during asynchrony. Upon return to the first \textit{good} interval, \sys{} immediately commits the entire un-committed backlog of all lanes.

\nc{I think this paragraph is a bit abstract for me. I would keep it much shorter so that you still highlight the "imporant" things, but your'e able to move to concrete details faster. It's also the case that I think you can merge 1) and 3). We've also already mentioned 1/3 in the data dissemination layer, so might feel a bit redundant?} \fs{I don't see how to merge 1 and 3? Each has a unique purpose -> hence the 3 following subsections that go in detail on each}

 % This allows \sys{} to commit a lane's entire history by achieving consensus on only a single PoA (\S\ref{sec:consensus}, thus (seamlessly) recovering from periods of asynchrony with cost independent from possibly generated backlogs
\fi 
%%%%%%%%%%%%%%%%%%%%%%%%% OLD PARA END %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5

\subsubsection{Seamless data synchronization.}

In order to process a committed lane cut, a replica must first ensure that, for each lane, it is in possession of all data proposals subsumed by the respective tip's history. If it has previously voted for the tip, then, by the FIFO voting rule, it must possess all relevant lane proposals. If it hasn't, then it must first acquire (\textbf{synchronize}) the tip's data (and possibly all of its history). To do so, it simply requests the missing digest's data proposal from the $f+1$ replicas that certified it (one must be honest and will reply). 
In the worst case, a replica may need to recursively learn of (and fetch) each data proposal in a tip's history. For instance, a byzantine lane governor $G$ may leverage a period of asynchrony to certify a long lane, yet broadcast any given proposal to only $f+1$ replicas.  \fs{you could also just get really unlucky with async on point to point channels, e.g. partial network partitions}
If done naively, synchronization can require sequential message exchanges in the order of a lane's length ($\sim$ length of asynchrony).
\nc{Worth mentioning that other systems don't do this?}\la{I need to understand what is that Natacha beleives is worth highlighting here.}

\par \textbf{Fast, bounded synchronization.} To bound synchronization latency, \sys{} lanes enforces strict FIFO delivery on all data proposals in a certified tip. An honest replica only votes for a data proposal for position $i$ if it has voted for its predecessor in $i-1$ -- consequently, any honest replica part of a certificate must possess the entire history, which by design has no position gaps. \nc{I feel like we're belabouring the point with these two separate paragraphs. Could we not merge them?}\la{Agreed}\sys{} leverages this invariant to synchronize in just a single message exchange, no matter the size of the history: a replica simply requests (from the tip's certifying replicas) to sync on \fs{(and will only commit) }\textit{all} proposals in the tip's history with positions greater than its locally last committed lane proposal ($\geq last_committed[tip.lane].pos +1 $, $\leq tip.pos$). 
\fs{I switched the order with the ordering section. Make sure that this is still clear}
By correctness of consensus, all honest replicas agree on the last committed lane proposal, and thus sync on the same content. 
\nc{I see what you mean where this is a bit confusing if we haven't talked about consensus yet}

%%Comments
\fs{NOTE: it's not guaranteed, nor is it important, that the last synced on data item is a child of our latest committed. If it is not, then technically we could sync on, and commit} 

\fs{NOTE: this optimization can also be applied with Best effort Broadcast. Instead of requesting from certifier, request from leader. Honest leader only proposes certificates for which it has locally received all history}
\fs{This way if leader is byz: we will just timeout. But if leader is honest, then it wouldn't propose a tip for which it hasn't seen the chain history itself (i.e. enforce FIFO sync)}



%%%%%%%%%%%%% BEGIN Certified tips:
\fs{TODO: Cert is not necessary to protect against "just" asynchrony; it's meant to safeguard against byz abuse.}

\par \textbf{Why propose \textit{certified} tips?}
\fs{moved sentence back up to original position as requested by comments -- TODO: remove some redundancy with the next sentence}
Chained certified lanes ensure that no synchronization is necessary on the critical path of consensus, thus ensuring smooth and reliable consensus progress.

Proposing only tips that are certified streamlines the voting step of consensus proposals, and allows data synchronization to be non-blocking (asynchronous), and in parallel with consensus. Every replica can assert locally that a tip's entire transitive history must be available at some correct replica (if not locally), and begins synchronizing on missing tip histories asynchronously upon receiving a consensus proposal. 
Using the fast synchronization optimization (2md to sync), this ensures that replicas will successfully synchronize on all requires tip histories by the time the proposed cut commits (subject to data bandwidth constraints). 
\nc{I feel like we could significantly shorten and merge the previous three paragraphs. I understand that each technique gives you slightly different things, but having the three separately feels unnecessary long. Especially as, for ex, you already talk about data sync in the first paragraph. The why propose certified tips only I feel is also better explained as we describe the data sync logic rather than afterwards, separately. Happy to give it a short and you can tell me what you think}
\fs{DATA amount = bit size can of course not be reduced. That is less principled -> impact changes depending on available bandwidth. I would just assume infinite bandwidth here.} \fs{TODO: Clean up definition of seamlessness to account for data size.} \fs{Note: most likely only have to fetch large amount of data on a byz lane. (unless direct channel extremely asyc)}


\fs{The important property is that synchronization is now "replica-local" -- see commented text. Mention explicitly?}
% Consequently, any required synchronization is local to each replica and does not hold up consensus progress: other replicas may already be able to locally commit and execute, and new consensus proposals can already proceed with agreement in parallel. 

In contrast, if \sys{}'s data lanes were to employ only best-effort-broadcast \nc{terminology? You've not mentioned the concept of best effort broadcast before} \la{Indeed. It all makes sense, but it is a bit stream of consciousness here.}\fs{does beb need explaining? Feel free to change the whole paragraph as you wish} and consensus proposed uncertified tips, replicas must synchronize \textit{before} voting on a consensus proposal to ensure that a tip (history) indeed exists and thus commitment is live. It must either wait to receive the original broadcast (which may never happen if the originator was Byzantine), or request it from the leader -- this \changebars{}{places an undue broadcasting burden on the leader} requires at least 2 additional message exchanges on the critical path. Blocking to vote can result in lack of timely Quorum formation, causing consensus to timeout and restart progress. %conflicting with our goal of seamlessness.
\fs{this is in conflict with the motivation of moving to multi-leader designs, and away from leader bottleneck, and}

% \nc{I think this sentence is super important and would be much better served at the start of the subsection, and then we describe "why" during the section}\la{hear hear}

%%%%%%%%%%%% END Certified tips

%%%%%%%%%%%% How to order lanes
\subsubsection{Ordering lane histories.} 
Once a replica has synchronized on all proposals subsumed by a committed lane cut $\langle tips \rangle$ it must establish a total order \changebars{across the lanes}{}. \nc{for all the commands included in the cut + why does it need to establish a total order? We should probably say}\fs{sentence already starts with all proposals subsumed by the cut? Add sth like "cut represents n independent lane-logs; need to combine them to arrive at one?". Not sure the "need for a TO" needs to be justified?}. Each replica maintains a $\texttt{log}$ of all ordered requests, and a map \texttt{latest\_committed: lane-id $\rightarrow$ pos} noting the latest committed position of each lane.
% \nc{By proposal here, do you mean the last batch, certified tip, or the consensus proposal which is itself a cut (I assume it's the certified tip)}
A replica first identifies, for each lane $l$, the oldest ancestor $start_l$ of $P.tips[l]$ with a position exceeding $latest\_committed[l]$ (i.e. $start.pos == latest[l]+1$). %that could not yet have been ordered (i.e. such that $start.pos > latest[l]+1$). 
We note that the latest committed lane position may not (and need not) be the parent of $start$; for instance, the replica governing $l$ may have equivocated. This does not affect safety--it merely causes ancestors of $start$ to be ignored. \fs{it would also be safe to commit both forks! this is just simpler}

%\nc{What is start in this case? If we're staying at the highest level here, maybe lets's skip the math? it would have been easier for me to just erad "the oldest ancestor in P.tips that has not yet been committed (or that r doesn't know has committed yet}
Next, a replica updates the latest committed position for each lane ($latest\_committed[l] = tips[l].pos$), and appends to the log all new proposals (all lane proposals between, and including, $start_l$ and $P.tips[l]$) using some deterministic function. For instance, we may zip all lanes new proposals (from oldest to newest) in round-robin fashion (to provide fairness). 

\fs{TODO: Want to discuss why this automatically reconciles forks? Or rather, why forks don't affect this?}
\nc{This seems too "simple", especially the "some determnisitic function". I would add "While this is seemingly simple, recall that our dissemination layer does not provide any consistency guarantee across nodes, thus, ... I think this is more interesting than giving examples of the determistic function and to bring fairness in}
\nc{Is it also worth making a distinction between committed and locally committed?}

%% Why do forks not matter?
% Car primitive does not preclude equivocation. While lanes governed by honest replica's will only ever consist of a single chain, byzantine lanes may fork arbitrarily. 
% This does not affect safety, because consensus commit's a tips chained history. I.e. it doesn't "see" forks %It only affects the rate of progress made by byzantine proposers. 
\fs{Note, that latest locally committed lane proposal doesn't have to be an ancestor of start. It also doesn't have to be +1. this could happen if the lane was forked. I explicitly didn't say ancestor that has not yet committed -> there might be older ancestors that will not ordered even though they have position < latest} \fs{we also don't HAVE to stop at > latest. We could go all the way back to 0. But we don't have to anything: this is a byz proposer. If we notice that there is a fork, we can also commit nothing and report the replica. But we don't care...}
\nc{I think we need to change this paragraph. It's both too detailed and not detailed enough. By the end, I don't think the reader has a clear idea yet of what invariants are true about this "locally committed" log, or what the relationship is between latest() and the tips when there's forking etc. We need to explicitly list the guarantees that hold ture, and the ones that don't because of forking}

%%%%%%%%%%%%%%%%%%
\iffalse
\par \textbf{Implementing consensus.}
\sys{}'s architecture allows for a flexible choice in implementing the precise consensus mechanism. In theory, any consensus protocol (including asynchronous ones) can be employed. Because \sys{} aims to minimize latency, we opt to design a mechanism that follows a classic two-round (linear) PBFT-style ~\cite{castro1999pbft, gueta2019sbft} (or Jolteon~\cite{jolteon-ditto}) agreement pattern, and augment it with a Fast Path inspired by Zyzzyva~\cite{kotla10zyzzyva} and SBFT~\cite{gueta2019sbft} that reduces latency to a single round in gracious intervals. 
While data dissemination and consensus in \sys{} are logically distinct, the highly regular lane structure allows us to easily map consensus rounds onto cars, thereby sharing physical messages (\S\ref{sec:base_consensus}). 
%Concretely, the message pattern of one consensus instance (in good intervals) can be mapped to two cars (Fig. \ref{fig:consensus}) of one lane -- we designate the lane owner as the consensus instance leader.
\fs{next paragraph is not very important, but it's kind of interesting. Feel free to just cut!!}
In general, cars and lanes can be considered a lightweight version of Provable Broadcast (PB) chains~\cite{provable_abraham}. This chained construction is at the core of a variety of consensus mechanisms~\cite{provable_abraham}, and allows \sys{} to embed a multitude of consensus mechanisms atop the data lanes. For instance, \sys{} could be instantiated with Hotstuff~\cite{yin2019hotstuff} mapped to three cars in a lane; or chained across lanes, with one car per lane (rotating leaders).
\fi


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5 OLD / NOTES %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\iffalse

\par \textbf{Why propose \textit{certified} tips?} Proposing only tips that are certified streamlines the voting step of consensus proposals, and ensures reliable consensus progress. Since proposals consist of a vector of tip certificates, every replica can assert that every tip's entire transitive history must be available at some correct replica (if not locally). If \sys{}'s data lanes used only best-effort-broadcast and tips were uncertified, then a replica that has not yet locally observed the lane cut must first acquire (\textbf{synchronize}) the tip's data (and possibly all of its history) \fs{which can be in the order of asychrony length} to ensure that it indeed exists and thus commitment is live. It must either wait to receive it from the original broadcaster (which may never happen if the originator was Byzantine), or request it from the leader. The latter places an undue broadcasting burden on the leader \fs{this is in conflict with the motivation of moving to multi-leader designs, and away from leader bottleneck}, and requires at least 2 additional message exchanges (up to O(hisotry-size) $\sim$ length of asynchrony in the worst case, to recursively learn and fetch the missing history).
Worse, blocking to vote can result in lack of timely Quorums, causing consensus to timeout and conflicting with our goal of seamlessness. %consensus progress does not smoothly return.
\sys{}'s chained certified lanes, in contrast, guarantee that no synchronization is necessary on the critical path of consensus, thus ensuring smooth consensus progress. 

\fi



% Cars and lanes can be considered a lightweight version of pipelined Reliable Broadcasts, and Provable Broadcast (PB) chains~\cite{provable_abraham}. This chained construction is at the core of a variety of consensus mechanisms~\cite{provable_abraham}, and allows \sys{} to embed a multitude of consensus mechanisms atop the data lanes. Unlike RB and PB, cars require Quorums of only size $f+1$. This minimizes tail latencies for quorum generation, and results in a 2x reduction of signatures compared to popular RB-based DAG constructions~\cite{danezis2022narwhal, spiegelman2022bullshark}. We note that the car primitive is weaker than PB as it does not preclude equivocation. While lanes governed by honest replica's will only ever consist of a single chain, byzantine lanes may fork arbitrarily. This does not affect safety, but only affects the rate of progress made by byzantine proposers. Consensus takes as input only tips, and orders only those proposals in the tips temporal history. 


% Consensus follows a ticketing-based approach in which a replica may only propose an input when in possession of a \textit{ticket}. In its simplest form, a ticket starts corresponds to a \textit{view} \neil{Instead of corresponds I would say initiates/starts a view} in traditional BFT protocols, which specifies a leader-replica and consists of either \one a Quorum certifying commitment of the previous proposal, or \two a Quorum of votes expressing discontent with the previous proposer's progress (\textit{View Change}). While this design is straightforward, a \textit{sequential} ticket-based approach has suboptimal end-to-end latency -- for simplicity, we defer discussion of potential issues and how to optimize in Section \S\ref{sec:end-to-end}. %For simplicity, we refer to tickets and views interchangeably for the moment.




==> Sections/3-System/Protocol/core-consensus-new.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%% Re-factored version (FP integrated, coverage delayed, view logic delayed)
\subsection{Core Consensus}
\label{sec:core_consensus}

%%%%%%%%%%%%%%%%%%%%%%%% Slot based version START %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\sys{} uses a paxos-style slot-based consensus model in which leaders are assigned to a slot $s$, and can start proposing a new lane cut upon observing committment of slot $s-1$, and sufficiently many new tips to ensure the proposal is doing useful work. Within each slot, \sys{} follows a classical view based structure~\cite{castro1999pbft} -- when a slot's consensus instance fails to make timely progress, replicas arm themselves and rebel, triggering a \textit{View Change} and electing a new leader. 


Each view of consensus consists of two phases (5md total), \textit{Prepare} and \textit{Confirm}, that respectively try to achieve agreement within a view (non-equivocation), and durability across views (Fig. \ref{fig:consensus}). During gracious intervals the \textit{Confirm} phase can be omitted (Fast Path), reducing consensus latency to only a single phase (3md).

\begin{figure}[h!]
   \centering
   \includegraphics[width=0.45\textwidth]{Figures/consensus.pdf}
   \caption{Consensus logic rides the existing cars, and modifies Quorums to be of size $2f+1$. P1 = Prepare, P2 = Confirm, C = Commit}
   \label{fig:consensus}
\end{figure}


For simplicity, we first discuss consensus for only a \textbf{single} slot $s$ during a \la{Is this different from gracious? So many names, so little time...} good interval; we therefore omit explicit mention of slot-number and view in most of the discussion. 

\subsubsection{Single slot consensus in the common case.}
The protocol proceeds as follows: 
\par \textbf{Prepare Phase (P1).}

\par \protocol{\textbf{1: L} $\rightarrow$ \textbf{R}: Leader $L$ broadcasts \textsc{Prepare}.}
A leader $L$ for slot $s$ begins processing (view $v=0$) once it has received a ticket $T \coloneqq CommitQC_{s-1}$, and "sufficiently" many new data proposals to propose a cut that advances the frontier committed in $s-1$; we coin this requirement \textit{lane coverage}, and defer discussion \la {of it} to the end of the section.

The leader broadcasts a message $\textsc{Prepare} \coloneqq (\langle P \rangle_L, T) $, where proposal $P \coloneqq s, \textit{new-tips}$ \textit{new-tips} $\coloneqq [lanes[r_1],tip, ..., lanes[r_n],tip]$ is a cut of the latest certified lane tips observed by $L$. \fs{fix formatting somehow}

%Replicas that receive a Prepare message underwrite its validity if it's the first they have seen in the view. 
\par \protocol{\textbf{2: R} $\rightarrow$ \textbf{L}: Replica $R$ processes \textsc{Prepare} and votes.}
$R$ first confirms the \textsc{Prepare}'s validity: it checks that \one the ticket endorses the leader's tenure ($s = T.slot +1$) and $Leader(s) = L$), and \two $R$ has not yet voted for this slot. If it is valid, $R$ stores a copy of the proposal ($prop[s] = P$), and returns a vote $\textsc{Prep-Vote} \coloneqq \langle dig=h(P) \rangle_R$ for it's \la{muscle memory -- its} digest.

\par \protocol{\textbf{3: L}: Leader $L$ assembles Quorum of PREP-VOTE messages.}
$L$ waits for at least $n-f = 2f+1$ matching \textsc{Prep-Vote} messages from distinct replicas and aggregates them into a \textit{Prepare Quorum Certificate (QC)} $PrepareQC \coloneqq (v, dig, \{\textsc{Prep-Vote}\})$. Because honest replicas vote at most once (per view), no two PrepareQC's with different $dig$ can exist (in view $v$); this ensures agreement \textit{within} a view. To make the decision durable across views as well (the safety requirement to commit), $L$ initiates the \textit{Confirm phase}.

\par \textbf{Fast Path.} During gracious intervals $L$ may receive $n$ votes by waiting for a small timeout beyond the first $n-f$. A Quorum of $n$ votes guarantees durability, thus allowing it to proceed on the FastPath. $L$ upgrades the QC into a \textit{Fast-CommitQC} and proceeds directly to the Commit step (skip Confirm phase): it broadcasts the \textit{CommitQC}, and commits locally. 


\par \textbf{Confirm Phase (P2).}
\par \protocol{\textbf{1: L} $\rightarrow$ \textbf{R}: Leader $L$ broadcasts \textsc{Confirm}.}
$L$ forwards the $PrepareQC_v$ by broadcasting a message $\textsc{Confirm} \coloneqq \langle PrepareQC_v  \rangle$ to all replicas.

\par \protocol{\textbf{2: R} $\rightarrow$ \textbf{L}: Replica $R$ receives and acknowledges \textsc{Confirm}.}
%$R$ validates that $PrepareQc.v \geq current-view$.
$R$ returns an acknowledgment $\textsc{Confirm-Ack} \coloneqq \langle dig \rangle_R$, and buffers the \textit{PrepareQC} locally ($conf[s] = PrepareQC$) in case it must ever vote to recover the decision in a View change.

\fs{should we call this something else than highQC?}
\nc{Add some intuition as to why it's necessary to store the highest prepareQC?}

\par \protocol{\textbf{3: L} $\rightarrow$ \textbf{R}: Leader $L$ assembles \textsc{CommitQC} and commits.}
$L$ aggregates $2f+1$ matching \textsc{Confirm-Ack} messages from distinct replicas into a \textit{Commit Quorum Certificate} $CommitQC \coloneqq (v, dig, \{Confirm-Ack\})$, and broadcasts it to all replicas. Replicas that observe a CommitQC commit the associated proposal.
%Additionally, the $CommitQC_v$ acts as ticket for slot $s+1$. \fs{IN PURE VIEW VERSION: $v+1$} 

This concludes the agreement process for a single slot during a good interval. Multi-slot agreement follows naturally via the $CommitQC$ ticket design: a new consensus slot begins when the previous slot commits a proposal. We discuss in \S\ref{sec:parallel} how to orchestrate agreement for slots in parallel to reduce end-to-end latencies.

\subsubsection{Committing cuts.} \fs{Could move the ordering commit logic here.}
A committed slot's proposal (cut of lanes) can be processed and applied to the log (short, \textit{finalized}) once all previous slots have committed and finalized. \fs{Could also call it \textit{totally ordered} instead of finalized} 

Once a replica has synchronized on all proposals subsumed by a committed lane cut $\langle tips \rangle$ it must establish a total order \changebars{across the lanes}{}. \nc{for all the commands included in the cut + why does it need to establish a total order? We should probably say}\fs{sentence already starts with all proposals subsumed by the cut? Add sth like "cut represents n independent lane-logs; need to combine them to arrive at one?". Not sure the "need for a TO" needs to be justified?}. Each replica maintains a $\texttt{log}$ of all ordered requests, and a map \texttt{latest\_committed: lane-id $\rightarrow$ pos} noting the latest committed position of each lane.
% \nc{By proposal here, do you mean the last batch, certified tip, or the consensus proposal which is itself a cut (I assume it's the certified tip)}
A replica first identifies, for each lane $l$, the oldest ancestor $start_l$ of $P.tips[l]$ with a position exceeding $latest\_committed[l]$ (i.e. $start.pos == latest[l]+1$). %that could not yet have been ordered (i.e. such that $start.pos > latest[l]+1$). 
We note that the latest committed lane position may not (and need not) be the parent of $start$; for instance, the replica governing $l$ may have equivocated. This does not affect safety--it merely causes ancestors of $start$ to be ignored. \fs{it would also be safe to commit both forks! this is just simpler}

%\nc{What is start in this case? If we're staying at the highest level here, maybe lets's skip the math? it would have been easier for me to just erad "the oldest ancestor in P.tips that has not yet been committed (or that r doesn't know has committed yet}
Next, a replica updates the latest committed position for each lane ($latest\_committed[l] = tips[l].pos$), and appends to the log all new proposals (all lane proposals between, and including, $start_l$ and $P.tips[l]$) using some deterministic function. For instance, we may zip all lanes new proposals (from oldest to newest) in round-robin fashion (to provide fairness). 



\subsubsection{View change.}
In the presence of a faulty leader the protocol is not guaranteed to create the CommitQC necessary to commit. To nonetheless make timely progress \sys{} relies on timeouts to elect a new leader: replicas that observe a lack of progress rebel, and create a special \textit{Timeout Certificate} (TC) ticket in order to force a \textit{View Change}~\cite{castro1999pbft, kotla10zyzzyva}.

Each view $v$ (for a slot $s$) is mapped to one designated leader (e.g. using round-robin); to prove its tenure a leader carries a ticket, corresponding to either (in $v=0$) a ($CommitQC_{s-1}$\footnote{The view associated with a CommitQC ticket is immaterial; by safety of consensus, all CommitQC's in a slot $s$ must have the same value.}, or (in $v>0$) a Quorum of mutineers (Timeout Certificate -- TC) in view $v-1$ of slot $s$ ($TC_{(s, v-1)}$. 

\textsc{Prepare} and \textsc{Confirm} messages contain the view $v$ associated with the sending leader's tenure. Each replica maintains a $\textit{current-view}_s$, and ignores all messages with smaller views; it it receives a valid message in a higher view $v'$, it advances it's current view to $v'$. Per view, a replica sends at most one \textsc{Prep-Vote} and \textsc{Confirm-Ack}.

%Prepare validity: \two the replica has not advanced to a higher view locally ($P.v > \textit{curr-view}_R$), and \three it has not previously voted for view $P.v$. If all the above is true, it advances its current view $\textit{curr-view}_R = v$,

A replica starts a timer for view $v$ upon first observing a ticket $T_v$. \fs{Note: We should mention somewhere that having the async layer/seamlessness makes it less important to have aggressive timeouts. Pick them conservatively. If we timeout late we lose latency under failures, but we never lose throughput!!}\neil{Agreed!}

%, i.e. upon observing a $CommitQC_{s-1$, or a $TC_{(s, v)}$.
\nc{Will people understand that observing a ticket T can happen when you receive a PREPARE message from a leader in a new view?}\fs{it's intentionally more than that. I hope it's clear with the addition of the ticket section above}
%, which may be either a $CommitQC_{s-1}$ \fs{PURE VIEW VERSION: v-1} or $TC_{(s, v-1)}$. 
It cancels a timer for $v$ upon locally committing slot $s$ or observing a ticket $T_{(s, v+1)}$. Upon timing out, it broadcasts a complaint message \textit{Timeout} in which it votes for any locally observed Proposal that \textit{could have} committed: \nc{By this do you mean that it includes its highQC?}\fs{highQC and highProp yes -- I'm not sure if there is value in mentioning this here already without also giving the intuition. (the protocol box has it}
%Concretely, it includes \one it's latest received \textsc{Prepare}, and \two it's current $highQC$. 

\par \protocol{\textbf{1: R} $\rightarrow$ \textbf{R}: Replica $R$ broadcasts \textsc{Timeout}.}
A replica $R$, whose timer $t_v$ expires, initiates a call to arms by broadcasting a message $Timeout \coloneqq \langle v, highQC, highProp \rangle_R$.
$highQC$ and $highProp$ are, respectively, the $PrepareQC_{v'}$ ($conf[s]$) and proposal$_v''$ ($prop[s$) with the highest views locally observed by $R$.

%This can either be a $prepareQC_{v'}$ with $v' <= v$, or a $commitQC_{v''}$ \nc{I don't think you've said anywhere that you store the last commitQC} with $v'' <= v-1$ ($R$ would not timeout if $v'' == v$); if $v'' == v'$, precedence is given to the $commitQC$.

%For simplicity, our implementation piggybacks timeouts on available car messages (propose or vote); one may also send them externally.
%A replica that receives a Quorum of $n-f$ relevant timeout votes assembles a \textit{Timeout Quorum Certificate} $TC$ and advances its local view -- if it is the designated view leader it uses the $TC$ as ticket to begin a new Prepare phase. 

\par \protocol{\textbf{2: R} Replica $R$ forms TC and advances view.}
A replica $R$ accepts a $Timeout$ message if it has not yet advanced to a higher view ($\textit{current-view}_R \leq Timeout.v$) or locally stored $CommitQC$; in the latter case it simply forwards the $commitQC$ to the sender of $Timeout$. %, and the contained $highQC$ is a valid PrepareQC/CommitQC. 
%It can adopt the $Timeout.highQC$ as its own local $highQC_R$ if it has a bigger view \nc{Explain the logic behind that?}. 

Upon accepting $f+1$ distinct timeouts for $v$ a replica $R$ joins the mutiny, and broadcasts a $Timeout$ of its own (if it has not already); this guarantees that if one honest replica locally forms a TC, all honest replicas will. 
Upon accepting $2f+1$ distinct timeouts for $v$ a replica assembles a \textit{Timeout Certificate} $TC \coloneqq (v, \{Timeouts\}$, and advances its local view $current-view_R \coloneqq v+1$, thus ignoring all consensus messages for $v' < v+1$. Since $TC$ qualifies as a ticket for $v+1$, $R$ starts a timer for $v+1$. If $R$ is the leader for $v+1$ it additionally begins a new Prepare phase, using the TC as ticket. 

\fs{optional small optimization:} To avoid repeatedly sending the same highQC in case of consecutive timeouts a replica can instead send only a digest of the highQC, and send the Quorum itself only the \textit{once} to each replica.
\nc{Makes sense but I would maybe leave out for now}

\fs{we use the all to all version -- explain. the simplest one is sending them to the next leader, but the all to all ensures that all replicas move to a new view within bounded time (only after GST of course). MENTION VIEW SYNCHRONIZER HERE FOR OUR DEAR FRIEND ALEXEY!!!!!!!!!!!!!!!!!!}

% For safety, a leader empowered by a TC ticket must recover and re-propose any proposal that \textit{could have} committed.
% \fs{pure view version in comments:}
% %Crucially, a leader empowered by a TC ticket \textbf{must} recover and extend all proposals that may have previously committed.  

A leader $L$ that uses a TC as ticket must recover any proposal that \textit{could have} been committed at some honest replica. Given a TC a replica determines a \textit{winning proposal} by selecting the greater of \one the highest $highQC$ contained in $TC$, and \two the highest proposal present $f+1$ times in $TC$; in a tie, precedence is given to the $highQC$. 
This guarantees that if in some view $v$ a $CommitQC$ was formed for a proposal $P$, all consecutive views may only re-propose $P$. Consequently, it is safe to select as winning proposal the eligible candidate with the highest view.
\par \textbf{Safety intuition.} If $P$ committed via a $Fast-CommitQC_v$ then any Quorum of $n-f$ Timeouts must contain $f+1$ proposals. Likewise, any "slow" $CommitQC$ implies the presence of at least one $PrepareQC_v$ in the TC. Note that \one no two $PrepareQC$ with the same view can exist, and \two the existence of a $PrepareQC$ ($n-f$ \textsc{Prep-Vote}s) in view $v$ implies that no conflicting proposal could have reached a $Fast-CommitQC$ in $v$. Thus there is a unique winning proposal.

\par \protocol{\textbf{3: L} $\rightarrow$ \textbf{R}: Leader $L$ sends $\textsc{Prepare}_{v+1}$.}
Empowered by a TC ticket, leader $L$ broadcasts a message $Prepare \coloneqq (\langle v+1, \textit{tips} \rangle_L), TC_v$, where \textit{tips} is the winning proposal derived from TC; or $L's$ local certified lane cut if no winning proposal exists. Replicas that receive such a Prepare message validate $TC$, and the correctness of $tips$, and otherwise proceed with Prepare as usual.  
\fs{In most cases, it suffices to send only a digest of TC, because other replicas likely see the same (though not guaranteed)}

%%%%%%%%%%%%%%%%%%%%%%%%% LANE COVERAGE %%%%%%%%%%%%%%%%%%%%%%%5
\subsubsection{Lane Coverage.}
To minimize the number of required consensus instances\fs{waste/redundancy}, honest leaders in \sys{} will only initiate a new proposal once data lanes have made ample progress. \changebars{}{(w.r.t the preceding slot's committed proposal)} 

We call this requirement \textit{lane coverage} -- it is a tunable hyperparameter presenting a trade-off between latency, efficiency, and fairness. By default we set coverage to $\geq n-f$ new tips ($\geq n-f$ lanes with $>=1$ new proposal each), the maximum possible in presence of failures, to maximize resource efficiency and ensure that at least half of the included tips are associated with honest governed lanes %(\S\ref{sec:fairness}).
However, flexible configurations are possible depending on system preference. \fs{Optional discussion, can cut:} A system with heterogeneous lane capacities and pace, for instance, may opt to reduce the coverage criterion to a single lane to minimize latency. Likewise, if latency is less imperative, one may strengthen the criterion to require $>1$ new cars per lane to minimize the number of required instances; in this case, one may consider replacing intermittent cars (all but the tip) by best effort broadcasts to further reduce costs. 

Intuitively, lane coverage governs the \textit{pace} of consensus: consensus need not make progress if data lanes have not advanced. We tune timeouts in the consensus layer to account for leaders waiting for coverage. 
Notably, lane coverage enforces only a lower bound on required progress, and does not cause \sys{} to discriminate against slow lanes. Unlike contemporary DAG-BFT protocols that are governed by only the fastest $n-f$ replicas, and are subject to \textit{orphaning} proposals of the $f$ slowest, proposals in \sys{} include cut's of \textit{all} $n$ lanes. Consequently, all (honest) replicas proposals are guaranteed to eventually commit. \fs{at most one consensus instance after not being included in the first n-f => this interplays nicely with the parallel consensus below!}.
\fs{TODO: Improve/Re-work the above paragraph: It would be nice to highlight that this is a property of logically independent layers. n-f fastest athletes drive consensus, but they are just the messengers for the mail of ALL replicas. In DAG consensus and dissemination roles are intertwined, so n-f that drives consensus implies n-f whose mail is delivered}

Lane coverage in \sys{} is best effort and not enforced. From a performance perspective, a Byzantine leader that disregards coverage is no different than a leader that stays silent; from a fairness perspective, it is equivalent to leaders in traditional BFT protocols assembling batches at will. The next honest leader in a good interval will make up for any "lost" coverage. 
\fs{if we are worried about a byz wasting resources (messages, sigs, etc) then we could enforce} 


% \fs{A nice thing of our design is that unlike DAG protocols, we don't have orphans. A consensus protocol can have up to $n$ new proposals. So if any honest becomes leader, and has seen another honest replicas lane state, then it will propose it. I.e. eventually an honest replica will always propose honest tips (DAGS artificially limit to n-f edges to ensure progress, and then need weak edges etc to save orphans)}
% \fs{The fast replicas partake in consensus progress, but this is independent from inclusion!!}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%% PARALLEL CONSENSUS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Parallel Multi-Slot Agreement}
\label{sec:parallel}

\sys{} consensus, by default, proceeds through a series of \textit{sequential} slots instances. Unfortunately, lane proposals that narrowly miss inclusion in the current slot's proposed consensus cut may, in the worst case, experience the sequential latency of up to two consensus instances. Tips that "miss the bus" experience wait-time for the current consensus proposal to commit -- including any number of view changes necessary to do so --, and the latency of the next consensus instance (in which they are covered). \fs{In expectation, the experienced consensus latency is thus 1.5x the advertised delay.}


\par \textbf{Parallel Consensus.}
To circumvent sequential wait-times, \sys{}, inspired by PBFT~\cite{castro1999pbft}, allows for a new slot instance to begin in parallel with ongoing slots; instead of only upon commitment of the preceding slot. 
We modify a slot ticket for $s$ to no longer require a $CommitQC_{s-1}$: the leader of slot $s$ can begin consensus for slot $s$ as soon as the first \textsc{Prepare}$_{s-1}$ message (the view is immaterial), and lane coverage is satisfied (w.r.t to \textsc{Prepare}$_{s-1}$). This encourages honest leaders to not issue redundant proposals, minimizing wastage. Lane coverage is once again best effort and, in fact, cannot be enforced as it is not guaranteed that $\textsc{Prepare}_{s-1}$ represents the proposal that is ultimately committed in slot $s-1$ (e.g. due to a View Change).

% \fs{NOTE: It actually CANNOT be strictly enforce. Reason in comments:}  
% While we may demand to reference \textit{some} $\textsc{Prepare}_{s-1}$ as ticket, we cannot guarantee that it represents the proposal that is ultimately committed in slot $s-1$. \fs{e.g. view change could change} \fs{Note: If we are not enforcing coverage, then there is no need for a ticket: I.e. the Prepare does not need to be included}

\fs{cutting figure since I've moved ride sharing into optimizations only}
% \begin{figure}[h!]
%     \vskip -5pt
%    \centering
%    \includegraphics[width=0.45\textwidth]{Figures/pipeline.pdf}
%    \vskip -5pt
%    \caption{$\textsc{Prepare}_{s+1}$ can begin upon receiving $\textsc{Prepare}_s$.}
%    \label{fig:pipeline}
%    \vskip -5pt
% \end{figure}


When instantiated with a stable leader there is no sequential wait-time imposed by consensus (still subject to lane coverage). %; a new slot begins as soon as $n-f$ lanes have made progress (coverage)\fs{THIS IS IMPRECISE. ONLY TRUE IF NOT RIDE SHARING. IF RIDE SHARING THEN WE HAVE TO WAIT FOR CAR ==> LATENCY IS ACTUALLY 2}. 
With rotating leaders, the wait-time is at most 1md; the time to receive $\textsc{Prepare}_{s-1}$. %\fs{this is why we have separate views per slots}. 
%Figure \ref{fig:pipeline} illustrates two pipelined instances embedded onto separate lanes.

To manage parallel slot instances we adjust \sys{} as follows.

\par \textbf{Managing concurrent instances.}
\sys{} maintains independent state for all ongoing consensus slot instances. Each instance has its own consensus messages, and is agnostic to consensus processing on all concurrent slots. 
%Messages of different instances can, however, ride the same cars; we discuss in Section \S\ref{sec:optimizations} how to share signature costs. 
Slots that commit wait to \textit{finalize} until all preceding slot instances have been finalized first. Upon finalizing a slot's proposal (a cut of tips), \sys{} replicas identify and order only proposals that are new. As discussed above, it is not guaranteed that consecutive slot's propose monotonic cuts; non-monotonic tip positions are simply ignored. \fs{i.e. we don't try to order/apply multiple forks.}  \fs{Sync happens asynchronously, and might do redundant work.}


\par \textbf{Adjusting view synchronization.}
To account for parallel, overlapping instances, replicas no longer begin a timer for slot $s$ upon reception of a $CommitQC_{s-1}$, but upon reception of the first $\textsc{Prepare}_{(s-1, v)}$ message. \fs{timeouts should account for time it might take to forward Prepare to the leader that needs it + time to get coverage}. 
Additionally, we adjust the leader-election scheme to decorrelate view changes across successive slots. If the same round-robin schedule were applied across and within slots, the worst case number of view changes to finalize $k$ successive slots is $\frac{k * (f+1)}{2}$, as each slot must rotate through the same faulty leaders. To avoid this, we shift round-robin assignment for slots by $f$; random election is feasible too. 

\par \textbf{Bounding parallel instances.}
During good intervals there will likely be at most 3-4 concurrent instances at a time\footnote{Each instance incurs $\leq 4md$ (Prepare + opt Confirm) before sending commit message. Thus up to 4 instances can open}. In periods of asynchrony (or in presence of faulty leaders) this number can grow arbitrarily large: new instances may keep opening (they only need to observe a proposal and coverage \fs{data layer keeps growing!}), but instances are not closing at the same rate. These instances are not beneficiary, as a single instance in the next good interval can subsume all such proposals with a single new cut.
To avoid wastage, and simplify garbage collection, we can bound the maximum number of open instances to some $k$ by (re-)introducing delayed CommitQC tickets. To begin slot instance $s$, one must include a ticket $CommitQC_{s-k}$. 
When committing slot $s$ we can thus garbage collect the commitQC for slot $s-k$ as $CommitQC_s$ transitively certifies commitment for slot $s-k$. \fs{(and $s-2k$, $s-3k$, ...).}\fs{(Note, cannot gc everything $< s-k$; need to wait for finalization to do that -- however, $s-k-1$ will have been GC by $s-1$ already, and so forth)}

\fs{Bonus argument: If we only use Prepare as ticket, then the commitQC for each slot must be kept around in order to reply to view changes. e.g. to help inform replicas that haven't committed). We'd like to bound this. Can do so either by active checkpointing (requires synchronization), or by leveraging the depth limiter} 

\par \textbf{Discussion.}
\fs{Reason for parallelizing this way (and not chained): READ IT!!! -> and then decide whether to cut or move to related work} 
\sys{}'s parallel proposals resemble modern chained-BFT protocols~\cite{2023beegees, yin2019hotstuff, jolteon-ditto} which pipeline consensus phases (e.g. piggyback $\textsc{Prepare}_{s+1}$ on $\textsc{Confirm}_s$). \sys{} too could be configured such a way, yet we opt against it for three reasons: \one pipelining phases is not latency optimal as it requires at least 2md between proposals \fs{rigid}, \two it introduces liveness concerns that require additional complexity to circumvent~\cite{2023beegees}, and \three it correlates the coverage criterion for successive slots, i.e. coverage for slot 2 affect progress of slot 1. 
\sys{}'s slot based consensus, in contrast, is straightforward to parallelize, and, so we hope, more easily accessible to a wider audience. 
%\fs{it does however introduce more signatures possible, which requires finicky optizations if it should be a bottleneck. If signatures are the bottleneck nothing stops us from just using a pipelined HS-like consensus alternatively}


==> Sections/3-System/Protocol/core-consensus.tex <==

\iffalse
%\subsection{On a highway to... throughput}
\subsection{Layering partially sync consensus.}
\label{sec:consensus}
%Motorway -- layering partially sync consensus atop async dissemination.

The role of the consensus layer in \sys{} is to totally order the disseminated proposals from all data lanes. Unlike traditional BFT consensus protocols, that take as input a batch of requests to commit, \sys{}'s consensus tries to commit each lanes' history by taking as input a snapshot (or \textit{cut}) of observed lane tips. This achieves two things:
\one First, proposing a vector of tips allows \sys to achieve consensus throughput that scales horizontally with the number of lanes ($n$ total) and their volume. Upon committing a consensus proposal (a vector of tips -- not to be confused with data proposals), \sys{} replicas deterministically zip the not yet committed data proposals of \textit{all} $n$ lanes into one consistent total order. 
\two \fs{this is a direct callback/duplicate of the data dissemination point} Second, proposing only tips it enables \sys{} to commit all proposals in a lane with constant complexity, irrespective of the lane's length. While consensus in \sys{} is partially synchronous, that is, it only guarantees to make progress committing during periods of synchrony, data lanes grow unimpeded even during asynchrony. Upon return to the first \textit{good} interval, \sys{} immediately commits the entire un-committed backlog of all lanes, thus achieving seamlessness.


\sys{}'s architecture allows for a flexible choice in selecting the precise consensus mechanism. In theory, any consensus protocol (including asynchronous ones) can be employed. Because \sys{} aims to minimize latency, we opt to design a mechanism that follows a classic two-round (linear) PBFT-style ~\cite{castro1999pbft, gueta2019sbft} (or Jolteon~\cite{jolteon-ditto}) agreement pattern, and augment it with a Fast Path inspired by Zyzzyva~\cite{kotla10zyzzyva} and SBFT~\cite{gueta2019sbft} that reduces latency to a single round in gracious intervals. 
While data dissemination and consensus in \sys{} are logically distinct, the highly regular lane structure~\cite{provable_abraham} allows us to easily map consensus rounds onto cars, thereby sharing physical messages (\S\ref{sec:base_consensus}). Concretely, the message pattern of one consensus instance (in good intervals) can be mapped to two cars (Fig. \ref{fig:consensus}) of one lane -- we designate the lane owner as the consensus instance leader.\footnote{Similarly, we could employ and map other popular protocols. For instance, Hotstuff~\cite{yin2019hotstuff} could be mapped to three cars in a lane; or chained across lanes, with one car per lane (rotating leaders).}

In the following, we outline and discuss in detail all components of \sys{} consensus. 
%We first discuss consensus for a single proposal (one consensus instance), and then generalize to multiple proposals necessary to realize State Machine Replication. 
Consensus follows a ticketing-based approach in which a replica may only propose an input when in possession of a \textit{ticket}. In its simplest form, a ticket starts corresponds to a \textit{view} \neil{Instead of corresponds I would say initiates/starts a view} in traditional BFT protocols, which specifies a leader-replica and consists of either \one a Quorum certifying commitment of the previous proposal, or \two a Quorum of votes expressing discontent with the previous proposer's progress (\textit{View Change}). While this design is straightforward, a \textit{sequential} ticket-based approach has suboptimal end-to-end latency -- for simplicity, we defer discussion of potential issues and how to optimize in Section \S\ref{sec:end-to-end}. %For simplicity, we refer to tickets and views interchangeably for the moment.

%TODO: Iterate through series of views. View corresponds to new leader -- view change indicates that we committed something
\fi

\subsection{Core Consensus}
\label{sec:base_consensus}

%%%%%%%%%%%%%%%%%%%%%%%% Slot based version START %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\fs{shorten this.}
\nc{I don't think most of the text is necessary here beyond the "paxos style" consensus protocol, where leaders are assigned to slots and can start proposing once they have 1) seen a commit QC for round s-1, and once they 2) have seen sufficiently many new tips to ensure each new proposal is "useful" *AND THAT'S IT*. The rest you can sprinkle in the pseudocode. Instead, I would focus on how "elegant" the relationship is with the data sync phase}
\sys{} uses a paxos-style slot-based consensus model. %, in which we try and commit a proposal for slot s before we commit slot s+1. 
We say that a slot commits upon reaching agreement on an input proposal; a slot finalizes (and can be applied to the log) if all previous slots have committed and finalized (or it is genesis). \fs{i.e finalized = proposal has finality, i.e. its log position is fixed. Could also call it \textit{totally ordered} instead of finalized} 

In its simplest form, a new consensus slot begins when the previous slot commits a proposal; only one slot is actively reaching consensus at a time. We discuss in \S\ref{sec:end-to-end} how to orchestrate agreement for slots in parallel to reduce end-to-end latencies.

\nc{Would be simpler I think (and more direct in the flow, to talk about committing consensus proposals here (and the cuts). Right now it looks like you're describing completely orthogonal protocols.}

Within each slot, \sys{} follows a classical view based structure. %that is rooted in (linear) PBFT~\cite{castro1999pbft, gueta2019sbft} and Jolteon~\cite{jolteon-ditto}. 

When a slot's consensus instance fails to make timely progress, replicas arm themselves and rebel, triggering a \textit{View Change}.
\nc{You say 1) consensus happens one slot at a time, but in SX we discuss how to make it parallel. For simplicity we only discuss for a single slot. I feel like this gets a little bit ocnfusing. I'd remove that first paragraph and just say, for simplicityl we talk about a single slot. We talk about multislot next (or something along those lines)}

Each (slot, view) pair $(s, v)$ is mapped to one designated leader (e.g. using round-robin); to prove its tenure a leader carries a ticket, corresponding to either a Quorum certifying successful commitment of a proposal in slot $s-1$ ($CommitQC_{s-1}$\footnote{The view associated with a CommitQC ticket is immaterial; by safety of consensus, all CommitQC's in a slot $s$ must have the same value.}) (ticket for $(s, v=0)$) \neil{would just explicitly write in parentheses that this is a ticket for the case v=0}, or a Quorum of mutineers (Timeout Certificate -- TC) in view $v-1$ of slot $s$ ($TC_{(s, v-1)}$ (ticket for $(s, v>0)$).
\fs{Should we just get rid of the CommitQC ticket? Since we don't enforce coverage, it's not "necessary" to have. However, it does explicitly make it such that slots cannot overlap (are sequential) which might simplify understanding. Our parallel optimization weakens this constraint.}

For simplicity, we discuss consensus for only a \textbf{single} slot $s$ during a good interval; we therefore omit explicit mention of slot-number in most of the discussion. Consensus naturally extends to multi-shot consensus via the above ticketing mechanism.

\par \textbf{Consensus Proposals.}
A leader $L$ for slot $s$ begins a new view $v=0$ once it has received a ticket $T_s \coloneqq CommitQC_{s-1}$.
%that is empowered with a ticket $T_s \coloneqq CommitQC_{s-1}$ begins a new view $v = 0$ by creating a new consensus proposal. \fs{find different name for Proposal in data lane and consensus}


%%%%%%%%%%%%%%%%%%%%%%%% Slot based version END %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%% Purely view based version START %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\iffalse 
Consensus in \sys{} follows a classical view based structure that is rooted in (linear) PBFT~\cite{castro1999pbft, gueta2019sbft} and Jolteon~\cite{jolteon-ditto}\fs{are we most similar to Jolteon?}\neil{Yeah, I lean more toward Jolteon rather than linear PBFT since technically we don't use multi/threshold signatures in the implementation}.\footnote{We discuss in \S\ref{sec:optimizations} how to use an all-to-all message paradigm to tradeoff increased complexity for lower latency.}

Consensus changes views whenever \one a consensus proposal commits, or \two progress times out, and replicas arm themselves and revolt. Each view $v$ is mapped to one designated leader (e.g. using round-robin); to prove its tenure a leader carries a ticket, corresponding to either a Quorum certifying successful commitment (good case) or a Quorum of mutineers in view $v-1$ (failure case). 
Each view of consensus consists of two phases, \textit{Prepare} and \textit{Confirm}, that respectively try to achieve agreement within a view (non-equivocation), and durability across views (Fig. \ref{fig:base_consensus}). For simplicity, we first outline the protocol during a good interval in which the ticket corresponds to a commitment.


%We describe the good and failure case in order.
\neil{I was a bit confused before since this seems like the "chained" version of Jolteon (but without the optimization where a single vote can be for multiple proposals) where there is not a distinction between views and slots whereas for the pipelined version each consensus instance is completely independent (the views are not shared across instances). Maybe add a sentence that once a commit happens, replicas move to the next height/sequence number in addition to going to the next view}
\neil{If this is intended to just be for single-shot consensus, then I would just say that views advance when enough replicas timeout (exception for view 1 which starts immediately)}
\neil{TLDR; there is a mix of single-shot/multi-shot that I find a little confusing. The fact that a ticket can be a commit QC in the previous view seems more like multi-shot since for single-shot you would just terminate once you receive a commit QC (specifically "chained" where views are incremented across multiple consensus instances (unlike pipelined where all instances are completely independent) but the rest seems to be more like a single-shot description}
\fs{It is multi-shot, but you are right it's not clear enough currently. Originally I was thinking of describing the slot based stuff first, but I felt like it was needlessly confusing because this section does not yet depend on it. So I tried to go with view changes that could either be QC or TC. Maybe it's easier to mention slot after all: Ticket with QC starts new slot. Ticket with TC extends view in a slot. } \fs{Technically one doesn't need to mention slot height's at all. It's implicit via the ticket chain.}\neil{Yeah in that case I would mention slot/height/sequence number in some capacity (even if it is implicit you can just note that because otherwise it's hard to tell whether it's single or multi-shot), so that way the transition to the pipelined version is smoother.}

\par \textbf{Consensus Proposals.}
A leader $L$ that is empowered with a ticket $T_v \coloneqq CommitQC_{v-1}$ begins a new view $v$ by creating a new consensus proposal. \fs{find different name for Proposal in data lane and consensus}

\fi
%%%%%%%%%%%%%%%%%%%%%%%%%%% Purely view based version END %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\iffalse 
 Unlike proposals in traditional BFT protocols (that consists of batches of requests), a consensus proposal in \sys{} corresponds to a snapshot \textit{cut} of all data lanes. Concretely, it consists of a vector of the $n$ \textit{certified} tips observed by the leader. \neil{Would just explicitly emphasize that what's proposed are certificates containing the metadata and not the tip (data) itself} Fig. \ref{fig:car_lanes} illustrates an example cut that might correspond to the latest certified tips at some replica.
\fs{proposing a vector of locally observed certified tips is pretty much analogous to having edges in the DAG. But I'm hoping that describing things bottom up, rather than comparing to DAG makes it easier for non-DAG experts.}

\fs{TODO: Cert is not necessary to protect against "just" asynchrony; it's meant to safeguard against byz abuse.}

\par \textbf{Why propose \textit{certified} tips?} Proposing only tips that are certified streamlines the voting step of consensus proposals, and ensures reliable consensus progress. Since proposals consist of a vector of tip certificates, every replica can assert that every tip's entire transitive history must be available at some correct replica (if not locally). If \sys{}'s data lanes used only best-effort-broadcast and tips were uncertified, then a replica that has not yet locally observed the lane cut must first acquire (\textbf{synchronize}) the tip's data (and possibly all of its history) \fs{which can be in the order of asychrony length} to ensure that it indeed exists and thus commitment is live. It must either wait to receive it from the original broadcaster (which may never happen if the originator was Byzantine), or request it from the leader. The latter places an undue broadcasting burden on the leader \fs{this is in conflict with the motivation of moving to multi-leader designs, and away from leader bottleneck}, and requires at least 2 additional message exchanges (up to O(hisotry-size) $\sim$ length of asynchrony in the worst case, to recursively learn and fetch the missing history).
Worse, blocking to vote can result in lack of timely Quorums, causing consensus to timeout and conflicting with our goal of seamlessness. %consensus progress does not smoothly return.
\sys{}'s chained certified lanes, in contrast, guarantee that no synchronization is necessary on the critical path of consensus, thus ensuring smooth consensus progress. 
 %It can commit a tip once it has learned of the required lane history. \fs{we can again separate meta data and data here.}
\fi

%%%%%%%%%%%%%%% BEGIN COVERAGE 
\fs{This discussion can also move later if we want}
\par \textbf{Coverage.} To minimize the number of required consensus instances\fs{waste/redundancy}, honest leaders in \sys{} will only initiate a new proposal once they have observed sufficiently many new tips \changebars{}{(w.r.t the preceding slot's committed proposal)} to conclude that the data lanes have made ample progress. 
%\neil{I find the the cut terminology clearer, maybe something like honest leaders only propose monotonic cuts} \fs{I'd like to say that, but it's not quite accurate. It would only be monotonic if all $n$ are newer}
We call this requirement \textit{lane coverage} \changebars{}{-- it is a tunable hyperparameter presenting a trade-off between latency, efficiency, and fairness}; by default we set coverage to $2f+1$ new tips ($2f+1$ lanes with $>=1$ new proposal each) % to ensure that at least half of them are associated with honest governed lanes (\S\ref{sec:fairness}.  
\nc{Why is 2f+1 the magic number? You could imagine f+1 as that would ensure that we're proposing honest nodes' proposals at least}\fs{see text continuation in comment (fairness) -- can add it back in; I had removed it because talking about chain quality is difficult} 
\fs{Can set coverage to 1 to allow any new proposal to commit asap -- this is a tradeoff between latency (useful if only few nodes have new proposals) vs efficiency (less consensus instances) and fairness (chain equality) } 
Intuitively, coverage governs the pace of consensus: consensus need not make progress if data lanes have not advanced. We tune timeouts in the consensus layer to account for leaders waiting for coverage. \fs{Note: We should mention somewhere that having the async layer/seamlessness makes it less important to have aggressive timeouts. Pick them conservatively. If we timeout late we lose latency under failures, but we never lose throughput!!}\neil{Agreed!}

Lane coverage in \sys{} is best effort and not enforced. From a performance perspective, a Byzantine leader that disregards coverage is no different than a leader that stays silent; from a fairness perspective, it is equivalent to leaders in traditional BFT protocols assembling batches at will. The next honest leader in a good interval will make up for any "lost" coverage. 
\nc{This feels like an unnecessarily lengthy discussion at this stage. I would remove this discussion fully and merge the "Consensus Proposal" paragraph into the first phase of the pseudocode, adding an extra sentence saying "when the leader has sufficient new data to propose.  We coin this term "lane coverage". }\fs{agree, will do}
\fs{if we are worried about a byz wasting resources (messages, sigs, etc) then we could enforce} 

% \fs{IGNORE: Note: Don't "need" a CommitQC ticket to start a new slot if we don't enforce coverage. It may be simpler didactically though to have it to illustrate this is sequential}
%\nc{Not sure that I understand your comment here}
\fs{A nice thing of our design is that unlike DAG protocols, we don't have orphans. A consensus protocol can have up to $n$ new proposals. So if any honest becomes leader, and has seen another honest replicas lane state, then it will propose it. I.e. eventually an honest replica will always propose honest tips (DAGS artificially limit to n-f edges to ensure progress, and then need weak edges etc to save orphans)}

%%%%%%%%%%%%%%%%% END COVERAGE
Each view of consensus consists of two phases, \textit{Prepare} and \textit{Confirm}, that respectively try to achieve agreement within a view (non-equivocation), and durability across views (Fig. \ref{fig:consensus}).

\begin{figure}[h!]
   \centering
   \includegraphics[width=0.45\textwidth]{Figures/consensus.pdf}
   \caption{Consensus logic rides the existing cars, and modifies Quorums to be of size $2f+1$. P1 = Prepare, P2 = Confirm, C = Commit}
   \label{fig:consensus}
\end{figure}

The protocol proceeds as follows: 
\par \textbf{Prepare Phase (P1).}

\par \protocol{\textbf{1: L} $\rightarrow$ \textbf{R}: Leader $L$ broadcasts \textsc{Prepare}.}
\nc{Note: we probably want to do the same we did for Basil regarding view logic. Defer it to later} A leader that has met sufficient lane coverage assembles and broadcasts to all replicas a message $\textsc{Prepare} \coloneqq \langle s, T, v=0, new-tips \rangle_L $, where $T \coloneqq CommitQC_{s-1}$ is its ticket \fs{IF PURE VIEW VERSION: $CommitQC_{v-1}$,  $v \coloneqq T.v+1$ the view for the leaders tenure}, and $new-tips \coloneqq <tips[1][lane-1.length], ..., tips[n][lane-n.length]>$ is a vector of the latest certified tips observed by $L$. \nc{Why[1] in this case?}

%Replicas that receive a Prepare message underwrite its validity if it's the first they have seen in the view. 
\par \protocol{\textbf{2: R} $\rightarrow$ \textbf{L}: Replica $R$ processes \textsc{Prepare} and votes.}
$R$ first confirms the \textsc{Prepare}'s validity. 
\textsc{Prepare} is considered valid if \one the ticket endorses the leader and the proposed view ($P.v = P.T.view + 1$ and $Leader(P.v) = L$), \two the replica has not advanced to a higher view locally ($P.v > \textit{curr-view}_R$), and \three it has not previously voted for view $P.v$. If all the above is true, it advances its current view $\textit{curr-view}_R = v$, stores a digest of the proposal $votes[v] = h(\textsc{Prepare})$, and returns a vote $\textsc{Prep-Vote} \coloneqq \langle v, h(\textsc{Prepare}) \rangle_R$.
\neil{May want to just move the view advancement logic to the synchronizer or mention that views only advance once you receive a TC (assuming you mean single-shot here)}
\par \protocol{\textbf{3: L}: Leader $L$ assembles \textsc{PrepareQC} \nc{of PREP-VOTE messages}.}
$L$ aggregates $2f+1$ \nc{2f+1 or n-f, 2f+1 right?} matching \textsc{Prep-Vote} messages from distinct replicas into a \textit{Prepare Quorum Certificate} $PrepareQC \coloneqq (v, dig=h(Prep), \{Prep-Vote\})$.
\nc{let's make sure capitalisation of prep-votes is consistent. Should we also mention that the leader will timeout if it fails to receive a quorum of prepareQCs?}

Because honest replicas vote at most once per view, no two PrepareQC's with different $dig$ can exist in view $v$. This ensures agreement \textit{within} a view. To make the decision durable across views as well, and thus commit, $L$ begins the \textit{Confirm phase}.

\par \textbf{Confirm Phase (P2).}
\par \protocol{\textbf{1: L} $\rightarrow$ \textbf{R}: Leader $L$ broadcasts \textsc{Confirm}.}
$L$ forwards the $PrepareQC_v$ by broadcasting a message $\textsc{Confirm} \coloneqq \langle PrepareQC_v  \rangle$ to all replicas.
\nc{is there a reason why we don't describe the fast path here as well? Seems like we want to talk about the fast path as the "default" rather than an optimisation afterwards}

\par \protocol{\textbf{2: R} $\rightarrow$ \textbf{L}: Replica $R$ receives and acknowledges \textsc{Confirm}.}
$R$ validates that $PrepareQc.v \geq current-view$. %, and \two confirms that all signatures are valid.
If so, it buffers the PrepareQC locally ($highQC = PrepareQC$) \fs{should we call this something else?} and return an acknowledgment $\textsc{Confirm-Ack} \coloneqq \langle v, dig \rangle_R$.
\nc{Add some intuition as to why it's necessary to store the highest prepareQC?}

\par \protocol{\textbf{3: L} $\rightarrow$ \textbf{R}: Leader $L$ assembles \textsc{CommitQC} and commits.}
$L$ aggregates $2f+1$ matching \textsc{Confirm-Ack} messages from distinct replicas into a \textit{Commit Quorum Certificate} $CommitQC \coloneqq (v, dig, \{Confirm-Ack\})$, and broadcasts it to all replicas. Replicas that observe a CommitQC commit the associated proposal.
%Additionally, the $CommitQC_v$ acts as ticket for slot $s+1$. \fs{IN PURE VIEW VERSION: $v+1$} 

This concludes the agreement process during a good interval. 
\nc{It feels like including the fast path in the description (or at least before the view change) would help make the protocol "interesting" soudning rather than put all the "meat" in an optimisation section? I also see the argument for starting as simple as possible}
%Next, we outline how to construct an ordered log from a committed vector of tips.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% ORDERING
\iffalse
\par \textbf{Commit: Ordering lane states.} Each replica maintains a commit state consisting of \one a log of all ordered requests, and \two a map $latest: r \rightarrow height$ noting the height of the latest committed proposal of each lane.
Upon committing a new proposal $P$, \sys{} replicas identify, for each lane $l$, the oldest ancestor $start_l$ of $P.new-tips[l]$ that could not yet have been ordered (i.e. such that $start.height > latest[l]+1$). 
Then, they update $latest[l] = P.new-tips[l].height$ for each lane, and append to the log all new proposals (all lane proposals between, and including, $start_l$ and $P.new-tips[l]$) using some deterministic function. For instance, to provide fairness, we may zip all lanes new proposals (from oldest to newest) in round-robin fashion. 

Note that in order to \textit{commit} a lane and execute a proposal, a replica may still need to first synchronize on missing data. Crucially, however, this wait is local to each replica and does not hold up consensus progress: other replicas may already be able to locally commit and execute, and new consensus proposals can already proceed with agreement in parallel. 
To minimize commit delays, \sys{} replicas begins synchronizing on missing data asynchronously and in parallel upon voting for a missing certified tip.


\fs{Note, that latest locally committed lane proposal doesn't have to be an ancestor of start. It also doesn't have to be +1. this could happen if the lane was forked. I explicitly didn't say ancestor that has not yet committed -> there might be older ancestors that will not ordered even though they have heights < latest} \fs{we also don't HAVE to stop at > latest. We could go all the way back to 0. But we don't have to anything: this is a byz proposer. If we notice that there is a fork, we can also commit nothing and report the replica. But we don't care...}

\fi

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% END GOOD INTERVAL BASICs %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\par \textbf{View change.}
In the presence of a faulty leader the protocol is not guaranteed to create the CommitQC necessary to commit in a view. To nonetheless make progress \sys{} relies on timeouts to elect a new leader: replicas that observe a lack of progress mutiny \nc{rebel}, and create a special \textit{Timeout Certificate} (TC) ticket in order to force a \textit{View Change}~\cite{castro1999pbft, kotla10zyzzyva}. 

A replica starts a timer for view $v$ upon first observing a ticket $T_v$.
\nc{Will people understand that observing a ticket T can happen when you receive a PREPARE message from a leader in a new view?}
%, which may be either a $CommitQC_{s-1}$ \fs{PURE VIEW VERSION: v-1} or $TC_{(s, v-1)}$. 
It cancels a timer for $v$ upon locally committing slot $s$ or observing a ticket $T_{(s, v+1)}$. Upon timing out, it broadcasts a complaint message \textit{Timeout} in which it votes for any locally observed Proposal that \textit{could have} committed\nc{By this do you mean that it includes its highQC?}. 

\par \protocol{\textbf{1: R} $\rightarrow$ \textbf{R}: Replica $R$ broadcasts \textsc{Timeout}.}
A replica $R$, whose timer $t_v$ expires, initiates a call to arms by broadcasting a message $Timeout \coloneqq \langle v, highQC \rangle_R$.
$highQC$ is the $PrepareQC$ with the highest view locally observed by $R$. 

\fs{Old Pure View version: This can either be a $prepareQC_{v'}$ with $v' <= v$, or a $commitQC_{v''}$ with $v'' <= v-1$ ($R$ would not timeout if $v'' == v$); if $v'' == v'$, precedence is given to the $commitQC$.}

%For simplicity, our implementation piggybacks timeouts on available car messages (propose or vote); one may also send them externally.
%A replica that receives a Quorum of $n-f$ relevant timeout votes assembles a \textit{Timeout Quorum Certificate} $TC$ and advances its local view -- if it is the designated view leader it uses the $TC$ as ticket to begin a new Prepare phase. 

\par \protocol{\textbf{2: R} Replica $R$ forms TC and advances view.}
A replica $R$ accepts a $Timeout$ message if it has not yet advanced to a higher view ($current-view_R \leq Timeout.v$).%, and the contained $highQC$ is a valid PrepareQC/CommitQC. 
It adopts the $Timeout.highQC$ as its own local $highQC_R$ if it has a bigger view \nc{Explain the logic behind that?}\fs{this is no different than receiving a new Confirm; one's own highQC could not possibly "win". TBH there isn't really much point in this... happy to just remove}. 
If it has locally stored a $CommitQC$ \fs{pure view version: $commitQC_v'$ with $v'>v$,} then it simply forwards it to the sender of $Timeout$.

Upon accepting $f+1$ distinct timeouts for $v$ a replica $R$ joins the mutiny, and broadcasts a $Timeout$ of its own (if it has not already); this guarantees that if one honest replica locally forms a TC, all honest replicas will. 
Upon accepting $2f+1$ distinct timeouts for $v$ a replica assembles a \textit{Timeout Certificate} $TC \coloneqq (v, \{Timeouts\}$, and advances its local view $current-view_R \coloneqq v+1$, thus ignoring all consensus messages for $v' < v+1$. Since $TC$ qualifies as a ticket for $v+1$, $R$ starts a timer for $v+1$. If $R$ is the leader for $v+1$ it additionally begins a new Prepare phase, using the TC as ticket. 

\fs{optional small optimization:} To avoid repeatedly sending the same highQC in case of consecutive timeouts a replica can instead send only a digest of the highQC, and send the Quorum itself only the \textit{once} to each replica.
\nc{Makes sense but I would maybe leave out for now}

\fs{we use the all to all version -- explain. the simplest one is sending them to the next leader, but the all to all ensures that all replicas move to a new view within bounded time (only after GST of course). MENTION VIEW SYNCHRONIZER HERE FOR OUR DEAR FRIEND ALEXEY!!!!!!!!!!!!!!!!!!}

% For safety, a leader empowered by a TC ticket must recover and re-propose any proposal that \textit{could have} committed.
% \fs{pure view version in comments:}
% %Crucially, a leader empowered by a TC ticket \textbf{must} recover and extend all proposals that may have previously committed.  

A leader $L$ that uses a TC as ticket must recover any proposal that \textit{could have} been committed at some honest replica. It thus must re-propose the $PrepareQC$ with the highest view contained in the TC; if none exist, the leader may propose a new cut. This is safe: If ever there existed $2f+1$ PrepareQC's in the same view (i.e. a CommitQC could exist), then (by Quorum intersection) all TC's must contain the PrepareQC (as the highest view) \nc{I could not understand this sentence, do you mean "will contain at least one instance of this prepareQC, and that instance will necessarily be the one with the highest view (that'd be my understanding of how it works)?}, and thus every consecutive view change must have recovered and re-proposed the same proposal. \fs{because every TC is of size 2f+1.}
\fs{pure view version in comments}
% We note that a PrepareQC in some view $v'$ (by quorum intersection) must extend all committed proposals (commitQC exists) in views $< v'$; if it does not, an honest replica must have cast a faulty Prepare-Vote -- a contradiction. \neil{Clarify what "extend all committed proposals means since it is not very well defined (ties back to the earlier comment about whether I should think of this as single-shot or multi-shot)} Moreover, there can be at most one PrepareQC and CommitQC per view, respectively.
% Consequently, re-proposing the PrepareQC or CommitQC with the \textit{highest} view in the TC ensures that one extends all committed proposals, maintaining safety. 

\par \protocol{\textbf{3: L} $\rightarrow$ \textbf{R}: Leader $L$ sends $\textsc{Prepare}_{v+1}$.}
Empowered by a TC ticket, leader $L$ broadcasts a message $Prepare \coloneqq v+1, \textit{winner-prop} \rangle_L$, where \textit{winner-prop} is the proposal associated with the QC that has the highest view amongst the $2f+1$ highQC's included in TC; or its local certified lane cut if no such QC exists \fs{how does this affect view change together with/without fast path? without fast path: no change. with fast path: now can have chains of proposals => must find common ancestor! }. Replicas that receive such a Prepare message validate $TC$, and the correctness of $winner-prop$, and otherwise proceed with Prepare as usual.  
\fs{In most cases, it suffices to send only a digest of TC, because other replicas likely see the same (though not guaranteed)}

%If no QC exists, then it is safe to propose anything: The next view's leader proposes either a no-op, the original proposal -- or more optimized: a new tip cut of its choice (that is greater than the original proposal;   => note: in non-pipeline mode can always do this. Pipeline mode distinguishes between consensus for new slots, and within slots. Cannot issue two proposals in one slot.

% \underline{Pedantic Details:} In case there is no winning proposal for the current slot a leader may propose its own local lane cut as tips. It sends $Prepare \coloneqq T: \langle TC, v+1, new-tips \rangle_L$. This is safe because no other proposal could be committed. \fs{(i.e. there can only ever be \textbf{one} committed proposal per slot) }

\fs{Pure view version in comments. Note: In slot based there must only be 1 committed proposal per slot} %Instead of only re-proposing, a Leader can always propose its own new tips in addition to the recovering ones. It sends $Prepare \coloneqq T: \langle TC, v+1, new-tips \rangle_L$. Upon committing this Proposal, replicas extract $winner-prop$ from the TC directly, and commit $new-tips$ \textit{after} $winner-prop$ has been ordered.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% FAST PATH

\par \textbf{Fast path.}
During good intervals, consensus requires 2 phases (5md total) \neil{pedantic but would say 2.5 round-trips since some people use rounds as equivalent to message delays}\fs{I was going for phases as in Prepare/Confirm} to commit a lane cut proposal. Inspired by Zyzzyva~\cite{kotla10zyzzyva} and SBFT~\cite{gueta2019sbft}, we augment \sys{} to include also a FastPath that takes advantage of graceful intervals~\cite{aardvark} in order to commit in a single phase (3md).
Rather than wait for $n-f$ Confirm-Votes to form a CommitQC, \sys{} can also construct a Fast-CommitQC by assembling $n$ Prepare-Votes. 
To maintain safety, we must adjust the view change protocol accordingly. In addition to a $highQC$, a $Timeout$ message includes also the proposal with the highest view that a replica has observed. In turn, we adjust the \textit{winner-prop} to be the greater of a) the highest highQC in $TC$, or 2) the highest proposal present $f+1$ times in $TC$. This ensures that a proposal that committed on the FastPath will be preserved. 
%\fs{the rule is imprecise/wrong when using the TC new proposal optimization from above: It should be the highest ancestor of proposals thats present $f+1$ times. E.g. consider seeing 2=f+1 proposals p1 and p2, where p2 extends p1. Then we should recover p1} \fs{Note: Without that optimization no change should be necessary: if somebody votes p2, then it must include a QC for p1.} \fs{I guess the fix is to also include the TC as highQC.}
\nc{Can you add intuition in the text for why that's correct?. I also couldn't follow your second comment}\fs{ack will re-iterate.}\fs{@Neil discuss how to best realize this subtelty}
\nc{Note: I feel that you shoul describe the slow path and the fast path together as one protocol. And then describe the view change in one go. Will help minimise length of text, it also makes it clear that we have 3MD in the "good case" as opposed to as a second thought}\fs{ok}

\subsubsection{Ride sharing.} %\textbf{Embedding on data lanes.}
Consensus phases and cars share the same message pattern. 
\fs{can cut:} This is no coincidence, as the car structure is a lightweight version of provable broadcast, the core building block of most consensus protocols~\cite{provable_abraham}.

\fs{Note: we currently piggyback consensus messages on cars, but don't yet share signatures}
To eschew message redundancies
\nc{we should explicitly say what redundancies we avoid here} \sys{} tries to avoid sending Consensus messages individually, but instead piggyback them atop cars when \textit{convenient}. Consensus message wait for a small timeout to see whether they can hitch a ride. If the timer expires, they drive themselves; this avoids having to, in the worst-case, wait for up to 2md until the next proposal (1md in expectation). \nc{This is a problem in system X and Y as they ...}\fs{it's something unique to us -- it's the tradeoff for sharing message timings}
\fs{the assumption here is that cars are available (i.e. consensus is the bottleneck); if they aren't, then should just always send messages externally for best latency}

We first describe the shared case.
\par \one Shared Cars: Each consensus view's communication is embedded on one lane (the lane governed by the leader) \nc{Could not parse this sentence. Did you mean "as embedded on one lane?"}: Prepare and Confirm phases are piggybacked on a car each; Commit and Timeout messages are piggybacked on Propose messages. To minimize the number of signature generations and verifications required, \sys{} can share a single signature across all passengers -- a replica simply batches all instance messages and signs once \nc{What is an instance message in this case? Given consensus is chained, can there ever be more than one prepare message (or confirmed) piggy backed on a car. I think will be good to specify what exactly you mean by piggy backing in this case}?~\footnote{This optimization is orthogonal to signature aggregation, and be employed jointly.}. 

\fs{NOTE: if we did Hotstuff pipelining instead of parallel pbft then we'd already be sharing consensus messages anyways --> we'd only need to still share with cars. }

Doing so poses a trade-off: when sharing certificates produced by other lanes (e.g. when proposing a certified tip, or when forwarding a PrepareQC/CommitQC during View Changes) a replica may need to forward all messages in the batch to prove validity of the signatures it has shared \nc{Define what you mean here by "sharing certificates produced by other lanes"} \footnote{Optimistically, a replica initially only sends a digest of the certificate's associated payload. The certificate itself must contain additional relevant meta data per batched message (e.g. the $pos$ of a car, or the $slot, view$ of a QC)}. To reduce such message costs, \sys{} may sign only the merkle root of a batch, and send only the relevant message plus the respective merkle path~\cite{suri2021basil}.


\fs{exact message specification of piggybacked car is commented out.}
% We augment car messages $Prop \coloneqq (\langle height, B\rangle_P, parent-cert, Opt:[Prepare/Confirm/Commit/Timeout])$ and $Vote \coloneqq \langle dig, height \rangle_R, Opt:[Prepare-Vote/Confirm-Vote]$. \fs{fo all to all we allow to piggyback any message. I.e. Vote is extended also with Consensus Instance}
% Consensus Instance = Prepare OR Confirm OR Commit + view (+ slot)

We note that cars by default only wait for $f+1$ votes -- too few to successfully assemble PrepareQCs and CommitQCs. To account for this, we upgrade any car carrying a \textsc{Prepare/Confirm} consensus message into a special ambassador car that waits for $n-f = 2f+1$ votes. \nc{Do you end up in a situation where most cars are ambassador cars? One of the "big" pitches was that we went as fast as possible in our lane, and that was enabled by f+1 best effort broadcast, but now, if we're anyways piggy backing, seems like we're back to waiting for 2f+1?} Fig. \ref{fig:consensus} illustrates the embedding, flags denote ambassadors. Data availability certificates (PoA) themselves remain of size $f+1$. 

Honest replicas always vote for data availability, but may omit a consensus-vote if they have locally timed out on the denoted view. To distinguish faulty voters from honest replicas (that timed out due to asynchrony) \sys{} reserves the right to delay cars following an ambassador: ambassador cars wait for either $n-f$ votes, or the expiration of the consensus view's timer -- in which case the leader abandons its tenure and proceeds with the next car (without a consensus Quorum). We note that although \nc{consensus?} proposal pace may decelerate, data lane growth remains asynchronous. \fs{TODO: clarify what "asynchronous growth" means? Are people confused by timeouts making it synchronous? => it WILL make progress even in asynchrony.}  \fs{NOTE: If we piggyback MULTIPLE consensus instances on a car, then we may need to wait for the biggest timeout. In that case we may want to send externally.}

Ambassador cars representing a \textsc{Prepare} employ an additional (smaller) timer to attempt waiting for the $n$ \textsc{Prepare-Votes} required to construct a Fast-CommitQC in gracious intervals. Alternatively, \sys{} can be configured to perform the standard execution and FastPath in parallel by continuing to wait beyond formation of a PrepareQC, and later forwarding possible Fast-CommitQCs externally (out-of-lane).
\nc{While I thought the disucssion of the various options wsa informative, I'm wondering if if we don't just want to pick one as otherwise it gets quite confusing "i could do this, but also this, or this". Maybe for the same of clarity and the paper, let's pick our poison?}

\fs{During good intervals, waiting for $n-f$ matching votes affects only tail latency -- we can expect all 2f+1 honest replicas to reply with a vote. Same for $n$ in gracious periods}
\fs{In face of asynchrony, however, honest replicas may have timed out on a consensus view, and thus vote against (they send a car vote without consensus vote). The leader waits for the consensus timeout to decide whether or not to keep waiting, or advance the car while giving up on its consensus tenure.}


\fs{We are assuming there is new proposals coming continuously, and therefore consensus can just share the messages. (I.e. just like in DAGS, consensus only happens if there is new nodes). If this is not the case, then instead of waiting for the batch timer to fire, we can of course also just send a consensus message separately. In this case, we don't even have to give the consensus message a height (it's just lane external) -- so we don't do consensus on a new tip thats empty }

\fs{special rule territory:} \fs{the below is actually more of a mess than I describe. It's not enough to just have a single off-lane car for Prepare, but Confirm also needs to go offlane. It may be worth to just describe as sending externally}
\par \two Riding Solo: Consensus messages that fail to attach to \textsc{Proposal}s or \textsc{Vote}s in a timely manner can issue a special \textit{off-lane} car. This car follows the usual structure, and may carry both multiple consensus instance messages \nc{How given that consensus is chained}\fs{a car is just the Prepare/Vote pattern; I'm specifically saying this car is not chained (i.e. off-lane)} and new data requests \nc{What is a data request?}. A few special rules apply:
Firstly, this car need not obey the typical chained lane rules. It has no position, and does not need to reference only certified proposals.
\nc{What does it mean for a car to "reference" a proposal"?} For instance, it can choose to reference the latest proposal (but yet to be certified) proposal sent by the leader. This is safe and live: only the leader itself will propose this special car as it's own tip, and thus is responsible for it's (history's) delivery.
Second, subsequent normal car's do not need to extend the off-lane car. To avoid orphaning an off-lane car whose payload was certified but did not commit, a subsequent car may include a special \textit{tow} reference to a certificate of the off-lane car (if it exists). This allows the off-lane car to eventually be committed alongside the normal car's history.

\iffalse
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% EMBEDDING
\par \textbf{Ride sharing.} %\textbf{Embedding on data lanes.}
Consensus phases and cars share the same message pattern. 
\fs{can cut:} This is no coincidence, as the car structure is a lightweight version of provable broadcast, the core building block of most consensus protocols~\cite{provable_abraham}.

To eschew message redundancies and simplify implementation \sys{} does not send Consensus messages individually, but instead piggybacks them atop cars. \fs{the assumption here is that cars are available (i.e. consensus is the bottleneck); if they aren't, then should just send messages externally for best latency}
Each consensus view's communication is embedded on one lane (the lane governed by the leader): Prepare and Confirm phases are piggybacked on a car each; Commit and Timeout messages are piggybacked on Propose messages. In its simplest form, we simply sign data votes and consensus votes separately; we discuss in \S\ref{sec:optimizations} how to also share signatures across car passengers.

\fs{cut exact message specification.}
% We augment car messages $Prop \coloneqq (\langle height, B\rangle_P, parent-cert, Opt:[Prepare/Confirm/Commit/Timeout])$ and $Vote \coloneqq \langle dig, height \rangle_R, Opt:[Prepare-Vote/Confirm-Vote]$. \fs{fo all to all we allow to piggyback any message. I.e. Vote is extended also with Consensus Instance}
% Consensus Instance = Prepare OR Confirm OR Commit + view (+ slot)

We note that cars by default only wait for $f+1$ votes -- too few to successfully assemble PrepareQCs and CommitQCs. To account for this, we upgrade any car carrying a \textsc{Prepare/Confirm} consensus message into a special ambassador car that waits for $n-f = 2f+1$ votes. Fig. \ref{fig:consensus} illustrates the embedding, flags denote ambassadors. Data availability certificates (PoA) themselves remain of size $f+1$. 

Honest replicas always vote for data availability, but may omit a consensus-vote if they have locally timed out on the denoted view. To distinguish faulty voters from honest replicas (that timed out due to asynchrony) \sys{} reserves the right to delay cars following an ambassador: ambassador cars wait for either $n-f$ votes, or the expiration of the consensus view's timer -- in which case the leader abandons its tenure and proceeds with the next car (without a consensus Quorum). We note that although proposal pace may decelerate, data lane growth remains asynchronous. \fs{TODO: clarify what "asynchronous growth" means? Are people confused by timeouts making it synchronous? => it WILL make progress even in asynchrony.}  \fs{NOTE: If we piggyback MULTIPLE consensus instances on a car, then we may need to wait for the biggest timeout. In that case we may want to send externally.}

Ambassador cars representing a \textsc{Prepare} employ an additional (smaller) timer to attempt waiting for the $n$ \textsc{Prepare-Votes} required to construct a Fast-CommitQC in gracious intervals. Alternatively, \sys{} can be configured to perform the standard execution and FastPath in parallel by continuing to wait beyond formation of a PrepareQC, and later forwarding possible Fast-CommitQCs externally (out-of-lane). 

\fs{During good intervals, waiting for $n-f$ matching votes affects only tail latency -- we can expect all 2f+1 honest replicas to reply with a vote. Same for $n$ in gracious periods}
\fs{In face of asynchrony, however, honest replicas may have timed out on a consensus view, and thus vote against (they send a car vote without consensus vote). The leader waits for the consensus timeout to decide whether or not to keep waiting, or advance the car while giving up on its consensus tenure.}


\fs{We are assuming there is new proposals coming continuously, and therefore consensus can just share the messages. (I.e. just like in DAGS, consensus only happens if there is new nodes). If this is not the case, then instead of waiting for the batch timer to fire, we can of course also just send a consensus message separately. In this case, we don't even have to give the consensus message a height (it's just lane external) -- so we don't do consensus on a new tip thats empty }

\fi
% \fs{TODO: DISCUSS DATA LAYER BLOCKING}  => blocking lane is fine. Next car couldn't commit anyways earlier.
% Think asynchrony: if consensus times out and doesn't make progress => no point in having speediest data layer. (latency is suspended during async anyways, just have bigger cars)
% Going as fast as you can (smaller cars) matters for latency during good intervals. And during good intervals we'd imagine getting 2f+1 we need before timing out anways. At least on a good leader. For byz leader we dont care about its lane progress.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

This concludes the core \sys{} consensus design. 
%In section \S\ref{sec:end-to-end} we discuss how to improve end-to-end latency in \sys{} by pipelining consensus of successive proposals.
\fs{we call this simplified version Motorway in experiments, and Autobahn = the full one.}

%\subsubsection{Chaining instances.}
%Don't have this here. Just generalize View change rule. If have committment, can propose new data. (Note: can also propose new data if TC empty). I.e. distinguish receiving QC and TC (pull this from Poster section)

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Discussion / More details %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



\input{Sections/3-System/Protocol/fairness}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% END HERE %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% NOTES  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% FAST PATH AFTER EMBEDDING only

\iffalse
\par \textbf{Fast path.}
During good intervals, consensus requires 2 phases (5md total) \neil{pedantic but would say 2.5 round-trips since some people use rounds as equivalent to message delays}\fs{I was going for phases as in Prepare/Confirm} to commit a lane cut proposal. Inspired by Zyzzyva~\cite{kotla10zyzzyva} and SBFT~\cite{gueta2019sbft}, we augment \sys{} to include also a FastPath that takes advantage of graceful intervals~\cite{aardvark} in order to commit in a single phase (3md).
Rather than wait for $n-f$ Confirm-Votes to form a CommitQC, \sys{} can also construct a Fast-CommitQC by assembling $n$ Prepare-Votes. Doing so has implications for two part of the protocol:

First, to maintain safety, we must adjust the view change protocol. In addition to a $highQC$, a $Timeout$ message includes also the proposal with the highest view that a replica has observed. In turn, we adjust the \textit{winner-prop} to be the greater of a) the highest highQC in $TC$, or 2) the highest proposal present $f+1$ times in $TC$. This ensures that a proposal that committed on the FastPath will be preserved.\fs{TODO: add intuition (if 3f+1 committed fast, f+1 are visible} %\fs{the rule is imprecise/wrong when using the TC new proposal optimization from above: It should be the highest ancestor of proposals thats present $f+1$ times. E.g. consider seeing 2=f+1 proposals p1 and p2, where p2 extends p1. Then we should recover p1} \fs{Note: Without that optimization no change should be necessary: if somebody votes p2, then it must include a QC for p1.}

Second, when trying to construct a Fast-CommitQC, we must once again be mindful to not unduly slow down the data layer. We consider two practical options; their choice is up to preference and demands of the system. \one \sys{} can enforce a small timeout (distinct from view timer) on ambassador cars to try and wait for $n$ \textsc{Prepare-Votes}. Notably, data lane growth remains asynchronous even in gracious intervals, albeit with slightly pulled brakes. \two \sys{} can perform the standard execution and FastPath in parallel by continuing to wait beyond formation of a PrepareQC, and later forwarding possible Fast-CommitQCs externally (out-of-lane). 
We choose option \two for our implementation in order to allow the data lanes to proceed unimpeded. \fs{maybe 1 is actually simpler and still practical if we are not that overrun for load. Easier to debug because only one path can be in the system at a time.}

\fs{another impractical option: 2) add small timeout, but don't make data layer wait. Con: both fast path and slow path are then delayed by 1 more car (increasing latency, which is no good)}
\fi 


\iffalse
\fs{just populating content/things to mention. Not prose.}

%%%%%%%%%%%%%%%%%%%%%%%%%%5555%%%%%%%%%% SLOT BASED 
\sys{} uses a paxos-style slot-based consensus model, in which we try and commit a proposal for slot s before we commit slot s+1. \fs{slots abstract views "cleaner". It distinguishes views that try to just finish the same proposal, from views that are doing new work}
\sys{} allows consensus for slots to occur in a parallel, pipelined fashion (\S \ref{sec:end-to-end}. For simplicity, we first discuss consensus on a \textbf{single} slot. \fs{Note: If we didn't use pipelining/parallel consensus, then there is no need for a concept of a slot. Going through views is enough} Each slot progresses through a series of views: In case of a faulty leader, we view change in order to finalize the slot. We say that a slot commits upon reaching agreement; a slot finalizes (and can be applied to the log) if all previous slots have committed and finalized (or it is genesis). \fs{i.e finalized = proposal has finality, i.e. its log position is fixed. Could also call it \textit{totally ordered} instead of finalized} 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Proposals
Consensus proposals in \sys{} are not data request (or batches of requests), but instead are \textit{snapshot cuts} of the data lanes (Fig.\ref{fig:car_lanes}). Concretely, a leader proposes a vector of \textit{tips}: A tip (for a given lane) is the latest completed car observed by the leader -- i.e. it is the latest (largest height) certified proposal received from the respective replica's lane. Fig. \ref{fig:car_lanes} shows an example cut that might correspond to the latest certified tips at some replica.
Upon reaching consensus on a cut of tips, \sys{} flattens every new (not already finalized) request into a total order. To do so fairly, we zip together all lanes in a deterministic order: For each tip, we identify the latest ancestor that has not already been finalized. Then, from oldest to newest (tip), we zip all lanes in round-robin fashion.

\par \textbf{Why propose only certified tips?} Proposing only tips that are certified streamlines the voting step of consensus proposals, and ensures seamlessness. Since proposals consist of a vector of tip certificates, every replica can locally assert that the entire tips transitive history must be available at some correct replica (if not locally). If tips were uncertified, and a replica has not seen the data item, then it must request the data first: It must either wait to receive it (which it might never, if the originator was byz), or require the leader to forward the request (which places broadcasting burden on the leader -- either it always sends it pessimistically, or it requires 2 extra md). If all data dissemination was best effort (chained) then we might have to recursively unravel sync (and add md's) in the order of lane length.

\sys{}'s chained certified lanes guarantees that no synchronization is necessary on the critical path of consensus. This ensures that consensus is \textit{seamless} because the cost of consensus is independent from the length of a lane (i.e. agnostic to periods of asynchrony). \fs{Note: For execution a replica may still need to locally synchronize on whatever it is missing. But importantly this does not hold up OTHER replicas. If we sync during consensus, then it may very well (unless replica is not part of quorum -- but consensus quorums are bigger than result quorums)}. We discuss in \S\ref{sec:optimizations} how to tradeoff some synchronization for latency benefits (while still being seamless).


%If all data dissemination was best effort (chained) then we might have to recursively unravel sync (and add md's) in the order of lane length.

Optimization: Fast Sync. Move to optimization section.

\fs{need to make compelling case why it matters to distinguish consensus seamlessness, from application seamlessnes... If sync -- possibly recursively -- is anyways required, then theres no win end-to-end}
\fs{problem: cannot possibly have seamless commit.}

\par \textbf{Fast Synchronization.}
If you accept a tip for Lane L, request from the f+1 replicas in the cert, all proposals between latest[L].height and tip.L.
Trick: since we required that a replica has seen the parent before voting => any replica that has cert has all of that history. Bonus: That replica must have something with latest[L].height +1 (because of the data layer rule!!) \fs{this is important, otherwise we couldnt tell if a replica sent everything I needed.}
So at most 1 round of sync (can be in parallel with consensus), but a lot of data.
Importantly, this doesn't stop other replicas that do have the data from committing) 

\fs{}

\fs{beb, chain get stuck synchronizing. Data might not exist. If Byz leader -> timeout on consensus. If honest leader -> expect honest leader to only propose tips for which itself has the history!!}

\fs{could sync by just asking the leader for everything?}
\fs{It can cause consenus to block -- might timeout etc. But it is constant latency}
\fs{cert based is better, because sync is asynchronous and per replica -- doesn't hold up consensus}

Note: data dissemination itself belongs to exec layer. Sync on "meta-data" in order to be able to commit everything.


Tips = cert. This means that there is +3 md latency (basically an RB). We discuss in Optimizations how to improve this.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Good case consensus
\par \textbf{Consensus.}
We adopt a linear pbft-style consensus pattern. We discuss in \S\ref{sec:optimizations} how to use an all-to-all message paradigm to tradeoff increased complexity for lower latency.
Consensus in good intervals consists of two phases. A \textit{Prepare} phase (P1) during which a designated leader proposes a cut of the data lanes, and tried to reach agreement within the current view (non-equivocation). And then a \textit{Confirm} phase (P2) \ref{fig:base_consensus}, in which the decision is made durable accross views. In both phases, we collect a Quourm of 2f+1 vote replies; respectively they form a PrepareQC (P-QC) and CommitQC (C-QC). A P-QC is necessary to start the Confirm phase, while a CommitQC signifies that the proposal can be committed.

Honest leaders in \sys{} will only initiate a proposal (Prepare) once they have observed sufficiently many new tips to conclude that the data lane has made progress. We call this property coverage. It's a hyperparameter -- we set it to a Quorum (2f+1) to make sure that at least half are honest lanes that advanced (\S\ref{sec:fairness} \fs{Can set coverage to 1 to allow any new proposal to commit asap -- this is a tradeoff between latency (useful if only few nodes have new proposals) vs efficiency (less consensus instances) and fairness (chain equality) } \fs{note, that this property makes timeouts a tad trickier. Should account for the wait }
Byz leaders don't  need to respect this. (we could check, but don't need to) -- no loss; byz could've just stayed silent as well. \neil{in this case would silence from byz be better than not respecting the coverage rule since proposing old data wastes resources, and could prevent the next leader from proposing new stuff if the old data ends up being committed} This is safety independent, and purely an efficiency optimizing decision: There is no need to do consensus if there is no data. "progress" at the consensus layer means nothing, if there is not progress at the data layer -(consensus works for the data layer)
\fs{A nice thing of our design is that unlike DAG protocols, we don't have orphans. A consensus protocol can have up to $n$ new proposals. So if any honest becomes leader, and has seen another honest replicas lane state, then it will propose it. I.e. eventually an honest replica will always propose honest tips (DAGS artificially limit to n-f edges to ensure progress, and then need weak edges etc to save orphans)}

We embed on data layer to minimize message redundancies -- this is easy, because they share the exact same communication pattern \fs{we don't have to since they are logically separate. But we make the choice to simplify implementation and to reduce messages sent}. Each lane is just a long chain of provable broadcast pattern. We can embed other consensus styles as well: E.g. hotstuff on a single lane -- or even rotating hotstuff with one phase = 1 car.

Extend message $Prop \coloneqq \langle height, request-batch, parent-cert: digest + f+1 sig, Opt: <Consensus-Instance>  \rangle_{P}$ 
and message: $Vote \coloneqq \langle prop_digest \rangle_R $ + separately signed consensus instance. \fs{fo all to all we allow to piggyback any message. I.e. Vote is extended also with Consensus Instance}
Consensus Instance = Prepare OR Confirm OR Commit + view (+ slot)

Details: Next car doesn't start before 2f+1 were formed. But in the simplest form we keep the quorums separate, so the data quorum is still only of size f+1. We discuss in Section \S\ref{sec:optimizations} (\textit{Ride sharing}) how to avoid redundant signatures.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% View change
In order to deal with faulty leaders that hold up consensus we need to change leaders. 
We use timeouts, and change views within a slot. 

We start a timer for view v:
1) view v==0: upon receiving the commit message for the previous slot  \fs{in pipeline we revise this: start timer upon receiving prepare from previous slot}
2) view v >= 1: upon receiving a TimeoutCertificate for view v -1 

If we commit (receive C-QC) we cancel all timers, and never start one again.

Upon timing out, replicas broadcast a message $Timeout/New-view \coloneqq \lange curr_view, high_QC \rangle_R $. 
They include the newest QC they have seen (i.e. highest view P-QC)
If one receives a timeout from others, but already has C-QC one can just forward C-QC
Upon collecting a Quorum (2f+1) of Timeout messages for the same view , a replica forms a TimeoutCertificate. It then moves to view v (and starts a timer) \fs{it cancels any old ones -- could still be running if we didn't time out ourselves}
If it is the leader for the next view: use TimeoutCertificate (TC) to start a new Prepare (in view 2)

The leader chooses a new proposal based on the TimeoutCertificate: If it contains any P-QC'sIt re-proposes the proposal vouched for by the highest P-QC. Doing so ensures, that IF any previous proposal could have been committed at some replica, no other proposal is ever committed. (if there was a commit, all future views must decide the same). 
If no QC exists, then it is safe to propose anything: The next view's leader proposes either a no-op, the original proposal -- or more optimized: a new tip cut of its choice (that is greater than the original proposal; 




\fs{we use the all to all version -- explain. the simplest one is sending them to the next leader, but the all to all ensures that all replicas move to a new view within bounded time (only after GST of course}

For simplicity, our implementation also piggybacks these messages on available cars (no reply is required) \fs{could also put them onto votes, or send externally}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Fast Path
 \fs{could move Fast path to optimizations? I like it as part of the speediness story though}.
We optimize \sys{} to take advantages of graceful intervals by adding a Fast Path (inspired and similar to the one in SBFT/Zyzzyva).
Can construct a Commit Certificate (C-QC) also by using $3f+1$ Prepare votes (short: Fast C-QC). In this case, we need to adjust the view change protocol accordingly: A timeout vote also includes the proposal with the highest view that a replica has observed (for the slot). A new prepare then uses a TC as follows It picks as proposal the greater between: 1) the highest P-QC, or 2) the highest Prepare (that exists f+1 times).

When trying to construct a Fast C-QC, we must be careful to not slow down the data layer. 
There are two practical options:
1) add small timeout to wait for fast Quorum before moving on (i.e. delay slow path and data layer slightly). This is still asynchronous (it will grow if the timeout expires), but it puts on some brakes. 
2) do fast and slow path in parallel, i.e. keep waiting, and do fast path too. This is only useful if we send FP messages externally (i.e. don't wait for cars); otherwise, if we wait for the next car, that car carries the round 2 of slow path anyways.

Either option is fine, and it's up to preference and demands of the system. We choose option 2 for our implementation in order to allow the data lanes to proceed unimpeded. \fs{maybe 1 is actually simpler and still practical if we are not that overrun for load}

\fs{another impractical option: 2) add small timeout, but don't make data layer wait. Con: both fast path and slow path are then delayed by 1 more car (increasing latency, which is no good)}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Slots
\sys{} starts consensus for a new slot $s$ upon receiving commit confirmation (a C-QC) for slot $s-1$, and sufficiently many new tips to fulfill the coverage criterion. We assign leaders for slots via round-robin in order to distribute load and ensure that byz (or honest slow leaders) don't stall progress. 
    \fs{could also use stable leader or random leader. With stable leader there is the risk of selecting a leader that doesn't optimize coverage. Can use orthogonal leader reputation schemes (cite shoal, carousel) to make the best connected replicas be leaders - reputation = proportional to volume of data committed} 

We note, that in the simple sequential consensus structure outlined so far, the concept of slots is not necessary. We can abstract the existence of slots entirely, and replace it with a simple ticketing-based design in which we increase views instead of incrementing slots: A given replica is the current leader of consensus if it holds a \textit{Ticket} for view $v$, where a ticket is either a Commit Certificate (C-QC), or a TimeoutCertificate for the previous view $v-1$.
We call this naive sequential mode of operation \textit{Motorway}. \fs{compare in experiments}

Next, we discuss how \sys{} improves upon Motorway to optimize end-to-end latency via means of pipelining.


-- 



\fi


%%%%%%%%%%%%%%%%%%%%%%%%% COMMENTS / NOTES
\iffalse
- Layering consensus: Start by describing a single instance: One slot (multiple views) 
    - what are proposals? Quorum of tip certs. Why certs? Could be more aggressive, but tradeoff for sync on critical path
            - if being more aggressive, only be aggressive for tip; needs to have cert parent. (otherwise we unravel are are no longer seamless)
    
-- base pattern
        - could use different protocols. we follow a linear pbft/sbft one (2 provable broadcasts. Describe how it is mapped onto cars (doesn't have to be!).
         - note: because the car structure is just provable broadcasts, one can map pretty much any protocol on top. Could do hotstuff (just do 3 cars); could spread rounds of hotstuff across lanes (different proposers), like rotating hotstuff.
     - create picture where there is a FLAG on a car that says P1^s P2^s (where s is the slot instance)

    
\fi
    


==> Sections/3-System/Protocol/end-to-end.tex <==
\subsection{Reducing end-to-end latency} %Pipelined consensus -> Rename: Reducing End-to-end latency}
\label{sec:end-to-end}

The \sys{} consensus protocol described so far is simple and, on paper, has low \textit{consensus} latency. %While the,..., it is subject to suboptimal end-to-end latency in practice.
%In the following we discuss two shortcomings and respective improvements in turn.
In the following we discuss two end-to-end latency shortcomings and respective improvements.



% \one First, we investigate how to leverage optimism when proposing tips to reduce the latency between payload dissemination and inclusion for consensus. \two Next, we discuss the worst-case for data synchronization, and how to bound latency to a single RT. \three Finally, we describe how to instantiate \sys{} with parallel/pipelined consensus slot instances to minimize sequential consensus latencies.

%OLD TEXT: Our discussion proceeds in two parts: \one First, we investigate in detail the purpose of proposing certified tips in \sys{}, and present two optimizations that, respectively, bound catch-up to one round-trip, and optimistically propose un-certified tips. \two Next, we describe a pipelined instantiation of \sys{} that minimizes \textit{sequential} consensus latencies.

\subsubsection{Reducing Latency from Proposal to Prepare}
%\par \textbf{Certification overhead.} 
By default, \sys{} consensus pessimistically only proposes \textit{certified} tips. This allows voting in consensus to proceed without blocking, a crucial requirement to achieve seamlessness (\S\ref{sec:cert-tips}). However, assembling and sharing certificates imposes a latency overhead of 3 message exchanges that must be paid \textit{in addition} to consensus latency. This results in a best-case end-to-end latency of 6md on the FastPath, and 8md otherwise.

%In the best case, proposing certified tips still incurs an inherent latency penalty -- it requires 3 message delays for the leader to learn of a new tip, resulting in 6md end-to-end latency on the FastPath, and 8md otherwise.

\fs{Notably, this is a redundant cost with consensus, which also proves availability...}


\sys{} employs two optimizations to improve a data proposal's latency from dissemination to cut-inclusion. 
\par \textbf{Leader tips.} First, we allow that, for its own lane, a leader may simply include as tip the proposal it is currently broadcasting in the car used to issue a new Prepare message. If the leader has failed to share its lane history then progress of its view may be interrupted; this will not occur for honest leaders. 
\par \textbf{Striking a balance on optimism.} Second, \sys{} allows leaders to adopt \textit{common-sense}: honest leaders may choose to optimistically propose non-certified tips for lanes that are historically reliable, at the risk of having to synchronize and losing its tenure. Notably, the responsibility for synchronization falls only to the leader in a view that originally proposes the tips. Views that re-propose winning proposals do not require blocking synchronization; all tips in a winning-proposal are implicitly considered certified since $\geq f+1$ replicas voted for it.

In gracious intervals, this optimization reduces latency to a single message exchange (the optimum). 
If the triangle inequality holds for point-to-point channels, all replicas will locally deliver all proposed tips before receiving a $Prepare$, thus avoiding synchronization. When it does not, replicas hold off from voting, and request synchronization from the leader directly. If a tip is delivered locally in the meantime, the replica resumes early, minimizing latency (at the cost of some wasted synchronization). 

During less gracious intervals proposing optimistic tips poses a risk to a leader's tenure. A byzantine proposer may forward its payload only to the leader, burdening it with synchronization, and potentially causing its view to time out. We note, however, that critical-path synchronization is only necessary for the tip itself -- by design, all ancestors must be certified, and thus can be synchronized asynchronously.
To improve the predictability of unwanted synchronization, \sys{} can be augmented with a simple reputation mechanism\fs{cite private communications with Sasha}. A leader that is forced to synchronize on a given lane's tip downgrades the lane's reputation. Below a threshold, it stops proposing optimistic tips for the lane %. Since beneath the optimistic tip, all other proposals must still be certified 
-- the leader simply falls back to proposing a certified tip. 
%Below a threshold, it simply falls back to proposing certified tips for the lane. 
Each replica is thus responsible for warranting optimism on its governed lane and consequently its own data proposals' latency. Reputation can be regained over time, e.g. for each committed lane proposal; the speed of recovery is determined by its work-rate. Pessimistic combinations are possible: a leader may pessimistically choose to forward the payload of lane tips of replicas whose reputation is in question, and collect hints about the pessimism necessity.


\iffalse

\subsubsection{Bounding data synchronization latency}
%\par \textbf{Unbounded worst-case commit latency.} 
For efficiency, \sys{} consensus proposals contain only a cut of tips of each lane. When \textit{committing} a proposed tip a replica first orders all of its (so-far uncommitted) history. But what happens if this history is not locally known to a replica? In the worst case \fs{after byzantine attack, or partial network partitions}, a replica may need to recursively learn of (and fetch) a given tip's history, requiring sequential message exchanges in the order of lane length, and compromising our goal of seamlessness.
%In the worst case, data synchronization (even with certified tips) may still have to recursively unravel one ancestor at a time to request the entire history. 
For instance, a byzantine lane governor $G$ may leverage a period of asynchrony to build a long lane backlog, yet broadcast any given proposal to only $f+1$ replicas. 

%We discuss next how to \one bound synchronization delay to a single round-trip, and \two strike a balance between occasional synchronization and optimistic latency.

\par \textbf{Fast synchronization.} To bound synchronization latency, \sys{} enforces strict FIFO on all certified proposals. An honest replica only delivers and votes for a proposal in height $h$ if it has voted for its predecessor in $h-1$ -- consequently, any honest replica part of a certificate must possess the entire history, which by design has no height gaps. \sys{} leverages this invariant to synchronize in just a single message exchange, no matter the size of the history: rather than request direct parents recursively, a replica requests to sync on (and will only commit) \textit{all} proposals with heights greater than its locally last committed lane proposal ($\geq lanes[G][length] +1 $, $\leq tip.height$). 
By correctness of consensus, all honest replicas agree on the last committed lane proposal, and thus sync on the same content. 

\fs{NOTE: it's not guaranteed, nor is it important, that the last synced on data item is a child of our latest committed. If it is not, then technically we could sync on, and commit} 
\fs{DATA amount = bit size can of course not be reduced. That is less principled -> impact changes depending on available bandwidth. I would just assume infinite bandwidth here.} \fs{TODO: Clean up definition of seamlessness to account for data size.} \fs{Note: most likely only have to fetch large amount of data on a byz lane. (unless direct channel extremely asyc)}

\fs{NOTE: this optimization can also be applied with Best effort Broadcast. Instead of requesting from certifier, request from leader. Honest leader only proposes certificates for which it has locally received all history}
\fs{This way if leader is byz: we will just timeout. But if leader is honest, then it wouldn't propose a tip for which it hasn't seen the chain history itself (i.e. enforce FIFO sync)}
%Solution: FIFO: Request sync in a single message step. Request all history between last-commit and tip.
%This optimization is applicable to BeB too. Instead of requesting from certifier, request from leader.
%\footnote{It can also be applied for DAG protocols, if they enforce FIFO}

\fi

\subsubsection{Avoiding sequential consensus latency}
%\par \textbf{Higher-than-expected consensus latency.} 
\sys{} employs a ticket-based consensus that proceeds through a series of \textit{sequential} slots instances. Unfortunately, lane proposals that narrowly miss inclusion in the current slot's proposed consensus cut may experience the sequential latency of up to two consensus instances. Tips that "miss the bus" experience wait-time for the current consensus proposal to commit -- including any number of view changes necessary to do so --, and the latency of the next consensus instance (in which they are covered). In expectation, the experienced consensus latency is thus 1.5x the advertised delay.


\par \textbf{Parallel Consensus.}
To circumvent sequential wait-times, \sys{}, inspired by PBFT~\cite{castro1999pbft}, allows for a new slot instance to begin in parallel with ongoing slots; instead of only upon commitment of the preceding slot. 
We modify a slot ticket for $s$ to no longer require a CommitQC for slot $s-1$. The leader of slot $s$ can begin consensus for slot $s$ as soon as the first \textsc{Prepare} message for slot $s-1$ is received, and sufficient additional coverage is achieved. This encourages honest leaders to not issue redundant proposals, minimizing wastage. Once again, coverage is best effort and cannot be strictly enforced. \fs{cut: probably just confuses people. (It's saying that even if we tried to enforce coverage, we couldn't). Hence "cannot be enforced"} While we may demand to reference \textit{some} $\textsc{Prepare}_{s-1}$ as ticket, we cannot guarantee that it represents the proposal that is ultimately committed in slot $s-1$. \fs{e.g. view change could change} \fs{Note: If we are not enforcing coverage, then there is no need for a ticket: I.e. the Prepare does not need to be included}

\begin{figure}[h!]
    \vskip -5pt
   \centering
   \includegraphics[width=0.45\textwidth]{Figures/pipeline.pdf}
   \vskip -5pt
   \caption{$\textsc{Prepare}_{s+1}$ can begin upon receiving $\textsc{Prepare}_s$.}
   \label{fig:pipeline}
   \vskip -5pt
\end{figure}

When instantiated with a stable leader there is no sequential wait-time; a new slot begins as soon as $n-f$ lanes have made progress (coverage)\fs{THIS IS IMPRECISE. ONLY TRUE IF NOT RIDE SHARING. IF RIDE SHARING THEN WE HAVE TO WAIT FOR CAR ==> LATENCY IS ACTUALLY 2}. With rotating leaders, the wait-time is at most 1md; the time to receive $\textsc{Prepare}_{s-1}$. \fs{this is why we have separate views per slots}. Figure \ref{fig:pipeline} illustrates two pipelined instances embedded onto separate lanes.

\fs{move next to related work:} \sys{}'s parallel proposals resemble modern chained-BFT protocols~\cite{2023beegees, yin2019hotstuff, jolteon-ditto} which pipeline consensus phases (e.g. piggyback $\textsc{Prepare}_{s+1}$ on $\textsc{Confirm}_s$). \sys{} too could be configured such a way, yet we opt for parallel proposals for two reasons: \one pipelining phases is not latency optimal as it requires at least 2md between proposals \fs{rigid}, and \two it introduces liveness concerns that require additional complexity to circumvent~\cite{2023beegees}.\fs{it also makes the coverage criterion easier to handle: E.g. coverage for slot 2 does not affect progress of slot 1} \sys{}'s slot based consensus is straightforward to parallelize, and, so we hope, easily accessible to a wider audience. \fs{it does however introduce more signatures possible, which requires finicky optizations if it should be a bottleneck. If signatures are the bottleneck nothing stops us from just using a pipelined HS-like consensus alternatively}

To realize parallel slot instances we must adjustments the system as follows.

\par \textbf{Managing concurrent instances.}
\sys{} maintains independent state for all ongoing consensus slot instances. Each instance has its own consensus messages, and is agnostic to consensus processing on all concurrent slots. Messages of different instances can, however, ride the same cars; we discuss in Section \S\ref{sec:optimizations} how to share signature costs. Slots that commit wait to \textit{finalize} until all preceding slot instances have been finalized first. Upon finalizing a slot's proposal (a cut of tips), \sys{} replicas identify and order only proposals that are new. As discussed above, it is not guaranteed that consecutive slot's propose monotonic cuts; non-monotonic tip positions are simply ignored. \fs{i.e. we don't try to order/apply multiple forks.}  \fs{Sync happens asynchronously, and might do redundant work.}





\par \textbf{Adjusting view synchronization.}
To account for parallel, overlapping instances, replicas no longer begin a timer for slot $s$ upon reception of a $CommitQC_{s-1}$, but upon reception of the first $\textsc{Prepare}_{(s-1, v)}$ message. \fs{timeouts should account for time it might take to forward Prepare to the leader that needs it + time to get coverage}. 
Additionally, we adjust the leader-election scheme to decorrelate view changes across successive slots. If the same round-robin schedule were applied across and within slots, the worst case number of view changes to finalize $k$ successive slots is $\frac{k * (f+1)}{2}$, as each slot must rotate through the same faulty leaders. To avoid this, we shift round-robin assignment for slots by $f$; random election is feasible too. 

\par \textbf{Bounding parallel instances.}
During good intervals there will likely be at most 3-4 concurrent instances at a time\footnote{Each instance incurs $\leq 4md$ (Prepare + opt Confirm) before sending commit message. Thus up to 4 instances can open}. In periods of asynchrony (or in presence of faulty leaders) this number can grow arbitrarily large: new instances may keep opening (they only need to observe a proposal and coverage \fs{data layer keeps growing!}), but instances are not closing at the same rate. These instances are not beneficiary, as a single instance in the next good interval can subsume all such proposals with a single new cut.
To avoid wastage, and simplify garbage collection, we can bound the maximum number of open instances to some $k$ by (re-)introducing delayed CommitQC tickets. To begin slot instance $s$, one must include a ticket $CommitQC_{s-k}$. 
When committing slot $s$ we can thus garbage collect the commitQC for slot $s-k$ as $CommitQC_s$ transitively certifies commitment for slot $s-k$. \fs{(and $s-2k$, $s-3k$, ...).}\fs{(Note, cannot gc everything $< s-k$; need to wait for finalization to do that -- however, $s-k-1$ will have been GC by $s-1$ already, and so forth)}

\fs{If we only extend proposals, then the commitQC for each slot must be kept around in order to reply to view changes. e.g. to help inform replicas that haven't committed). We'd like to bound this. Can do so either by active checkpointing (requires synchronization), or by leveraging the depth limiter} 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% END SECTION %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%
\iffalse 


\fs{Could go with a Jolteon style pipelined implementation. But we also find this didactically easier. We want each component to be nicely logically isolated} \fs{Hotstuff based has the k-consec leader requirement. Begees fixes it, but it complicates the whole design}


\sys{} uses a paxos-style slot-based consensus model, in which we try and commit a proposal for slot s before we commit slot s+1. \fs{slots abstract views "cleaner". It distinguishes views that try to just finish the same proposal, from views that are doing new work}
\sys{} allows consensus for slots to occur in a parallel, pipelined fashion (\S \ref{sec:pipeline}. For simplicity, we first discuss consensus on a \textbf{single} slot. \fs{Note: If we didn't use pipelining/parallel consensus, then there is no need for a concept of a slot. Going through views is enough} Each slot progresses through a series of views: In case of a faulty leader, we view change in order to finalize the slot. We say that a slot commits upon reaching agreement; a slot finalizes (and can be applied to the log) if all previous slots have committed and finalized (or it is genesis). \fs{i.e finalized = proposal has finality, i.e. its log position is fixed. Could also call it \textit{totally ordered} instead of finalized} 


\fS{Below is only placeholder text}


While the consensus mechanism describe so far has low latency for consensus proposals, it suffers from suboptimal end-to-end latency. 
Due to the consensus mechanisms sequential nature, cars that narrowly miss inclusion in the cut, experience the \textit{sequential} latency of up to two consensus slot instances \fs{i.e. slot abstracts view change cost into an instance}: Cars that "miss the bus" pay for the wait-time of the current slot to finalize (including any number of view changes necessary to do so), and the latency of the consensus instance covering them. In the worst case, the total latency (of a car waiting to be proposed) is 2x consensus latency; in expectation, it is 1.5x.

\fs{talk a bit about how this problem is sort of the root of the bad DAG latency. They must always wait for the previous leader to finish (9md). This really penalizes "siblings" of the leader}

To sidestep this issue, and thus minimize end-to-end latency \fs{want to get close to 1x consensus latency}, \sys{} begins consensus for a new slot in parallel (pipelined) with ongoing slots; as opposed to upon commitment of the prior slot. In spirit, this approach resembles a combination of parallel proposals issued by a stable leader in pbft, and chained pipelined proposals issued by rotating leaders in Hotstuff.

\sys{} begins consensus for slot $s$ as soon as the first $Prepare$ message for slot $s-1$ is received, and sufficient coverage is ensured. The worst-case wait time is thus 1md \fs{(+ time for coverage -- which doesn't count as wait time really)}
Consensus for concurrent slot instances is logically independent. They operate in parallel: normal case processing and view changes are agnostic to other slots. To finalize (be applied to the log), a slot must simply wait for all preceeding slots to be committed (and finalized) first.

Waiting for preceeding slot proposals guarantees that, in good intervals, two concurrent consensus instances do not perform redundant work. Put differently, slot instance $s$ provides \textit{additional} lane coverage over $s-1$'s proposal. We note, that this property is purely best effort. The proposed cuts of finalized slots may or may not extend each other. For instance, while the proposal of slot $s$ extended the \textit{first} proposal of slot $s-1$, view changes may have resulted in $s-1$ finalizing a different cut entirely. This is safe: since slots are finalized in-order, non-monotonic tip (-histories) are simply considered out-dated and are ignored (during the log flattening process). \fs{i.e. we discard everything that's already been done, and apply all new. Recall: there might be forks in byz lanes: we can either apply them too (no problem), or be lazy and ignore things with height <= already applied height} 

%%%%%%%%%%%%%%%%%%%%%% Timeouts 
Pipelining consensus requires us to adapt the view synchronization logic. For one, replicas no longer begin timers upon reception of the previous slots committment, but upon reception of the first (logical) Prepare message \fs{timeouts should account for time it might take to forward Prepare to the leader that needs it + time to get coverage}. Second, the leader-election scheme must be adjusted to decorrelate view changes across successive slots. If the same round-robin schedule is applied across and within slots, the worst case latency to complete $k$ successive slots is $k * (f+1)$. To avoid this, we shift round-robin assignment for slots by $f$ \fs{random election can also work}.

%%%%%%%%%%%%% Bounding instances
During good intervals there will be (in practice) at most 3-4 concurrent instances at a time \fs{there is 4 md before commit message => up to 4 instances can open}. In periods of asynchrony this can grow larger: new instances may keep opening (they only need to see a proposal), but instances are not closing at the same rate. Note: each new instance might still meet the coverage criterion (since data layer keeps growing)!
To avoid wastage we can bound the maximum number of open instances by introducing an additional criterion: To start slot instance s, one must include a commit certificate for slot instance $s-k$. 

%%%%%%%%%%%%% Garbage Collection
The same technique can be used to help us garbage collect. When extending proposals only, the commitQC for each slot must be kept around in order to reply to view changes \fs{e.g. to help inform replicas that haven't committed). We'd like to bound this. Can do so either by active checkpointing (requires synchronization), or by leveraging the depth limiter: When committing slot $s$, we can garbage collect the commitQC for slot $s-k$ because the cert for $s$ can be used to certify $s-k$'s committment (and $s-2k$, $s-3k$, and so on).
(Note, cannot gc everything $< s-k$; need to wait for finalization to do that -- however, $s-k-1$ will have been GC by $s-1$ already, and so forth)

\fi
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% NOTES / COMMENTS / OLD STUFF %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\iffalse
- Autabahn in all its glory: Describe Pipelining; managing multiple instances  (this reduces effective/end-to-end latency; i.e. it tries to AVOID sequential latency)
    - slots no longer sequential (view changes within slots)
    - when to start (+wait for new coverage); how to commit (wait for prev slots -- similar to parallel PBFT/pipelining in hotstuff); how to do view changes (when to start timeouts? how to rotate leaders); proposing new tips if
    - how to flatten into log?
        - slots not guaranteed to extend each other; keep only whats "new"
    - bounding #concurrent instances; in practice not many (2,3? up to f+x). Can bound to a fixed k (need as part of ticket also cert from s-k). This will allow GC older certs. (GC only < s-k once s commits)

\fi

==> Sections/3-System/Protocol/fairness.tex <==
%\subsection{Chain (E)quality}

\par \textbf{Chain (E)quality.}

\label{sec:fairness}
\fs{want to talk about fairness at all?}

\iffalse

%\subsection{Fairness: A tale of equity and equality}
- talk about chain quality:
typically guarantees that output log is 50/50 (equity)
 => DAGs get this by slowing everybody down to the same pace
    DAGs throttle all replicas into lock step (speed of the slowest in the Quorum).
    Lower resource replicas (slower replicas) get the same value as the higher resource ones (faster)
    Is this fair? 
    Our design is more merit based. Arguably, this is what leader reputation schemes end up with anyways! (i.e they negate the equity)

instead we guarantee chain equality: 
- opportunity for output log to be 50/50
  ==> need coverage to be 2f+1 new tips in order for this to hold

How many cars in each lane depends purely on the lanes connectivity (bandwidth, latencies) and load 

Note: Like DAGS we don't deal with request de-duplication; it is orthogonal. Some nice work that targets this problem explicitly is ISS/BFT-Mir

%%%%%%%%%%%%%%%%%%%%%%%%%%

Subtlety: This property may not hold for specific prefixes of the log. 
A byzantine proposer may choose to not respect coverage growth (e.g. only propose a bigger tips for the byz guys, but not for honest). Even if we forced that there is new from 2f+1 => byz leader could just propose 1 new for every honest, and 100 new for byz. => Consequently, if you look at the prefix of the log right after this byz leader then there was not equal opportunity.
However, by the next honest proposer it will have balanced out. 
\fs{even if we enforce: a view change could result in a different proposal being chosen -> thus the following pipeline proposal may not be an extension}

Note, that this is still an abuse of "fairness" in some way: In its tenure the leader could control what to include. However, I'd argue that this is not much different than a normal single leader BFT protocol that picks what TX to order how in its batch. One can try to implement orthogonal techniques that deal with ordering fairness (This is not OUR goal here.)

Bonus: If one really wants chain quality, then one can also parameterize the coverage growth with some k. E.g. for every lane you must include exactly $k_l$ new (k could be different per lane). We find this to be overly restrictive though.

%%%%%%%%%%%%%%%%%%%%%%5
Subtelty2:
Lose chain equality with pipelining? Cannot guarantee that two successive slots extend one another: coverage was checked for first proposal of slot s-1; but another may end up committing. 
=> This should not be a problem for the same reason as above => it all balances out..

%%%%%%%%%%%5

Bottom line: 
- we want to maximize tput
- we are "more or less" equal opportunity.


\fi


==> Sections/3-System/Protocol/optimizations-trial.tex <==
\subsection{Optimizations}
Finally, we discuss a number of optimizations, that, while not central to \sys{}'s ethos, can improve performance.

\subsubsection{Further reducing latency.}
\label{sec:optimistic_tips}
By default, \sys{} consensus pessimistically only proposes \textit{certified} tips. This allows voting in the consensus layer to proceed without blocking, which is crucial for seamlessness (\S\ref{sec:consensus_on_lanes}). Assembling and sharing certificates, however, imposes a latency overhead of three message exchanges in addition to the unavoidable consensus latency. This results in a best-case end-to-end latency of six message delays on the fast path, and eight otherwise. \sys{} employs two optimizations to reduce the latency between the dissemination of a data proposal and it being proposed as part of consensus (inclusion latency).  %\fs{Notably, this is a redundant cost with consensus, which also proves availability...}
\par \textbf{Leader tips.} First, we allow a leader to include a reference to the latest proposal ($dig, pos$) it has broadcast as its own lane's tip, even as the tip has not yet been certified.
%\fs{note: if ride sharing, the car carrying Prepare can be used as the tip}
If a Byzantine leader intentionally does not disseminate data, yet includes  the proposal as a tip, it is primarily hurting itself. Correct nodes will, at most, make a single extra data sync request before requesting a view change.  Moreover, if the Byz leader ever wants to propose additional data, it will have to backfill the data for this proposal (in-order voting).
%If the leader has failed to disseminate its own lane's history then progress of its tenured view may be interrupted; this will not happen for correct leaders that reliably disseminate (in order).} 

\par \textbf{Optimistic tips.} Second, \sys{} \changebars{may choose to relax seamlessness and allow leaders}{allows leaders} to optimistically propose non-certified tip references ($dig, pos$) for lanes that have, historically, remained reliable. \changebars{In gracious intervals, this optimization lowers inclusion latency to a single message exchange, which is optimal. However, this}{. This} comes at the risk of incurring blocking synchronization and triggering additional view changes. Replicas that have not received a tip locally hold off from voting, and request the tip from the leader directly. We note, that critical-path synchronization is only necessary for the tip itself (and thus has constant cost) -- by design, all ancestors must be certified, and thus can be synchronized asynchronously. \fs{this might be more detail than is necessary}\changebars{}{Moreover, synchronization is only necessary in either view $v=0$ or in subsequent views that did not select a winning proposal from a prior view. In all other cases, the selected proposal $P$ included in \textsc{Prepare}$_{v' > 0}$ is, by design, implicitly certified ($\geq f+1$ replicas voted for $P$).}

\fs{this discussion seems not that relevant.}
\changebars{}{In gracious intervals, this optimization lowers inclusion latency to a single message exchange, which is optimal. When the triangle inequality holds all replicas will locally deliver all proposed tips histories before receiving a \textsc{Prepare}; when it does not, replicas may over-eagerly request unnecessary synchronization. During less gracious intervals proposing optimistic tips poses a risk to a leader's tenure. For instance, a Byzantine proposer may forward its batch only to the leader, burdening it with synchronization, and potentially causing its view to time out.} %\changebars{Although the amount of required synchronization is bounded (only one car per lane), and thus remains practical, we classify the optimistic tip optimization as not fully seamless since synchronization is on the critical path of consensus.}{}
\iffalse 
\fs{CUT REPUTATION SCHEME. MOVE TO APPENDIX}
\changebars{To reduce unwanted synchronization in practice}{To improve the predictability of unwanted synchronization}, \sys{} can be augmented with a simple (replica-local) reputation mechanism\fs{Our current prototype does not implement this}. A leader forced to synchronize on some lane $l$'s tip downgrades its local perception of $l$'s reputability. Below a threshold, the leader stops proposing optimistic tips for $l$, and simply falls back to proposing a certified tip. Each replica is thus responsible for warranting optimism for its own lane and consequently its own data proposals' latency. Reputation can be regained over time, e.g. for each committed car.
\nc{I would remove this reputation scheme discussion. We don't do it, and it opens up to questions about how to design reputation schemes }
%\changebars{We remark that such a reputation scheme serves exclusively to minimize \textit{redundant} dissemination, and is not necessary for safety, liveness, or seamlessness; without, the worst case synchronization effort on the critical path remains constant.}{}
\fi


\subsubsection{Other optional modifications.}
\fs{could possibly be cut/replaced with a reference to appendix. If cut, then consolidate the section intro.}
\sys{} can, if desired, be further augmented with several standard techniques. We discuss them briefly for completeness.

\par \textbf{Signature aggregation.}
\sys{}, like others~\cite{gueta2019sbft, yin2019hotstuff, Bullshark} can be instantiated with threshold (TH) signatures~\cite{boldyreva2002threshold, shoup2000practical} that aggregate matching vote signature of any Quorum Certificate (PoA, PrepareQC, CommitQC) into a single signature. This reduces \sys{}'s complexity per car and consensus instance (during good intervals) to $O(n)$; view changes require $O(n^2)$ messages~\cite{yin2019hotstuff}. 
%In the presence of asynchrony or faults TH-aggregation may be at odds with ride sharing: if some correct replicas do not vote for all consensus passengers (e.g. due to timing out or advancing views) there may be non-matching; one must fall back to un-aggregated signatures, or employ aggregate signature schemes with support for multiple messages~\cite{boneh2003aggregate, lu2018lattice}.

\iffalse
\par \textbf{Signature aggregation.}
\sys{}, like many related works~\cite{gueta2019sbft, yin2019hotstuff, Bullshark} can be instantiated with Threshold (TH) Signatures~\cite{boldyreva2002threshold, shoup2000practical}. A leader can aggregate matching vote signature of any Quorum Certificate (PoA, PrepareQC, CommitQC) into a single signature, thus ensuring that all messages carrying a QC are constant-sized. This reduces \sys{}'s complexity per car and consensus instance (during good intervals) to $O(n)$; view changes require $O(n^2)$ messages~\cite{yin2019hotstuff}.
\fs{Don't talk about this, but simply put it into the list of aggregates.}
During asynchronous periods TH aggregation may be at odds with ride sharing: if some correct replicas do not vote for all passenger consensus instances (e.g. due to timing out or advancing views) the leader may receive $n-f$ different votes that cannot be aggregated; it must fall back to un-aggregated signatures, or employ aggregate signature schemes with support for multiple messages~\cite{boneh2003aggregate, lu2018lattice}.
%\fs{Problem/Tension with ride sharing: if some replicas don't vote on a consensus instance piggybacked on a car (e.g. due to having view changed) then the n-f votes are different and cannot be aggregated using Threshold signatures. One can use aggregate signatures instead, or has to resort to un-aggregated sigs for this car}
\fs{in the common case can still use TH sigs}
\fi

\par \textbf{All-to-all communication.}
\sys{} follows a linear-PBFT communication pattern~\cite{gueta2019sbft} that allows it to achieve linear complexity (during good intervals) when instantiated with aggregate signatures. \sys{} can, of course, also be instantiated with all-to-all communication for better latency (but no linearity). In this regime, consensus consists of only 3 message exchanges (2md on FastPath): replicas broadcast \textsc{Prepare-Vote}s and \textsc{Confirm-Ack}s, and respectively assemble $PrepareQC$s and $ConfirmQC$s locally. %To continue ride-sharing, ambassador cars can adopt all-to-all communication too.
\fs{Slightly more discussion in comments:}
%\one the leader broadcasts \textsc{Prepare}, \two all replicas broadcast \textsc{Prepare-Vote}s, and locally form a \textsc{Prepare-QC}, and \three all replicas broadcast a \textsc{Confirm} message, and locally assemble a \textsc{Commit-QC}. 
% Two design options exist to continue ride sharing: \one Ambassador cars become all-to-all, or \two the messages of a consensus view are piggybacked on car's of \textit{any} lane -- a replica simply uses the earlier of any locally available \textsc{Propose} (own lane) or \textsc{Vote} (possibly other lane); this option amplifies tension with TH signature aggregation as, for any given car, not all votes may include the same message batch.


==> Sections/3-System/Protocol/optimizations.tex <==
\subsection{Optional optimizations}
\label{sec:optimizations}

\sys{} can be augmented with several standard performance optimizations. Our prototype does not implement these. \fs{should we cut them all-together? They don't necessarily work out smoothly, so i'd consider this more of a discussion section, rather than straightforward optimizations}

% \par \textbf{Optimistic (non-certified) tips.}
% The leader can propose uncertified tips (i.e. the proposal on the latest car; rather than the latest certificate) at the risk of having to synchronize on the critical path. 

% The idea is simple: Effectively let Consensus handle the certification, and avoid redundant work.

% Tradeoff: 
% Pro: if things go smoothly, latency is 2md lower (don't need to wait to get certificate first)
% Con: if things don't go smoothly: leader has to supply the proposed tip (adds 2md + makes leader do more work).
%      In this case: replica cannot reply yet -> its vote needs to move into a new car, which complicates sig ride sharing \fs{Cleaner: ask for sync externally. Hold off on replying to car until vote. This makes signature sharing cleaner}
%      -> Makes consensus latency less predictable. Allows byz to offload broadcasting work.

% Note: In the gracious case this optimization is probably quite desirable. Although some replicas might not have the payload yet at the time they receive a proposal for a tip (e.g. due to asymmetric link latencies), they will eventually get it. So it's not true that we will pay a +2md latency penalty. A replica might ask for sync, but then shortly after receive the message normally and proceed to vote. Triangle relationship mostly holds:\fs{this wastes some bandwidth for syncing, but it's whatever} \fs{note: No matter how skewed the latency assymmetry, it should always be faster to go from R1 to R2, than from R1 to L1 to R2 to L1 to R2}
% Only byzantine/crashed senders result in the +2md cost (for the leader to forward).

% Bound: Still don't allow chains of Best effort broadcasts. This way, if we recover from a period of sync, it's still seamless: we may just need to do a sync on n  proposals (but it's independent from the length of async). If instead, we built a hash chain without certs, then we'd have to potentially wait for a replica to sync on all of it.

% Improving predictability:  + Honest leader does not want to lose its tenure!
% To make consensus latency more predictable in non-gracious intervals, the leader can try to either a) pessimistically forward the data itself (but this is a lot of redundant broadcasting work), or b) try to manage a reputation scheme for replicas: If the leader was forced to provide sync on a tip issued by replica R, then it can downgrade R's reputation. If the reputation is below a threshold, it may stop including uncertified tips. This only affects the end-to-end latency of R's proposals! (Reputation can be regained slowly over time. E.g. a performance related metric could be "how many cars have been committed on this lane" -> this indicates workrate) \fs{cite private discussions with Sasha..}

\par \textbf{Signature aggregation.}
\sys{}, like many related works~\cite{gueta2019sbft, yin2019hotstuff, Bullshark} can be instantiated with Threshold (TH) Signatures~\cite{boldyreva2002threshold, shoup2000practical}. A leader can aggregate matching vote signature of any Quorum Certificate (PoA, PrepareQC, CommitQC) into a single signature, thus ensuring that all messages carrying a QC are constant-sized. This reduces \sys{}'s complexity per car and consensus instance (during good intervals) to $O(n)$; view changes require $O(n^2)$ messages~\cite{yin2019hotstuff}.
We want to point out, however, that TH aggregation may be at odds with ride sharing during asynchronous periods. If some correct replicas do not vote for all passenger consensus instances (e.g. due to having view changed) the leader may receive $n-f$ different votes that cannot be aggregated using TH signatures; it must fall back to un-aggregated signatures, or employ aggregate signature schemes with support for multiple messages~\cite{boneh2003aggregate, lu2018lattice}.
\fs{Problem/Tension with ride sharing: if some replicas don't vote on a consensus instance piggybacked on a car (e.g. due to having view changed) then the n-f votes are different and cannot be aggregated using Threshold signatures. One can use aggregate signatures instead, or has to resort to un-aggregated sigs for this car}
\fs{in the common case can still use TH sigs}

% Quorums from same instance can be flattened via use of TH sigs.
% - Note: this is not compatible with Basil based batching (merkle paths may be different) -> need aggregate sig for this.


% \par \textbf{Signature ride sharing.}
% \fs{this is so small it feels like it can just move into the Embedding section.}

% Move the whole embedding section here. Then talk about the tradeoff that this introduces.
% Introduce special rule back:
% - try to ride share if convenient
% - ride yourself otherwise:

% A car's \textsc{Proposal} and \textsc{Vote} messages may piggyback messages from several consensus instances. To minimize the number of signature generations and verifications required, \sys{} can share a single signature across all passengers -- a replica simply batches and signs

% Propose messages obviously can share a sig, no implications
% If vote messages share sig => Quorum is on a multi-message.
%  -> this is fine: QC's are propagated per lane (send's all messages anyways). Syncing on only ONE Qc becomes more expensive (need all messages). Can use Basil style merkle tree batching to reduce this to log b bits.

%  Can aggregate sigs for the shared messages.

%Optimistic sigs unaffected: We currently describe them as BLOCKING on the leaders lane == leader takes responsibility (no new cars while outstanding sync)
 % ---------------

% We can try to share the signatures of data dissemination and (multiple) instances of consensus that are using the same car.
% -> this will reduce signature generation and verification costs.  \fs{and might let us show a tput improvement because our cars have smaller Quorums than DAG -- assuming sigs become the bottleneck}

% If we are using the most basic protocol (without aggressive tips, all to all communication) then Quorums are formed WITHIN lanes only, and all vote replies should have the same set of messages (if the leader was honest). => so technically can just sign the batch (and then can even use TH sig to collapse the batch). 

% Challenge: 
% - to verify only one instance, need the messages of all instances that were signed. => can use Basil batching to turn into merkle tree.
% - note: this is not a problem on the normal path: all replicas want to verify all the content of a car anyways. But it's annoying to have to send all batched messages to prove just a single instance (for example for a view change). Though maybe it's not worth optimizing since the size might be small anyways, it's just meta data for a couple consensus instances.

% - if we do all-to-all or aggressive tips, then it may no longer be true that all votes (used to form a quorum for a given instance i) have the same set of messages. In that case, cannot do Th sigs (only aggregate). To avoid having to include all the messages for verification => use Basil sig batching.


% \par \textbf{Special Rule}:
% Problem: Consensus is waiting for up to 2md for car to be done.
% We might not want to wait for the next car to start.
% Start a special car directly. Special car has no parent cert requirement (no position). It's just extra. It's covered by the leader tip optimization.

% I think we should just bring back the simplest special rule where a consensus can start it's own car (after a tiny timeout?). This car is "special" because it needs to have no parent cert. Since it's the leader tip that's fine.
% it can extend the directly preceeding proposal if we want, in order to commit it as well
% and it can be referenced with a bonus edge by the next proposal (in case it doesn't commit, this way the proposal on the special car survives)


\par \textbf{All-to-all communication.}
\sys{} follows a linear-PBFT communication pattern~\cite{gueta2019sbft} that allows it to achieve linear complexity during good intervals (when instantiated with threshold signatures). \sys{} can, of course, also be instantiated with an all-to-all communication pattern to further reduce consensus latency--at the cost of linearity. In this discipline, consensus consists of only 3 message exchanges (2md on FastPath): \one the leader broadcasts \textsc{Prepare}, \two all replicas broadcast \textsc{Prepare-Vote}, and locally form a \textsc{Prepare-QC}, and \three all replicas broadcast a \textsc{Confirm} message, and locally assemble a \textsc{Commit-QC} from $n-f$ matching confirmations.

Two design options exist to continue ride sharing: \one Ambassador cars become all-to-all, or \two the messages of a consensus view are piggybacked on car's of \textit{any} lane -- a replica simply uses the earlier of any locally available \textsc{Propose} (own lane) or \textsc{Vote} (possibly other lane). We note that the latter option exists in tension with signature aggregation: for any given car, not all votes may include the same message batch, and thus threshold signatures are not applicable. \fs{could use aggregate sigs if one really wanted}

% Instead of linear pbft, use all-to-all.
% Prepare. Broadcast Prepare-vote (form PrepareQC locally). Upon having PrepareQC, broadcast Confirm (form commitQC locally). 

% View change: stays the same. Vote with PrepareQC. 

% Two options:
% 1) Make one lane all to all (also changes car structure)
% 2) Try to map it to multiple lanes (since there is already an "all to all" happening)

% --> 2: Problematic when combined with aggregation and ride sharing.
%     1. Prepare message can be mapped to car proposal
%     2. Then every replica must broadcast to all a Confirm. This can be piggybacked on a Car proposal   (easy), or a Car Vote (problematic)
%     3. Same goes for the Commit msg

% - It is not guaranteed that all car votes look the same => thus we cannot aggregate vote signatures if we are using ride sharing   (+ we need to send multiple messages)
% - If you only send on Car Proposal, then you may be waiting same time it takes linearly!!

% TLDR: Mapping all to all is in tension with signature aggregation + ride share.
% -> To nonetheless ride share (not have to send message for all in quorum), and aggregate, one can use Basil style batching + aggregate sigs.

% -----------------

% Can make Data lane and consensus all to all.

% Alternatively, can also Map consensus onto any proposal/vote, instead of just into one lane. 
% => in this case, proposals/votes don't necessarily have the same set of consensus messages => can't just batch sig. Use Basil style batching. 
% => NOTE: this makes consensus wait possibly: Need proposal on each lane in order to drive

% Pro: lower latency: Slow path 3md, Fast path 2md
% Con: all-to-all has $O(n^2)$ - cannot be reduced by TH sigs. BUT: it's just embedded on the already existing "all-to-all" of the Data layer

% \fs{alternatively: Could also make lanes themselves all to all, but this increases complexity to $n^3$ }



\subsubsection{Other possible modifications.} \fs{Do not mention any of these. Currently commented out.}

% \par \textbf{TC Tickets.}   A ticket to start the next slot is a Prepare message for the current slot. This, however, could delay the start of the next slot if there is a sequence of consecutive faulty leaders that fail to send a Prepare message. To minimize this delay, a ticket to start the next slot can alternatively be a TC itself (not as part of a Prepare message). This TC can contain the latest tips for each replica that send a Timeout message, which the next slot leader must extend for its Prepare message, providing greater coverage.

% \fs{we're doing this anyways already in the description}
% \par \textbf{Timeout Messages Riding Cars.} Timeout messages are sent externally (not on cars) so view changes are not affected by delays from possibly missing the bus. This however, adds small overhead to just the data layer (albeit small since these messages just contain metadata). Alternatively, these timeout messages could ride cars so that the consensus layer has no message overhead on the data layer. Note: They should ride the propose message (not the vote message) to ensure that the simpler (i.e. without Basil batch) signature ride sharing still works.

% \par \textbf{Chaining Consensus Instances.} Autobahn pipelines single-decree linear pbft instances to minimize end-to-end latency. This, however, adds additional complexity by having replicas keep track of slots AND views. One could instead adapt a protocol like Chained HotStuff, which simplifies some overhead with managing slots. and allows signatures to be shared for multiple consensus instances.

==> Sections/3-System/Protocol/pseudocode.tex <==


%\textbf{Goals.}
%\begin{itemize}
%    \item High throughput of DAG protocols with low latency 
%    of traditional leader based BFT
%    \item DAG protocols decouple data dissemination from consensus
%    \item However, both layers are intertwined together
%    \item Consensus crucially relies on the structure/causal ordering of the 
%    data dissemination layer
%    \item Like other protocols we separate out data dissemination from 
%    consensus to maximize throughput
%    \item Our data dissemination layer is much less restrictive than DAG protocols since we do not rely on its structure
%\end{itemize}

%\par \textbf{Data Dissemination Layer Design}
%\begin{itemize}
%    \item Goal: Provide async responsive throughput
%    \item To maximize throughput we want to guarantee data availability while also minimizing 
%    the latency to complete broadcasts
%    \item For data availability we just need proof that f+1 replicas stored the data, ensures 
%    that if we fetch at least 1 honest will respond with the data
%    \item The DAG adds unnecessary synchronization for pure data dissemination. Replicas have to wait to complete n-f broadcasts from other replicas before disseminating a new block of data, adding extra latency
%    \item We get rid of of the DAG structure and instead use n parallel chains. Each replica can grow its own chain independently without waiting to complete broadcasts from other replicas
%\end{itemize}

%\par \textbf{Consensus Layer Design.}
%\begin{itemize}
%    \item Goal: Avoid sequential latency
%    \item We use a traditional BFT consensus protocol: linear PBFT/HotStuff to have as low latency as possible
%\end{itemize}

\fs{TODO:}

\begin{algorithm}
\begin{algorithmic}[1]
\Procedure{Block}{$tip,tipCert,infoList$}
%\State{$B\gets \Call{NormalBlock}{tip,tipCert}$}
\State{$B.height\gets tip.height+1$}
\State{$B.parent\gets \Call{H}{tip}$}\Comment{H is a cryptographic hash 
function}
\State{$B.parentCert\gets tipCert$}
\State{$B.batch\gets $ a batch of client transactions}
\State{$B.infoList\gets infoList$}
\State{\Return $B$}
\EndProcedure

\Procedure{Cert}{$votes$}
\State{\textbf{parse} $votes$ as set of \msg{Vote}{hash,height,infoList}}
\State{$C.hash\gets hash$}
\State{$C.votes\gets votes$}
\State{$C.height\gets height$}
\State{$C.infoList \gets infoList$}
\State{\Return $C$}
\EndProcedure

\Procedure{PrepareInfo}{$slot,view,ticket,proposals$}
\State{$PI.slot\gets slot$}
\State{$PI.view\gets view$}
\State{$PI.ticket\gets ticket$}
\State{$PI.proposals\gets proposals$}
\State{\Return $PI$}
\EndProcedure

\Procedure{ConfirmInfo}{$slot,view,cert,type$}
\State{$CI.slot\gets slot$}
\State{$CI.view\gets view$}
\State{$CI.qc\gets cert$}
\State{$CI.type\gets type$}
\State{\Return $CI$}
\EndProcedure

\Procedure{TC}{$votes$}
\State{\textbf{parse} $timeouts$ as $n-f$ \msg{Timeout}{v,qc_i}}
\State{$TC.view\gets v$}
\State{$TC.timeouts\gets timeouts$}
\State{\Return $TC$}
\EndProcedure
\end{algorithmic}
\caption{\sys{} Data Structures}
\end{algorithm}

\begin{algorithm}
\begin{algorithmic}[1]
\State{$//$\textit{Haven't added yet: special edge rule, fast path, checkpointing/gc}}
\State{$tips_i \gets \{\}$}\Comment{Local view of tips for each chain}
\State{$infoList_i \gets \{\}$}\Comment{Consensus information to be included}

\State{$//$ \textit{Initial broadcast}}
\If{$tips_i[i]=\bot$}
\State{$tips_i[i]\gets \Call{Block}{\bot,\bot,infoList_i}$}
\State{\textbf{send} \msg{Propose}{tips_i[i]}}
\State{$infoList_i.\Call{Clear}{\null}$}\Comment{Reset info after proposing}
\EndIf

\Event{receiving a valid \msg{Propose}{B_j} from replica $j$}
\If{$\Call{IsNormalValid}{B_j}$}
\State{$//$\textit{Add block to our local view of the chain}}
\If{$B_j.height>tips_i[j].height$}
\State{$tips_i[j]\gets B_j$}
\EndIf
\State{\textbf{send} \msg{Vote}{\Call{H}
{B_j},B_j.height,\{\}}}\Comment{H is a cryptographic hash 
function}
\EndIf
\EndEvent

\Event{receiving $V\gets f+1$ \msg{Vote}{\Call{H}{B_i},height,-}}
\State{$cert \gets \Call{Cert}{V}$}\Comment{$f+1$ votes guarantees availability}
\State{$//$\textit{Once we have a cert, we can propose a new block}}
\If{$cert.height>tips_i[i].parentCert.height$}
\State{$tips_i[i]\gets \Call{Block}{tips_i[i], cert, infoList_i}$}
\State{\textbf{send} \msg{Propose}{tips_i[i]}}
\State{$infoList_i.\Call{Clear}{\null}$}
\EndIf
\EndEvent
\end{algorithmic}
\caption{\sys{} data dissemination}
\end{algorithm}

\begin{algorithm}
\begin{algorithmic}[1]


\Procedure{ProcessPrepare}{$B,info$}
\State{$pValid\gets \Call{IsPrepareValid}{info}$}
\If{$pValid$}
\State{$view_i[info.slot]\gets info.view$}\Comment{Enter new view}
\State{$timers_i[info.slot].\Call{Start}{\null}$}\Comment{Start the view timer for the new view}
\State{$proposed\gets proposedSlots_i.\Call{Contains}{info.slot+1}$}
\State{$//$\textit{If we are the leader of the next slot and haven't already proposed the next slot, then we have our ticket to propose}}
\If{$i=\Call{Leader}{info.slot+1,1}\land \neg proposed$}
\State{$ticket_i\gets B$}
\EndIf
\State{$//$\textit{Add newer block to our local view of the chain}}
\If{$B.height>tips_i[j].height$}
\State{$tips_i[j]=B$}
\EndIf
\EndIf
\EndProcedure

\Procedure{ProcessConfirm}{$B,info$}
\State{$cValid\gets \Call{IsConfirmValid}{info}$}
\If{$cValid$}
\If{$B.parentCert.view>qc_i[info.slot].view$}
\State{$qc_i[info.slot]\gets B.parentCert$}
\EndIf
\State{$//$\textit{The commit condition}}
\If{$qc_i[info.slot].type="Commit"$}
\State{$committed_i[info.slot]\gets info$}
\EndIf
\If{$B_j.height>tips_i[j].height$}
\State{$tips_i[j]=B_j$}
\EndIf
\EndIf
\EndProcedure

\Procedure{EnoughCoverage}{$ticket, tips$}
\State{$newerHeights\gets 0$}
\For{$r\in R$}
\State{$newHeight\gets tips[r].parentCert.height$}
\State{$oldHeight\gets ticket[r].height$}
\If{$newHeight>oldHeight$}
\State{$newerHeights\gets newerHeights+1$}
\EndIf
\EndFor
\State{\Return $newerHeights\geq n-f$}
\EndProcedure

\end{algorithmic}
\caption{\sys{} Consensus Utilities}
\end{algorithm}


%\begin{algorithm}
%\begin{algorithmic}[1]
%\Procedure{IsProposeValid}{$B_j$}
%\State{\textbf{assert} $\Call{CheckCoverage}{B_j.ticket,B_j.proposals}$}
%\State{\textbf{assert} $B_j.slot=B_j.ticket.slot+1$}
%\State{\Return $true$}
%\EndProcedure

%\Procedure{IsNormalValid}{$B_j$}
% 1. Check block is at the correct height
% 2. Ensure voting at most once per height semantics
% 3. Check that block height is 1 more than parent cert
%\State{\textbf{assert} $|B_j.parentCert.votes|\geq f+1$}
%\State{\textbf{assert} $B_j.height=B_j.parentCert.height+1$}
%\State{\Return $true$}
%\EndProcedure

%\Procedure{CheckCoverage}{$ticket, tips$}
%\State{$newerHeights\gets 0$}
%\For{$r\in R$}
%\State{$newHeight\gets tips[r].parentCert.height$}
%\State{$oldHeight\gets ticket[r].height$}
%\If{$newHeight>oldHeight$}
%\State{$numNewHeights\gets numNewHeights+1$}
%\EndIf
%\EndFor
%\State{\Return $numNewHeights\geq n-f$}
%\EndProcedure

%\Procedure{IsSpecialValid}{$B_j$}
%\State{$B_{parent}\gets \Call{Sync}{B_j.parentCert.hash}$}
%\State{\textbf{assert} $B_j.parentCert.hash=\Call{H}{B_{parent}}$}
%\State{\textbf{assert} $B_j.height-B_{parent}.height\leq 2$}
%\State{\textbf{assert} $B_j.view\geq view_i$}
%\State{\textbf{assert} $B_j.view=B_j.ticket.view+1$}
%\State{\Return $\Call{CheckCoverage}{B_{parent}.proposals, B_j.proposals}$}
%\EndProcedure

%\end{algorithmic}
%\caption{Block Validity Checks}
%\end{algorithm}




\begin{algorithm}
\begin{algorithmic}[1]
\State{$view_i \gets \{\}$}
\State{$qc_i \gets \{\}$}
\State{$tc_i\gets \{\}$}
\State{$timers_i \gets \{\}$}
\State{$ticket_i \gets \bot$}

\State{$proposedSlots_i\gets \{\}$}
\State{$committed_i\gets \{\}$}
%\State{$chainCerts_i\gets \{\}$}
%\State{$proposedHeights\gets \{\}$}
%\State{$committedHeights \gets \{\}$}

\State{$//$ \textit{Initial consensus}}
\If{$i=\Call{Leader}{1,1}$}
\State{$PI\gets \Call{PrepareInfo}{1,1,\bot,\bot}$}
\State{$infoList_i.\Call{Insert}{PI}$}
%\State{$tips_i[i]\gets \Call{SpecialBlock}{1,1,\{PI\}}$}
%\State{\textbf{send} \msg{Propose}{tips_i[i]}}
\EndIf

\Event{receiving a valid \msg{Propose}{B_j} from replica $j$}
% Don't need if statement, create valid vector, and check if it's all false afterwards
\State{$specialValids\gets \{\}$}
\For{$info\in B_j.infoList$}
\State{$\Call{ProcessPrepare}{B_j,info}$}
\State{$\Call{ProcessConfirm}{B_j,info}$}
\State{$pValid\gets \Call{IsPrepareValid}{info}$}
\State{$cValid\gets \Call{IsConfirmValid}{info}$}
\State{$specialValids[info]\gets pValid\lor cValid$}
\EndFor

\If{$specialValids\neq \{\} \lor \Call{IsNormalValid}{B_j}$}
\State{\textbf{send} \msg{Vote}{\Call{H}{B_j}, B_j.height, specialValids}}
\EndIf
\EndEvent

\Event{receiving $V\gets n-f$ \msg{Vote}{\Call{H}{B_i},h,infoList}}
\State{$confirmInfos\gets \{\}$}
\For{$info \in infoList$}
\If{$\Call{IsPrepareValid}{info}$}
\State{$type\gets "Prepare"$}
\Else
\State{$type\gets "Commit"$}
\EndIf
\State{$CI\gets \Call{ConfirmInfo}{info.slot,info.view,info.hash,type}$}
\State{$confirmInfos.\Call{Insert}{CI}$}
\EndFor
\State{$qc \gets \Call{QC}{V,confirmInfos}$}
%\If{$h>tips_i[i].parentCert.height$}
\State{$tips_i[i]\gets \Call{Block}{tips_i[i],qc,infoList_i}$}
\State{\textbf{send} \msg{Propose}{tips_i[i]}}
\State{$infoList_i.\Call{Clear}{\null}$}
%\EndIf
\EndEvent

\Event{$\Call{EnoughCoverage}{ticket_i,tips_i}\land ticket_i\neq \bot$}
%\State{$tips_i[i]\gets \Call{CreateProposeBlock}{ticket_i}$}
%\State{$tips_i[i]\gets \Call{CreateSpecBlock}{B,view_i,ticket_i}$}
\State{$slot\gets ticket_i.slot$}
\State{$certs\gets \{tip.parentCert: tip \in tips\}$}

\State{$PI\gets \Call{PrepareInfo}{slot+1,1,ticket_i,certs}$}
\State{$proposedSlots_i.\Call{Insert}{slot}$}
\State{$infoList_i.\Call{Insert}{PI}$}
\State{$ticket_i\gets \bot$}
%\State{\textbf{send} \msg{Propose}{tips_i[i]}}
\EndEvent


%\Event{receiving $V\gets n-f$ \msg{Vote}{H(B'),-}}
%\State{$cert \gets \Call{CreateCert}{V}$}
%\If{$B'=B^i_{tip}$}
%\State{$highCert_i\gets cert$}
%\State{$b_h\gets $ a batch of transactions}
%\State{$height_i\gets height_i+1$}
%\State{$B^i_{tip}\gets (\Call{H}{B^i_{tip}}, height_i, highCert_i, b_h)$}
%\State{\textbf{send} \msg{Propose}{B^i_{tip}}}
%\EndIf
%\EndEvent

\end{algorithmic}
\caption{\sys{} parallel chains consensus}
\end{algorithm}

\begin{algorithm}
\begin{algorithmic}[1]
\Procedure{WinningProposals}{$tc$}
\State{$PI\gets \bot$}
\For{$timeout\in tc.timeouts$}
\State{\textbf{parse} timeout as \msg{Timeout}{v,qc_i,info}}
\If{$qc_i.view>PI.view$}
\State{$PI\gets info$}
\EndIf
\EndFor
\If{$PI=\bot$}
\State{\Return{$tips_i$}}
\EndIf
\State{\Return{$PI.proposals$}}
\EndProcedure

\Event{$timers_i[slot].\Call{Expire}{\null}$}
\State{\textbf{send} \msg{Timeout}{slot,view_i[slot],qc_i[slot]} to all}
\EndEvent

\Event{receiving $T\gets n-f$ \msg{Timeout}{slot,v,qc_i}}
\State{$tc \gets \Call{CreateTC}{T}$}
\If{$v>view_i[slot]$}
\State{$view_i[slot]\gets v+1$}
\State{\textbf{send} $tc$ to all}
\EndIf
\EndEvent

\Event{receiving a Timeout Certificate (TC) $tc$}
\If{$i=\Call{Leader}{tc.slot,tc.view+1}$}
\State{$tc_i[slot]\gets tc$}
\State{$//$\textit{If view change says none of the prior tip certs could have been committed, then winning info returns the current certs this replica has for each chain}}
\State{$certs\gets \Call{WinningProposals}{tc}$}
\State{$PI\gets \Call{PrepareInfo}{tc.slot,tc.view,tc,certs}$}
\State{$infoList_i.\Call{Insert}{PI}$}
\EndIf
\State{$//$\textit{Check whether we have already proposed something for the slot}}
\State{$proposed\gets proposedSlots_i.\Call{Contains}{slot+1}$}
\If{$i=\Call{Leader}{slot+1,1} \land \neg proposed$}
\State{$ticket_i\gets tc$}
\EndIf
\EndEvent
\end{algorithmic} 
\caption{\sys{} view change}
\end{algorithm}


%\begin{algorithm}
%\begin{algorithmic}[1]
%\Procedure{CommitRule}{$B_j$}
%\If{$\Call{IsQC}{B_j.ticket}$}
%\State{$B_1\gets \Call{Sync}{B_j.ticket}$}
%\If{$\Call{IsQC}{B_1.ticket}$}
%\State{$B_0\gets \Call{Sync}{B_1.ticket}$}
%\If{$B_0.view+1=B_1.view$}
%\State{\Return $B_0$}
%\EndIf
%\EndIf
%\EndIf
%\State{\Return $\bot$}
%\EndProcedure

%\Procedure{ViewChange}{$B_{commit}$}
%\State{$stack = \{B_{commit}\}$}
%\State{$B'\gets B_{commit}$}

%\While{$B'.view < v_c$} \Comment{$v_c$ is the view of the last committed block}
%\If{$\Call{IsQC}{B'.ticket}$} \Comment{QC from previous view}
%\State{$B\gets \Call{Sync}{B'.ticket.hash}$}
%\State{$stack.\Call{push}{B}$}
%\State{$B'=B$}
%\ElsIf{$\Call{IsTC}{B'.ticket}$}
%\State{$tcBlocks\gets \Call{Sync}{B'.ticket}$}
%\State{$B\gets \Call{WinningProposal}{tcBlocks}$}
%\State{$stack.\Call{push}{B}$}
%\State{$B'=B$}
%\EndIf
%\EndWhile

%\While{$\neg stack.\Call{empty}$} \Comment{Iterate over committed special blocks}
%\State{$B=stack.\Call{pop}$}
%\State{Commit $B$'s causal history is some deterministic order}\Comment{Indirect commit}
%\EndWhile

%\EndProcedure

%\end{algorithmic}
%\caption{Sailfish Commit Rule and View Change}
%\end{algorithm}



==> Sections/3-System/Sailfish_notes/protocol_details.tex <==
\section{Protocol Details}
\protocol{
\underline{Block:}
\begin{itemize}
    \item $r$: the round (for \textbf{DAG}) of the header
    \item $edges$: hash pointers to $n-f$ certificates in round $r-1$ if normal 
    block, OR pointers to $k \geq 1$ headers in round $r-1$ if special block
    rule is satisfied
    \item $b_h$: payload containing batches of client transactions
\end{itemize}
\underline{Additional State for a Special Block:}
\begin{itemize}
    \item $v$: the view (for \textbf{consensus}) of the block
    \item $special\_edges$: hash pointers to blocks in round $r-1$
    \item $ticket$: a Timeout Certificate (TC) in view $v-1$ OR
    a Commit Quorum Certificate (Commit QC) for a special block in view $v-1$
\end{itemize}
}

\protocol{
\underline{Quorum Certificate (QC):}
\begin{itemize}
    \item $H(B)$: hash of the block
    \item $V$: either 1) $n-f$ matching \msg{Vote}{H(B)} messages (DAG QC) or 2) $n-f$ matching \msg{Accept}{H(B)} messages (Commit QC)
\end{itemize}
}

\protocol{
\underline{Replica $R$ Local State:}
\begin{itemize}
    \item $r$: current DAG round number
    \item $DAG_R$: the local DAG 
    \item $v$: current view number
    \item $commitQC_R$: the highest (by view) CommitQC received.
    \item $dagQC_R$: the highest (by view) DagQC received for a special block 
    \item $highPropose_R$: highest (by view) valid \textsc{Propose} message received 
    for a special block
    \item $highAccept_R$: highest (by view) valid \textsc{Accept} message sent for a
    special block
\end{itemize}
}

\subsection{Block Life cycle}

%\todo{I would change our signature description to $\msg{Type}{Content}_\sigma$. The Type needs to be signed too after all.}

We assume all messages are signed. We distinguish between two block types that are proposed to the DAG: normal and special. For all DAG purposes, normal and special blocks are (mostly) the same, but special blocks contain additional meta data that drives consensus. We detail the common protocol on the DAG below, and indicate special block specifics as add-ons.\\

\par \textbf{Propose.}
A proposer $P$ can propose a new block, $B_p$, in round $r$, once it receives $n-f$ DAG 
certificates from round $r-1$ (more detail later), which is satisfied when $|DAG_P[r-1]|\geq n-f$.
To propose $B_p$, $P$ assembles a batch of client transactions
into $b_h$, and collects $DAG_P[r-1]$ as $parents$. Each parent edge is a DAG certificate from the prior round ($r-1$). Note, that it is immaterial whether $parents$ contain "normal" or "special" blocks. 
A block proposal includes two additional special fields $v$ and $ticket$ that are empty by default, and are only set for special blocks (see below).
It additionally signs $(r, edges, b_h, v, ticket)$. 

\underline{Additonal Special Block Considerations:}
If $P$ is the designated leader $L_v$ for a current view $v$, it may upgrade its block to be \textit{special} if it collects a ticket. A ticket is either
\begin{enumerate}
    \item at least $n-f$ \msg{Vote}{H(B), true} messages (QC) OR
    \item at least $n-f$ \msg{Timeout}{v-1,-,-,-} messages (TC).
\end{enumerate}
Detailed information about \textsc{Vote} and \textsc{Timeout} messages are discussed later.
$P$ includes such a QC or TC in $B_p$ as $ticket$, indicating that the block is special.

\protocol{\underline{Step 1: $P$ to all $R$} \\
Send \msg{Propose}{B_p} where 
$B_p=(r, parents, b_h, v, ticket)$
}

\par \textbf{Vote.} 
Upon receiving a Proposal for $B_p$, a replica $r$ checks the validity of $B_p$: It confirms the 
message proposal is well-formed, it's signature is valid, that it contains $n-f$ parent edges to DAG certificates in 
round $r-1$, and that it has received no previous \textsc{Propose} request from $P$ in round $r$. 
If these checks do not pass, replica $R$ discards the \textsc{Propose} message.

\underline{Additonal Special Block Considerations:}
If $B_p$ is special (contains $v$ and $ticket$) replica $R$ performs additional validation: 
\begin{enumerate}
    \item It confirms that $B_p.v\geq v$. Otherwise, this proposal is outdated, and $R$ treats $B_p$ as a normal block for the remainder and sets $specialValid := false$.
    \item It confirms that $P=L_v$, and that $B_p$ is the first proposal it has received in view $v$.
    \item It confirms that $ticket$ contains either a) a valid QC for a special block in view $v-1$, or b) a TC containing $n-f$ \textsc{Timeout} messages for view $v-1$.
\end{enumerate}
%If these special validation checks fail, $R$ sets this serves as PoM of $P$.
If the special block validation checks pass successfully, replica $R$ sets the flag $specialValid := true$, updates its local view $v := B_p.v$, and updates its local highest proposal to $highPropose_R :=$ \msg{Propose}{B_p}. Additionally, if $B_p.ticket$ is a valid QC then $R$ updates its $QC_R := B_p.ticket$ and adds it to the DAG by setting $DAG_R[r][P]=QC_R$. Replica $R$ then resets its view timer, and sends a signed \textsc{Vote} message containing $H(B_p)$ and $specialValid$.  
%((Note to self: Our view change should be able to produce a Commit QC implicitly; i.e. a view change quorum that includes a block f+1 times in highest view $v$ implies commit(?)

\protocol{\underline{Step 2: $R$ to $P$} \\ Send \msg{Vote}{H(B_p), specialValid}}

\par \textbf{Confirm.}
The Confirm step is only for normal blocks. $P$ waits to collects a set of $n-f$ signed \msg{Vote}
{H(B_p),-} messages, and forms a DAG certificate, $C(B_p)$, from these messages.

%\underline{Additional Special Block Considerations:}
%If $B_p$ is special, replica $R$ performs additional validation:
%\begin{enumerate}
%    \item $P$ waits to collect $n-f$ valid \msg{Vote}{H(B_p), true} messages or until $specialValidTimer$ expires. If $specialValidTimer$ expires before collecting $n-f$ valid \msg{Vote}{H(B_p), true} messages, $R$ sets $specialValid := false$ and forms a DAG certificate for $B_p$.
%    \item After receiving $n-f$ valid \msg{Vote}{H(B_p), true}, $P$ waits to collect an additional $f$ \msg{Vote}{H(B_p), true} messages ($n$ in total).
%\end{enumerate}
%If condition $1$ holds but not condition $2$, $P$ forms a QC using the $n-f$ \msg{Vote}{H(B_p), true} messages it received. Otherwise if condition $2$ holds, $P$ sends a \textsc{Fast-Commit} message containing a fast QC ($n$ \msg{Vote}{H(B_p), true} messages).

%After $P$ forms either a DAG certificate, a QC, or a fast QC, it proposes a new block.
%TODO: Also wait for some timer, if 3f+1 matching commit also. ((Put this under optimizations probably))

\protocol{\underline{Step 3: $P$ to all $R$} \\ Send \msg{Confirm}{C(B_p)}} 
When a replica $R$ receives $C(B_p)$, it adds the certificate to its local DAG by setting 
$DAG_R[B_p.r][P]=C(B_p)$.

%\par \textbf{Accept.}

%A replica $R$ checks the validity of $dagQC$, and that it is well-formed (contains $n-f$ \textsc{Vote} messages containing $H(B_p)$).
%If $dagQC$ is valid, then replica $R$ adds the certificate and corresponding 
%block to its DAG.

%\underline{Additonal Special Block Considerations:}
%If $dagQC$ is valid and $B_p.v >= v$, $R$ updates its $dagQC_R$ to be $dagQC$. 
%\todo{Note, that at this point, the replica could also indirectly commit any past View Changes.}
%It sends an \textsc{Accept} message for $H(B_p)$ to $L_{v+1}$. (Note, that with a stable leader $L_{v+1} = P$.

%\protocol{\underline{Step 4: $R$ to $L_v$} \\ Send \msg{Accept}{H(B_v)}}



%\protocol{\underline{Step 5: $L_v$ to $R$} \\ Send \msg{Decide}{commitQC}}
%When a replica $R$ receives a \textsc{Decide} message, it directly commits $B_p$ and updates its $commitQC_R := commitQC$.

%Note that $L_{v+1}$ propagates the commit QC to all replicas as part of its next special block proposal.\\

\subsection{View Change}
If replica $R$ does not receive a commit QC within its view $v$ timeout, it broadcasts a \textsc{Timeout} message to all replicas indicating it wishes to move to the next view. This \textsc{Timeout} message contains $v$, the current view number of replica $R$, $highPropose_R$, the highest (by view) \textsc{Propose} message $R$ received, and $QC_R$, the highest (by view) QC $R$ received.

\protocol{\underline{Step 5: $R$ to all} \\ Send \msg{Timeout}{v, highPropose_R, QC_R}}

Once a replica receives $n-f$ matching \textsc{Timeout} messages for view $v$, it forms a timeout certificate (TC), and forwards it to $L_{v+1}$, the leader of view $v+1$. Once $L_{v+1}$ receives the TC it proposes a new special block using the TC as its ticket.

\todo{"fix" view change/choice of who to forward Accept to (curr Leader, next Leader, all to all)}
((One weird thing: If Lv+1 was faulty, then this view change only moves v  to v+1, so its Lv+1 turn again... 
--> this is a result of the optimization that does not send Accepts back to Lv -- and then requires Lv to forward again (can do so inside its DAG, but must wait for physical round... The only way to keep the optimized latency without this view change issue is to use all to all communication for the vote step.)

%\par \textbf{Slow Path Commit.}\\
%$L_v$ waits for $n-f$ matching Accept messages with valid signatures, and assembles a commit QC containing these messages. $L_v$ then sends a \textsc{Commit} message containing the commit QC to all replicas.


\subsection{Commit Rules}
There are two ways a special block can be committed. Either 1) it is committed directly on the fast or slow path or 2) it is committed indirectly once a direct commit happens by examining the prior tickets. Once a special block is committed all of its causal history can be committed in some deterministic order. Normal blocks can only be committed as part of the causal history of a committed special block.

\par \textbf{Fast Direct Commit.} A block $B$ can be committed directly on the fast path if there are $n$ \msg{Vote}{H(B),true} messages.
\newline \newline
\protocol{$n$ \msg{Vote}{H(B),true} messages}

\par \textbf{Slow Direct Commit.} 
\newline \newline
\protocol{Upon receiving $n-f$ matching \msg{Accept}{H(B_r)}: \\ Send
$n-f$ matching \msg{Accept}{H(B_r)} to all $R$ (commit certificate)}

\par \textbf{Indirect Commit.} Once a replica $R$ directly commits a block $B_p$, it must go back and order previously proposed blocks that may have been committed by an honest replica. To do so, replica $R$ recursively considers all of the tickets starting with $B_p.ticket$. If the ticket is a TC, $R$ finds the highest DAG QC (by view) among the $n-f$ \textsc{Timeout} messages. $R$ also finds the highest (by view) special block which has $f+1$ matching votes for it. Let $v_d$ be the view of the highest DAG QC, and the corresponding block proposal $B_d$. Also let $v_p$ be the view of the highest special block with $f+1$ matching \textsc{Propose} messages $R$ commits the corresponding block to the higher of the two by pushing it onto a stack, and then repeats the process by considering that block's ticket. If the ticket is a commit QC rather than a TC, $R$ stops the indirect commit process and orders each block by stack order.

Tie together View Change msg in Block Protocol, and View Change indirect commit (below):
1. The next proposer of a special block only uses a view change quorum as a "ticket". 
2. Only once the chain extending the view change quorum is committed (next Commit-QC), then we need to inspect the VC quorum contents to decide what to indirectly commit.
\todo{Add some intuition/detail on view change correctness}

\par \textbf{View Change.}
Can indirectly commit via view change one next block reaches Commit QC -- thus guaranteeing that there will be no other extended view change quorum for the transition from $v$ to $v+1$ (i.e. the chain is durable). Note that a DAG-QC does not suffice. A different chain head might be committed, that does not include the view change quorum (thus one cannot preemptively commit it)\\
Can commit via view change, if one sees f+1 matching. (implies nothing else could be committed, thus safe to commit this value). If no such value exist, can commit some deterministic value ((Note: This must be signed by proposer. I.e. in signed view change message the replicas include a signed propose, instead of just the proposal. \\
Hierarchy: Pick highest view. If tie, break by DAG QC > f+1 propose > 1 propose. \\
Should be ok to just pick the highest view. Why: Because consensus is sequential, the next smaller view must be present in the previous CommitQC or ViewChange Quorum too. If the VC Quorum for v (moving to v+1) contains a proposal for view v, then this proposal must have referenced a CommitQC or VC-QC in v-1. That QC will guarantee that anything proposed in v-1 will be committed (and so on recursively.)
\todo{Add this single propose case to Indirect Commit Algorithm too?}



\subsection{Refinements}
\par \textbf{Special Block Extension Rule.} 
-- Talk a bit about the problem: if special block waits for edges, then it needs to wait for next physical round.
Instead of including $n-f$ edges, a special block need only extend $k \geq 1$ blocks, e.g. the proposers own prior block.
Note that edges can extend either special or normal blocks -- From the DAGs perspective there is no difference.



Before $L_v$ creates a special block it waits until the special block
rule is satisfied (see the special block rule paragraph for details).

\par \textbf{Special Block Proposal Rule.} To maximize DAG coverage (the amount
of new uncommitted blocks that are added), a leader waits until the special block
proposal rule is satisfied before proposing a new special block. This is to avoid
the case that special blocks only have a single edge to the previous special
block, which essentially degenerates to the throughput of a non-DAG BFT protocol.
Different rules will make different trade-offs, however, we propose a simple
rule that strikes a balance between latency and throughput. The rule requires
that a special block in round $r$ must have at least $n-f$ blocks in round $r-2$
and at least one block in round $r-1$ contained in its causal history. This
ensures that there is still sufficient coverage for throughput but not restrictive
enough that latency suffers from having to wait for $n-f$ blocks in round $r-1$.

\par \textbf{Fast Path.}
\todo{add fast path precise protocol details}
TODO: 
- wait for timeout for 3f+1; Confirm still sent Async in parallel
- View Change proof implication.


\begin{algorithm}
If you receive a Commit-QC for block B, then you may transitively commit all parents (in the consensus chain) of B without waiting for their Commit-QCs. Realistically, this will rarely/never happen, as consensus is sequential, and thus replicas will likely receive all CommitQC broadcasts in sequence. However, if channels are asynchronous, and a lagging replica receives a CommitQC far ahead of it's latest (i.e. all the intermediary ones are in flight but slow / were not sent by the leader, then this lagging replica can immediately commit the chain and catch up. 
\textbf{I would also add that this indirect commit is necessary for when there is a faulty
leader (not just when there is asynchrony/honest replica is slow)}
\caption{Indirect Commit}\label{commit:rule}
\begin{algorithmic}
\Event{Received Commit-QC($B$)}   \Comment{Direct Commit of Block $B$}
\State{$stack = \bot$}

\While{$B.v < v_c$} \Comment{$v_c$ is the view of the last committed block}
\If{$ B.\pi == Commit-QC_{B.v-1}$} \Comment{QC from previous view}
\State{$B'$ is a block s.t. $H(B')==B.\pi.H$}
\State{$stack.push(B')$}
\State{$B=B'$}
\Else \Comment{$B.\pi$ is View Change Quorum}
\State{$QC_h=$ highest (by view) DAG-QC contained in $B.\pi$}
\State{$B_w=$ highest (by view) block such that there exists $f+1$ 
\msg{Propose}{B'} messages in $B.\pi$, where $B'$ contains a 
\msg{Propose}{B} message in some ancestor block}

%\State{$sQC_h =$ $wQC_h$ highest (by view) \textsc{Propose} in $B.\pi$}


\State{$B_h=\bot$}
\If{$ QC_h.v \geq B_w.v$} %\land QC_h.v \geq sQC_h  $}
\State{$B_h$ is set s.t. $H(B_h)==QC_h.H$}
\Else
\State{$B_h$ is set to $B_w$}

\EndIf
\State{$stack.push(B_h)$}
\State{$B=B_h$}
\EndIf
\EndWhile

\While{$\neq stack.empty()$} \Comment{Iterate over committed special blocks}
\State{$B=stack.pop()$}
\State{Commit $B$'s causal history is some deterministic order}\Comment{Indirect commit}
\EndWhile

\EndEvent
\end{algorithmic}
\end{algorithm}





\iffalse
\subsection{Normal Block}

\par \textbf{Proposer Logic.} Let $P$ be the designated proposer of block $B_p$,
and $R$ the set of all replicas. To propose $B_p$, $P$ assembles a batch of client transactions
into $b_h$, and collects a set of $n-f$ $edges$: Each $edge$ is comprised of the hash $H(B')$ of a block $B'$ from round $r-1$, and it's associated $DAG-QC$ (see below). Note, that it is immaterial whether $B'$ is a "normal" or "special" block.
It signs $(r, edges, b_h)$ as $\sigma_p$. 

\protocol{\ul{Step 1: $P$ to all $R$} \\ Send \msg{Propose}{B_p} where 
$B_p=(r, edges, b_h, \sigma_p)$} 

\par \textbf{Replica Logic.} Upon receiving a Proposal for $B_p$, a replica $r$ checks the validity of $B_p$: It confirms the message proposal
is well-formed, it's signature is valid, that it contains $n-f$ edges to blocks in round $r-1$, and that it has received no previous Propose request from $P$ in round $r$. If $B_p$ is valid, $r$ signs $H(B_p)$ as $\sigma_r$ -- where $H$ is a collision resistant hash function. 

\protocol{\ul{Step 2: $R$ to $P$} \\ Send \msg{Vote}{H(B_p), \sigma_r}}

\par \textbf{Proposer Logic.} $P$ collects a set of $n-f$ valid \textsc{Vote} messages
for $H(B_p)$, and forms a quorum certificate $DAG-QC_p$ by aggregating all the \textsc{Vote}
signatures. % into $\sigma$.

\protocol{\ul{Step 3: $P$ to all $R$} \\ Send \msg{Confirm}{DAG-QC_p} where 
$DAG-QC_p=(H(B_p), \{\sigma_r\})$} 

\par \textbf{Replica Logic.} A
replica $r$ checks the validity of $DAG-QC_p$ and that it is well-formed (signature 
is an aggregation of $n-f$ distinct signatures, and are valid).
If $DAG-QC_p$ is valid, then it adds the certificate and corresponding block to its
DAG.

\subsection{Special Block}

\par \textbf{Leader Logic.} Let $L_v$ be the designated leader for the current
view, and $R$ be the set of all replicas. 
To propose a new Special Block $S_v$ $L_v$ must first collect either
\begin{enumerate}
    \item a $Commit-QC$ ($n-f$ matching \textsc{Accept} messages) for a special block $S_{v-1}$ in view $v-1$ or
    \item a $VC-QC$ ($n-f$ \textsc{NewView} messages) for view $v$
\end{enumerate}
and include it in $S_v$ as proof $\pi$.

$L_v$ then completes the block akin to a normal block: It assembles a batch of client transactions $b_h$,
and collects a set of $n-f$ edges to blocks in round $r-1$. It signs $S_v = (r, edges, b_h, v, \pi)$ as $\sigma_p$.\\

$S_v$ can be viewed/treated as a normal block $B$ that additionally has additional meta-data $v$ and $pi$ that indicates the block is special / carries consensus information. The Propose, Vote, and Confirm steps are mostly identical to the Normal Block processing, but additionally do some consensus related processing. For clarity, we outline the full processing (including redundancy) below. ==> TODO: Merge the description into one.


\protocol{\ul{Step 1: $L_v$ to all $R$} \\ Send \msg{Propose}{S_v} where 
$S_v=(r, edges, b_h, v, \pi, \sigma_p)$} 

\par \textbf{Replica Logic.} A
replica $r$ checks the validity of $S_v$ and that it is well-formed (signature is 
valid, $\pi$ contains a valid quorum certificate for a special block from view $v-1$
or $n-f$  \textsc{NewView} messages). If $S_v$ is valid, and $v > view_r$ then $r$ updates its local view $view_r := v$, and updates its local highest proposal to $p_r := S_v$. Additionally, if $S_v.\pi$ contains a $Commit-QC$ s.t. $Commit-QC.v > commit_r.v$ (i.e. larger than local highest qc), $r$ updates $commit_r := Commit-QC$. $r$ then resets its view timer, and signs $H(S_v)$ as $\sigma_r$.  ((Note to self: Our view change should be able to produce a Commit QC implicitly; i.e. a view change quorum that includes a block f+1 times in highest view $v$ implies commit(?)


\protocol{\ul{Step 2: $R$ to $L_v$} \\ Send \msg{Vote}{H(S_v), \sigma_r}}

\par \textbf{Leader Logic.} $L_v$ collects a set of $n-f$ \textsc{Vote} messages
for $H(B_v)$, and forms a quorum certificate $DAG-QC_{l_v}$ by aggregating all the 
\textsc{Vote} signatures. % into $\sigma$.

\protocol{\ul{Step 3: $L_v$ to all $R$} \\ Send \msg{Confirm}{DAG-QC_{l_v}} where 
$DAG-QC_{l_v}=(H(S_v), {\sigma_r})$} 

\par \textbf{Replica Logic.} A
replica $r$ checks the validity of $DAG-QC_{l_v}$ and that it is well-formed 
(signature formed from $2f+1$ valid signatures). If $DAG-QC_{l_v}$ is valid, then it 
updates its $qc_r$ to be $DAG-QC_{l_v}$, and signs $H(B_v)$ as $\sigma_r$.

\protocol{\ul{Step 4: $R$ to $L_v$} \\ Send \msg{Accept}{H(B_v), \sigma_r}}

\par \textbf{Leader Logic.} The leader waits for $n-f$ Accept messages with valid signatures, and aassembles a $Commit-QC_v = {H(S_v), {\sigma_r}$. 
It then broadcasts the $Commit-QC$ to all replicas. (Edit: This can be piggybacked on next Dag proposal).
Note, that with rotating leaders, Replicas may send the Accept to the next leader already.

\par \textbf{Replica Logic.} When a replica waiting for a $Commit-QC_v$ times out (timer expires) it 
collects $vp_r$ and $QC_r$ and sends a signed \textsc{NewView} message to the 
leader of view $v+1$. It includes its highest valid propose message $p_r$, and it's highest local $DAG-QC$ $qc_r$.

\protocol{\ul{Step 5: $R$ to $L_{v+1}$} \\ Send \msg{NewView}{v+1, p_r, qc_r}}


\begin{algorithm}
\caption{View Change}\label{commit:rule}
\begin{algorithmic}
\Event{Direct Commit of Block $B$)}  
\State{$stack = \bot$}

\While{$B.v < v_c$} \Comment{$v_c$ is the view of the last committed block}
\If{$|B.S| == 1$} \Comment{QC from previous view}
\State{$B'$ is a block s.t. $H(B')==B.S.H$}
\State{$stack.push(B')$}
\State{$B=B'$}
\Else
\State{$QC_h=$ highest QC (by view) contained within $B.S$}
\State{$wQC_h=$ highest (by view) set of $f+1$ matching \textsc{Vote1} messages within $B.S$}
\State{$B_h=\bot$}
\If{$QC_h.v \geq wQC_h.v$}
\State{$B_h$ is set s.t. $H(B_h)==QC_h.H$}
\Else
\State{$B_h$ is set s.t. $H(B_h)==wQC_h.H$}
\EndIf
\State{$stack.push(B_h)$}
\State{$B=B_h$}
\EndIf
\EndWhile

\While{$\neq stack.empty()$} \Comment{Iterate over committed special blocks}
\State{$B=stack.pop()$}
\State{Commit $B$'s causal history is some deterministic order}\Comment{Indirect commit}
\EndWhile

\EndEvent
\end{algorithmic}
\end{algorithm}


\fi

==> Sections/3-System/Sailfish_notes/pseudocode.tex <==
\section{Protocol Pseudocode}
\begin{figure*}
\fbox{\begin{minipage}{\linewidth}
\textbf{Normal Block Protocol:}
\begin{enumerate}
    \item \textbf{Propose}. Upon receiving $n-f$ blocks in DAG round $r$,
    set $r=r+1$, collect the hashes of $n-f$ blocks in round $r-1$ into
    $edges$, collect a batch of client transactions into $b_h$, and create a signature on $(r, edges, b_h)$ as $\sigma_p$.
    Multicast block $B_r=(r, edges, b_h, \sigma_p)$ to all replicas.
    \item \textbf{Vote}. Upon receiving a block $B_r$, check signature validity,
    and check that no other block from the proposer replica has been received in
    round $r_r$. If checks pass, send a \textsc{Resp}{($H(B_r)$, 
    $\sigma_i$)} to the proposer replica, where $H(B_r)$ is a hash of $B_r$, and 
    $\sigma_i$ is a signature on $H(B_r)$ message.
    \item \textbf{Certify}. Upon receiving $n-f$ \textsc{Resp}{($H(B_r)$)} 
    messages, form a certificate $C_r$ on $B_r$. Multicast $C_r$ to all replicas.
    \item \textbf{DAG}. Upon receiving a certificate $C_r$, add it to $DAG_i[r]$.
\end{enumerate}
\end{minipage}
}
\caption{\textbf{Protocol for a Normal Block}}
\label{fig:cert}
\end{figure*}

\begin{figure*}
\fbox{\begin{minipage}{\linewidth}
\textbf{Special Block Happy Path Protocol:}
\begin{enumerate}
    
    \item \textbf{Propose}. After committing block $B$ in view $v-1$,
    increment $r_r$, collect the hashes of $k \geq 1$ blocks in round $r_r-1$ into
    $edges$, collect a batch of client transactions into $b_h$, and create a signature on $(r_r, edges, b_h)$ as $\sigma_p$.
    Multicast special block $B_r=(r_r, edges, b_h, \sigma_p, v_r, C_{v-1})$ to all replicas.
    
    \item \textbf{Vote}. Upon receiving a special block $B_r$, check signature 
    validity of proposer, validate parent block certificate ($C_{v-1})$),
    and check that no other block from the proposer replica has been received in
    round $r_r$ and in view $v_r$. If all checks pass, send a \textsc{Vote-Resp-1}{($H(B_r)$, 
    $\sigma_i$)} to the proposer replica, where $H(B_r)$ is a hash of $B_r$, and 
    $\sigma_i$ is a signature on $H(B_r)$ message.
    
    \item \textbf{Certify}. Upon receiving $n-f$ \textsc{Vote-Resp-1}{($H(B_r)$)} 
    messages, form a certificate $C_r$ on $B_r$. Multicast $C_r$ to all replicas.
    
    \item \textbf{Fast Direct Commit}. If $n$ \textsc{Vote-Resp-1}{($H(B_r)$)} 
    messages are received, form a \textit{fast} commit certificate $CC_r$ on $B_r$
    and directly commit $B_r$.
    Forward $CC_r$ to all replicas.
    
    \item \textbf{Slow Path}. Upon receiving a valid certificate $C_r$, add
    it to $DAG_i[r]$ and send a \textsc{Vote-Resp-2}{($H(B_r)$)} to the leader.
    
    \item \textbf{Slow Direct Commit}. Upon receiving $n-f$ \textsc{Vote-Resp-2}{(H(B))} messages, form a commit certificate $C_v$ on $B$, and locally 
    directly commit $B$. Forward $C_v$ to all replicas. Replicas that receive $C_v$ commit B.
        
\end{enumerate}
\end{minipage}
}
\caption{\textbf{Fast View Change Protocol for a Special Block}}
\label{fig:cert}
\end{figure*}

\begin{figure*}
\fbox{\begin{minipage}{\linewidth}
\textbf{Special Block Sad Path Protocol:}
\begin{enumerate}

    \item \textbf{NewView}. Once the timeout expires without receiving a
    \textsc{Vote-Req} message for a special block in the current view, send
    a \textsc{NewView}{($v_R+1, vp1_R, vp2_R$)} message to the leader of view $v_R+1$,
    and increment $v_R$.
    
    \item \textbf{Propose}. After collecting $n-f$ valid \textsc{NewView} messages
    for the current view into $S$,
    increment $r_r$, collect the hashes of $k \geq 1$ blocks in round $r_r-1$ into
    $edges$, collect a batch of client transactions into $b_h$, and create a signature on $(r_r, edges, b_h)$ as $\sigma_p$.
    Multicast special block $B_r=(r_r, edges, b_h, \sigma_p, v_r, S)$ to all replicas.
    
    \item \textbf{Vote}. Upon receiving a special block $B_r$, check signature 
    validity of proposer, validate \textsc{NewView} messages are valid ($S$),
    and check that no other block from the proposer replica has been received in
    round $r_r$ and in view $v_r$. If all checks pass, send a \textsc{Vote-Resp-1}{($H(B_r)$, 
    $\sigma_i$)} to the proposer replica, where $H(B_r)$ is a hash of $B_r$, and 
    $\sigma_i$ is a signature on $H(B_r)$ message.
    
    \item \textbf{Certify}. Upon receiving $n-f$ \textsc{Vote-Resp-1}{($H(B_r)$)} 
    messages, form a certificate $C_r$ on $B_r$. Multicast $C_r$ to all replicas.
    
    \item \textbf{Fast Direct Commit}. If $n$ \textsc{Vote-Resp-1}{($H(B_r)$)} messages are
    received, form a \textit{fast} commit certificate $CC_r$ on $B_r$ and directly commit $B_r$.
    Forward $CC_r$ to all replicas.
    
    \item \textbf{Slow Path}. Upon receiving a valid certificate $C_r$, add
    it to $DAG_i[r]$ and send a \textsc{Vote-Resp-2}{($H(B_r)$)} to the leader.
    
    \item \textbf{Slow Direct Commit}. Upon receiving $n-f$ \textsc{Vote-Resp-2}{(H(B))} messages, form a commit certificate $C_v$ on $B$, and locally 
    directly commit $B$. Forward $C_v$ to all replicas. Replicas that receive $C_v$ commit B.
        
\end{enumerate}
\end{minipage}
}
\caption{\textbf{Slow View Change Protocol for a Special Block}}
\label{fig:cert}
\end{figure*}

\begin{figure*}
\fbox{\begin{minipage}{\linewidth}

\textbf{Indirect Commit Protocol:}

\begin{enumerate}
    \item \textbf{Initialize.} Create an empty stack.
    
    \item \textbf{Trigger.} Upon directly committing a special block $B$, check 
    whether $B.S \neq \bot$ or $B.C \neq \bot$.
    
    \item \textbf{$B.C \neq \bot$}. Let $B'$ be the block s.t. $H(B')=B.C.H$.
    Push $B'$ onto the stack, and set $B=B'$.
    
    \item \textbf{$B.S \neq \bot$}. Let $QC_h$ be the highest (by view) quorum
    certificate in $B.S$, and let $wQC_h$ be the highest set of $f+1$ matching
    $vp1_R$ messages for a special block in $B.S$. If $QC_h.v \geq wQC_h.v$, then
    set $B_h$ to be the block s.t. $H(B_h)=QC_h.H$. If $wQC_h.v < QC_h.v$, then
    set $B_h$ to be the block s.t. $H(B_h)=wQC_h.H$. Push $B_h$ onto the stack, 
    and set $B=B_h$.
    
    \item \textbf{Repeat.} Recursively go through this procedure until $B.v<v_c$,
    where $v_c$ is the view of the last committed block. Then update $v_c$ to be
    the view of the special block that was directly committed.
    
    \item \textbf{Indirect Commit.} Pop an element, $B$, off the stack. Commit
    all of $B$'s uncommitted causal history according to some deterministic 
    order. Repeat until the stack is empty.
\end{enumerate}
\end{minipage}
}
\caption{\textbf{Indirect Commit Protocol}}
\label{fig:cert}
\end{figure*}


==> Sections/3-System/Sailfish_notes/sailfish_protocol.tex <==
\section{Protocol}

In a Nutshell: We do virtual consensus on top of a physical DAG -- somewhat akin to doing a logical DAG atop a physical DAG (as explored in bullshark). We sidestep the weakness of waiting for next physical round via special rule.

We're sort of inbetween Fin and Narwahl-HS


\ia{my take:}

Virtual voting: consensus is done inside the DAG

Narwahl-HS: consensus is done outside the DAG

Our path: in between - the consensus is "taking control" of the DAG link and making it faster

\ia{goals theory:}

1. Like Fin, but make it formal: obtain asynchronous responsiveness  or responsive throughput: throughput moves at network speed (even in asynchrony), only latency needs GST. So this is a stengtherning  of responsiveness definition

2. After GST: get the best latency possible: 3 network delays to commit in slow path, 2 network delays to commit in fast path



- Next: Add 4 steps:
1) Conceptually, how we re-use the above multicast as first round of Consensus, and simply add a voting phase on top.
2) How we embed a Total order/Chain, by creating Special Blocks -- Abstractly, both DAG and Consensus can be viewed separately. Next special block cannot start before previous one has been "learned" (Sequential Consensus)
3) Add View Change
4) Add parallel Fast Path (does not affect view change)
- Add a figure that shows how our messages correspond to DAG and consensus.\\
%\includegraphics[width=0.8\textwidth]{figures/sailfish_high_level.png}

- Add a table comparing the end to end latency for client. Latency until Superblock that includes/extends + Latency of Consensus.

Refinements:
1) Special Block extension rule: Superblock doesn't need to have n-f edges --> Ensures we don't have to wait for next physical round. -- In theory, special blocks don't need to be part of DAG rounds at all, but we want this in an effort to minimize extra messages 
2) Refinement of extension rule: only extend blocks with enough edges. Ensures "coverage"  -- otherwise, super blocks could just extend themselves infinitely, degenerating back to a single chain 
3) Special Block learning rule (skip ahead rounds if last special block has higher): Ensures consensus progress ("no loss" of throughput; just means DAG is not fully oblivious to consensus)
4) Modularity: We picked Linear PBFT, but can make quadratic. Can use Hotstuff instead (3 rounds) if one wants linear VC. Can use single leader vs rotating. Can parallelize with single leader (though not really advantageous). Cannot pipeline.
5) Notes on orphans: Will be caught with rotation. Can propose older rounds if one wants; for simplicity of progress checks we don't
6) Garbage Collection: Can use simple Timeout mech like in Bullshark
7) Fairness


Talk about DAG committment procedure:
standard: commit special blocks causal history in order. Declare a deterministic order for everything in leaders causal history that is not already part of previous leaders commit (e.g. stop recursive branch extension if a node is already committed), and order this sequence AFTER the last committed leader
-- Note/Subtelty: DAG rounds do not imply a PO (only edges do). E.g. a node from Dag round 1 can be ordered for commit after Dag round 100, if there is no edge between them.


Analysis:
If Consensus as fast as DAG --> (almost) Every round is special block (==> every other block latest, using our tagging rule)
If Consensus slower/stopped due to async; DAG grows --> as soon as synchrony is back, next special block is at the tip of DAG
Overhead is just 1 signature per replica per special block round (minimal),
amortized it's basically as good as zero message


\subsection{Latency comparisons}
End-to-End Latency = Consensus Latency + 2md

Consensus Latencies:
Sailfish: 4md slow path, 2md fast path.    (If not using all to all, or rotating leader optimization, need 5md on slow path).
(can make fast path 1md, if we optimistically want to reply directly to the client, instead of the leader; but since we're doing consensus on batches (of batches) whose requests can be from different clients, it's much easier if leader manages this. + To reply, not only need the commit proof, but also the actual request result (which requires committing the DAG and executing first. How can one prove that the commitQC vouches for a result? -- it only vouches for an ordering committment)
        
Bullshark: 6md for even rounds, 9md for odd rounds ==> amortized = 15/2 = 7.5 rounds
Narwahl + BFT = 3md + BFT. E.g. Hotstuff = 3md + 6md = 9md; PBFT = 3md + 4md = 7md; Zyzzyva= 3md + 2 md   (maybe even just 1, if super clever and reply directly to client for quorum).

End-to-end: We can get about 2x over Bullshark/Narwahl-Hs

==> Sections/3-System/Sailfish_notes/system.tex <==
\section{System Overview}
\begin{itemize}
    \item Sailfish designed to be scalable, and have low latency
    \item Consists of two layers: data propagation, and consensus
\end{itemize}

\textbf{Data Propagation.} 
\begin{itemize}
    \item Like other approaches Sailfish decouples data dissemination from 
    consensus
    \item Data propagation layer provides an asynchronous, high throughput 
    substrate for disseminating transactions
    \item Each replica sequentially sends a batch of transactions, collects 
    a quorum of $n-f$ signed votes (a certificate), and sends next batch 
    containing certificate and a hash pointer to previous batch
    \item Forms $n$ parallel chains, one for each replica
    \item No timeouts making it asynchronous and responsive
    \item Certificates guarantee data availability and non-equivocation
\end{itemize}

\textbf{Consensus.} 
\begin{itemize}
    \item Partially synchronous, and guarantees total ordering
    \item Departs from other designs where blackbox consensus is separated 
    completely by running on top of data propagation layer
    \item Incurs high latency since data propagation layer is doing redundant 
    work with consensus
    \item Consensus is logically separated from data propagation but it reuses 
    the same physical messages as the data propagation layer
\end{itemize}

\textbf{Challenges.}
\begin{itemize}
    \item How to compose a partially synchronous consensus layer with a fully 
    asynchronous data propagation layer without making the data propagation 
    layer partially synchronous?
    \item How to ensure that a logical split between data propagation and 
    consensus doesn't mean that consensus has to synchronize with data 
    propagation?
    \item How to integrate an optimistic fast path for even faster latency 
    under no failures?
\end{itemize}

==> Sections/3-System/background.tex <==
\section{Background}

 \item Challenge \#1: Ensuring that a partially synchronous consensus protocol doesn't also cause data growth to be partially synchronous, violating asynchronous responsive throughput
    
%\includegraphics[width=\textwidth]{figures/lightningspeed.jpg}
\fs{describe Trad BFT or DAG more? don't think we really need to}

\fs{DAG background; old notes from sailfish}
\begin{itemize}

    \item There is an emerging class of BFT-SMR protocols that are DAG-based
    \item The DAG is an abstraction for reliable data dissemination that 
    provides high throughput but does not provide total ordering (An example is 
    Narwhal)
    \item A separate consensus protocol takes as input the DAG and outputs a 
    total ordering over those blocks (An example is Tusk)
    \item DAG BFT Protocols are known to have high throughput but also high latency
    \item The high throughput is largely a result of a DAG design like Narwhal, which does reliable 
    data dissemination in parallel, while also continuing to grow during asynchronous periods
    \item We formalize this notion with a property called asynchronous responsive throughput
    \item The high latency is largely a result of most of these protocols being "zero-message" 
    overhead, (Tusk, DAG-Rider, Bullshark, Fino, Shoal etc.), which require multiple 
    instances of RB to commit a single block.
\end{itemize}



\begin{definition} (Asynchronous Responsive Throughput.)

\end{definition}

%DAGs are for high throughput.
%Emphasize zero message overhead consensus as feature.
%Advertise lack of view change + pacemaker as feature.
%Neglect commit latency in the process. 
%--> E.g. either layer consensus atop separately (high latency, not "free" overhead); or use async randomized consensus embedded
% --> Bullshark tries to improve it by using pre-determined leaders, and waiting on timeouts
%     --> Latency still high: 2 full rounds; latency "starts" only every other round; latency not responsive (uses timeouts)

%Our pitch:
%- Latency of traditional agreement
%- Responsive
%- Async responsive throughput: Consensus only with partial sync, but Dag grows while async ==> when Consensus recovers, directly commit tip of DAG
%- Add minimal redundant messages

%Tradeoff: Prioritize latency
%- only vote messages are extra
%- we need view change + pacemaker (arguably most complex part of consensus engine)


\subsection{Characterizing prior DAG protocols}
\begin{itemize}
    \item We characterize prior work into two categories: protocols that have 
    zero message overhead and those that don't, and whether consensus is 
    logically independent of the DAG
    \item Zero message overhead pros: high throughput, no view change or view 
    synchronization mechanism. cons: latency is high since commitment requires 
    at least 2 full rounds of reliable broadcast, which itself takes at least 
    three rounds
    \item Consensus logically independent of DAG, pros: consensus is not blocked 
    if the DAG is slow, high throughput. cons: tail latency can be high since dependent on DAG for 
    piggybacking consensus messages
\end{itemize}


%Normal Consensus:\\
%PBFT, Hotstuff \\

%DAG Consensus\\
%- Narwahl https://arxiv.org/pdf/2105.11827.pdf \\
%- Bullshark https://arxiv.org/pdf/2201.05677.pdf  \\
%- Partial Sync Bullshark  https://arxiv.org/pdf/2209.05633.pdf \\
%- Fin/Fino:https://blog.chain.link/bft-on-a-dag/  , https://arxiv.org/pdf/2208.00940.pdf  \\ 
%- DAG-Rider https://arxiv.org/pdf/2102.08325.pdf \\

%- Cordial Miners https://arxiv.org/pdf/2205.09174.pdf \\
%- Aleph https://arxiv.org/pdf/1908.05156.pdf \\
%- Swirlds Hashgraph https://www.swirlds.com/downloads/SWIRLDS-TR-2016-01.pdf \\
%- Blockmania https://arxiv.org/abs/1809.01620 \\

%Parallel Chains \\
%Dashing and Star: https://eprint.iacr.org/2022/625.pdf 
   %  --> older version with parallel BFT + fast path: https://eprint.iacr.org/archive/2022/625/1653294713.pdf

==> Sections/4-Evaluation/calculations.tex <==
Async experiments

Autobahn with 30 sec async window:
210k txn/s input rate * 30 sec = 6.3 million txn backlog
last committed slot before async car heights:
196, 343, 196, 656
first prepare after async car heights:
536, 1116, 524, 1719
in total 2504 new cars are proposed
on average each car contains 2.5 payloads of 1000k txns = 6.26 million txns 
committed after just a single slot, which is roughly the size of the backlog

==> Sections/5-RelatedWork/related-not-shortened.tex <==
\section{Related Work - unshortened}
\label{sec:related}

\fs{Let's talk in the CR also about the value of our flexible proposal speed. Traditional BFT *allows* only the leader to propose. DAG protocols *force* everybody to propose; that might not always be good. Dahlia's new work: https://eprint.iacr.org/2024/923 argues to let people propose accordingly to their speed -- but it's a ticketing based design. OURS achieves it *organically*. We allow everyone to propose as much or little as they can! (Lane Coverage can simply be tuned) }
% \nc{General question: do we want to cite protocols that have been released on Arxiv only? (Shoal, Mystecityi, BBCA. I also don't think STAR has been published anywhere yet}\fs{I don't feel strongly about that. For OSDI submission I'd say we can remove them if you prefer; but for arxiv/public version I think it makes us look more serious} 

\sys{} draws inspiration from several existing works. Scalog~\cite{ding2020scalog} demonstrates how to separate data dissemination from ordering to scale throughput at low latencies (for crash failures); akin to \sys{}'s lanes, Scalog disseminates data, and reaches consensus on cuts of independent log segments. Narwhal~\cite{danezis2022narwhal} discusses how to implement a scalable and BFT robust asynchronous broadcast layer, a core tenet for achieving seamlessness. \sys{} shares the spirit of layering consensus over asynchronous dissemination, but improves efficiency at both levels. \sys{}'s consensus itself is closely rooted in traditional, latency-optimal BFT-protocols, most notably PBFT's core consensus logic and parallelism~\cite{castro1999pbft}, Zyzzyva's fast path~\cite{kotla10zyzzyva, gueta2019sbft}, and Aardvark's doctrine of robustness~\cite{aardvark}. 

\par \textbf{Motorizing Consensus Protocols.} We note that \sys{}'s architecture, by design, isn't tied to a specific consensus mechanism, and thus can easily accommodate future algorithmic improvements (including advances in asynchronous protocols).
Furthermore, existing consensus deployments may easily be \textit{motorized} to enjoy both improved throughput and seamlessness without adopting the custom consensus protocol described in \sys{}: a blackbox consensus mechanism of choice may be augmented by adding lanes, replacing consensus proposals with cuts, and adopting the synchronization and ordering logic presented.

%\fs{cut:} Finally, \sys{} draws on Shoal~\cite{spiegelman2023shoal} and Carousel~\cite{carousel} for inspiration on reputation-schemes \fs{to enable optimistc tips}.

%a BFT way that is robust to async -- Dags sync on history before voting. (2f+1 sync on 2f+1). (For us f+1 sync on n; later we propose n -- no orphans by design.)


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Psync protocols
\subsection{Partially synchronous BFT consensus}

%%Traditional
\par \textbf{Traditional BFT} protocols such as PBFT~\cite{castro1999pbft}, HotStuff~\cite{yin2019hotstuff}, and their respective variants~\cite{kotla10zyzzyva, gueta2019sbft}\cite{jalalzai2020fasthotstuff, jolteon-ditto}
optimize for good intervals: they minimize latency in the common (synchronous) case, but guarantee neither progress during periods of asynchrony\fs{blips? Here it seem correct/find to just say asynchrony.}, nor resilience to asynchrony hangovers.\fs{exact latencies in comment:}
%\fs{(5md (linear)/3md (all) PBFT, 2md (fast)/ 5md (slow) Zyzzyva, 5md? Jolteon, 7md Hotstuff) +2 for all end to end (only +1 zyzzyva because reply goes to client). say \sys follows same?}
%Unfortunately, this class of protocols is prone to asynchrony hangovers. %This is because request batches are only disseminated alongside consensus proposals; backlogs generated during asynchrony must be "worked off" over time by increasing batch sizes. %after even a brief period of asynchrony, such protocols do not gracefully resume operation processing once synchrony returns.

Protocols in this class employ a dedicated (single) leader that disseminates data and drives agreement in the classic \textsc{Prepare}/\textsc{Confirm} pattern adopted by \sys{}.
PBFT~\cite{castro1999pbft} rotates leaders only in presence of faults (or asynchrony), and allows a stable leader to drive consensus for multiple slots in parallel. HotStuff~\cite{yin2019hotstuff} rotates leaders for every proposal, but pipelines consecutive consensus phases to reduce latency and share signature costs. \sys{} incorporates features of both approaches: it allows parallel proposals for minimal latency, \changebars{and}{} rotates leaders eagerly for fairness and robustness~\cite{aardvark}\changebars{.}{, and is amenable to ride sharing for optimal resource efficiency.}\fs{feel free to cut; I think "amenable" is fair wording}

%(proposal bandwidth is limited to one replica)
\par \textbf{Multi-log frameworks}~\cite{stathakopoulou2019mir, stathakopoulou2022state, gupta2021rcc, arun2022scalable}  partition the request space across multiple proposers to sidestep a perceived leader bottleneck. They carefully orchestrate traditional BFT instances in parallel, and intertwine their logs to arrive at a single, total order. %Doing so demands careful and complex orchestration, and can result in suboptimal performance in the presence of faults.
Multi-log frameworks inherit both the good and the bad of their BFT building blocks: consensus has low latency, but remains prone to hangovers. %\fs{alt: \textit{network robustness remains poor}.} 

\par \textbf{Directed Acyclic Graph (DAG) BFT}, a new class of BFT protocols \cite{baird2016swirlds, keidar2021all, danezis2022narwhal, malkhi2022maximal, Bullshark} originate in the asynchronous model and enjoy both excellent throughput and network resilience; recent designs \cite{spiegelman2022bullshark, spiegelman2023shoal, keidar2023cordial} make use of partial synchrony to improve consensus latency. 
DAG protocols employ a highly parallel asynchronous data dissemination layer that proceeds through a series of structured, tightly synchronized rounds. Each proposal references $n-f$ proposals in the prior round, forming a DAG of causally related, data proposals. Consensus uses this structure as a common clock, and is embedded with no message overhead~\cite{Bullshark}: in every other round, the consensus protocol \textit{interprets} the DAG structure to identify a leader node, and constructs an ordered log by committing and flattening the leader's topological (or \textit{causal}) history in the DAG.
% However, while asynchronous consensus protocols make progress consistently, they do so at a higher, often prohibitive latency; consequently, these protocols see little practical adoption. Recent DAG protocols \cite{spiegelman2022bullshark, spiegelman2023shoal, keidar2023cordial} make use of partial synchrony to improve consensus latency (data dissemination remains asynchronous). 
%-- the DAG grows asynchronously, and replicas need not block in order to synchronize on missing data--,
\textit{Certified} DAGs are close to achieving seamlessness (data synchronization on the timeout-critical path aside) but use Reliable Broadcast~\cite{bracha1985asynchronous} (RB) to implement the voting steps of traditional BFT consensus, resulting in high latencies. Bullshark~\cite{spiegelman2022bullshark}, for instance, alternates between (even) rounds (of RB) with a leader, and odd rounds without. It requires 2 rounds of RB (3md per RB) to commit leader blocks and up to 4 round for non-leader blocks leader rounds, for a worst case total latency of 12 md. Shoal~\cite{spiegelman2023shoal} optimizes latency to 9md by increasing leader frequency to every round.

%requires \changebars{12md to commit (9md when optimized by Shoal~\cite{spiegelman2023shoal}}{between 3 and 4 rounds of RB (3 when optimized by Shoal~\cite{spiegelman2023shoal})}. %exhibiting an average case consensus latency of 9 message exchanges.
%\fs{Note: the implementation's actually do block to synchronize; in a way, this implements the FIFO requirement required to let other replicas catch up fast. But because dag growth and consensus are intertwined it is implicitly on the critical path of consensus.}

% . Concretely: Bullshark alternates between (even) rounds with a leader, and odd rounds without. It requires 2 rounds to commit leader blocks; 3 rounds to commit blocks in non-leader (odd) rounds; and 4 round for non-leader blocks in (even) leader rounds, for a worst case total of 4 * 3 md. We will add back additional details about DAG protocols and related work, currently in our supplementary material.



\fs{Added bbca-chain because it is now published at FC.}
\changebars{Recent works propose (but do not empirically evaluate) un-certified DAGs~\cite{keidar2023cordial, malkhi2024bbca}. These designs aim to improve latency by replacing the RB in each round with best-effort-broadcast (BEB), but forgo seamlessness because they must synchronize (possibly recursively) on missing data before voting.}{}
Cordial Miners~\cite{keidar2023cordial} matches PBFT's latency in gracious intervals, but to guarantee progress must wait in each round (up to a timer) for a message from the leader. BBCA-chain~\cite{malkhi2024bbca} modifies Bullshark by weakening non-leader proposals to BEB, and strengthening leader proposals to single-shot PBFT instances; it chains these instances via a ticket-based design akin to \sys{} but is subject to up to 2x sequential consensus latency (\S\ref{sec:parallel}).

% \fs{Added bbca-chain because it is now published at FC.}
% \changebars{A few recent works propose (but have not empirically evaluated) un-certified DAGs; these designs aim to improve latency, but forgo seamlessness because they must synchronize (possibly recursively) on missing data before voting. Cordial Miners~\cite{keidar2023cordial} replaces the RB in each round with best-effort-broadcast (BEB), allowing it to match PBFT's latency in gracious intervals; to guarantee progress, however, it must wait in each round (up to a timer) for a message from the leader. BBCA-chain~\cite{malkhi2024bbca} modifies Bullshark by weakening non-leader proposals to BEB, and strengthening leader proposals to single-shot PBFT instances; it chains these instances via a ticket-based design akin to \sys{} but is subject to up to 2x sequential consensus latency (\S\ref{sec:parallel}).}{OLD (only cordial) IN COMMENTS}
%A recent work, Cordial Miners~\cite{keidar2023cordial} proposes instead an un-certified DAG, which improves latency, but forgoes seamlessness. It replaces the RB in each round with best-effort-broadcast, allowing it to match PBFT's latency in gracious intervals; to guarantee progress, however, it must wait in each round (up to a timer) for a message from the leader, and synchronize on missing data before voting.

% Several un-certified DAGs have been proposed recently; these designs improve latency, but forgo seamlessness. Cordial Miners~\cite{keidar2023cordial} uses best-effort-broadcast (BEB) rounds (instead of RB), matching PBFT's latency at the cost of 
% introducing a timer-constraint for advancing rounds and ensuring progress. \la{This "timing constraint" is a bit mysterious.}  % \fs{they wait a timeout to see the leader -- this "materializes" the pbft on the Dag}

% \fs{Mysticeti and BBCA are arxiv only} \la{If we are tight in space, I would remove them}\nc{I also would remove them - at least in the non arxiv version}
% Mysticeti-C~\cite{babel2023mysticeti}) extends Cordial Miners by optimizing non-leader block latencies via pipelining and a more robust commit rule. BBCA-chain modifies Bullshark by weakening non-leader proposals to BEB, and strengthening leader proposals to single-shot PBFT instances; it chains these instances via a ticket-based design akin to \sys{} but is subject to up to 2x sequential consensus latency (\S\ref{sec:parallel}). 


\par \textbf{DAG vs Lanes}. Lanes in \sys{} loosely resemble the DAG structure, but minimize quorum sizes and eschew rigid dependencies across proposers. 
%, and propose requests on behalf of their entity (with varying loads)~\cite{liu2023flexible}.
DAGs must operate at the proposal rate of the $n-f'th$ fastest (i.e. slowest correct, in presence of faults), while \sys{}'s independent lanes allow for flexible proposal rates (each replica can propose at their load and resource capability); this is desirable in modern permissioned blockchains, where replicas might be operated by heterogeneous entities (with varying resource capacities)~\cite{liu2023flexible}. 
Notably, \sys{} proposes a cut of all $n$ replica lanes; in contrast, DAGs can reliably advance proposals simultaneously from only $n-f$ replicas, and are thus subject to orphaning some proposals~\cite{Bullshark}. \fs{DAGs bigger quorums also increase tail latencies and make it less robust to partitions?}


%\nc{Cutting for space} Sonic~\cite{duan2022dashing} adopts a construction similar to \sys{}. It uses $n$ parallel proposers that create "weak-certificates" that only prove availability (equivalent to PoA), but retains a rigid round-based DAG-like construction. For \textit{each} round it requires an external single-shot PBFT instance that commits $n-f$ weak-certificates; this design is prone to asynchrony hangovers as the number of required consensus instances is directly proportional to duration of asynchrony. 

% Star~\cite{duan2022dashing} adopts a construction similar to \sys{}; it uses  "weak-certificates" ($f+1$) \fs{instead of RB} that only prove availability -- very much akin to PoA's in \sys{}. It retains a round-based DAG construction, but for each round, requires an external single-shot PBFT instance to reach consensus. 
% \fs{I'd cut this actually. They removed this from their public version: }Like \sys{}, it allows consensus instances to operate in parallel; in the worst case, however, an arbitrary amount of instances may open (in the order of async duration), all of which must commit before resuming gracefully.

% \neil{It feels a bit weird to me to classify Star as a Dag protocol since it doesn't have edges in the traditional sense. Could we just keep the part that says it takes inspiration from Dags by using an epoch/round based structure and it separates data dissemination from consensus but uses PoA and PBFT.} 
% \fs{I see your point. They do wait for n-f to advance round, they just don't explicitly reference them. That's because it's not necessary.}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% async protocols
\subsection{Asynchronous BFT consensus}
%\fs{Personally I want to talk about async protocol as little as possible...}
Asynchronous BFT~\cite{vaba, danezis2022narwhal, jolteon-ditto, liu2023flexible, honeybadger} protocols sidestep the FLP impossibility result~\cite{fischer1985impossibility} and guarantee liveness even during asynchrony by introducing randomization. 
They typically use a combination of reliable broadcast (RBC)~\cite{bracha1987asynchronous} and asynchronous Byzantine Agreement, either Binary BBA~\cite{bracha1987asynchronous, mostefaoui2014signature, abraham2022efficient, cachin2000random} or Multi-Valued (MVBA)~\cite{vaba, cachin2001secure}, to implement asynchronous Byzantine atomic broadcast (BAB)~\cite{honeybadger, beat, gao2022dumbo}.
%They typically avoid a using a single predetermined leader to dictate a proposal, and instead generate shared common coins using asynchronous Byzantine Agreement, either Binary (BBA)~\cite{bracha1987asynchronous, mostefaoui2014signature, abraham2022efficient, cachin2000random} or Multi-Valued (MVBA)~\cite{vaba, cachin2001secure}, to determine a single winning proposal.} 
Unfortunately, these protocols require expensive cryptography and (in the worst case) tens of rounds of message exchanges, resulting in impractical latency.\fs{(Threshold-signatures (for coin generation) and -encryption (to handle network adversary))} \neil{complexity measures for single-shot async (mvba) in message delays: vaba - 13-19.5 md, dumbo mvba 19-47 md, speeding dumbo 6-12 md. For multi-shot need to add in 3 md for RB in beginning}
%VABA~\cite{vaba} aims to minimize overall message complexity, and generates a shared coin from $n$ consensus instances using Threshold Signatures in only $O(n^2)$ messages.
The asynchronous systems closest related to \sys{} are Honeybadger~\cite{honeybadger} and Dumbo-NG~\cite{gao2022dumbo}. 
Honeybadger~\cite{honeybadger} achieves high throughput by operating $n$ instances of Reliable Broadcast (RB) in parallel and trading off latency for large batch sizes; it uses $n$ BBA instances to select $n-f$ proposals that may commit. Dumbo-NG~\cite{gao2022dumbo} separates data dissemination from consensus to ameliorate batching/latency trade-offs. It constructs parallel chains of RB and layers a sequential multi-shot MVBA protocol atop; this architecture closely resembles the spirit of \sys{}, but incurs significantly higher latency.\fs{which proposes cuts of RB certificates}

\iffalse
%\neil{while a single BA instance takes expected constant rounds to complete, running n instances results in expected log(n) rounds to complete};
\la{The next paragraph seem to go into really aficionado-level details, but if you think they are important to satisfy some referees... I was already game with ignoring these protocols after you mentioned those latency figures. But the details certainly show your mastery of the literature, oh mighty Neil and Florian duo.}
Honeybadger~\cite{honeybadger} achieves high throughput by operating $n$ instances of Reliable Broadcast (RB) in parallel, and trades off latency further in favor of large batch sizes. \la{Is the following sentence (just before Dumbo) necessary?} It uses $n$ BBA instances to select $n-f$ proposals that may commit; Dumbo~\cite{guo2020dumbo} improves message complexity by using a single MVBA instance instead. Dumbo-NG~\cite{gao2022dumbo} separates data dissemination from consensus to ameliorate batching/latency trade-offs. It constructs parallel chains of RB and layers a sequential multi-shot MVBA protocol atop \fs{which proposes cuts of RB certificates}; this architecture closely resembles the spirit of \sys{}, but incurs significantly higher latency. \fs{some more comparison details in comments}
% Dumbo-NG follows a similar structure as Autobahn lanes but they only 1) use n-f quorums for all reliable broadcasts 2) only use an external blackbox MVBA protocol for agreement on cuts, which they do not piggyback on the data lane messages 3) only use certified cuts for consensus, and 4) don't use pipelined consensus to reduce end-to-end latency

%\neil{add ACE (abstract consensus encapsulation)?}

Tusk~\cite{danezis2022narwhal} avoids blackbox BBA/MVBA protocols, and instead constructs a DAG using Narwhal~\cite{danezis2022narwhal} whose structure it interprets to derive a common coin; this requires an expected 4.5 rounds of RB. %\neil{A common coin can be generated by a single dag round, so would change the wording slightly}

Ditto~\cite{jolteon-ditto} and Bullshark~\cite{Bullshark} improve the common-case performance of asynchronous protocols by, respectively, augmenting a 2-round-HotStuff variant to use MVBA only as a fallback, and introducing a partially synchronous fast path (2 rounds of RB) to Tusk. However, these protocols must explicitly switch between modes of operation (to ensure that at most one commits), and may not gracefully respond to changing network conditions. \fs{Ditto hastily switches to the optimistic path, while Bullshark remains in one mode for several rounds (responds sluggishly)}

%\fs{WHAT is the downside here? Switchover time?}\neil{yes and that Ditto hastily switches back to the optimistic path if it commits on the fallback even if the network is async}
% Bullshark~\cite{Bullshark} improves consensus latency in Tusk for the common (synchonous) case by introducing a partially synchronous fast path (2 rounds of RB) but must explicitly switch between modes of operation to ensure that at most one mode commits; it must remain in one mode for several rounds, and thus may respond to changing network conditions sluggishly (e.g. operate asynchronously after return of synchrony, and vice versa). %\fs{TODO: if you want can mention other hybrid designs that require BA to reconcile parallel modes. Some notes in comments below.}

%\neil{orthogonal but any reason why you didn't put these paragraphs on Tusk, Narwhal, and Bullshark in the DAG-BFT subsection?}
MyTumbler~\cite{liu2023flexible} targets low latency for heterogeneous participants by leveraging a combination of Timestamp-based parallel consensus, and BA with a fast path for good intervals (SuperMA). %\neil{I would say the fast path is not about synchrony (since there isn't timeouts) but rather about whether there are any failures or not. The RBC will succeed and everybody will reach agreement and terminate if the proposer/leader is honest, otherwise a binary agreement protocol is needed if there are failures} 
Like \sys{}, it allows for flexible proposal speeds, but requires trading off latency and throughput by tuning the pace at which consensus terminates; notably, each proposal requires its own consensus instance, while \sys{} requires only one per cut. \sys{} could, like SuperMA, be augmented with an asynchronous fallback---we leave such exploration to future work.
%istances become stable \fs{subject to aborting}

% \sys{} consensus too could be augmented with an asynchronous fallback path akin to SuperMA. We chose against it due to the increased protocol complexity, and the risk of entering a slow asynchronous path when a single view change may suffice (e.g. when narrowly failing a system-set timeout).  %efficiency concerns (communication cost $O(n^3)$
\fs{SuperMA details in comment} 
%SuperMA operates in three speed-tiers--it returns if a tier commits, and moves to the next otherwise: \one a best-effort PBFT-style agreement round (no view-changes), followed by \two a randomized binary agreement protocol which under optimistic conditions can terminate without generating a common coin, and finally \three a classic common coin generation. 
%\neil{I would phrase this differently: i) a Bracha style RBC protocol (to differentiate it from the full consensus that PBFT guarantees with view change)} %ii) a randomized binary agreement protocol which under optimistic conditions can terminate without generating a common coin (the common coin and coin skipping steps are apart of the binary agreement)

\fi

% \fs{In ADDITION \sys also allows for parallel proposals, but that's a latency optimization}
% Unlike MyTumbler's TS based mechanism is not subject to any proposals aborting.
% \sys also has tuneable coverage, which can help configure chain quality (MyTumbler proceeds as soon as theres one new proposal)
%\sys{} instead can support flexible proposal capacities via the independent data lanes (replicas can go as fast or slow as they want) -- we have to tradeoff coverage for latency though.\fs{there's no free wins here, one must always tradeoff between lat and tput/effifiency/redundancy in some manner when having replicas of different proposal speeds}


% \par \textbf{Hybrid designs} strive to combine the best of both asynchronous and partially synchronous consensus protocols. However, such designs introduce complexity, and can, in practice, be prone to performing suboptimally in either setting.
% Bullshark~\cite{Bullshark} improves consensus latency for the common (synchonous) case by introducing a partially synchronous fast path but must explicitly switch between modes of operation and remain in them for several rounds; consequently it may respond to changing network conditions sluggishly (e.g. operate asynchronously after return of synchrony, and vice versa). 




% HoneyBadgerBFT family of protocols construct an atomic broadcast protocol by having each node reliably broadcast their input (for a total of n instances of reliable broadcast running in parallel), and then running n corresponding binary agreements to determine which reliable broadcast outputs to deliver. The Dumbo family replaces the n binary agreement instances with just a single multi-valued byzantine agreement that determines a set of at least n-f reliable broadcast outputs to deliver.
 

% \subsection{Hybrid Psync/Async BFT consensus}
%  - two protocol modes, or an async "fallback"

% MyTumbler:
% - could end up in async fallback even though we just had a too aggressive timeout: It would be enough to view change and re-propose on sync with slightly bigger timeout. Instead we go async path, which can take a while in the worst case -> other slots are then forced to wait too.

%  Bullshark:
% - psync fast path
% - async slow path
% - once you switch to steady state/fallback for a wave -> cannot switch back in the middle of wave => loses 4 rounds.
%     - e.g. if everybody commits in the async path, then everybody will be in steady mode for the next 4 rounds, and it's not possible to commit in the fallback until the next wave.
%     - if nobody commits on the fallback path, then replicas enter fallback mode again (even though network may now be sync). Thus one is missing out on the better latency one could get.

%  ParBFT:
%  - run psync and async path in parallel. 
%  - requires binary agreement to choose between both outputs.

% Pro:
% - in theory, best of both worlds

% Con:
% - complex
% - in practice: may switch too late to psync optimistic mode when network becomes sync => results in longer recovery time (higher end to end latency) than necessary (from staying in async pessimistic mode). 
% - running both paths in parallel is redundant work, that is often wasteful. requires to run BA to agree between both results (this adds extra latency)


% these protocols can switch too late




%%%%%%%%%%%%%%%%%%%%%%%%%%% Notes: %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% A recent class of DAG-based BFT protocols achieves both high throughput and seamlessness by leveraging a highly parallel asynchronous data dissemination as protocol backbone. They then either layer a separate consensus on top (Hotstuff over Narwhal) or embedd it on the DAG by interpreting the structure (Bullshark, Fin, Shoal). DAGs basically constantly view change -- they leverage the DAG structure as "clock" that drives consensus.
% In addition to the rigid round structure Bullshark requires a timeout in each round for progress. This doesn't affect tput because data layer keeps growing at the worker layer, but impacts latency (makes it non-responsive)

% \sys{} in spirit is very similar to NarwhalHS, but improves effifiency at all levels: break up Dag structure, cheaper RBS, propose tips directly (instead of one cert that points to parents) -- this saves 1 RB latency), use faster consensus, pipeline consensus, share messages. \fs{I'm not really happy with the realization that we are so similar in spirit, like a NarwhalHS 2.0 -- it makes us feel less innovative, even though it's kind of a coincidence that we ended up back here}

% Shoal inherits the foundation of Bullshark (same DAG structure and consensus) but leverages a relay/pipelining of consensus instances to reduce worst case latency compared to bullshark- its a re-interpretation of the schedule really. Latency is still high though (6md for leaders, 9 md for non leaders -- vs our 5 for leaders, 8 for non (slow); 3/5 (fast); 2/3 (all-to-all)
% Shoal additionally employs a reputation scheme (taken from Carousel) to favor leaders with better connectivity and reliability -- this allows them to get rid off timeouts, which makes the protocol quite elegant.
% Reputation schemes are orthogonal to our design, and could be integrated too to improve leader selection (however, we have to keep timeouts because consensus on its own has no "engine".)


%Dashing and Star
% Quite similar to ours. But: rigid rounds; no fast path; no pipelining
% - pbft per round (can be in parallel per round). Proposes 2f+1 certs (we can do up to n new)
% - each round does PoA with f+1 like we do; but rounds are rigid (wait for 2f+1 from prev round)
% - bad: if async, can have infinite consensus instances running. need to wait for all of them to finish before we are caught up. (we can catch up on the entire async backlog with one consnesus instance instead)


% TODO: mention cordial miners \cite{keidar2023cordial}
% - DAG without certification in each round. 
% - basically pbft embedded onto the DAG. Use timeout to make the embedding "visible"
% - need timeout in leader round + next round to guarantee progress. 
% - Latency: 4.5md expected. Async version too: needs more RTs 
% TODO: Mysticeti extends the cordial miners protocol with pipelining (to reduce non-leader latencies), and backup leaders to make committment more robust to crash faults.
% It runs in lockstep, and is not seamless(?) -> may have to sync on edges of proposal before voting (byz replica can force you to sync arbitrarily long)


% \fs{mention BBCA or not? }
% \nc{I would say concurrent unpublished work}
% A recent work BBCA-Chain proposes a rough design (has no implementation) that is similar to our Motorway one. It uses a DAG backbone, but turns some nodes into single-shot pbft instances (they call these "BBCA" \fs{so dumb}), and all others into best effort broadcast. Consequently, it is not seamless: Have to possibly sync on the critical path.
% Furthermore it has no fast path (they just use a bare single-shot pbft instance that they rename to "BBCA") and no pipelining. In the worst case, their end-to-end latency is 2x consensus.



%%%%%%%%%%%%%%%%%%%%%
\iffalse

BBCA-chain is similar, concurrent work:
- however, they use BEB, which places sync on critical path (makes for bad recovery)
- they use only sequential consensus, which can have high end-to-end latency for proposals that miss the bus (no better than normal Dag!)
- they don't have FP
- they don't pipeline backbone blocks (related to high sequential latency) => FS: don't think this matters: they use BeB so there's nothing to pipeline...
- DAG rounds are slowed down by backbone block (data dissemination slowed down) -- I don't think this matters much though, it stays async. I think the egregious part is that their "DAG" layer has lost all robustness / async benefit
-yeah I was confused because I originally thought non-backbone blocks had edges but now looking at the diagram they may not have edges? -> It's just underspecified since they didn't build anything.  Even if they do have edges, since they are not certified, it doesn't give you a "quick" commit upon recovery. You have to sync on anything a byz leader references before being able to vote. ((NOTE: you still need to sync on everything to be able to execute in our case too...) But voting sync is sequential: You need to sync on the latest, and then its parent, and then ... (unless you include EVERYTHING new in each proposal -- we just keep it small by making it just the tip)
-> yeah agreed with everything regarding sync, still think they didn't carefully think it through because for sailfish we had a way for consensus to output certified blocks to the dag layer so that the anchor block wouldn't dominate the dag round latency, whereas they may always have to wait 5 md to go to the next dag round


Note: refuse to call it BBCA -- say one-shot PBFT. Probing = view change messages
they also make it seem like BBCA and CBC are just as expensive but BBCA is 5 md whereas CBC is 3 md (linear). Yeah, they compare all-to-all to linear. So much for linearity ;) lol "BBCA, a lightly modified
Byzantine Consistent Broadcast (CBC) primitive" -> should've said pbft here instead of cbc

similarities: 
- ticket based approach -- theirs is our naive version
    - view change 

other differences :
- their VC quorum is taken as 2f+1 edges   
- ours it taken just as a Quorum (2f+1 cars received)

Note:
- we could also do all to all if we want for consensus.
- if we want all to all to ride cars, it can just be mapped across lanes, instead of only within a lane.


\fi

==> Style-Files/neil-defs/defs.tex <==
\usepackage{xparse}
\newcommand{\bnm}{\begin{newmath}}
\newcommand{\enm}{\end{newmath}}

\newcommand{\bea}{\begin{eqnarray*}}%
\newcommand{\eea}{\end{eqnarray*}}%

\newcommand{\bne}{\begin{newequation}}
\newcommand{\ene}{\end{newequation}}

\newcommand{\bal}{\begin{newalign}}
\newcommand{\eal}{\end{newalign}}

\newenvironment{newalign}{\begin{align}%
\setlength{\abovedisplayskip}{4pt}%
\setlength{\belowdisplayskip}{4pt}%
\setlength{\abovecaptionskip}{1pt}%
\setlength{\belowcaptionskip}{1pt}%
\setlength{\abovedisplayshortskip}{6pt}%
\setlength{\belowdisplayshortskip}{6pt} }{\end{align}}
\setlength{\abovedisplayskip}{2pt}%
\setlength{\belowdisplayskip}{2pt}%

\newenvironment{newmath}{\begin{displaymath}%
\setlength{\abovedisplayskip}{4pt}%
\setlength{\belowdisplayskip}{4pt}%
\setlength{\abovedisplayshortskip}{6pt}%
\setlength{\belowdisplayshortskip}{6pt} }{\end{displaymath}}

\newenvironment{neweqnarrays}{\begin{eqnarray*}%
\setlength{\abovedisplayskip}{-4pt}%
\setlength{\belowdisplayskip}{-4pt}%
\setlength{\abovedisplayshortskip}{-4pt}%
\setlength{\belowdisplayshortskip}{-4pt}%
\setlength{\jot}{-0.4in} }{\end{eqnarray*}}

\newenvironment{newequation}{\begin{equation}%
\setlength{\abovedisplayskip}{4pt}%
\setlength{\belowdisplayskip}{4pt}%
\setlength{\abovedisplayshortskip}{6pt}%
\setlength{\belowdisplayshortskip}{6pt} }{\end{equation}}



\newcounter{ctr}
\newcounter{savectr}
\newcounter{ectr}

\newenvironment{newitemize}{%
\begin{list}{\mbox{}\hspace{5pt}$\bullet$\hfill}{\labelwidth=15pt%
\labelsep=4pt \leftmargin=12pt \topsep=3pt%
\setlength{\listparindent}{\saveparindent}%
\setlength{\parsep}{\saveparskip}%
\setlength{\itemsep}{3pt} }}{\end{list}}


\newenvironment{newenum}{%
\begin{list}{{\rm (\arabic{ctr})}\hfill}{\usecounter{ctr} \labelwidth=17pt%
\labelsep=5pt \leftmargin=22pt \topsep=3pt%
\setlength{\listparindent}{\saveparindent}%
\setlength{\parsep}{\saveparskip}%
\setlength{\itemsep}{2pt} }}{\end{list}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% Figure and table macros
%

\newcounter{mytable}
\def\mytable{\begin{centering}\refstepcounter{mytable}}
\def\endmytable{\end{centering}}

\def\mytablecaption#1{\vspace{2mm}
  \centerline{Table \arabic{mytable}.~{#1}}
  \vspace{6mm}
  \addcontentsline{lot}{table}{\protect\numberline{\arabic{mytable}}~{#1}}
}


\newcounter{myfig}
\def\myfig{\begin{centering}\refstepcounter{myfig}}
\def\endmyfig{\end{centering}}

\def\myfigcaption#1{
             \vspace{2mm}
             \centerline{\textsf{Figure \arabic{myfig}.~{#1}}}
             \vspace{6mm}
             \addcontentsline{lof}{figure}{\protect\numberline{\arabic{myfig}}~{#1}}}


\newlength{\saveparindent}
\setlength{\saveparindent}{\parindent}
\newlength{\saveparskip}
\setlength{\saveparskip}{\parskip}

\newcommand{\decOracle}{\textbf{Dec}}

\newcommand{\negsmidge}{{\hspace{-0.1ex}}}
\newcommand{\cdotsm}{\negsmidge\negsmidge\negsmidge\cdot\negsmidge\negsmidge\negsmidge}

\def\suchthatt{\: :\:}
\newcommand{\E}{{\rm I\kern-.3em E}}
\newcommand{\Prob}[1]{{\Pr\left[\,{#1}\,\right]}}
\newcommand{\Probb}[2]{{\Pr}_{#1}\left[\,{#2}\,\right]}
\newcommand{\CondProb}[2]{{\Pr}\left[\: #1\:\left|\right.\:#2\:\right]}
\newcommand{\CondProbb}[2]{\Pr[#1|#2]}
\newcommand{\ProbExp}[2]{{\Pr}\left[\: #1\:\suchthatt\:#2\:\right]}
\newcommand{\Ex}[1]{{\textnormal{E}\left[\,{#1}\,\right]}}
\newcommand{\Exx}{{\textnormal{E}}}
\newcommand{\given}{\ensuremath{\,\big|\,}}


\newcommand{\true}{\mathsf{true}}
\newcommand{\false}{\mathsf{false}}
\def\negl{\mathsf{negl}}


\newcommand{\secref}[1]{\mbox{Section~\ref{#1}}}
\newcommand{\appref}[1]{\mbox{Appendix~\ref{#1}}}
\newcommand{\thref}[1]{\mbox{Theorem~\ref{#1}}}
\newcommand{\defref}[1]{\mbox{Definition~\ref{#1}}}
\newcommand{\corref}[1]{\mbox{Corollary~\ref{#1}}}
\newcommand{\lemref}[1]{\mbox{Lemma~\ref{#1}}}
\newcommand{\clref}[1]{\mbox{Claim~\ref{#1}}}
\newcommand{\propref}[1]{\mbox{Proposition~\ref{#1}}}
\newcommand{\factref}[1]{\mbox{Fact~\ref{#1}}}
\newcommand{\remref}[1]{\mbox{Remark~\ref{#1}}}
\newcommand{\figref}[1]{\mbox{Figure~\ref{#1}}}
\renewcommand{\algref}[1]{\mbox{Algorithm~\ref{#1}}}
% \newcommand{\eqref}[1]{\mbox{Equation~(\ref{#1})}}
% Have to use \renewcommand because exists already in amsmath
\renewcommand{\eqref}[1]{\mbox{Equation~(\ref{#1})}}
\newcommand{\consref}[1]{\mbox{Construction~\ref{#1}}}
\newcommand{\tabref}[1]{\mbox{Table~\ref{#1}}}

\newcommand{\get}{{\:{\leftarrow}\:}}
\newcommand{\gett}[1]{\:{\leftarrow}_{#1}\:}
\newcommand{\getsr}{{\:{\leftarrow{\hspace*{-3pt}\raisebox{.75pt}{$\scriptscriptstyle\$$}}}\:}}
\newcommand{\getm}{{\:\leftarrow_{\mdist}\:}}
\newcommand{\getd}{{\:\leftarrow_{\ddist}\:}}
%\newcommand{\getm}{{\:{\leftarrow{\hspace*{-3pt}\raisebox{.75pt}{$\scriptscriptstyle \mdist$}}}\:}}
\newcommand{\getk}{{\:\leftarrow_{\kdist}\:}}
%\newcommand{\getk}{{\:{\leftarrow{\hspace*{-3pt}\raisebox{.75pt}{$\scriptscriptstyle \kdist$}}}\:}}
\newcommand{\getp}{{\:\leftarrow_{p}\:}}



\newcommand{\gamesfontsize}{\small}
\newcommand{\fpage}[2]{\framebox{\begin{minipage}[t]{#1\textwidth}\setstretch{1.1}\gamesfontsize  #2 \end{minipage}}}
\newcommand{\mpage}[2]{\begin{minipage}[t]{#1\textwidth}\setstretch{1.1}\gamesfontsize  #2 \end{minipage}}

\newcommand{\hpages}[3]{\begin{tabular}{cc}\begin{minipage}[t]{#1\textwidth} #2 \end{minipage} & \begin{minipage}[t]{#1\textwidth} #3 \end{minipage}\end{tabular}}

\newcommand{\hpagess}[4]{
        \begin{tabular}[t]{c@{\hspace*{.5em}}c}
        \begin{minipage}[t]{#1\textwidth}\gamesfontsize #3 \end{minipage}
        &
        \begin{minipage}[t]{#2\textwidth}\gamesfontsize #4 \end{minipage}
        \end{tabular}
    }

\newcommand{\hpagesss}[6]{
        \begin{tabular}[t]{c@{\hspace*{.5em}}c@{\hspace*{.5em}}c@{\hspace*{.5em}}c}
        \begin{minipage}[t]{#1\textwidth}\gamesfontsize #4 \end{minipage}
        &
        \begin{minipage}[t]{#2\textwidth}\gamesfontsize #5 \end{minipage}
        &
        \begin{minipage}[t]{#3\textwidth}\gamesfontsize #6 \end{minipage}
        \end{tabular}
    }

\newcommand{\hpagessss}[8]{
        \begin{tabular}{c@{\hspace*{.5em}}c@{\hspace*{.5em}}c@{\hspace*{.5em}}c}
        \begin{minipage}[t]{#1\textwidth}\gamesfontsize #5 \end{minipage}
        &
        \begin{minipage}[t]{#2\textwidth}\gamesfontsize #6 \end{minipage}
        &
        \begin{minipage}[t]{#3\textwidth}\gamesfontsize #7 \end{minipage}
        &
        \begin{minipage}[t]{#4\textwidth}\gamesfontsize #8 \end{minipage}
        \end{tabular}
    }


\newcommand{\hfpages}[3]{\hfpagess{#1}{#1}{#2}{#3}}
\newcommand{\hfpagess}[4]{
        \begin{tabular}[t]{c@{\hspace*{.5em}}c}
        \framebox{\begin{minipage}[t]{#1\textwidth}\setstretch{1.1}\gamesfontsize #3 \end{minipage}}
        &
        \framebox{\begin{minipage}[t]{#2\textwidth}\setstretch{1.1}\gamesfontsize #4 \end{minipage}}
        \end{tabular}
    }
\newcommand{\hfpagesss}[6]{
        \begin{tabular}[t]{c@{\hspace*{.5em}}c@{\hspace*{.5em}}c}
        \framebox{\begin{minipage}[t]{#1\textwidth}\setstretch{1.1}\gamesfontsize #4 \end{minipage}}
        &
        \framebox{\begin{minipage}[t]{#2\textwidth}\setstretch{1.1}\gamesfontsize #5 \end{minipage}}
        &
        \framebox{\begin{minipage}[t]{#3\textwidth}\setstretch{1.1}\gamesfontsize #6 \end{minipage}}
        \end{tabular}
    }
\newcommand{\hfpagessss}[8]{
        \begin{tabular}[t]{c@{\hspace*{.5em}}c@{\hspace*{.5em}}c@{\hspace*{.5em}}c}
        \framebox{\begin{minipage}[t]{#1\textwidth}\setstretch{1.1}\gamesfontsize #5 \end{minipage}}
        &
        \framebox{\begin{minipage}[t]{#2\textwidth}\setstretch{1.1}\gamesfontsize #6 \end{minipage}}
        &
        \framebox{\begin{minipage}[t]{#3\textwidth}\setstretch{1.1}\gamesfontsize #7 \end{minipage}}
        &
        \framebox{\begin{minipage}[t]{#4\textwidth}\setstretch{1.1}\gamesfontsize #8 \end{minipage}}
        \end{tabular}
    }

\newcommand{\vecw}{\mathbf{w}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\load}{L}
\newcommand{\coll}{\mathsf{Coll}}
\newcommand{\nocoll}{\overline{\mathsf{Coll}}}


\newcommand{\Img}{\textsf{Img}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%% Fonts and symbols
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand\funcfont{\textsf}
\newcommand\variablefont{\texttt}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% NEW COMMANDS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def \Perm {\funcfont{Perm}}
\def \calC {{\mathcal{C}}}
\def \calU {{\mathcal{U}}}
\renewcommand{\u}{\ensuremath{u}}
\newcommand{\unew}{\ensuremath{\tilde{u}}}

\newcommand{\calN}{\mathcal{N}}
\def \sspace {{\mathcal{S}}}
\def \strings {{\mathcal{S}}}
\def \slen {{s}}
\def \kspace {{\mathcal{K}}}
\def \kspacesize {{m}}
\def \mspacesize {{n}}
\def \kdict {D}
\def \dictsize {d}
\newcommand{\kdist}{p_k}
\newcommand{\mdist}{\ensuremath{{W}}}
\newcommand{\alldist}{\rho}
\newcommand{\pwdist}{\transgen}
\newcommand{\ddist}{\rho_{dec}}
\newcommand{\PWset}{{\mathcal{P}}}  % TODO: fix, same as \pwdist
\newcommand{\PWsetvec}{\vec{\mathcal{P}}}
\newcommand{\PWvec}{\vec{P}}
\newcommand{\domvec}{\vec{D}}
\newcommand{\humanornot}{\vec{h}}
\newcommand{\dom}{\textsf{dom}}
%\def \kdist {{\kappa}}
%\def \mdist {{\mu}}
%\def \ddist {{\delta}}
\def \pspace {{\mathcal{P}}}
\def \mpspace {{\mathcal{MP}}}
\def \cspace {{\mathcal{C}}}
\def \key {\kappa}
%\def \msg {M}
\def \seed {S}
\def \ctxt {C}
\def \ctxtpart {C_2}
\newcommand{\genprime}{{\textsf{GenPrime}}}
\newcommand{\isprime}{{\textsf{IsPrime}}}
\newcommand{\LeastLesserPrime}{{\textsf{PrevPrime}}}
\newcommand{\pwset}{\mathcal{S}}
\newcommand{\DTE}{{\textsf{DTE}}}
\newcommand{\encode}{{\textsf{encode}}}
\newcommand{\decode}{{\textsf{decode}}}

\newcommand{\DTEsingle}{{\textsf{1PW-DTE}}}
\newcommand{\encodesingle}{{\textsf{1PW-encode}}}
\newcommand{\decodesingle}{{\textsf{1PW-decode}}}

\newcommand{\DTErss}{{\textsf{RSS-DTE}}}
\newcommand{\encoderss}{{\textsf{RSS-encode}}}
\newcommand{\decoderss}{{\textsf{RSS-decode}}}

\newcommand{\DTEindep}{{\textsf{MPW-DTE}}}
\newcommand{\encodeindep}{{\textsf{MPW-encode}}}
\newcommand{\decodeindep}{{\textsf{MPW-decode}}}


\newcommand{\DTEsub}{{\textsf{SG-DTE}}}
\newcommand{\encodesub}{{\textsf{SG-encode}}}
\newcommand{\decodesub}{{\textsf{SG-decode}}}
\newcommand{\decodekamf}{{\textsf{KAMF-decode}}}
\newcommand{\DTEis}{{\textsf{IS-DTE}}}
\newcommand{\encodeis}{{\textsf{is-encode}}}
\newcommand{\decodeis}{{\textsf{is-decode}}}
\newcommand{\DTErej}{{\textsf{REJ-DTE}}}
\newcommand{\encoderej}{{\textsf{rej-encode}}}
\newcommand{\decoderej}{{\textsf{rej-decode}}}
\newcommand{\DTErsarej}{{\textsf{RSA-REJ-DTE}}}
\newcommand{\encodeRSAREJ}{{\textsf{rsa-rej-encode}}}
\newcommand{\decodeRSAREJ}{{\textsf{rsa-rej-decode}}}
\newcommand{\DTErsainc}{{\textsf{RSA-INC-DTE}}}
\newcommand{\encodeRSAINC}{{\textsf{rsa-inc-encode}}}
\newcommand{\decodeRSAINC}{{\textsf{rsa-inc-decode}}}
\newcommand{\DTEunf}{{\textsf{UNF-DTE}}}
\newcommand{\DTEnunf}{{\textsf{NUNF-DTE}}}


%\newcommand{\encodeis}{{\textsf{encode}_{\textrm{is}}}}
%\newcommand{\decodeis}{{\textsf{decode}_{\textrm{is}}}}
\newcommand{\rep}{\textsf{rep}}
\newcommand{\isErr}{\epsilon_{\textnormal{is}}}
\newcommand{\incErr}{\epsilon_{\textnormal{inc}}}
\def \enc {{\textsf{E}}}
\def \dec {{\textsf{D}}}
\def \SEscheme {{\textsf{SE}}}
\def \HEscheme {{\textsf{HE}}}
\def \CTR {{\textsf{CTR}}}
\def \encHE {{\textsf{HEnc}}}
\def \HIDE {{\textsf{HiaL}}}
\def \encHIDE {{\textsf{HEnc}}}
\def \decHIDE {{\textsf{HDec}}}
\def \decHE {{\textsf{HDec}}}
\def \encHEt {{\textsf{HEnc2}}}
\def \decHEt {{\textsf{HDec2}}}

\newcommand{\myind}{\hspace*{1em}}
\newcommand{\thh}{^{\textit{th}}} % th
\newcommand{\concat}{\,\|\,}
\newcommand{\dotdot}{..}
\newcommand{\emptystr}{\varepsilon}

\newcommand{\round}{\textsf{round}}

\newcommand{\alphabar}{\overline{\alpha}}
\newcommand{\numbinsbar}{\overline{b}}
\newcommand{\numballs}{a}
\newcommand{\numbins}{b}

%\def \encHE {{\sf{enc}^{HE}}}
%\def \decHE {{\sf{dec}^{HE}}}
%\def \encHEt {{\sf{enc}^{HE2}}}
%\def \decHEt {{\sf{dec}^{HE2}}}
\def \idealHE {{\mathcal{HE}}}
\def \IEnc {{\mathbf{\rho}}}
\def \IDec {{\mathbf{\rho^{-1}}}}
\def \OEnc {{\mathbf{Enc}}}
\def \ODec {{\mathbf{Dec}}}
\newcommand{\SimuProc}{\mathbf{Sim}}
\newcommand{\ROProc}{\mathbf{RO}}
\newcommand{\PrimProc}{\mathbf{Prim}}
\def \stm {g}
\def \istm {\hat{g}}
\def \kts {{f}}
\def \lex {{\sf lex}}
\def \part {part}
\def \kd {{\sf{kd}}}
\def \msgdist {{d}}
\def \keydist {{r}}
\def \ind {{\sf{index}}}
\def \kprf {z}
\def \adv {\ensuremath{\mathcal A}\xspace}
\def \pwds {u}
\newcommand{\mpw}{mpw}
\newcommand{\pw}{w}
\newcommand{\pwvec}{\vec{\pw}}
\newcommand{\vecx}{\vec{x}}
\def \tokens {v}
\def \calP{{\mathcal{P}}}
\def \template{{\mathcal{T}}}
\def \vaultset{{\mathcal{V}}}
\def \ext {{\sf ext}}
\def \offset {\delta}
\def \maxweight {\epsilon}
\def \advo {{\mathcal{A}}^{*}}

\newcommand{\Chall}{\textsf{Ch}}
\newcommand{\Test}{\textnormal{\textsf{Test}}}
\newcommand{\RoR}{\textsf{RoR}}
\newcommand{\MI}{\textnormal{MI}}
\providecommand{\MR}{\textnormal{MR}}
\newcommand{\MRCCA}{\textnormal{MR-CCA}}
\newcommand{\SAMP}{\textnormal{SAMP}}
\newcommand{\DTEgame}{\textnormal{SAMP}}
\newcommand{\KR}{\textnormal{KR}}
\newcommand{\advA}{{\mathcal{A}}}
\newcommand{\advR}{{\mathcal{R}}}
\newcommand{\advB}{{\mathcal{B}}} % 
\newcommand{\advC}{{\mathcal{C}}} % C
\newcommand{\advD}{{\mathcal{D}}} % D
\newcommand{\advE}{{\mathcal{E}}}
\newcommand{\advF}{{\mathcal{F}}}
\newcommand{\advG}{{\mathcal{G}}}
\newcommand{\advI}{{\mathcal{I}}}
\newcommand{\nextval}{\;;\;}
\newcommand{\TabC}{\texttt{C}}
\newcommand{\TabR}{\texttt{R}}
\newcommand{\Hash}{H}
\newcommand{\Cipher}{\pi}
\newcommand{\CipherInv}{\pi^{-1}}
\newcommand{\simu}{{\mathcal S}}
\newcommand{\prim}{P}
\newcommand{\maxguess}{\gamma}


\newcommand{\bigO}{\mathcal{O}}
\newcommand{\calG}{{\mathcal{G}}}

\def\sqed{{\hspace{5pt}\rule[-1pt]{3pt}{9pt}}}
\def\qedsym{\hspace{2pt}\rule[-1pt]{3pt}{9pt}}

\newcommand{\Colon}{{\::\;}}
\newcommand{\good}{\textsf{Good}}

\newcommand\Tvsp{\rule{0pt}{2.6ex}}
\newcommand\Bvsp{\rule[-1.2ex]{0pt}{0pt}}
\newcommand{\TabPad}{\hspace*{5pt}}
\newcommand\TabSep{@{\hspace{5pt}}|@{\hspace{5pt}}}
\newcommand\TabSepLeft{|@{\hspace{5pt}}}
\newcommand\TabSepRight{@{\hspace{5pt}}|}


\DeclareMathOperator*{\argmin}{argmin}
\DeclareMathOperator*{\argmax}{argmax}
\newcommand{\comma}{\textnormal{,}}

\renewcommand{\paragraph}[1]{\vspace*{6pt}\noindent\textbf{#1}\;}

\newcommand{\weirvault}{\textsf{Pastebin}\xspace}
\newcommand{\ndssvault}{\textsf{DBCBW}\xspace}




\newcommand{\reminder}[1]{ [[[ \marginpar{\mbox{$<==$}} #1 ]]] }

%
% New theorem types: (Already in CCS template)
%
%\newtheorem{observation}{Observation}
%\newtheorem{definition}{Definition}
%\newtheorem{claim}{Claim}
\newtheorem{assumption}{Assumption}
\newtheorem{fact}{Fact}
% \newtheorem{theorem}{Theorem}[section]
% \newtheorem{lemma}{Lemma}[section]
% \newtheorem{corollary}{Corollary}[section]
% \newtheorem{proposition}{Proposition}
% \newtheorem{example}{Example}

%
% Definitions:
%
\def \blackslug{\hbox{\hskip 1pt \vrule width 4pt height 8pt
    depth 1.5pt \hskip 1pt}}
\def \qed{\quad\blackslug\lower 8.5pt\null\par}
% In-line QED, for ending a proof with a $$ formula
% In-line QED, for ending a proof with a $$ formula
\def \inQED{\quad\quad\blackslug}
\def \Qed{\QED}
\def \QUAD{$\Box$}
\def \Proof{\par\noindent{\bf Proof:~}}
\def \proof{\Proof}
\def \poly {\mbox{$\mathsf{poly}$}}
\def \binary {\mbox{$\mathsf{binary}$}}
\def \ones {\mbox{$\mathsf{ones}$}}
\def \rank {\mbox{$\mathsf{rank}$}}
\def \bits {\mbox{$\mathsf{bits}$}}
\def \factorial {\mbox{$\mathsf{factorial}$}}
\def \fr {\mbox{$\mathsf{fr}$}}
\def \pr {\mbox{$\mathsf{pr}$}}
\def \zon {\{0,1\}^n}
\def \zo  {\{0,1\}}
\def \zok {\{0,1\}^k}
\def \mo {s}


\def\utilcnt{\ensuremath{\mu_{\mathrm{cnt}}}}
\def\utiltime{\ensuremath{\mu_{\mathrm{time}}}}
\def\ex{\ensuremath{{\mathrm{ex}}}}
\def\rlx{\ensuremath{{\mathrm{rlx}}}}
\def\tp{\textsf{TP}}
\def\cp{\textnormal{\textsf{CP}}\xspace}
\def\edistcutoff{\edist}
\def\entcutoff{\ensuremath{m}}
\def\relentcutoff{{\sigma}}
\def\mutt{\mu_{\mathrm{tt}}}

\newcommand{\Hdot}{H(\mbox{ } \cdot \mbox{ }  , \mbox{ } \del)}


\newcounter{mynote}[section]
\newcommand{\notecolor}{blue}
%\renewcommand{\thenote}{\thesection.\arabic{mynote}}
%\renewcommand{\tnote}[1]{\refstepcounter{mynote}{\bf \textcolor{\notecolor}{$\ll$TomR~\thenote: {\sf #1}$\gg$}}}

\newcommand{\fixme}[1]{{\textcolor{red}{[FIXME: #1]}}}
\newcommand{\todo}[1]{{\textcolor{red}{[TODO: #1]}}}


\newcommand\ignore[1]{}


\newcommand\simplescheme{simple}


\newcommand{\KDF}{\mathsf{KDF}}
\newcommand{\salt}{\mathsf{sa}}
\newcommand{\PRF}{F}
\newcommand{\subgram}{\mathsf{SG}}
\newcommand{\popdomains}{\mathcal{D}}

\newcommand{\retrieve}{\textsf{Sync}}
\newcommand{\update}{\textsf{Insert}}

\newcommand{\dictW}{\textbf{D1}\xspace}
\newcommand{\dictF}{\textbf{D2}\xspace}

\newcommand{\str}{\text{str}}
\newcommand{\calS}{{\mathcal S}}

% \newcommand{\new}[1]{\textcolor{red}{\sf #1}}
\newcommand{\new}[1]{#1}


%% ------------------------- Rahul -----------------------
\newcounter{rcnote}[section]
\newcommand{\rcthenote}{\thesection.\arabic{rcnote}}
\newcommand{\rcnote}[1]{\refstepcounter{rcnote}{\bf \textcolor{magenta}{$\ll$RC~\rcthenote: {\sf #1}$\gg$}}}

\newcounter{mrnote}[section]
\newcommand{\mrthenote}{\thesection.\arabic{mrnote}}
\newcommand{\mrnote}[1]{\refstepcounter{mrnote}{\bf \textcolor{green}{$\ll$MR~\mrthenote: {\sf #1}$\gg$}}}

\newcounter{fknote}[section]
\newcommand{\fkthenote}{\thesection.\arabic{fknote}}
\newcommand{\fknote}[1]{\refstepcounter{fknote}{\bf \textcolor{blue}{$\ll$FK~\fkthenote: {\sf #1}$\gg$}}}

\newcounter{anote}[section]
\newcommand{\ajthenote}{\thesection.\arabic{anote}}
\newcommand{\anote}[1]{\refstepcounter{anote}{\bf \textcolor{cyan}{$\ll$AJ~\ajthenote: {\sf #1}$\gg$}}}



\newcommand{\mytab}{\hspace*{.4cm}}
\def\half{{1\over 2}}
\newcommand{\NT}[1]{\texttt{#1}}
\DeclareMathSymbol{\mlq}{\mathord}{operators}{``}
\DeclareMathSymbol{\mrq}{\mathord}{operators}{`'}
\newcommand{\calO}{{\mathcal O}}
\newcommand{\calA}{{\mathcal A}}
\newcommand{\kamfplus}{Kamouflage\textbf{+}\xspace}
% \newcommand{\genfrom}[1]{\;{\stackrel{\,#1}{\leftarrow}}\;}
\newcommand{\genfrom}[1]{{\:{\leftarrow{\hspace*{-3pt}\raisebox{.75pt}{$\scriptscriptstyle#1$}}}\:}}
%\newcommand{\genfrom}[1]{\;\leftarrow{\tiny \$} #1\;}
\newcommand{\twopartdef}[4]
{
  \left\{
    \begin{array}{ll}
      #1 & \mbox{if } #2 \\[4pt]
      #3 & #4
      \end{array}
      \right.
}
\newcommand{\threepartdef}[6]
{
  \left\{
    \begin{array}{lll}
      #1 & \mbox{if } #2 \\
      #3 & \mbox{if } #4 \\
      #5 & \mbox{if } #6
      \end{array}
      \right.
}

\newcommand{\gt}[1]{\gamma_{#1,\maxdist}}
\newcommand{\gmt}[2]{\gamma_{#1,#2}}
\def\nh{\ensuremath{N}}
\def\ball{\ensuremath{B}}
\def\anh{\ensuremath{\tilde{N}_k}}
% \newcommand{\nh}[2]{{N_{#1}(#2)}}

\newcommand{\ballsizet}[1]{{\beta_{#1,\maxdist}}}
\newcommand{\ballsize}[2]{{\beta_{#1,#2}}}
\newcommand{\rh}[2]{{\bf R}_{#1, #2}}
\newcommand{\rhf}[2]{R_{f, \gamma}}
\newcommand{\realm}{{m}}
% \newcommand{\inputm}{{\tilde{m}}}
\newcommand{\lmid}{\ell_{\realm, m'}}
\newcommand{\cipherlength}{n}
\renewcommand{\SS}{\textsf{SS}}
\newcommand{\Rec}{\textsf{Rec}\xspace}
\newcommand{\rec}{\textsf{rec}\xspace}
\newcommand{\Rep}{\textsf{Rep}\xspace}
\newcommand{\Gen}{\textsf{Gen}}
\newcommand{\dis}{\textsf{dis}}

\def\chk{\textnormal{\textsf{Chk}}\xspace}
\def\reg{\textnormal{\textsf{Reg}}\xspace}
\def\exchk{\textnormal{\textsf{ExChk}}\xspace}
\def\adpchk{\textnormal{\textsf{AdpChk}}\xspace}
\def\RKROR{\textnormal{MKROR}\xspace}
\def\SRKROR{\textnormal{SKROR}\xspace}
\def\ROR{\textnormal{ROR}\xspace}
\def\ROBUST{\textnormal{ROB}\xspace}
\def\OFFDIST{\textnormal{OFFDIST}\xspace}
\def\POFFDIST{\overline{\textnormal{OFFDIST}}\xspace}
\def\OFFGUESS{\textnormal{OFFGUESS}\xspace}
\def\ONGUESS{\overline{\textnormal{ONGUESS}}\xspace}
\def\ONATTACK{\textnormal{ONATTACK}\xspace}
\def\adp{\ensuremath{\Pi\xspace}}
\def\Check{\textnormal{\textsf{Checker}}}
\def\CheckPtxt{\textnormal{\textsf{PChecker}}}
\def\trans{\textnormal{\ensuremath{T}}}
\def\transgen{\textnormal{\ensuremath{\mathcal{T}}}}
\def\pke{\ensuremath{\mathcal{E}}}
\def\pkenc{\ensuremath{\pke^{\mathrm{enc}}}}
\def\pkdec{\ensuremath{\pke^{\mathrm{dec}}}}
\def\sH{\ensuremath\mathrm{H}^s}
\def\H{\ensuremath{\mathsf{H}}\xspace}
\def\T{\ensuremath{\mathsf{T}}\xspace}
\def\W{\ensuremath{\mathsf{W}}\xspace}
\def\F{\ensuremath{\mathsf{F}}\xspace}
\def\ret{\ensuremath{\mathrm{return}}\xspace}
\def\cs{\ensuremath{t}} % Cache Size
\def\waitlen{\ensuremath{\omega}\xspace} %waitlist size
\newcommand{\M}{{\mathcal{M}}}
\newcommand{\ent}{{\bf H}}
\newcommand{\Hfuzzy}{{\mathrm{H}}^{\rm fuzz}}
\newcommand{\Hminfuzzy}{{\mathrm{H}}^{{\rm{fuzz}}}_{t,\infty}}
\newcommand{\Hpfuzzy}{{\mathrm{H}}^{{\rm{pfuzz}}}}
\newcommand{\Hinf}{{\bf H}^{{\rm \min}}_{\infty}}
\newcommand{\Hminpfuzzy}{{\bf H}^{{\rm pfuzz}}_{t,\infty}}


\def\sa{{\sf sa}}
\def\err{{\varepsilon}}%^{(e)}}}
\newcommand{\dist}{\mathcmd{p}}
\newcommand{\distest}{\hat{\mathcmd{p}}}
\newcommand{\distvec}{\mathbf{\dist}}
\newcommand{\distvecest}{\hat{\mathbf{p}}}
\newcommand{\w}{{w}}
\newcommand{\wnew}{\tilde{w}}
\newcommand{\m}{{w}}
\newcommand{\mnew}{{\tilde{m}}}
\newcommand{\mspacevec}{\mathcmd{\mathbf{W}}}
\newcommand{\mvec}{\mathcmd{\mathbf{\m}}}
\newcommand{\mvecss}[1]{\mvec_1\ldots\mvec_{#1}}
\renewcommand{\mspace}{\mathcmd{W}}
\newcommand{\mspacebot}{{\mspace}_\bot}

\newcommand{\similar}{\mathrm{sim}}
\newcommand{\similarvec}{\mathrm{\mathbf{sim}}}

\def \mvecnew{{\tilde{\mvec}}}
\newcommand{\mvecnewss}[1]{\mvecnew_1\ldots\mvecnew_{#1}}

\DeclareDocumentCommand{\edist}{o o}{
  \ensuremath{
    \IfNoValueTF{#1}{{d}}{{\sf d}(#1,#2)}
  }
}

\newcommand{\utilinc}{\mu}
\newcommand{\secloss}{\Delta}
\newcommand{\seclossg}{\Delta^\textnormal{greedy}}
\newcommand{\seclosso}{\Delta}
%\newcommand{\maxlambda}{\lambda^*}
%\newcommand{\maxfuzzlambda}{\tilde{\lambda}^*}
\newcommand{\fuzzlambda}{\lambda^\textnormal{fuzzy}}
\newcommand{\greedylambda}{\lambda^\textnormal{greedy}}
\newcommand{\greedylambdaon}{\tilde{\lambda}^\mathrm{on}}
\newcommand{\greedylambdaoff}{\tilde{\lambda}^\mathrm{off}}
\newcommand{\seclosson}{\secloss^\mathrm{on}}
\newcommand{\seclossoff}{\secloss^\mathrm{off}}
\def \edit {\ensuremath{e}}
\newcommand\error{e}
\newcommand\tab[1][1cm]{\hspace*{#1}}

\newcommand{\mathcmd}[1]{\ensuremath{#1}\xspace} % to use a command both in math mode and non-math mode
\newcommand{\minentropy}[1]{\ensuremath{\operatorname{H_\infty}\olrk{#1}}}
\newcommand{\fuzzyminentropy}[1]{\ensuremath{\operatorname{H^{fuzz}_{\maxdist, \infty}}\olrk{#1}}}
\providecommand{\condminentropy}[2]{\ensuremath{\operatorname{\tilde{H}_\infty}\olrk{#1|#2}}}
\newcommand{\s}{\mathcmd{s}}
\newcommand{\typo}{\mathcmd{\tilde{\m}}}
\newcommand{\typoj}[1]{\ensuremath{(\typo_{#1}, j_{#1})}}
\newcommand\typojprime[1]{{(\typo_{#1}, j'_{#1})}}
\newcommand\contrib[2]{\mathsf{cont}\left[{#1}/{#2}\right]}
\def\typovec{\ensuremath{\{\typo_i\}_{i=1}}}
\def\opttypovec{\ensuremath{\{\typo^*_i\}_{i=1}}}
\def\slotguess{\textsf{SlotGuess}}
\def\typodist{\ensuremath{\tau_\pw}}
\def\cachedtypodist{\ensuremath{{\tilde{\tau}}_{\pw}}}
\def\typodistest{\ensuremath{{\hat{\tau}}_{\pw}}}
\def\incache{T_\pw}
\newcommand{\fuzzylambda}{\ensuremath{\lambda^{\mathrm{fuzzy}}}}
%\newcommand{\errorprob}[2]{\mathcmd{\tau_{#1}({#2})}}
\newcommand{\errordist}{\mathcmd{\tau}}
\newcommand{\famdist}{\mathcmd{\mathcal{W}}}
\def\guessw{\ensuremath{W}}
\newcommand{\precdist}{W}
\newcommand{\entdef}{Z}
\newcommand{\PW}{\mathcmd{\mathcal{W}}}
\newcommand{\cachedom}{\mathcmd{\mathcal{S}}}
\newcommand{\supp}{\mbox{supp}}
\newcommand{\olrk}[1]{\ifx\nursymbol#1\else\!\!\mskip4.5mu plus 0.5mu\left(\mskip0.5mu plus0.5mu #1\mskip1.5mu plus0.5mu \right)\fi}

\newcommand{\errorprob}[1]{\mathcmd{\tau_{#1}}}
\newcommand{\errorpr}[2]{\mathcmd{\errorprob{#1}{(#2)}}}
\newcommand{\Expectation}{\mathop{\mathbb E}}
\newcommand{\hash}[2]{\mathcmd{F(#1, #2)}}
\newcommand{\hashj}[3]{\mathcmd{F_{#3}(#1, #2)}}
\newcommand{\rhh}{\mathcmd{y}}
\newcommand{\x}{\mathcmd{x}}
\newcommand{\range}{\mathcmd{R}}
\newcommand{\lmm}{\mathcmd{l_\w}}
\newcommand{\rmm}{\mathcmd{r_\w}}
\newcommand{\conflict}[2]{\mathcmd{C_{#1, #2}}}
\newcommand{\Probsub}[2]{{\Pr_{#1}\left[\,{#2}\,\right]}}
\newcommand{\Condprobsub}[3]{{\Pr}_{#1}\left[\: #2\:\left|\right.\:#3\:\right]}
\newcommand{\wmid}{l_{\w, \w^\prime}}
\newcommand{\realhash}{\mathcmd{z}}
\newcommand{\collhash}{\mathcmd{z^\prime}}
\newcommand{\floor}[1]{\left \lfloor #1 \right \rfloor }
\newcommand{\ceiling}[1]{\left \lceil #1 \right \rceil }
\newcommand{\interval}{I}
% \newcommand{\p}[2]{p_{#1}(#2)}
\newcommand{\ssketch}{\mathcmd{\mathsf{S}}}
\newcommand{\tsketch}{\mathcmd{\msgsettingsym\mathsf{S}}}
\newcommand{\trivsketch}{\mathcmd{\tsketch_{\emptystr}}}
\newcommand{\WREC}{\mathcmd{\pcnotionstyle{W\pcmathhyphen{}REC}}}
\newcommand{\AREC}{\mathcmd{\pcnotionstyle{A\pcmathhyphen{}REC}}}
\newcommand{\WUTIL}{\mathcmd{\pcnotionstyle{W\pcmathhyphen{}UTIL}}}
\newcommand{\AUTIL}{\mathcmd{\pcnotionstyle{A\pcmathhyphen{}UTIL}}}
\newcommand{\indexset}{I}
\newcommand{\topset}{Z_1^*}
\newcommand{\cachedist}{T}
\newcommand{\pwdis}{R}
\newcommand{\onbudget}{q}
\newcommand{\blacklist}{\textsf{B}}
\newcommand{\blacklistlen}{\alpha}
\newcommand{\plaintextstate}{\bar{\state}}
\newcommand{\typocutoff}{\delta}
\newcommand{\plfuprob}{\ensuremath{\nu}}

\def\ballweight{\ensuremath{e_{\tilde{\tau}}}}
\newcommand{\Adv}{\textnormal{\textsf{Adv}}}
\newcommand{\AdvOFFLINE}[1]{\Adv^{\footnotesize\textnormal{\textrm{offdist}}}_{\footnotesize #1}}
\newcommand{\AdvOFFLINEP}[1]{\Adv^{\overline{\footnotesize\textnormal{\textrm{{offdist}}}}}_{\footnotesize #1}}
\newcommand{\AdvOFFGUESS}[1]{\Adv^{\footnotesize\textnormal{\textrm{offguess}}}_{\footnotesize #1}}
\newcommand{\AdvONGUESS}[1]{\Adv^{{\footnotesize\textnormal{\textrm{onguess}}}}_{\footnotesize #1}}
\newcommand{\AdvONATTACK}[1]{\Adv^{\footnotesize\textnormal{\textrm{onattack}}}_{\footnotesize #1}}
\newcommand{\AdvRKROR}[1]{\Adv^{\footnotesize\textnormal{\textrm{mk-ror}}}_{\footnotesize #1}}
\newcommand{\AdvSRKROR}[1]{\Adv^{\footnotesize\textnormal{\textrm{sk-ror}}}_{\footnotesize #1}}
\newcommand{\AdvROR}[1]{\Adv^{\footnotesize\textnormal{\textrm{ror}}}_{\footnotesize #1}}
\newcommand{\AdvROBUST}[1]{\Adv^{\footnotesize\textnormal{\textrm{rob}}}_{\footnotesize #1}}

\newcommand{\advantage}[3]{\pcnotionstyle{\Adv}^{#1}_{#2}(#3)}
\newcommand{\neighbourhood}[2]{N_{#1}({#2})}
\newcommand{\rhhdist}{Y}
\newcommand{\fullerhash}{z}
\newcommand{\errorball}[2]{{B}^{\errordist}_{#1}(#2)}
\newcommand{\f}{f}
\newcommand{\pwmaxlen}{\ell}
\newcommand{\indexi}{i}
\newcommand{\indexq}{q}
\newcommand{\indexx}{x}
\newcommand{\replace}{\textsf{replace}}
\newcommand{\vecca}{\vecc{a}}
\newcommand{\veccb}{\vecc{b}}
\newcommand{\veccv}{\vecc{v}}
\newcommand{\coins}{r}
\newcommand{\state}{\ensuremath{\mathsf{s}}}
\newcommand{\win}{\mathsf{win}}
\newcommand{\Chk}{\textsf{Chk}}
\newcommand{\PChk}{\textsf{PChk}}
\newcommand{\indexh}{h}
\newcommand{\randomZ}{Z}
\newcommand{\Cache}{\textnormal{\textsf{Cache}}}
\newcommand{\WarmupCache}{\textnormal{\textsf{WarmupCache}}}
\newcommand{\CacheUpdate}{\textnormal{\textsf{CacheUpdt}}}
\newcommand{\CacheInit}{\textnormal{\textsf{CacheInit}}}
\newcommand{\cachestate}{\ensuremath{\mathtt{S}}\xspace}
\newcommand{\cachestatelen}{\ensuremath{\sigma}\xspace}
\newcommand{\CacheLRU}{\textnormal{\textsf{CacheLRU}}}
\newcommand{\CacheLRUUpdate}{\textnormal{\textsf{UpdateLRU}}}
\newcommand{\CacheLRUInit}{\textnormal{\textsf{InitLRU}}}


\newcommand{\zxcvbn}{\textnormal{\textsf{zxcvbn}}\xspace}
\newcommand{\bad}{\textnormal{\textsf{bad}}}
\newcommand{\wait}{z}
\newcommand{\PKE}{\textnormal{\textsf{PKE}}}
\newcommand{\pkegen}{\mathcal{K}}
\newcommand{\pkeenc}{\mathcal{E}}
\newcommand{\pkedec}{\mathcal{D}}
\newcommand{\pkectxtspace}{\mathcal{C}_{\pkeenc}}
\newcommand{\pk}{\ensuremath{\mathsf{pk}}\xspace}
\newcommand{\sk}{\ensuremath{\mathsf{sk}}\xspace}
\newcommand{\PBE}{\textnormal{\textsf{PBE}}}
\newcommand{\utility}{\textsf{Utility}}

\newcommand{\skegen}{\ensuremath{\mathsf{K}}}
\newcommand{\skeenc}{\ensuremath{\mathsf{E}}}
\newcommand{\skedec}{\ensuremath{\mathsf{D}}}
\newcommand{\skectxtspace}{\ensuremath{\mathcal{C}_{\skeenc}}}
\newcommand{\ske}{\textnormal{\textsf{SKE}}}
\newcommand{\SE}{\textnormal{\textsf{SE}}}
\newcommand{\sekg}{\mathcal{K}}
\newcommand{\seenc}{\mathcal{E}}
\newcommand{\sedec}{\mathcal{D}}
\newcommand{\saltlen}{{\ell_{\mathrm{salt}}}}

\newcommand{\skk}{\textnormal{\textsf{k}}}
\newcommand{\cipherske}{{c}}
\newcommand{\cipherpke}{{c}}
\newcommand{\SH}{\textnormal{\textsf{SH}}}
\newcommand{\FH}{\textnormal{\textsf{H}}}
\newcommand{\counter}{\textnormal{\textsf{Count}}}
\newcommand{\indexp}{p}
\newcommand{\ciphertextspace}{\mathcal{C}}
\newcommand{\states}{\mathcal{S}}
\newcommand{\indexr}{r}
\newcommand{\vecc}[1]{\mathbf{#1}}
\newcommand{\sawait}{\overline{\sa}}
\newcommand{\skkwait}{\overline{\skk}}
\newcommand{\hwait}{\overline{\indexh}}
\newcommand{\randomY}{Y}
\newcommand{\indexm}{m}
\newcommand{\hashtable}[1]{H[#1]}
\newcommand{\SHlen}{k_1}
\newcommand{\FHlen}{k_2}
\newcommand{\valid}{\textnormal{\textsf{valid}}}
\newcommand{\skepsilon}{\epsilon_{ske}}
\newcommand{\pkepsilon}{\epsilon_{pke}}
\newcommand{\hybindex}{j}

\newcommand{\DL}{\textnormal{DL}}
\newcommand{\vecb}{\mathbf{b}}
\newcommand{\indicator}{\mathbb{I}}
\newcommand{\cipherspace}{\mathcal{C}}
\newcommand{\pkemsgspace}{\mathcal{M}_\pkeenc}

\newcommand{\pkecipher}{c}
\newcommand{\skecipher}{{c}}
\newcommand{\pkemsg}{m}
\newcommand{\skemsg}{{m}}
\newcommand{\skemsgspace}{ \msgspace_{\skeenc}}
\newcommand{\upperb}{\alpha}

\newcommand{\ffbox}[1]{
   \setlength{\fboxsep}{-1\fboxrule}
   \fbox{\hspace{1.2pt}\strut#1\hspace{1.2pt}}}


\newcommand{\statespace}{S}
\newcommand{\targuess}{\textsf{TarGuess}}
\newcommand{\untarguess}{\textsf{UnTarGuess}}

\newcommand{\accept}{\texttt{accept}}
\newcommand{\reject}{\texttt{reject}}
\newcommand{\threshold}{\ensuremath{\tau}}
\newcommand{\clfthreshold}{\ensuremath{\theta}}
\newcommand{\far}{\ensuremath{\alpha}}
\newcommand{\frr}{\ensuremath{\beta}}
\newcommand{\fpr}{\ensuremath{\nu}}
\newcommand{\fnr}{\ensuremath{\gamma}}
\newcommand{\FPR}{\textrm{FPR}}
\newcommand{\FNR}{\textrm{FNR}}


\newcommand{\matchalgo}{\mathcal{L}}
\newcommand{\matchalgovec}{\mathcal{\mathbf{L}}_\sslen}
\def \score {\theta}
\newcommand{\indexjvec}{\ensuremath{\mathcmd{\mathbf{j}}\xspace}}
\def\k{k}
\newcommand{\add}{\funcfont{Add}}
\newcommand{\accuracy}{\funcfont{Accuracy}}
\def\acc{\delta}
\def \MS {\funcfont{MS}}
\def \MRec {\funcfont{MRec}}
\newcommand \MSt{\MS^{\matchalgo}_\sslen}
\newcommand \MRect{\MRec^{\matchalgo}_\sslen}
\def \nmatches {\ensuremath{l}}
\def \D{D}
\def \Dmod{\tilde{D}}
\def \mlen{n}
\def \sslen{t}
\def \secret{s}
\def \secretvec{\mathbf{s}}
\newcommand{\sketch}{{\funcfont{sketch}}}
\newcommand{\sketchval}{v}
\def \recover{\funcfont{recover}}
\def \verify{\funcfont{verify}}
\def \q{q}
\def\fp{\alpha}
\def\fn{\beta}
\def\tp{\gamma}
\newcommand{\one}{\ensuremath{\mathbbm{1}}}
\newcommand{\seclen}{\ell}
\newcommand{\Overify}{{\mathcal{O}_\funcfont{vrfy}}}
\newcommand{\Omatch}{\mathcal{O}_\funcfont{match}}
\newcommand{\ith}[2]{#1_{#2}}
\newcommand{\jth}[2]{#1^{#2}}
\newcommand{\mspacei}{\ith{\mspace}{i}}
\newcommand{\errori}{\ith{\error}{i}}
\newcommand{\matchalgoi}{\ith{\matchalgo}{i}}
\newcommand{\mvecbar}{\overline{\mvec}}
\newcommand{\mvectilde}{\tilde{\mvec}}
\newcommand{\angbrac}[1]{\ensuremath{\langle #1 \rangle}}
\newcommand{\clf}{\mathcal{C}}
\newcommand{\clft}{\clf_\sslen}
\newcommand{\clfest}{\mathcal{\hat{\clf}}}
\newcommand{\clfq}[1]{{\clf^q_{#1}}}
\newcommand{\nclf}{r}
\newcommand{\oclf}{\omega}
\newcommand{\biosketch}{\funcfont{TenSketch}\xspace}
\newcommand{\tensketch}{\funcfont{TenSketch}\xspace}

\newcommand{\hvec}{\mathbf{h}}
\newcommand{\insertr}{\mathsf{insert{\scriptstyle\$}}}
\newcommand{\dbmsg}{\ensuremath{\mathcal{F}}}
\newcommand{\dbmsgs}{\ensuremath{\{\dbmsg_i\}}}
\newcommand{\dbid}{\mathcal{I}}
\newcommand{\db}{\ensuremath{D}}
% \newcommand{\dbs}{\ensuremath(\dbid,\{\dbmsg_i\})}
\newcommand{\dbs}{\ensuremath(\dbid,\dbmsg)}
\newcommand{\dbsprime}{\ensuremath(\dbid',\dbmsg')}
\newcommand{\dbsize}{N}
\def \dblen{N}
\def\mhat{\hat{\mvec}}
\def\findmatches{\funcfont{\footnotesize FindMatches$^{\matchalgo}$}}
\newcommand{\setss}[1]{\SS^\Delta_{#1}}
\newcommand{\setrec}[1]{\Rec^\Delta_{#1}}
\newcommand{\setsst}{\setss{\sslen}}
\newcommand{\setrect}{\setrec{\sslen}}
\newcommand{\costs}{{c_s}}
\newcommand{\costc}{{c_c}}
\NewDocumentCommand{\indseq}{ O{1} O{r} }{{#1}\ldots {#2}}
\newcommand{\seq}[2]{{{#1}_1,\ldots,{#1}_{#2}}}
\newcommand{\relu}{\funcfont{ReLu}}
\newcommand{\fcrelu}[1]{\funcfont{FC}_{\relu}^{#1}}
\newcommand{\gencliq}{\funcfont{GenTupIncr}}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:
%
% Comments/annotations
%
\newcommand{\neil}[1]{\textcolor{red}{\textbf{Neil:} #1}}
\newcommand{\heidi}[1]{\textcolor{blue}{\textbf{Heidi:} #1}}
\newcommand{\natacha}[1]{\textcolor{cyan}{\textbf{Natacha:} #1}}
\newcommand{\nc}[1]{\textcolor{cyan}{\textbf{Natacha:} #1}}
\newcommand{\alin}[1]{\textcolor{ForestGreen}{\textbf{Alin:} #1}}
\newcommand{\ittai}[1]{\textcolor{brown}{\textbf{Ittai comment:} #1}}
\newcommand{\IA}[1]{\textcolor{brown}{\textbf{IA:} #1}}
\newcommand{\fs}[1]{\textcolor{teal}{\textbf{FS:} #1}}

\newcommand{\changebars}[2]{\textcolor{red}{(#1)\st{(#2)}}}
%
% Crypto things
%
\newcommand{\badv}{\ensuremath{\mathcal{B}}\xspace}


\newcommand{\Gr}{\ensuremath{\mathbb{G}}\xspace}

\setlength{\fboxsep}{6pt}

%
% Math things
%
\newcommand{\randin}{\ensuremath{\in_R}\xspace}
\newcommand{\Fp}{\ensuremath{\mathbb{Z}_p}\xspace}
%
% Algorithms things
%
\algnewcommand{\LineComment}[1]{\State \(\triangleright\) \textcolor{gray}{#1}}

%
% Aggregate signature things
%
\newcommand{\apk}{\ensuremath{\mathsf{apk}\xspace}}

\newcommand{\aggKeygen}{\ensuremath{\mathsf{AS.KGen}}\xspace}
\newcommand{\aggSignShare}{\ensuremath{\mathsf{AS.SignShare}}\xspace}
\newcommand{\aggVerifyShare}{\ensuremath{\mathsf{AS.VerifyShare}}\xspace}
\newcommand{\aggAgg}{\ensuremath{\mathsf{AS.Agg}}\xspace}
\newcommand{\aggVerifyAgg}{\ensuremath{\mathsf{AS.VerifyAgg}}\xspace}

\newcommand{\bglsKeygen}{\ensuremath{\mathsf{BGLS.KGen}}\xspace}
\newcommand{\bglsSignShare}{\ensuremath{\mathsf{BGLS.SignShare}}\xspace}
\newcommand{\bglsVerifyShare}{\ensuremath{\mathsf{BGLS.VerifyShare}}\xspace}
\newcommand{\bglsAgg}{\ensuremath{\mathsf{BGLS.Agg}}\xspace}
\newcommand{\bglsVerifyAgg}{\ensuremath{\mathsf{BGLS.VerifyAgg}}\xspace}

\newcommand{\blsKeygen}{\ensuremath{\mathsf{BLS.KGen}}\xspace}
\newcommand{\blsSignShare}{\ensuremath{\mathsf{BLS.SignShare}}\xspace}
\newcommand{\blsVerifyShare}{\ensuremath{\mathsf{BLS.VerifyShare}}\xspace}
\newcommand{\blsAgg}{\ensuremath{\mathsf{BLS.Agg}}\xspace}
\newcommand{\blsVerifyAgg}{\ensuremath{\mathsf{BLS.VerifyAgg}}\xspace}

\makeatletter
% defined only inside "algorithmic" environment
\algblockdefx[Upon]{Upon}{EndUpon}
  [1]{\textbf{upon} #1 \textbf{do}}
  {end}
\algtext*{EndUpon}

% Protocol
% Custom upon ... do block.:w
\algblockdefx[Upon]{Upon}{EndUpon}
  [1]{\textbf{upon} #1 \textbf{do}}
  {end}
\algtext*{EndUpon}
\newcommand{\algolabel}[1]{\genericlabel{alg}{#1}}
\newcommand{\linelabel}[1]{\genericlabel{line}{#1}}
\newcommand{\msgfont}[1]{\textsc{#1}}
%\newcommand{\msg}[2]{\msgfont{#1}$\langle #2 \rangle$}
\newcommand{\msg}[2]{$\langle$\msgfont{#1}, $#2\rangle$}
%\newcommand{\smsg}[2]{$\langle$\msgfont{#1}, $#2\rangle$}$_{#3}$
\newcommand{\emsg}[2]{$\langle$\msgfont{#1}$\rangle$}
% Custom State: block.
\algnewcommand{\algorithmicstate}{\textbf{State:}}
\algnewcommand{\GlobalState}{\item[\algorithmicstate]}
%\newcommand{\msg}[1]{\langle #1 \rangle}
\newcommand{\light}[1]{\textcolor{gray}{#1}}

